DexTrack: Towards Generalizable Neural Tracking Control for Dexterous Manipulation from Human References

We address the challenge of developing a generalizable neural tracking controller for dexterous manipulation from human references. This controller aims to manage a dexterous robot hand to manipulate diverse objects for various purposes defined by kinematic human-object interactions. Developing such a controller is complicated by the intricate contact dynamics of dexterous manipulation and the need for adaptivity, generalizability, and robustness. Current reinforcement learning and trajectory optimization methods often fall short due to their dependence on task-specific rewards or precise system models. We introduce an approach that curates large-scale successful robot tracking demonstrations, comprising pairs of human references and robot actions, to train a neural controller. Utilizing a data flywheel, we iteratively enhance the controller's performance, as well as the number and quality of successful tracking demonstrations. We exploit available tracking demonstrations and carefully integrate reinforcement learning and imitation learning to boost the controller's performance in dynamic environments. At the same time, to obtain high-quality tracking demonstrations, we individually optimize per-trajectory tracking by leveraging the learned tracking controller in a homotopy optimization method. The homotopy optimization, mimicking chain-of-thought, aids in solving challenging trajectory tracking problems to increase demonstration diversity. We showcase our success by training a generalizable neural controller and evaluating it in both simulation and real world. Our method achieves over a 10% improvement in success rates compared to leading baselines. The project website with animated results is available at https://meowuu7.github.io/DexTrack/.

==> articles/ablations.tex <==
% \section{Ablation Studies}

==> articles/abstract.tex <==
\input{articles/teaser_figure}


\begin{abstract}

We address the challenge of developing a generalizable neural tracking controller for dexterous manipulation from human references. This controller aims to manage a dexterous robot hand to manipulate diverse objects for various purposes defined by kinematic human-object interactions. Developing such a controller is complicated by the intricate contact dynamics of dexterous manipulation and the need for adaptivity, generalizability, and robustness. Current reinforcement learning and trajectory optimization methods often fall short due to their dependence on task-specific rewards or precise system models. We introduce an approach that curates large-scale successful robot tracking demonstrations, comprising pairs of human references and robot actions, to train a neural controller. Utilizing a data flywheel, we iteratively enhance the controller's performance, as well as the number and quality of successful tracking demonstrations. We exploit available tracking demonstrations and carefully integrate reinforcement learning and imitation learning to boost the controller's performance in dynamic environments. At the same time, to obtain high-quality tracking demonstrations, we individually optimize per-trajectory tracking by leveraging the learned tracking controller in a homotopy optimization method. The homotopy optimization, mimicking chain-of-thought, aids in solving challenging trajectory tracking problems to increase demonstration diversity. We showcase our success by training a generalizable neural controller and evaluating it in both simulation and real world. Our method achieves over a 10\% improvement in success rates compared to leading baselines. The project website with animated results is available at  \href{https://projectwebsite7.github.io/gene-dex-manip/}{DexTrack}.
% and the number and quality of successful tracking demonstrations. 


% % We explore the problem of obtaining a generic controller for dexterous robotic hands 
% % learning a generalizable neural tracking controller for dexterous manipulation from human references. 
% We explore the problem of learning a generalizable neural tracking controller for dexterous manipulation from human references.
% % The task wishes for a versatile controller that can control a dexterous robot hand to accomplish various, challenging and expressive manipulation tasks specified by kinematic human-object manipulations. 
% This task wishes for a versatile controller capable of managing a dexterous robot hand to execute various complex and expressive manipulation tasks, as defined by kinematic human-object interactions.
% It is inherently challenged by the optimization difficulty resulting from intricate dynamics involved in dexterous manipulation and the expectation in the versatility, generalization ability, and robustness of the tracking controller.
% % to various, novel, and challenging manipulation tasks. 
% Either advanced model-free reinforcement learning (RL)-based techniques or model-based trajectory optimization fall short in resolving such huge challenges due to the demand on task-specific reward designs that largely hinder the generalization capability and the difficulty in complex system modeling in the dexterous manipulation scenario.
% Our key idea lies in leveraging high-quality abundant imitation-ready data to train a tracking controller and tackling the difficulties in acquiring such data by leveraging the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner.
% % by carefully combining reinforcement learning and imitation learning, 
% % jointly with RL and tackling the difficulties in acquiring such data by leveraging the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner.
% % leverage abundant, high-quality, imitation-ready data to facilitate the learning of a generalizable tracking controller.
% We carefully combine reinforcement learning and imitation learning to train the neural tracking controller to enhance its versatility, generalization ability, and robustness towards dynamic environment variations. To curate abundant high-quality imitation-ready data, we devise a per-trajectory tracking strategy using the tracking controller and a homotopy path generator, mimicking chain-of-thought, that can propose beneficial homotopy optimization paths to help us solve difficult single trajectory tracking problems. We showcase our success in training a versatile neural tracking controller with high generalization ability and robustness. Through extensive experiments conducted in both simulation and real world, our method demonstrates an improvement in success rates of over 10\% compared to the best-performing baseline. The project website with animated results is available at \href{https://projectwebsite7.github.io/gene-dex-manip/}{DexTrack}.
% % We demonstrate our success in training a versatile neural tracking controller with high generalization ability and robustness. We conduct extensive experiments in both the simulator and the real world, demonstrating capability of our method in boosting the success rate by 10\%+ from the best-performed baseline. The project website is available at \href{https://projectwebsite7.github.io/gene-dex-manip/}{DexTrack}. 
% % We conduct extensive experiments in both the simulator the real world, demonstrating the versatility, generalization ability, and robustness of our tracking controller,  capability of boosting the success rate by 10\%+ from the best-performed baseline. The project website is available at \href{https://projectwebsite7.github.io/gene-dex-manip/}{DexTrack}.
% % Isaac Gym and 
% % that effectively improves single trajectory tracking results via the tracking controller and a homotopy path generator, mimicking chain-of-thought, that can propose beneficial homotopy optimization paths. 
% % We leverage imitation learning and reinforcement learning to train the neural tracking controller to let it benefit from a large number of high-quality data and also be able to cope with dynamic state disturbances. To curate abundant high-quality imitation-ready data, we devise a per-trajectory tracking scheme that effectively improves single trajectory tracking results via the tracking controller and a homotopy path generator, mimicking chain-of-thought, that can propose beneficial homotopy optimization paths. 
% % We successfully train a universal tracking controller that enables a dexterous robot hand to adeptly interact with diverse objects to accomplish a wide range of novel and expressive manipulation tasks. 
% % with dynamics, rich hand-object contacts. 

% % Previous approaches are typically restricted to task-specific manipulation skill acquisition or only demonstrate the versatility in relatively simple tasks such as grasping, leaving 
% % the general dexterous tracking control largely unsolved~\eric{``Dexterous tracking control'' is not a good term. Dexterous is used to describe manipulation other than tracking.}. 
% % are typically limited by the unsatisfactory capability and versatility, leaving the universal dexterous tracking control largely unsolved. 
% % unsatisfactory task difficulties or being restricted in single trajectory tracking, leaving the universal dexterous tracking control largely unsolved. 
% % We propose to leverage the joint effort of reinforcement learning (RL) and the diverse and high-quality action-labeled data to open the possibility of training general tracking control policy. 
% % We wish to learn a versatile and generalizable neural controller by imitating abundant, high-quality data with actions to obtain the generalization ability towards veraious situations, and leveraging reinforcement learning to maintain the robustness and unepxted situations. However, acquiring  a large number of imitation-ready data itself is tricky and challenging. 
% % We propose to leverage abundant, high-quality, imitation-ready data to facilitate the learning of a generalizable tracking controller.
% % Since acquiring a large amount of imitiation-ready data with hgih-quality action sequences itself is very challenging, we devise a strategy w
% % But acquiring a large amount of imitation-ready data itself is very challenging. We propose to learn a tracking task structure prior model which is further leveraged to plan optimization paths so that we can solve difficult tracking problems via a homotopy method. 
% % model tracking task structure 
% % by 
% % transferring tracking data prior and a homotopy method propose
% % with the optimization paths generated by a homotopy generator. 
% % We design an iterative way to improve the imitation-ready data by data prior from the tracking controller and the tracking task structure prior, and enhance the tracking controller in a bootstrapping manner. 
% % improve the tracking controller 
% % But acquiring high-quality data itself
% % data to facilitate the tracking 
% % We design an iterative approach where we 1) curate high-quality action-labeled data taking the joint power of tracking prior from the tracking controller and tracking curriculum proposed by a learned curriculum scheduler, and 2) train the tracking controller taking advantage of the guidance from the labeled data. 
% % a universal controller that can generalize to adeptly complete various novel and challenging manipulation tasks. 
% % challenged by inherent difficulties from 
% % We explore the problem of learning a universal tracking controller from human references. The task wishes for a versatile controller that can control a dexterous robot hand to accomplish various challenging and expressive manipulation tasks specified by kinematic motions. It is challenged by inherent difficulties from the complex and intricate dynamics involved in dexterous manipulation and the wish for a universal controller that can generalize to adeptly complete various novel and challenging manipulation tasks. Previous approaches are typically limited by unsatisfactory task difficulties or being restricted in single trajectory tracking, leaving the universal dexterous tracking control largely unsolved. We propose to leverage the joint effort of reinforcement learning (RL) and the diverse and high-quality action-labeled data to open the possibility of training genera tracking control policy. We design an iterative approach where we 1) curate high-quality action-labeled data taking the joint power of tracking prior from the tracking controller and tracking curriculum proposed by a learned curriculum scheduler, and 2) train the tracking controller taking advantage of the guidance from the labeled data. We successfully train a universal tracking controller that enables a dexterous robot hand to adeptly interact with diverse objects to accomplish a wide range of novel and expressive manipulation tasks. We conduct extensive experiments in both Isaac Gym and the real world, demonstrating the capability of boosting the success rate by xx\%+ from the best-performed baseline. 
\end{abstract}

==> articles/conclusions.tex <==
\section{Conclusions and Limitations}

% In this work, we propose \modelname to tackle the challenge of developing a generalizable tracking controller for dexterous manipulation. By leveraging abundant high-quality robot tracking demonstrations and employing a pre-trajectory tracking scheme to mine imitation-ready data, we progressively refine the controller using a bootstrapping strategy. Extensive experiments validate the effectiveness of our approach, establishing it as a strong foundation for future advancements in generalizable tracking control. \noindent\textbf{Limitations.} The primary limitation of our method is the efficiency of acquiring high-quality demonstrations. Currently, searching for optimal homotopy optimization paths to improve demonstrations is time-consuming. Future research could focus on finding faster, approximate homotopy optimization methods to accelerate the training process.

We propose \modelname to develop a generalizable tracking controller for dexterous manipulation. Leveraging high-quality tracking demonstrations and a pre-trajectory tracking scheme, we refine the controller through bootstrapping. Extensive experiments confirm its effectiveness, establishing a strong foundation for future advancements. \noindent\textbf{Limitations.} A key limitation is the time-consuming process of acquiring high-quality demonstrations. Future work could explore faster, approximate methods for homotopy optimization to speed up training.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this work, we propose \modelname to address the challenge of developing a generalizable tracking controller for dexterous manipulation. 
% By leveraging abundant high-quality robot tracking demonstrations to train the tracking controller and employing a pre-trajectory tracking scheme that effectively mines high-quality imitation-ready data, we gradually solve problems in each side and finally arrive at a strong tracking controller via a bootstrapping strategy. 
% Extensive experiments demonstrate the effectiveness of our method, evidencing it as a promising foundation for future developments in generalizable tracking control. 
% \noindent\textbf{Limitations.} The main limitation of our method lies in the efficiency of acquiring high-quality demonstrations. Currently, searching for good homotopy optimization paths to improve demonstrations is a little bit time-consuming. A meaningful future research direction is approximately finding beneficial homotopy optimization in a time-efficient way, therefore accelerating the homotopy generator's training. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The main limitation of our approach lies in the efficiency of acquiring high-quality action-labeled data. Currently, searching for good tracking curricula for training the curriculum scheduler is the most time-consuming part of our method. How to improve the efficiency such as using approximate curricula for training the scheduler is an interesting future research direction. 


% To address the difficulties in acquiring abundant and high-quality data 
% universal tracking controller for dexterous robot hand manipulation. By combining reinforcement learning with high-quality action-labeled data, we unleash the possibility of using RL to train a tracking controller for solving difficult manipulation problems. To address the ``chicken-and-egg'' problem by 1) training the controller using both RL and action-labeled datasets, and 2) optimizing for high-quality action-labeled data effectively in an acceptable time-budget, we design an interactive approach. 
% Leveraging the joint power of a learned tracking curriculum and data guidance, we can effectively improve the quality of the labeled dataset. We then progressively improve the capability of the tracking controller by curating data with higher quality. Extensive experiments demonstrate the effectiveness of our method, evidencing it as a promising foundation for future developments in universal tracking control.

% \noindent\textbf{Limitations.} The main limitation of our approach lies in the efficiency of acquiring high-quality action-labeled data. Currently, searching for good tracking curricula for training the curriculum scheduler is the most time-consuming part of our method. How to improve the efficiency such as using approximate curricula for training the scheduler is an interesting future research direction. 
% The process of curating this data is resource-intensive, requiring significant time and effort to generate diverse and accurate labels that effectively guide the training of the tracking controller. While our method achieves notable performance improvements, the dependence on large amounts of labeled data could hinder scalability, particularly when expanding to more complex tasks or environments. Future work could explore strategies to reduce the reliance on labeled data, such as incorporating self-supervised learning or more efficient data-generation techniques, to enhance both the practicality and scalability of the approach.
% we can create enough high-quality data in an acceptable time budget for training 
% demonstrates significant improvements in manipulation performance across a range of novel and expressive tasks. Extensive experiments, both in simulation and real-world environments, validate the effectiveness of our approach, with notable improvements in success rates over existing baselines. This research opens new avenues for advancing dexterous robot manipulation, providing a promising foundation for future developments in universal tracking control.

==> articles/exp.tex <==

\vspace{-5pt}
\section{Experiments} \label{sec:exp}
\vspace{-5pt}
% TODO: overview part




% and adaptability 
% We conduct extensive experiments to demonstrate the effectiveness, generalization ability, and robustness, of our tracking controller. We evaluate our method on two HOI datasets containing complex functional daily manipulation featured by difficult trajectories with non-trivial object movements and subtle in-hand re-orientations, challenging object geometries, as well as rich and changing contacts. 
% We train our model in the Isaac Gym environment and conduct evaluations both in the simulator and the real world (see Section~\ref{sec:exp_setting}). We compare strong baselines with dedicated designs for dexterous manipulations to demonstrate the superiority of our method. Our tracking controller can track diverse, difficult, and novel hand-object interactions involving challenging and functional movements, extremely thin objects, as well as rich and changing contacts (see Section~\ref{sec:exp_results}).  However, previous approaches either fail to generalize or behave unsatisfactorily in challenging cases. On average, we can boost the tracking success rate by 10\% from the previously best-performed method. We make further analysis of our method on its robustness and the generalization ability to out-of-distribution test cases (see Section~\ref{sec:exp_analysis}) to illustrate its capability and utility (see Section~\ref{sec:exp_analysis}).  

We conduct extensive experiments to evaluate the effectiveness, generalization ability, and robustness of our tracking controller. Our method is tested on two HOI datasets featuring complex, functional, daily manipulation tasks.
% characterized by difficult trajectories with non-trivial object movements, subtle in-hand re-orientations, challenging object geometries, and dynamic, rich hand-object contact patterns. 
% The controller is trained in the Isaac Gym environment. 
We conduct both through experiments both in the simulation and evaluations in the the real world (see Section~\ref{sec:exp_setting}). 
% thorough evaluations both in the simulation and 
% with evaluations performed in both simulation and the real world (see Section~\ref{sec:exp_setting}). 
We compare our method against strong baselines to demonstrate its superiority. Our tracking controller successfully handles novel, difficult, and intriguing manipulations, including those involving intricate functional movements, extremely thin objects, and dynamic contacts (see Section~\ref{sec:exp_results}). In contrast, previous approaches fail to generalize well. 
% in these challenging scenarios. 
% fail to  or perform poorly in these challenging scenarios. 
% On average, our method improves the tracking success rate by 10\% over the best-performing prior methods on both two datasets. 
On average, our method improves the tracking success rate by more than 10\% over the best prior methods across both datasets.
We further analyze our controller's robustness towards significant kinematic noise such as unrealistic states and large penetrations (see Section~\ref{sec:exp_analysis}). 
% showcasing its versatility and practical utility.
% , as well as the generalization capabilities towards out-of-distribution test cases (see Section~\ref{sec:exp_analysis}), 
% , specifically designed for dexterous manipulations, 
% Empowered by our proposed training pipeline, we demonstrate that our tracking controller can effectively generalize to novel and challenging interaction trajectories involving unseen object geometry and unobserved manipulations. 
% , demonstrating strong capability and robustness. 


% , which are crucial properties that we expect for a general controller, to demonstrate its capability and utility (see Section~\ref{sec:exp_analysis}). 
% With a single policy, we 





% \textcolor{red}{TODO: track some interesting and long motions?}

\vspace{-5pt}
\subsection{Experimental Settings} \label{sec:exp_setting}
\vspace{-5pt}


% \todo{add the retargeting to the appendix} 

\noindent\textbf{Datasets.}
We test our method on two public human-object interaction  datasets:
% Our dexterous robot hand-object manipulation dataset is built by retargeting two public human-object interaction datasets: 
GRAB~\citep{taheri2020grab}, featuring daily interactions, and 
% single-hand interaction and 
TACO~\citep{liu2024taco}, containing functional tool-use interactions. 
% (single-hand interactions) and TACO~\citep{liu2024taco} (functional tool-use interactions). 
In simulation, we use the Allegro hand, with URDF adapted from IsaacGymEnvs~\citep{makoviychuk2021isaac}, and in real-world experiments, the LEAP hand~\citep{Shaw2023LEAPHL}, due to hardware constraints. Human-object interaction trajectories are retargeted to create robot hand-object sequences using PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. We fully retargeted the GRAB and TACO datasets, producing 1,269 and 2,316 robot hand manipulation sequences, respectively. The evaluation on GRAB focus on testing the model’s generalization to unseen interaction sequences. 
Specifically, we use sequences from subject \texttt{s1} (197 sequences) as the test data while the remaining trajectories as the training set. 
% sequences from subject \texttt{s1} (197 sequences) are used as the test dataset. 
% while the training dataset includes the remaining sequences from other subjects. 
For the TACO dataset, we follow the generalization evaluating setting suggested by the authors~\citep{liu2024taco} and split the dataset into a training set with 1,565 trajectories and four distinct test sets at different difficulty levels. The primary quantitative results are reported on the first-level set. More details are provided in Appendix~\ref{sec:supp_exp_details}. 
% and results are provided in Appendix~\ref{sec:supp_exp_details}. 
% More details on the dataset splitting and our results on remaining test sets are provided in Appendix~\ref{sec:supp_exp_details}. 
% to assess generalization at different levels. 
% evaluation setting suggested by the authors~\citep{liu2024taco}. The dataset is split into a training set with 

% GRAB focuses on testing generalization to unseen sequences, while TACO evaluates generalization across four distinct test sets. More details on dataset splitting and results are provided in Appendix~\ref{sec:supp_exp_details}.

% Our dexterous robot hand-object manipulation dataset is constructed by retargeting two public human-object interaction datasets: GRAB~\citep{taheri2020grab}, which focuses on single-hand interactions with everyday objects, and TACO~\citep{liu2024taco}, which features functional tool-use interactions. For simulation experiments, we use the Allegro hand, while in real-world experiments, the LEAP hand~\citep{Shaw2023LEAPHL} is employed due to constraints in the hardware resources. In simulation, the URDF file for the Allegro hand is adapted from IsaacGymEnvs~\citep{makoviychuk2021isaac}, while the LEAP hand URDF is adapted from dex\_urdf~\citep{bunnyvisionpro}. We retarget human-object interaction (HOI) trajectories to simulated robot hand to create the robot hand-object interaction sequences. We use the forward kinematics implemented in PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024} in the retargeting method. Further details are provided in Appendix~\ref{sec:supp_method}. We fully retargeted the GRAB and released TACO datasets, yielding 1,269 and 2,316 robot hand manipulation sequences, respectively. The GRAB dataset evaluation focuses on testing the model’s generalization to unseen interaction sequences, given the large variations in object geometries. Specifically, sequences from subject \texttt{s1} (197 sequences) are used as the test dataset, while the training dataset includes the remaining sequences from other subjects. For the TACO dataset, we follow the generalization evaluation setting suggested by the authors~\citep{liu2024taco}. The dataset is split into a training set with 1,565 trajectories and four distinct test sets to assess generalization at different levels. The primary quantitative results are reported on the first-level test set. More details on the dataset splitting and our results on remaining test sets are provided in Appendix~\ref{sec:supp_exp_details}. 

% The forward kinematics algorithm in  the retargeting method is
% We describe these hands in simulation using URDF files from dex\_urdf~\citep{bunnyvisionpro} and retarget human-object interaction (HOI) trajectories to both hands, generating corresponding kinematic trajectories through PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. 

% the test set S0. More details on the dataset splitting and visualizations are provided in Appendix~\ref{sec:supp_exp_details}. 
% : 1) S0: Both the tool object geometries and interaction triplets are seen during training; 2) S1: Novel tool geometries, but the interaction triplets are seen during training; 3) S2: Novel interaction triplets, but familiar object categories and geometries; 4) S3: Both object geometries and interaction triplets are novel. The primary quantitative results are reported on the test set S0. More details on the dataset splitting and visualizations are provided in Appendix~\ref{sec:supp_exp_details}. 

% Our dexterous robot hand-object manipulation dataset is created by retargeting two public human-object datasets, namely GRAB~\citep{taheri2020grab}, containing single-hand interactions with daily objects, and TACO~\citep{liu2024taco}, featured by functional tool using interactions. We use simulated Allegro hand in our simulation experiments while LEAP hand~\citep{Shaw2023LEAPHL} in the real world experiments due to the hardware constraints. We use URDF files from dex\_urdf~\citep{bunnyvisionpro} as their descriptions in the simulation. We retarget HOI trajectories to these two hands to create their corresponding kinematic trajectories leveraging PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. 
% For details of the retargeting method that we leverage in our method, please refer to Appendix~\ref{sec:supp_method}. 
% We retarget the full GRAB dataset and the full released TACO dataset, obtaining 1269 and 2316 robot hand manipulation sequences respectively. The evaluation on GRAB mainly aims at testing the model's generalization ability toward unseen interaction sequences considering the large distinctions between their object geometries. Specifically, we use sequences of subject \texttt{s1}, with  197 sequences in total, as the test dataset.  The training dataset is constructed by remaining sequences from other subjects. 
% For the TACO dataset, we create one training set with four distinct test sets with different generalization levels for a detailed evaluation of the model's generalization performance, as suggested by authors~\citep{liu2024taco}. Specifically, the whole dataset is split into a training dataset, containing 1565 trajectories, and the test set S0 where both the tool object geometries and the interaction triplets are seen during training, the test set S1 where the tool geometry is novel but the interaction triplets are seen during training, the test set S2 with novel interaction triplets but seen object categories and geometries, and the test set S4 with new object geometries and interaction triplets. Main quantitative results are reported on the test set S0.  Details w.r.t. the dataset splitting and visualizations are deferred to Appendix~\ref{sec:supp_exp_details}. 
% robot hand manipulation sequences and 2316 sequences
% obtaining 1269 manipulation sequences in total, and the full released TACO data which contains 2316 sequences in total. 
% For TACO dataset, to balance the time consumption and the final data amount, we randomly select 1800 sequences from 2316 sequences in total for retargeting.


% create four different test sets to evaluate the generalization 
% For GRAB, we mainly evaluate the model's generalization ability towards novel interaction sequences considering the large distinctions between their object geometries. For 
% To evaluate the model's generalization capability towards novel manipulation trajectories, we further split them into train and test splits. For the GRAB dataset, we use sequences of the \texttt{subject s1}, with 197 sequences in total, as the test dataset. The train dataset is constructed by remaining sequences from other subjects. For the TACO dataset, we 190 trajectories randomly selected from 1800 sequences for test, while the remaining trajectories as the training data. 
% \todo{unboserved objects? a different splitting method for TACO that considers the object category?}  For evaluating the model's generalization ability towards unseen geometry, we additionally construct a subset from the TACO's training dataset and a subset from TACO's test dataset as a new test split. \todo{details about that}
% For the GRAB datset, although there are existing previous splitting routines~\citep{Zhou2022TOCHSO,Liu2024GeneOHDT}, they mainly focus on cross object generalization. 




\noindent\textbf{Metrics.} 
We introduce five metrics to evaluate the racking accuracy and task success: 1) Per-frame average object rotation error: \( R_{\text{err}} = \frac{1}{N+1} \sum_{n=0}^N \text{Diff\_Angle}(\mathbf{q}_n, \hat{\mathbf{q}}_n) \), where \( \hat{\mathbf{q}}_n \) and  \( \mathbf{q}_n \)  are reference and tracked orientation.
2) Per-frame average object translation error: \( T_{\text{err}} = \frac{1}{N+1} \sum_{n=0}^N \Vert \mathbf{t}_n - \hat{\mathbf{t}}_n \Vert \), where \( \mathbf{t}_n \) and \( \hat{\mathbf{t}}_n \) are the tracked and reference translations. 3) Per-frame average wrist position and rotation error: \( E_{\text{wrist}} = \frac{1}{N+1} \sum_{n=0}^N \left( 0.5 \, \text{Diff\_Angle}(\mathbf{q}_n^{\text{wrist}}, \hat{\mathbf{q}}_n^{\text{wrist}}) + 0.5 \Vert \mathbf{t}_n^{\text{wrist}} - \hat{\mathbf{t}}_n^{\text{wrist}} \Vert \right) \), where \( \mathbf{q}_n^{\text{wrist}} \) and \( \hat{\mathbf{q}}_n^{\text{wrist}} \) are wrist orientations, and \( \mathbf{t}_n^{\text{wrist}} \) and \( \hat{\mathbf{t}}_n^{\text{wrist}} \) are translations. 4) Per-frame per-joint average position error: \( E_{\text{finger}} = \frac{1}{N+1} \sum_{n=0}^N \left( \frac{1}{d} \Vert \mathbf{\theta}_n^{\text{finger}} - \hat{\mathbf{\theta}}_n^{\text{finger}} \Vert_1 \right) \), where $\mathbf{\theta}$ denotes finger joint positions, \( d \) is the degrees of freedom.
% (16 for both Allegro and LEAP hands).  
% and \( \Vert \cdot \Vert_1 \) denotes the 1-norm. 
5) Success rate: A tracking attempt is successful if \( T_{\text{err}} \), \( R_{\text{err}} \), and \( 0.5E_{\text{wrist}} + 0.5E_{\text{finger}} \) are all below the thresholds. Success is calculated with two thresholds: \( 10\text{cm} \)-\(20^\circ\)-\(0.8\) and \( 10\text{cm} \)-\(40^\circ\)-\(1.2\).
% object tracking quality, hand tracking accuracy, and 
% We introduce five metrics to evaluate the quality of object tracking, hand tracking accuracy, and overall success in the tracking task: 
% 1) Per-frame average object rotation error: $R_{\text{err}} = \frac{1}{N} \sum_{n=1}^N \text{Diff\_Angle}(\mathbf{q}_n, \hat{\mathbf{q}}_n) $, where $\mathbf{q}_n$ is the ground-truth orientation, $\hat{\mathbf{q}}_n$ is the tracked result, represented in quaternion, $\text{Diff\_Angle}(\cdot, \cdot)$ computes the angular difference between two quaternions.
% 2) Per-frame average object translation error: $T_{\text{err}} = \frac{1}{N} \sum_{n=1}^N \Vert \mathbf{t}_n - \hat{\mathbf{t}}_n \Vert$, where $\mathbf{t}_n$ and $\hat{\mathbf{t}}_n$  represent the ground-truth and tracked translations, respectively.
% 3) Per-frame average wrist position and rotation error: $E_{\text{wrist}}=\frac{1}{N}  \sum_{n=1}^N (0.5 \text{Diff\_Angle}(\mathbf{q}_n^{\text{wrist}}, \hat{\mathbf{q}}_n^{\text{wrist}})  + 0.5 \Vert \mathbf{t}_n^{\text{wrist}} - \hat{\mathbf{t}}_n^{\text{wrist}} \Vert )$, where $\mathbf{q}_n^{\text{wrist}}$ and $\hat{\mathbf{q}}_n^{\text{wrist}}$ represent the orientation of the wrist in the reference motion and the tracking result, respectively, while $\mathbf{t}^{\text{wrist}}_n $ and $\hat{\mathbf{t}}_n^{\text{wrist}}$ denote the wrist translation in the reference trajectory and the tracking result, respectively. 
% 4) Per-frame per-joint average position error: 
% $E_{\text{finger}}= \frac{1}{N}  \sum_{n=1}^N (\frac{1}{d} \Vert \mathbf{\theta}_n^{\text{finger}} - \hat{\mathbf{\theta}}_n^{\text{finger}} \Vert_1 )$, where $d$ is the number of degree-of-freedom (DoF) of the dexterous robot hand, \emph{i.e.,} 16 for Allegro hand and the LEAP hand used in our experiments, $\Vert \cdot \Vert_1$ denote the $1$-norm of the vector. 
% 5) Success rate: A tracking attempt is deemed successful if the object translation error $T_{\text{err}}$, object rotation error $R_{\text{err}}$, and the hand tracking error $0.5E_{\text{wrist}} + 0.5E_{\text{finger}}$ are all below their specified thresholds. Success rates are calculated using two thresholds: $10\text{cm}$-$20^\circ$-$0.8$, $10\text{cm}$-$40^\circ$-$1.2$. 

% are smaller than their corresponding threshold. Three success rates are calculated using two different thresholds, namely $10\text{cm}-20^\circ-0.8$, $10\text{cm}-40^\circ-1.2$. 
% a tracking is regarded as successful if the object rotation error object translation error 
% $15\text{cm}-40^\circ-1.6$.



\noindent\textbf{Baselines.} 
To our knowledge, no prior model-based methods have directly tackled tracking control for dexterous manipulation. Most existing approaches focus on single goal-driven trajectory optimization with simplified dynamics models~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex}, limiting their adaptability for our framework's generalizable tracking controller. Thus, we primarily compare our method with model-free approaches: 1) DGrasp~\citep{christen2022d}: Adapted to track by dividing sequences into subsequences of 10 frames, with each subsequence solved incrementally. 2) PPO (OmniGrasp rew.): We re-implemented OmniGrasp's reward~\citep{Luo2024GraspingDO} to train a policy for tracking object trajectories. 3) PPO (w/o sup., tracking rew.): We trained a policy using PPO with our proposed tracking reward and observation design.
% To the best of our knowledge, no prior model-based methods have specifically addressed tasks identical or comparable to the tracking control for dexterous manipulation. 
% Most existing approaches are constrained to single goal-driven trajectory optimization~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex} with a simplified dynamics model, making them difficult to adapt for optimizing a versatile tracking controller as required by our framework.
% Therefore, we primarily compare our method against model-free approaches: 1) DGrasp~\citep{christen2022d}: We adapt DGrasp to address the tracking problem by dividing the entire sequence into several subsequences, each consisting of 10 frames. The last frame of each subsequence is defined as its reference frame. This transforms each subsequence tracking task into a solvable problem for DGrasp. We then train a policy to incrementally solve each subproblem. 2) PPO (OmniGrasp rew.): OmniGrasp proposes a universal controller for grasping objects from a table and following the given object trajectory. Since the original implementation has not been open-sourced, we re-implemented the reward as described in the paper~\citep{Luo2024GraspingDO}. Using this reward and PPO, we train a policy aimed at tracking each training trajectory. 3) PPO (w/o sup., tracking rew.): We directly train a policy using PPO and our proposed tracking reward, along with our observation design (see Section~\ref{sec:method_il_rl}). 
% To our best knowledge, there is no previous model-based methods aiming to solve the task same or similar to our dexterous manipulation tracking control. Most of them are restricted in single goal-driven trajectory optimization~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex} which is hard to be adapted to align with our goal of  optimizing a tracking controller.
% which does not and can hardly be adapted to align with our goal in optimizing a tracking controller. 

% Therefore, we mainly compare model-free approaches: 1) DGrasp~\citep{christen2022d}. We adapt DGrasp to solve the tracking problem. We divide the whole sequence into several subsequences with a length of 10 frames. We then define the last frame of each subsequence as its reference frame. After that, each subsequence tracking becomes a problem that DGrasp can solve. We then train a policy to solve each subproblem gradually. 2) PPO (OmniGrasp rew.). OmniGrasp proposes a universal controller for grasping objects from the table and following the given object trajectory. Since it has not been open-sourced yet, we re-implement the reward as described in the paper~\citep{Luo2024GraspingDO}. We then train a policy using the reward and PPO, with the goal of tracking each trajectory in the training dataset. 3) PPO (w/o sup., tracking rew.). We directly train a policy using PPO and our proposed tracking reward as well as the observation design (see Equation~\ref{eq:observations}~\ref{eq:rew_obj}~\ref{eq:rew_hand}~\ref{eq:rew_affinity}). 

% Since in the tracking phase, 

% We re-implement the reward as described in the paper~\citep{Luo2024GraspingDO}. A PPO is trained 
% divide the whole sequence into several subsequences, each of which has 10 frames, and define the end frame of the subsequence as the reference frame. Then the grasping policy is used to guide the hand and gradually track the object according to the hand and the object pose of each reference frame. 
% We compare our method with previous model-free approaches. 
% omni grasp reward o not considerthe 



\noindent\textbf{Training and evaluation settings.} 
% The training process involves three stages, each using different tracking demonstrations. 
We use PPO~\citep{Schulman2017ProximalPO}, implemented in {rl\_games}~\citep{rlgames2021}, with Isaac Gym~\citep{makoviychuk2021isaac} for simulation. Training is performed with 8192 parallel environments for both the per-trajectory tracker and the tracking controller. For the dexterous hand, the position gain and damping coefficient are set to 20 and 1 per finger joint. Evaluation results are averaged across 1000 parallel environments, and for real-world evaluations, we use LEAP~\citep{Shaw2023LEAPHL} with a Franka arm and FoundationPose~\citep{Wen2023FoundationPoseU6} for object state estimation. Additional details are provided in Appendix~\ref{sec:supp_exp_details}.
% for the tracking controller 
% without transferring weights between models.
% The training process for the tracking controller consists of three stages, as outlined in the method section. In each stage, we retrain the model using different labeled datasets, without transferring weights from the previous model.  We use PPO~\citep{Schulman2017ProximalPO}, implemented in {rl\_games}~\citep{rlgames2021}, as our reinforcement learning algorithm. Isaac Gym~\citep{makoviychuk2021isaac}, a widely-used simulated physical environment, is utilized for training. We employ 8192 parallel environments to train both the per-trajectory tracker and the tracking controller. For the articulated dexterous hand, the position gain and damping coefficient are set to 20 and 1, respectively, for each finger joint. During the evaluation phase, we average evaluation results obtained in 1000 parallel execution environments as the final result.  For real-world evaluations, we use LEAP~\citep{Shaw2023LEAPHL} with Franka arm. We use FoundationPose~\citep{Wen2023FoundationPoseU6} to estimate the object states. 
% Further details, such as the simulation environment and the real setup, are provided in Appendix~\ref{sec:supp_exp_details}. 
% During the evaluation phase, we sample the policy 1000 times across 1000 parallel execution environments and average the metrics to obtain the evaluation result for the current trajectory. 

% such as the simulation  setup, are provided in Appendix~\ref{sec:supp_exp_details}. 
% including the simulation environment setup, 
% This is because we found that transferring weights makes the model more difficult to train, rather than speeding up the training process.
% The tracking controller training is composed of three stages as we detailed in the method section. In each stage, we re-train the model with different labeled datasets without transferring weights from the previously trained model. It is because we observe that weight transferring would make the model even harder to train, other than accelerating the training process. We leverage PPO~\citep{Schulman2017ProximalPO} implemented in {rl\_games}~\citep{rlgames2021} as our RL algorithm. We use the widely appreciated Isaac Gym~\citep{makoviychuk2021isaac} as the simulated physical environment. We use 8192 parallel environments to train both the per-trajectory tracker and the tracking controller. For articulated dexterous hands, the position gain and the damping coefficient are set to 20 and 1 respectively for each finger joint. During the evaluation phase, we sample from the policy 1000 times (using 1000 parallel execution environments) and average their metrics as the evaluation result of the current trajectory. More details such as the simulation environment setting are deferred to Appendix~\ref{sec:supp_exp_details}. 
% For both the per-trajectory tracker and the tracking controller, 
% the single trajectory specialist tracking policy training and the general tracking policy optimization, we use 8192 parallel environments to train RL. 






% take the widely appreciated Isaac Gym as our simulated environment where we train our 


% rich and changing contacts, j
\vspace{-5pt}
% \subsection{Generalizable Dexterous Manipulation Tracking Control } \label{sec:exp_results}
\subsection{Generalizable Tracking Control for Dexteroous Manipulation } \label{sec:exp_results}
\vspace{-5pt}


% \todo{add the time consumption}

\begin{figure}[ht]
  \centering
  \vspace{-10pt}
  \includegraphics[width=\textwidth]{figs/robustness_noise.pdf}
  \vspace{-20pt}
  \caption{\footnotesize
  \textbf{Robustness w.r.t. unreasonable states. }
  Please check \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{video}}}} for animated results.
  % ~\eric{the subsection title has been occluded by the figure... please adjust.}
  }
  \label{fig_res_robustness}
  \vspace{-10pt}
\end{figure}

% \todo{change the w/o prior, w/o curri. to w/o data, w/o structure}

\begin{figure}[ht]
  \centering
  % \vspace{-10pt}
  % \includegraphics[width=\textwidth]{figs/res_5.pdf}
  \includegraphics[width=\textwidth]{figs/eval_res_all_v2.pdf}
  % \vspace{-20pt}
  \caption{\footnotesize
  \textbf{Qualitative comparisons. }
  Please check \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
  }
  \label{fig_res}
  \vspace{-10pt}
\end{figure}




% \begin{table*}[t]
%     \centering
%     \caption{ 
%     \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
%     } 
%     % \vspace{-10pt}
%     \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{@{\;}llccccc@{\;}}
%         \toprule
%         %         
%         Dataset & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

        
%         \cmidrule(l{0pt}r{1pt}){1-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}

%         % \multirow{5}{*}{ GRAB } & ControlVAE & - & -  & -  & - 
%         % \\ 
%         % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         % \\ 
%         % % \cmidrule(l{15pt}r{17pt}){3-9}

%         % % \cmidrule(l{15pt}r{17pt}){3-9}
%         % \cmidrule(l{1pt}r{1pt}){2-3}
%         % % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         \multirow{2}{*}{ GRAB } & DGrasp & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (w/o sup., tracking rew.)  & 0.3945 & 6.11  & 0.1076 & 0.5899 & 38.78/55.05/60.58 
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){2-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}
        
        
%         % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         % \\ 
%         ~ & \model~(w/ sup.)  & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         \\ 
%         ~ & \model~(w/ sup., w/ curriculum)  & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         \\ 
%         ~ & \model  & \bred{0.3303} & \bred{4.53} & {0.1118} & \bred{0.5048} & \bred{47.12}/\bred{65.52}/\bred{72.41}
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){1-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}


%         % \multirow{5}{*}{ TACO } & ControlVAE & - & -  & -  & - 
%         % \\ 
%         % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         % \\ 
%         % % \cmidrule(l{15pt}r{17pt}){3-9}

%         % % \cmidrule(l{15pt}r{17pt}){3-9}
%         % \cmidrule(l{1pt}r{1pt}){2-3}
%         % % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
%         % \\ 

%         \multirow{2}{*}{ TACO } & DGrasp & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (Tracking rew.)  & 0.4815 & 7.82  & 0.1195  & 0.4682 & {35.13}/{47.69}/61.54
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){2-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}
%         % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
%         % \\ 
%         ~ & \model~(w/ sup.)  &  0.4444 & 2.33  & 0.1782  & 0.5438 & 47.97/67.12/73.66
%         \\ 
%         ~ & \model~(w/ sup., w/ curriculum)  & {0.4854} & {1.99} & { 0.1298} & {0.4772} & 54.90/72.55/79.74
%         \\ 
%         ~ & \model & {0.4953} &  {2.10} & {0.1510} & {0.4661} & \bred{49.02}/\bred{74.50}/\bred{81.05}
%         \\ 

%         \bottomrule
 
%     \end{tabular}
%     }
%     \vspace{-10pt}
%     \label{tb_exp_main}
% \end{table*} 



% \todo{change the w/o prior, w/o curri. to w/o data, w/o structure}
\begin{table*}[t]
    \centering
    \caption{ 
    \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
    } 
    % \vspace{-10pt}
    \resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{\;}llccccc@{\;}}
        \toprule
        %         
        Dataset & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$) \\

        
        \cmidrule(l{0pt}r{1pt}){1-2}
        \cmidrule(l{2pt}r{2pt}){3-7}

        

        % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
        % \\ 
        \multirow{6}{*}{ GRAB } & DGrasp & 0.4493 & 6.75  & 0.1372  & 0.6039 & 34.52/52.79
        \\ 
        ~ & PPO (OmniGrasp rew.) & 0.4404 & 6.69  & 0.1722 & 0.6418  & 35.53/54.82
        \\ 
        ~ & PPO (w/o sup., tracking rew.)  & 0.3945 & 6.11  & \bred{0.1076} & 0.5899 & 38.58/54.82 % & 
        \\ 
        
        \cmidrule(l{0pt}r{1pt}){2-2}
        \cmidrule(l{2pt}r{2pt}){3-7}
        
        
        % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
        % \\ 
        % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
        % \\ 
        ~ & \model~(w/o data, w/o homotopy)  & {0.3443} & {7.81} & {0.1225} & \iblue{0.5218} & 39.59/57.87 
        \\ 
        ~ & \model~(w/o data)  & \iblue{0.3415} & \iblue{4.97} & { 0.1483} & {0.5264} & \iblue{43.15}/\iblue{62.44} % 
        \\ 
        ~ & \model  & \bred{0.3303} & \bred{4.53} & \iblue{0.1118} & \bred{0.5048} & \bred{46.70}/\bred{65.48} 
         \\ 
        
        \cmidrule(l{0pt}r{1pt}){1-2}
        \cmidrule(l{2pt}r{2pt}){3-7}


        % \multirow{5}{*}{ TACO } & ControlVAE & - & -  & -  & - 
        % \\ 
        % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
        % \\ 
        % % \cmidrule(l{15pt}r{17pt}){3-9}

        % % \cmidrule(l{15pt}r{17pt}){3-9}
        % \cmidrule(l{1pt}r{1pt}){2-3}
        % % \cmidrule(l{2pt}r{2pt}){8-12}


        % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
        % \\ 
        % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
        % \\ 
        % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
        % \\ 

        \multirow{6}{*}{ TACO } & DGrasp & 0.5021 & 5.04  & \bred{0.1129}  &  0.4737 & 38.42/47.78
        \\ 
        ~ & PPO (OmniGrasp rew.) & 0.5174 & 5.43  & 0.1279  & 0.4945 & 33.5/46.31
        \\ 
        ~ & PPO (w/o sup., tracking rew.)  & \iblue{0.4815} & 4.82  & \iblue{0.1195}  & \iblue{0.4682} & {34.98}/{57.64} 
        \\ 
        
        \cmidrule(l{0pt}r{1pt}){2-2}
        \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){8-12}
        % \cmidrule(l{2pt}r{2pt}){1-2}
        % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
        % \\ 
        % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
        % \\ 
        ~ & \model~(w/o data, w/o homotopy)  &  \bred{0.4444} & 2.33  & 0.1782  & 0.5438 & 44.83/67.00
        \\ 
        ~ & \model~(w/o data)  & {0.4854} & \iblue{2.21} & { 0.1698} & {0.4772} & \iblue{47.78}/\iblue{72.41}
        \\  
        ~ & \model & {0.4953} &  \bred{2.10} & {0.1510} & \bred{0.4661} & \bred{48.77}/\bred{74.38}
        \\ 

        \bottomrule
 
    \end{tabular}
    }
    \vspace{-10pt}
    \label{tb_exp_main}
\end{table*} 


% \todo{do not claim the efficiency and jmove the timeconsumption to the appendix}



% \begin{table*}[t]
%     \centering
%     \caption{ 
%     \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
%     } 
%     % \vspace{-10pt}
%     \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{@{\;}lllccccc@{\;}}
%         \toprule
%         %         
%         Dataset & ~ & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

        
%         \cmidrule(l{0pt}r{1pt}){1-3}
%         \cmidrule(l{2pt}r{2pt}){4-8}

%         \multirow{5}{*}{ GRAB } & \multirow{2}{*}{ \makecell[c]{Model \\ Based} } & ControlVAE & - & -  & -  & - 
%         \\ 
%         ~ & ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         \\ 
%         % \cmidrule(l{15pt}r{17pt}){3-9}

%         % \cmidrule(l{15pt}r{17pt}){3-9}
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         ~ & \multirow{2}{*}{ \makecell[c]{Model \\ Free} }  & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & ~ & PPO (Tracking rew.)  & 0.3945 & 6.11  & 0.1076 & 0.5899 & 38.78/55.05/60.58 
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}

%         % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         % \\ 
%         ~ & ~ & Ours  & \bred{0.3303} & \bred{4.53} & {0.1118} & \bred{0.5048} & \bred{47.12}/\bred{65.52}/\bred{72.41}
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){1-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}


%         \multirow{5}{*}{ TACO } & \multirow{2}{*}{ \makecell[c]{Model \\ Based} } & ControlVAE & - & -  & -  & - 
%         \\ 
%         ~ & ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         \\ 
%         % \cmidrule(l{15pt}r{17pt}){3-9}

%         % \cmidrule(l{15pt}r{17pt}){3-9}
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
%         % \\ 

%         ~ & \multirow{2}{*}{ \makecell[c]{Model \\ Free} }  & PPO (OmniGrasp rew.) & - & -  & -  & - 
%         \\ 
%         ~ & ~ & PPO (Tracking rew.)  & 0.4815 & 10.11  & 0.1195  & 0.4682 & {5.13}/{5.13}/61.54
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}
%         % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
%         % \\ 
%         ~ & ~ & Ours & {0.4953} &  {2.10} & {0.1510} & {0.4661} & \bred{49.02}/\bred{74.50}/\bred{81.05}
%         \\ 

%         \bottomrule
 
%     \end{tabular}
%     }
%     \vspace{-10pt}
%     \label{tb_exp_main}
% \end{table*} 




% \begin{figure}[h]
%   \centering
%   % \vspace{-10pt}
%   \includegraphics[width=\textwidth]{figs/res.pdf}
%   % \vspace{-20pt}
%   \caption{
%   \textbf{Qualitative comparisons. }
%   Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig_res_bak}
%   % \vspace{-10pt}
% \end{figure}




% \begin{wraptable}[6]{r}{0.5\textwidth}
% \vspace{-30pt}
%     \centering
%     \caption{ 
%     % \textbf{Ablation studies} on the GRAB dataset. 
%     Total training time consumption (GRAB dataset). 
%     } 
%     % \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccc@{\;}}
%         \toprule
%         ~ & \makecell[c]{PPO \\ (w/o sup)} & \makecell[c]{Ours \\ (w/ sup.)}  & \makecell[c]{Ours \\ (w/ sup., \\ w/ curri.)} & Ours   \\

%         \midrule % 

%         Time  &  $\sim$1 day & $\sim$4.5 days & $\sim$9 days & $\sim$5 days
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_exp_timeconsumption}
% \end{wraptable}





% decompose 

% \todo{which card and the hardware settings}

% We demonstrate the generalization ability of our tracking controller to unseen trajectories involving difficult manipulations and novel, thin objects. Our controller has no difficulty in dealing with very intricate motions involving thin objects, subtle in-hand re-orientations, and expressive functional manipulations. As presented in Table~\ref{tb_exp_main}, we can achieve significantly higher success rates calculated under two thresholds than the best-performed baseline in both two datasets. Figure~\ref{fig_res} illustrates qualitative examples and comparisons. Please check out our website and video for animated results. 
We demonstrate the generalization ability and robustness of our tracking controller on unseen trajectories involving challenging manipulations and novel, thin objects. Our controller has no difficulty in handling intricate motions, subtle in-hand re-orientations, and expressive functional manipulations, even when dealing with thin objects. 
As shown in Table~\ref{tb_exp_main}, we achieve significantly higher success rates, calculated under two different thresholds, compared to the best-performing baseline across both datasets. Figure~\ref{fig_res} provides qualitative examples and comparisons. We show the real-world effectiveness of our method and the superiority over best-performing baselines (Figure~\ref{fig_res},Table~\ref{tb_real_world_results}). For animated results, please visit our \href{https://projectwebsite7.github.io/gene-dex-manip/}{project website} and the \href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{accompanying video}.
% in two HOI datasets. Empowered by xxx, our policy can generalize well and robustly track challenging manipulations unseen during training. Most impressively and perhaps even surprising to us, our policy has no difficulty in dealing with very intricate motions involving thin objects, subtle in-hand re-orientations, and expressive functional manipulations. 



% \textcolor{red}{(TODO: cross-object generalization test? and that should be delivered in a small table)}


% \noindent\textbf{Expressive and functional motions with subtle in-hand re-orientations.} 

\noindent\textbf{Intriguing in-hand manipulations.}
% Expressive motions with s
% ubtle in-hand manipulations.} 
Our method effectively generalizes to novel, complex, and challenging functional manipulations, featured by subtle in-hand re-orientations, essential for precise tool-use tasks. For instance, in Figure~\ref{fig_res}a, the shovel is lifted, tilted, and reoriented with intricate finger movements to complete a {stirring} motion. Similarly, in Figure~\ref{fig_res}c, the small shovel is reoriented using minimal wrist adjustments. These results demonstrate the robustness and generalization of our controller, outperforming the PPO baseline, which struggles with basic lifting. 
% tasks like lifting thin tools.
% including
% complex object movements and 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method effectively generalizes to unseen, challenging manipulations that involve complex functional object movements and subtle in-hand re-orientations, which are crucial for achieving precise reorientations during tool-use tasks. For example, in Figure~\ref{fig_res}a, the shovel must first be lifted with the inner side facing down, then tilted so the inner part faces upward, while the fingers control the handle to complete a \texttt{stirring} motion. Our results nearly achieve this goal, despite the intricate finger movements required to re-orient the object.
% In Figure~\ref{fig_res}c, the trajectory demands that the small shovel be re-oriented to face right so it can be used to hold things. Although our method initially lifts the shovel with the inner side facing left (as shown in the third frame), it successfully re-orients the tool using detailed finger adjustments, with minimal change in wrist orientation (as shown in the fourth frame).
% These results highlight the robust performance and exceptional generalization ability of our controller. In contrast, the best-performing baseline, PPO (w/o sup.), which attempts to train a general controller using our designed rewards, struggles even with basic tasks like lifting thin tools from the table.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalizes well to unseen challenging manipulations involving complex functional object movements, and detailed and subtle in-hand re-orientations that are crucial to achieve correct orientations for accurately mimicking tool-using motions. In Figure~\ref{fig_res}a, the shovel should be lifted at first with the inner side facing towards and then tiled down with the inner part facing upwards and fingers controlling the handle to complete the \texttt{stirring} motion. Our results can almost fulfill the goal despite the need to use detailed finger movements to re-orient the object. As demonstrated in Figure~\ref{fig_res}c, the trajectory requires the hand to make the small shovel face towards the right side so that it can use it to hold things. Despite the fact that our method manage to lift the object up from the table with the object facing towards the left side (shown in the third frame), it can then successfully re-orient the small shovel so that it faces towards the right side mainly using fingers without varying the wrist orientation a lot (as shown in the forth frame). 
% These great performance convincingly demonstrate the strong capability and notable generalization ability of our controller. 
% In comparison to ours' adeptly tracking functional interactions, the best-performed baseline PPO (w/o sup.), which attempts to directly train a general controller using PPO with our carefully designed rewards but without additional guidance, even faces challenges in lifting such thin tools up from the table. 
% However xxx (baseline methods). \todo{baseline's performance}
% Such tool using method demonstrates the high generalizable dexterity enabled by our general tracker. 



% \begin{wraptable}[5]{r}{0.6\textwidth}
% \vspace{-23pt}
%     \centering
%     \caption{ 
%     % \textbf{Ablation studies} on the GRAB dataset. 
%     % \textbf{Generalization ability evaluations} on the TACO dataset. 
%     % \textbf{Gen} on the TACO dataset. 
%     \footnotesize
%     Generalizability evaluations on the TACO dataset. 
%     } 
%     \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{@{\;}lccccc@{\;}}
%         \toprule
%         Test set & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

%         % \\
%         \midrule % 


%         % \\
%         % \cmidrule(l{15pt}r{17pt}){2-4}
        
%         % \model (w/o SpatialDiff) & 2.94 & 3.45  & 31.67
%         % \\ 

%         % \model (w/o TemporalDiff) & \bred{1.72} & \bred{1.90} & 34.25 % 18.65 %
%         % \\

%         % \model (w/o Diffusion) & 3.16 & 3.83  & 18.65 

%         % S0 & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\
        
%         S1 & 0.5787 & {2.43} & {0.1481} & {0.4703} & 35.97/67.63
%         \\ 

%         % 
%         % \model (w/o Canon.) & {2.36} & {3.57} & \iblue{13.26}
%         S2 & {0.6026} & {2.46} & { 0.1455} & {0.4709} & 30.83/65.00
%         \\ 

%         S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % }
%     % \vspace{-16pt}
%     \label{tb_exp_taco_generalization_test}
% \end{wraptable}



\noindent\textbf{Intricate manipulations with thin objects. } 
Our method also generalizes well to challenging manipulations involving thin objects. In Figure~\ref{fig_res}b, despite the thin \texttt{shovel}'s complexity and missing CAD model parts, our method successfully lifts and controls it using a firm grasp with the second and third fingers. Similarly, in Figure~\ref{fig_res}e, our controller adeptly lifts and manipulates a thin \texttt{flute}, while the best-performing baseline struggles with the initial grasp. These results highlight the advantages of our approach in handling complex and delicate manipulations.
% that are difficult to grasp and control. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalizes effectively to unseen, challenging manipulations involving extremely thin objects that are both difficult to grasp and control. As shown in Figure~\ref{fig_res}b, the shovel is extremely thin, with some triangles missing from the CAD model, which adds to the complexity. Additionally, controlling such a long and thin object from the end further increases the difficulty. Despite these challenges, our method performs well, successfully lifting the object using the second and third fingers while maintaining a firm grip to follow the trajectory, even with this unconventional grasping pose.
% In the scenario depicted in Figure~\ref{fig_res}e, the task involves lifting a notably thin flute from the table and manipulating it. Our controller demonstrates remarkable proficiency in interacting with such objects. In contrast, the best-performing baseline struggles significantly during the initial grasping phase, highlighting the advantages of our approach in handling complex and delicate manipulations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalize well to unseen challenging manipulations involving extremely thin objects that are both difficult to grasp and control. As demonstrated in Figure~\ref{fig_res}b, the shovel is very thin here even with some triangles missing from the CAD model. Besides, controlling such a long and thin object from the end side further adds huge difficulties. Despite such challenges, our method can still generalize well and achieve good performance in this case. It manages to lift the object up using the second and the third fingers and control the hand to firmly hold the objects to follow its trajectory, using this unfriendly grasping pose. 
% In the case drawn in Figure~\ref{fig_res}f, the challenging task involves lifting an extremely thin flute from the table and playing with it. Our controller has no difficulty in interacting with this kind of object. 
% In comparison, the best-performed baseline faces significant challenges in the initial grasping stage. 
% Our controller can even perform robustly in this unfriendly grasping pose, controlling the hand to firmly hold the object and follow its trajectory. 

% complex object movements, extremely thin objects that are very difficult to grasp
% has no difficult in resolving challenging manipulation

% \begin{wrapfigure}[6]{r}{0.45\textwidth} % {0pt}
% \vspace{-4ex}
% \includegraphics[width = 0.45\textwidth]{./figs/real_eval_figs.pdf}
% \vspace{-24pt}
%     \caption{\footnotesize
%     Qualitative results in the real world.
%     }
%     \label{fig:fig_real_eval_figs}
% \vspace{-20pt}
% \end{wrapfigure}


% \todo{add this part}







\begin{table*}[t]
    \centering
    \caption{ \footnotesize
    \textbf{Real-world quantitative comparisons.}  \bred{Bold red} numbers for best values.
    % and \iblue{italic blue} values for the second best-performed ones. 
    } 
    % \vspace{-10pt}
        \resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{\;}lcccccccccc@{\;}}
        \toprule
       Method & \texttt{apple} & \texttt{banana} & \texttt{duck}  & \texttt{elephant} & \texttt{flashlight}    & \texttt{flute}   & \texttt{hammer}  & \texttt{hand}  & \texttt{phone}  & \texttt{waterbottle}     \\

        % \\
        \midrule % 

        PPO (w/o sup., tracking rew) & 0/0/0 & 25.0/25.0/0.0 & 50.0/25.0/0 & 50.0/0.0/0.0 & 50.0/0/0 & 0/0/0 & 25.0/0/0 & 66.7/33.3/0 & 25.0/0/0 & 33.3/33.3/0
        \\ 

        % 
        \model & \bred{25.0}/0/0 & \bred{50.0}/\bred{50.0}/\bred{25.0} & \bred{75.0}/\bred{50.0}/\bred{25.0} & \bred{75.0}/\bred{50.0}/\bred{50.0} & \bred{50.0}/\bred{25.0}/\bred{25.0}  & \bred{25.0}/\bred{25.0}/\bred{25.0} & \bred{50.0}/\bred{50.0}/\bred{50.0} & \bred{66.7}/\bred{33.3}/\bred{33.3} & \bred{50.0}/\bred{50.0}/\bred{25.0} & \bred{50.0}/\bred{33.3}/\bred{33.3} 
        \\ 

        % S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
        % \\ 
        
        \bottomrule
 
    \end{tabular}
    }
    \vspace{-20pt}
    \label{tb_real_world_results}
\end{table*} 

% % \begin{wraptable}[5]{r}{0.6\textwidth}
% \begin{table*}[t]
% \vspace{-23pt}
%     \centering
%     \caption{ 
%     \footnotesize
%     Generalizability evaluations on the TACO dataset. 
%     } 
%     \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccccccccc@{\;}}
%         \toprule
%        Method & apple & banana & duck  & elephant & flashlight    & flute   & hammer  & hand  & phone  & waterbottle     \\

%         % \\
%         \midrule % 

        
%         PPO (w/o sup., tracking rew) & 0.5787 & {2.43} & {0.1481} & {0.4703} & 35.97/67.63
%         \\ 

%         % 
%         % \model (w/o Canon.) & {2.36} & {3.57} & \iblue{13.26}
%         \model & {0.6026} & {2.46} & { 0.1455} & {0.4709} & 30.83/65.00
%         % \\ 

%         % S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
%         % \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_real_world_results}
% % \end{wraptable}
% \end{table*}


% \begin{figure}[ht]
%   \centering
%   \vspace{-10pt}
%   \includegraphics[width=0.8\textwidth]{figs/real_exp_cmp_3.pdf}
%   \vspace{-20pt}
%   \caption{\footnotesize
%   \textbf{Qualitative real-world evaluations and comparisons. }
%   % Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig:fig_real_eval_figs}
%   \vspace{-10pt}
% \end{figure}


\noindent\textbf{Real-world evaluations and comparisons.} 
% We transfer tracking results directly to the real world to assess tracking quality and also transfer the state-based controller to evaluate its robustness to noises in the state estimator. Success rates are measured under three thresholds and compared with the best baseline. Table~\ref{tb_real_world_results} summarizes per-object success rates averaged over their manipulation trajectories (transferred controller setting). Demonstrated in Figure~\ref{fig_res}f~\ref{fig_res}g, we enable the robot to track complex object movements in real-world scenarios. Further details are in Appendix~\ref{sec:supp_real_world}.
We directly transfer tracking results to the real world to assess tracking quality and evaluate the robustness of the state-based controller against noise in the state estimator. Success rates are measured under three thresholds and compared with the best baseline. Table~\ref{tb_real_world_results} summarizes the per-object success rates averaged over their manipulation trajectories in the transferred controller setting. As demonstrated in Figures~\ref{fig_res}f and \ref{fig_res}g, we enable the robot to track complex object movements and successfully lift a hard-to-grasp round apple in real-world scenarios. While the baseline fails. Further details can be found in Appendix~\ref{sec:supp_real_world}.

% We transfer tracking results directly to the real world to assess tracking quality and evaluate the robustness of the state-based tracker to noise in the state estimator. We measure success rates under three success thresholds for both settings and compare them with the best-performing baseline. Table~\ref{tb_real_world_results} summarizes the performance of the transferred tracker. We report per-object success rates averaged over their corresponding manipulation trajectories. As shown in Figure~\ref{fig_res}f,g, our method enables the robot to successfully track complex object movements in real-world scenarios. Additional details and results are provided in Appendix~\ref{sec:supp_real_world}.
% reports the 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We directly transfer tracking results to the real world to demonstrate the tracking quality and also transfer the state-based tracker to the real world to evaluate its robustness to noises in the state estimator. We evaluate the success rate under three types of success thresholds for both settings and compare it with the best-performed baseline method. Values reported in Table~\ref{tb_real_world_results} are the per-object success rate averaged over their corresponding manipulation trajectories, achieved via the transferred tracker. As shown in Figure~\ref{fig_res}f,g, our results executed in the real world can successfully let the robot track difficult manipulations with complex object movements. More details and results are deferred to the Appendix~\ref{sec:supp_real_world}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% success rate of each object averaged over the number of manipulation trajectories, 
% and evaluate the success rate. Moreover, we also transfer the state-based tracker to the real world to evaluate its robustness to noises in the state estimator. 




\vspace{-5pt}
\subsection{Further Analysis and Discussions} \label{sec:exp_analysis}
\vspace{-5pt}


\noindent\textbf{Robustness to noise in the kinematic reference motions.} 
% Our method is robust to significant kinematic noise. 
Despite severe hand-object penetrations in Figure~\ref{fig_res}c (frames 2 and 3) and Figure~\ref{fig_res}a (frame 2), the hand still interacts effectively with the object, highlighting the resilience of our tracking controller in challenging scenarios.
% Our method is robust to significant noise in the kinematic motions. For example, even with severe hand-object penetrations occurring in the motions depicted in Figure~\ref{fig_res}c (in the second and third frames) and Figure~\ref{fig_res}a (in the second frame), we can still effectively control the hand to interact correctly with the object. This resilience underscores the effectiveness of our tracking controller in handling challenging scenarios.
% We would not be affected by obvious noise in the kinematic motions. For instance, although there are severe hand-object penetrations in the motion shown in Figure~\ref{fig_res}c (the second and the third frame) and Figure~\ref{fig_res}a (the second frame), we can successfully control the hand to correctly interact with the object. 



% \begin{figure}[ht]
%   \centering
%   \vspace{-10pt}
%   \includegraphics[width=\textwidth]{figs/robustness_2.pdf}
%   \vspace{-20pt}
%   \caption{
%   \textbf{Robustness towards unreasonable references and novel object categories. }
%   Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig_res_robustness}
%   \vspace{-10pt}
% \end{figure}





\noindent\textbf{Robustness to unreasonable references. }
As shown in Figure~\ref{fig_res_robustness}, our method remains unaffected by significant noise in the kinematic references with unreasonable states.
% , even when they include unreasonable or unreachable states.
We effectively track the entire motion trajectory, demonstrating the controller's robustness in handling unexpected noise.
% As shown in Figure~\ref{fig_res_robustness}a, our method remains unaffected by significant noise in the kinematic references, even when they include unreasonable or unreachable states. We can effectively track the entire motion trajectory despite these challenges, demonstrating our controller's robustness in handling unexpected noise. 
% The kinematic reference trajectory is obtained by interpolating a different trajectory from the TACO dataset, demonstrating our controller's robustness in handling complex and noisy inputs.
% As demonstrated in Figure~\ref{fig_res_robustness}a, we would not be affected by the large noise in the kinematics references containing unreasonable and unreachable states and can still manage to track the whole motion trajectory. The kinematic reference trajectory is obtained by interpolating a different trajectory with a sequence from TACO. 
% \todo{xxx}




% \noindent\textbf{Further generalization ability evaluations.}
% We further evaluate the model's generalization ability across various test sets within the TACO dataset. As shown in Table~\ref{tb_exp_taco_generalization_test}, the controller performs well in the category-level generalization setting (S1), where object categories are known but manipulation trajectories and object geometries are novel. Performance on S2, involving novel interaction triplets, is satisfactory, demonstrating the controller's capacity to handle new manipulation sequences. However, results from S3 reveal challenges when dealing with new object categories and unseen interaction triplets. For instance, generalizing from interactions with shovels and spoons to using bowls for holding objects is particularly difficult. As shown in Figure~\ref{fig_res_robustness}b, despite unfamiliar objects and interactions, we successfully lift the knife and mimic the motion, though execution is imperfect, highlighting areas for improvement and adaptability in challenging scenarios.

% We further evaluate the model's generalization ability across different levels of test sets within the TACO dataset. As shown in Table~\ref{tb_exp_taco_generalization_test}, the controller performs well in the category-level generalization setting, where the object category is known during training, but the manipulation trajectories and object geometries are novel, as evidenced by its strong performance on test set S1.
% The performance on S2, which involves novel interaction triplets, remains relatively satisfactory, demonstrating the controller's capacity to generalize to new manipulation sequences. However, results from S3 highlight the challenges faced when dealing with novel object categories and unseen interaction triplets. For instance, generalizing from interactions that involve lifting and waving shovels and spoons to using bowls for holding objects proves to be too difficult for the current design. 
% As illustrated in Figure~\ref{fig_res_robustness}b, despite the unfamiliar object category and interaction triplet, we still manage to lift the knife and mimic the intended motion, although the execution is not perfect. This indicates potential areas for improvement while showcasing the model's adaptability in challenging scenarios.

% We further test the model's generalization ability on different levels of test sets on the TACO dataset. As indicated in Table~\ref{tb_exp_taco_generalization_test}, the controller can perform well in the category-level generalization setting, where the object category is observed during the training while the manipulation trajectories and the object geometry are novel, as indicated by its good performance in the test set S1. 
% The performance on S2 contains novel interaction triples is still relatively satisfactory, indicating its ability to generalize to control novel manipulation sequences. However, results on S3 indicate the model's being challenged by novel object categories and unseen interaction triplets. Generalizing from interactions demonstrating lifting and waving shovels and spoons to using bowls to hold things is still too challenging for the current design. As shown in Figure~\ref{fig_res_robustness}b, given the unobserved object category and the interaction triplet, though not perfect, we can still manage to lift the knife up and mimic the motion. 
% \todo{add the qualitative evals}
% The object position error is still kept to a small value, indicating 

% Specifically, the whole dataset is split into a training dataset, containing 1565 trajectories, and the test set S0 where both the tool object geometry and the interaction triplets are seen during training, the test set S1 where the tool geometry is novel but the interaction triplets are seen during training, the test set S2 with novel interaction triplets but seen object categories and geometries, and the test set S4 with new object geometries and interaction triplets. Details w.r.t. the dataset splitting and visualizations are deferred to Appendix~\ref{}. 

% \begin{wraptable}[6]{r}{0.5\textwidth}
% \vspace{-30pt}
%     \centering
%     \caption{ 
%     Total training time consumption (TACO dataset). 
%     } 
%     % \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccc@{\;}}
%         \toprule
%         ~ & \makecell[c]{PPO \\ (w/o sup)} & \makecell[c]{Ours \\ (w/ sup.)}  & \makecell[c]{Ours \\ (w/ sup., \\ w/ curri.)} & Ours   \\

%         \midrule % 

%         Time  &  $\sim$1 day & $\sim$5 days & $\sim$13 days & $\sim$4 days
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_exp_timeconsumption}
% \end{wraptable}


% \noindent\textbf{Time consumption.} Table~\ref{tb_exp_timeconsumption} summarizes the total time consumption of different methods on the TACO dataset. Directly training PPO without any supervision is the most efficient approach while the performance lagged behind due to no proper guidance. Exact curriculum learning for acquiring high-quality per-trajectory trackers, though as we observe in Table~\ref{tb_exp_main}, is an effective strategy, which also aligns with conclusions in previous approaches, is extremely time-consuming. For 400 trajectories that we finally select to optimize to produce an action-labeled dataset, searching the exact curriculum costs about 13 days to complete. However, our method requires only slightly more time than the version without tracking prior or curriculum scheduling (Ours w/ sup.). However we can achieve a much higher success rate than this version, taking advantage of the increased diversity and the quality of action-labeled data. 




\vspace{-5pt}
\section{Ablation Studies} 
\vspace{-5pt}


\noindent\textbf{Diversity and quality of robot tracking demonstrations.} 
We propose enhancing the diversity and quality of tracking demonstrations using the tracking controller and homotopy generator. We ablate these strategies by creating two variants: ``Ours (w/o data, w/o homotopy)'', where the dataset is built by optimizing each trajectory without prior knowledge, and ``Ours (w/o data)'', which uses only the homotopy optimization scheme to improve demonstrations. Despite using the same number of demonstrations, both variants produce lower-quality data. As shown in Table~\ref{tb_exp_main}, they underperform compared to our full method, underscoring the importance of data quality in training the controller.
% We propose to improve the diversity and the quality of the robot tracking demonstrations via the tracking controller and the homotopy generator. We ablate these two strategies by creating two variants: ``Ours (w/o data, w/o homotopy)'', where the dataset is built by directly optimizing each trajectory without prior knowledge, and ``Ours (w/o data)'', where we only leverage the homotopy optimization scheme to improve demonstrations. Both strategies, despite using the same amount of demonstrations, result in lower data quality. As shown in Table~\ref{tb_exp_main}, they underperform compared to our full method, highlighting the importance of data quality in training the controller.
% 
% where optimization combines trajectory-specific efforts with the controller's tracking prior.
% We propose transferring tracking knowledge from the controller and curriculum before optimization to handle more difficult and diverse trajectories in the dataset. We ablate these strategies 
% We propose to transfer general tracking knowledge encoded in the tracking controller and the curriculum prior to the optimization process for solving difficult-to-solve problems so that we can include more difficult and diverse labeled trajectories into the dataset. We've tried to ablate such two strategies and create ``Ours (w/o data, w/o structure)'' where the final labeled dataset is created by directly optimizing each trajectory without any prior from the tracking controller or the curriculum scheduler, and ``Ours (w/o data)'' where each trajectory is optimized under the joint effort of the per-trajectory tracking optimization and the tracking prior provided by the tracking controller. Such two strategies, though using the same amount of labeled data as our full method to provide supervision, may fall short in the data quality aspect. As shown in Table~\ref{tb_exp_main}, they would lag behind our full version, illustrating the role of data quality in training the tracking controller. 
% This approach can potentially let us get better per-trajectory tracker under expansive tracking curriculum trail-and-error. However, it is extremely time-consuming and unaffordable. As presented in Table~\ref{tb_exp_main}, Ours (w/ sup.), as restricted by the quality and the diversity of the action-labeled data, typically lags behind our full method on both the GRAB dataset and the TACO dataset. It validates the importance of data quality and coverage used to train the tracking controller. Ours (w/ sup., w/ curriculum) leverages the power of curriculum learning and the benefit of per-trajectory searched accurate curriculum, and can sometimes outperform out proposed strategy, which uses the tracking controller to provide tracking priors and the curriculum scheduler to propose the tracking schedule for tracking difficult trajectories. However, leveraging this approach is highly time-consuming, and would become extremely unaffordable when the number of data increases. Our proposed strategy can not only effectively improve the data quality, but smartly reduces the time consumption. 
% using per-trajectory tracking optimization and the tracking prior from the tracking controller. 
% optimized with per-trajectory searched curriculum, other than the curriculum planned by the scheduler. 
% This demonstrate the effectiveness of the tracking curriculum and the quality of our mined curricula. 
% typically lags behind our full method,
% \todo{xxxx} 
% \todo{for the curriculum, say that the trajectories between TACO is a little bit similar so we can observe the the one with exact curriculum can achieve better performance some times}


\begin{wrapfigure}[13]{r}{0.45\textwidth} % {0pt}
\vspace{-3ex}
\includegraphics[width = 0.45\textwidth]{./figs/scaling.pdf}
\vspace{-30pt}
    \caption{\footnotesize
    Scaling the amount of demonstrations.
    }
    \label{fig:fig_scaling}
% \vspace{-30pt}
\end{wrapfigure}


\noindent\textbf{Scaling the number of demonstrations.} 
To investigate the relationship between the tracking controller's performance and the number of demonstrations, we vary the size of the demonstration dataset during training and tested performance on the TACO dataset. Specifically, in the final training iteration, we down-sampled the dataset to 0.1, 0.3, 0.5, and 0.9 of its original size and re-trained the model. As shown in Figure~\ref{fig:fig_scaling}, there is a clear correlation between the amount of demonstrations and model performance. Since the curve has not plateaued, we hypothesize that increasing the amount of high-quality data could further improve performance.
% general tracking controller's performance and the amount of labeled data, 
% To explore the relation between the performance of the general tracking controller and the number of labeled data, we try to vary the number of final labeled data to train the model and test the model's performance on the TACO dataset. To be more specific, in the last training iteration, we try to down-sample the \emph{final action-labeled dataset} into $0.1, 0.3, 0.5, 0.9$ of its original size and re-train the model. As summarized in Figure~\ref{fig:fig_scaling}, there exists an obvious relation between the amount of labeled data used for training and the model's performance. Besides, the curve has not yet reached a flat raising mode in our trails. So we hypothesize that our method's performance could still be enhanced if we can manage to create more high-quality data to train the general tracking controller. 
 
% \todo{a scaling law that demonstrate the role of the data } 

% \todo{time consumption and the time efficiency}



% \todo{repro statement}



==> articles/intro.tex <==
\section{Introduction}
Robotic dexterous manipulation refers to the ability of a robot hand skillfully handling and manipulating objects for various target states with precision and adaptability. This capability has attracted significant attention because adept object manipulation for goals such as tool use is vital for robots to interact with the world. Many efforts have been devoted previously to push the ability of a dexterous hand toward human-level dexterity and versatility~\citep{rajeswaran2017learning,chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact,liu2024quasisim,Li2024ReinforcementLF}. This also aligns with our vision. 

Achieving human-level robotic dexterous manipulation is challenging due to two main difficulties: the intricate dynamics of contact-rich manipulation, which complicates optimization~\citep{pang2021convex,pang2023global,liu2024quasisim,Jin2024ComplementarityFreeMM}, and the need for robots to master a wide range of versatile skills beyond specific tasks. Previous approaches mainly resort to model-free reinforcement learning (RL)~\citep{chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi} or model-based trajectory optimization (TO)~\citep{pang2021convex,pang2023global,Jin2024ComplementarityFreeMM,hwangbo2018per}. While RL requires task-specific reward designs, limiting its generalization, TO depends on accurate dynamics models with known contact states, restricting adaptability to new objects and skills. A promising alternative is to leverage human hand-object manipulation references, widely available through videos or motion synthesis, and focus on controlling a dexterous hand to track these references. This approach separates high-level task planning from low-level control, framing diverse skill acquisition as the development of a universal tracking controller.
However, challenges remain due to noisy kinematic references, differences in morphology between human and robotic hands, complex dynamics with rich contacts, and diverse object geometry and skills.
Existing methods struggle with these issues, often limiting themselves to simple tasks without in-hand manipulation~\citep{christen2022d,zhang2023artigrasp,wu2023learning,xu2023unidexgrasp,Luo2024GraspingDO,Singh2024HandObjectIP,Chen2024ViViDexLV} or certain specific skills~\citep{qin2022dexmv,liu2024quasisim,rajeswaran2017learning}.

In this work, we aim to develop a general-purpose tracking controller that can follow hand-object manipulation references across various skills and diverse objects. In particular, given a collection of kinematics-only human hand-object manipulation trajectories, the controller is optimized to drive a robotic dexterous hand to manipulate the object so that the resulting hand and object trajectories can closely mimic their corresponding kinematic sequences. 
We expect the tracking controller to exhibit strong versatility, generalize well to precisely track novel manipulations, and have strong robustness towards large kinematics noises and unexpected reference states. 


To achieve the challenging goal above, we draw three key observations: 1) learning is crucial for handling heterogeneous reference motion noises and transferring data prior to new scenarios, supporting robust and generalizable tracking control; 2) leveraging large-scale, high-quality robot tracking demonstrations that pair kinematic references with tracking action sequences can supervise and significantly empower neural controllers, as demonstrated by data-scaling laws in computer vision and NLP~\citep{Achiam2023GPT4TR,Brown2020LanguageMA}; 3) acquiring large and high-quality tracking demonstrations is challenging but we could utilize the data flywheel~\citep{Chiang2024ChatbotAA,Bai2023QwenTR} to iteratively improve the tracking controller and expand the demonstrations in a bootstrapping manner.


Based upon the previous observations, we propose \modelnamenspace, a novel neural tracking controller for dexterous manipulation, guided by human references. Specifically, given a collection of human hand-object manipulation trajectories, we first retarget the collection to kinematic robotic dexterous hand sequences to form a set of reference motions as data preparation. Our method then alternates between mining successful robot tracking demonstrations and training the controller with the mined demonstrations. To make sure the data flywheel functions effectively, we introduce two key designs. First, we carefully integrate reinforcement and imitation learning techniques to train a neural controller, ensuring its performance improves with more demonstrations while maintaining robustness against unexpected states and noise. Second, we develop a per-trajectory tracking scheme that uses the trained controller to mine diverse and high-quality tracking demonstrations through a homotopy optimization method. The scheme transfers the tracking prior from the controller to individual trajectories to ease per-trajectory tracking for better demonstration quality. Moreover, the scheme will convert a tracking reference into a series of gradually simplified reference motions so that tracking these references from simple to complex could help better track the original reference motion. This is akin to chain-of-thought and is very suitable for tracking complex reference motions to increase the demonstration diversity. The two designs above together with the iterative training enable \modelname to successfully track novel and challenging human references.


We demonstrate the superiority of our method and compare it with previous methods on challenging manipulation tracking tasks in two datasets, describing expressive hand-object interactions in daily and functional tool-using scenarios, involving complex object movements, difficult and subtle in-hand re-orientations, interactions with thin objects, and frequent hand-object rich contact variations. 
% We both conduct extensive experiments in the simulator, \emph{i.e.,} Isaac Gym~\citep{makoviychuk2021isaac}, to demonstrate the efficacy, generalization ability, and robustness of our tracker to accomplish a wide range of manipulation tracking tasks and even excellently track novel manipulation trajectories, and evaluate 
We conduct both extensive experiments in the simulator, \emph{i.e.,} Isaac Gym~\citep{makoviychuk2021isaac}, and evaluations in the real world, to demonstrate the efficacy, generalization ability, and robustness of our tracker to accomplish a wide range of manipulation tracking tasks and even excellently track novel manipulation trajectories (Figure~\ref{fig_intro_teaser}).
% both conduct 
% We conduct experiments in both the simulator, \emph{i.e.,} Isaac Gym~\citep{makoviychuk2021isaac},  and the real world to demonstrate the efficacy, generalization ability, and robustness of our tracker to accomplish a wide range of manipulation tracking tasks and even excellently track novel manipulation trajectories (Figure~\ref{fig_intro_teaser}). 
% We can track difficult manipulations involving expressive and complex object movements, detailed and subtle in-hand re-orientations, and frequent rich hand-object contact variations.
Our approach successfully surpasses the previous methods both quantitatively and qualitatively, achieving more than 10\% success rate than the previous best-performed method. Besides, we conduct further analysis and demonstrate the various recovery behaviors of our controller, demonstrating its robustness to unexpected situations. Thorough ablations are conducted to validate the efficacy of our designs.

Our contributions are threefold:
\begin{itemize} % [noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=.5cm]
    \item We present a generalizable neural tracking controller that progressively improves its performance through iterative mining and incorporating high-quality tracking demonstrations.
    \item We introduce a training method that synergistically combines reinforcement learning and imitation learning. This approach leverages abundant high-quality robot tracking demonstrations to produce a controller that is generalizable, versatile, and robust.
    \item We develop a per-trajectory optimization scheme that employs our tracking controller within a homotopy optimization framework. We propose a data-driven way to generate homotopy paths, enabling solving challenging tracking problems.
\end{itemize}





==> articles/intro_old.tex <==
\section{Introduction}

% \todo{}

% \todo{problem and the motivation -- problem is still the general tracker but to motivate the method --- should not assume the single trajectory tracking is solved, especially efficiently tracking}

% \todo{method -- it seems that the current statement is a little bit uncesary complex..?}


% \todo{how to describe the task? -- the control the robot hand to accomplish what?}
% \todo{llm for helping?}


% \eric{1. What problem you are focusing on and why it is important?
% \begin{itemize}
%     \item The definition of dexterous manipulation.
%     \item The importance of dexterous manipulation.
%     \item Since developing dexterous robotic hands aims to achieve versatility similar to that of human hands, it becomes essential to develop robotic systems with diverse dexterous manipulation skills, which is also our goal in this paper.
% \end{itemize}}

% Advancing an embodied agent's ability to interact with the physical world is a critical step toward achieving powerful artificial intelligence. 
% Dexterous manipulation i
% Dexterous manipulation involves manipulating objects to change the object state for specific purposes. 
Robotic dexterous manipulation refers to the ability of a robot hand to skillfully handle and manipulate objects for various target states with precision and adaptability.
% similar to human hand movements.
Empowering an embodied agent with dexterous manipulation skills has attracted lots of attention since smartly and adeptly manipulating objects to fulfill goals such as tool-using is a crucial part of interacting with the world. 
% is a crucial part of 
% interacting with objects with dexterous hand is the most basic and effective way to change the object states to fulfill goals such as tool-using. 
The ultimate goal of developing robotic dexterous hand skills is letting it achieve human-level dexterity and versatility~\citep{rajeswaran2017learning,chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact,liu2024quasisim,Li2024ReinforcementLF}. To fulfill this ambitious yet essential vision, an essential milestone is equipping robotic system with diverse manipulation skills, which is also our goal in this work. 

% so that it has the capability to accomplish a wide range of manipulation tasks, wh
% Fulfilling this ambitious yet essential vision 
% It is an important topic nowadays since interacting with object using dexterous hand is a most basic way of using objects to fullfilll our goals. 
% aims at equipping a multi-finger robotic dexterous hand with the ability to interact with the 
% Equipping an embodied agent with human-level dexterity is an ambitious yet essential milestone in developing future super-intelligent robots capable of smart interactions with the environment~\citep{rajeswaran2017learning,chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,yao2022controlvae,fussell2021supertrack,grandia2023doc,peng2018deepmimic,wang2023physhoi,mordatch2012contact,liu2024quasisim,Jenelten2023DTCDT,Li2024ReinforcementLF}. 
% With this as the ultimate goal of developing dexterous robot hands, it becomes essential to equip robotic systems with diverse dexterous manipulation skills, which is also our goal in this work. 

% Developing dexterous hands with such dexterity 
% As the final goal of developing dexterous robot hands aims to achieve human
% Learning expressive and dexterous skills from human demonstrations is a promising and increasingly popular approach to advancing robot capabilities toward human-level dexterity. Human-object interactions (HOI) offer rich, semantically meaningful manipulations, supported by diverse data sources such as motion capture datasets~\citep{taheri2020grab,fan2023arctic,liu2024taco} and large-scale online video collections~\citep{Wu2024ReconstructingHO}. However, existing approaches predominantly focus on learning goal-driven or task-specific skill acquisitions~\citep{rajeswaran2017learning,qin2022dexmv,Xiong2022RoboTubeLH,liu2024quasisim} falling short of delivering a versatile controller capable of handling a broad range of complex manipulations.
% In this work, we aim to develop a general-purpose tracking controller from human manipulation references that can universally control a robotic hand to perform a wide variety of dexterous tasks. 

% task-specific, goal-driven 
% task-specific, goal-driven skills~\citep{rajeswaran2017learning,qin2022dexmv,Xiong2022RoboTubeLH}, or are constrained by single-trajectory optimization~\citep{liu2024quasisim}, 

% Advancing an embodied agent's capability to interact with the world is undoubtedly a significant step towards powerful artificial intelligence. Equipping an agent with high eligibility and human-level dexterity is an ambitious yet extremely vital waypoint towards future super-intelligent robot to smartly interact with the physical world~\citep{rajeswaran2017learning,chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,yao2022controlvae,fussell2021supertrack,grandia2023doc,peng2018deepmimic,wang2023physhoi,mordatch2012contact,liu2024quasisim,Jenelten2023DTCDT,Li2024ReinforcementLF}. 
% % \todo{cite some locomotion related papers}
% Learning expressive and dexterous skills from human references is a promising a popular trend to push the boundary of the robot library towards human-level dexterity taking advantage of highly dexterous, semantically meaningful and expressive manipulations contained in human-object interactions (HOI) and abundant data sources covering MoCap datasets~\citep{fan2023arctic,liu2024taco} and internet scale YouTube videos~\citep{Wu2024ReconstructingHO}. However, previous efforts are mainly limited to acquiring specific and relatively simple goal-driven skills~\citep{rajeswaran2017learning,qin2022dexmv,Xiong2022RoboTubeLH} or are restricted to single trajectory optimization~\citep{liu2024quasisim}, still a far way from a versatile controller wiht the ability to accomplish a wide range of challenging maipulations. 
% % are restricted to single trajectory offline tracking\todo{need to say their limitations here?} 
% In this work, we wish to learn a general tracking controller from human manipulation reference that can universally control the robot hand to accomplish a wide and versatile range of dexterous manipulations. 


% In this work, we investigate this issue and illustrate how optimizing the simulator concurrently with skill acquisition can benefit a popular yet challenging task in robot manipulation -- dexterous manipulation transfer.

% ~\citep{rajeswaran2017learning,Xiong2022RoboTubeLH,qin2022dexmv,liu2024quasisim}. \todo{more? } 
% Considering the complex and changing environments as well as novel tasks that an embodied agent would frequently encounter during real execution, a general policy capable of 
% a general policy capable of tackling a wide range of tasks with high robustness and adaptivity is more appealing and more practically useful. Despite the impressive achievement in general and robust local motion skill learning \todo{cite the robust tracker..?}, what's the best strategy to acquire a dexterous manipulation generalist that still lacks a mature and truly workable solution? In this work, we aim to explore the possibility of training a dexterous manipulation general police for a popular yet challenging family of tasks -- dexterous manipulation tracking. 





% \eric{2. What are the challenges and why previous methods are not good enough?
% \begin{itemize}
%     \item Dexterous manipulation is challenging due to …
%     \item RL based methods require task specific reward designs and are usually restricted to a specific manipulation skill. TO based methods require accurate dynamic models with known contact states, preventing it from generalizing to new objects and skills.
%     \item A seemingly attractive idea to tackle the above issues is to leverage reference motions of human hands manipulating objects, e.g., from videos or from motion synthesis methods. When available, these data can be tracked via a controller, allowing dexterous hands to quickly perform very diverse manipulation skills.
%     \item However, dexterous manipulation tracking is also challenging due to noises, complex dynamic contacts, diverse object geometry and manipulation trajectory… and existing methods fail…
%     \item Our work aims to tackle the above challenges and introduce …
% \end{itemize}}

This vision is super-challenging due to several inherent difficulties coming from 1) the intricate dynamics involved in contact-rich dexterous manipulation, which often challenges the optimization~\citep{pang2021convex,pang2023global,liu2024quasisim,Jin2024ComplementarityFreeMM}, and 2) the wish for letting the robot master versatile manipulation skills, not limited to single tasks or specific problems. Previous works mainly resort to model-free reinforcement learning (RL) techniques~\citep{chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi} and model-based trajectory optimization (TO) approaches~\citep{pang2021convex,pang2023global,Jin2024ComplementarityFreeMM,hwangbo2018per} to empower the dexterous hand with fantastic manipulation skills. Despite their impressive achievements, solely leveraging these methods can hardly let us arrive at a universal dexterous skill. RL requires methods that require task-specific reward designs and are usually restricted to a specific manipulation skill. Trajectory optimization, though free of designing rewards, relies on accurate dynamics models with known contact states. These assumptions severely prevent it from generalizing to new objects and skills. Jumping out of previous common routines, a seemingly attractive idea to tackle the above issues is to leverage references trajectories of human hands manipulating objects, which have abundant resources such as videos or motion synthesis methods, and convert the universal dexterous skill acquisition puzzle into a tracking control problem. In this way, we can isolate the high-level task planning and the low-level controlling. It further frees us from designing a general skill for tackling heterogeneous tasks by unifying diverse dexterous manipulation skill learning into a tracking control task.
% offers us the possibility of getting rid of a general
% by unifying diverse dexterous manipulation skill learning into a tracking control task.
% to isolate the high-level task planning and the low-level control problem, leverage references motions of human hands manipulating objects, which have abundant resources such as videos or motions synthesis methods, and convert the universal dexterous skill acquisition problem into a tracking control problem. 
With a controller that can track abundant and diverse human object manipulations with high generalization ability and robustness, we enable a dexterous hand to perform very diverse manipulation skills via high-level kinematics commands.
However, dexterous manipulation tracking control is also extremely challenging due to noisy kinematic references resulting from inaccurate capturing systems and the morphology difference between the robot hand and the human hand, the complex and dynamic, rich hand-object contacts, diverse and even challenging objects (\textit{e.g.,} very thin objects) and manipulation. Existing methods always fail to fully resolve these challenges, restricting their achievements in learning from sparse human references~\citep{christen2022d,zhang2023artigrasp,wu2023learning}, demonstrating versatility in relatively simple tasks such as grasping, trajectory following, and re-locating~\citep{xu2023unidexgrasp,Luo2024GraspingDO,Singh2024HandObjectIP,Chen2024ViViDexLV}, and task-specific or single skill acquisition~\citep{qin2022dexmv,liu2024quasisim,rajeswaran2017learning}. 
% \todo{more refs}
% Existing methods always fail to fully resolve these challenges, restricting their achievement in specific skill acquisition or the versatility only in relatively simple tasks such as grasping. \todo{add ref} 
In this work, we try to tackle these challenges and introduce a learning-based versatile neural tracking controller for dexterous manipulation from human references. 
% \todo{check this}

% \eric{3. Add a paragraph talking about the specific problem formulation. Train time, test time, input, output.}

The tracking control problem for dexterous manipulations from human references aims at developing a versatile and generalizable tracking controller leveraging abundant human-object interaction data. 
% at leveraging abundant kinematics-only human-object manipulation trajectories to learn a versatile and generalizable tracking controller.
Given a collection of kinematics-only human hand-object manipulation trajectories, the controller is optimized to drive a robotic dexterous hand to manipulate the object so that the resulting hand and object trajectories can closely mimic their corresponding kinematic sequences. 
% the robotic dexterous 
% track every trajectory in the dataset.
% At the test time, w
We expect the tracking controller to exhibit strong versatility, generalize well to precisely track novel manipulations, and have strong robustness towards large kinematics noises and unexpected reference states. 
% generalization ability to novel manipulations, and robustness towards large kinematics noise. Given an unseen manipulation trajectory with new and challenging interactions and unobserved object geometry, we wish it to generalize well and can precisely track these sequences. 
% to be able to generalize well to unseen manipulation trajectories and precisely track novel and challenging interactions such as complex object movements and subtle in-hand re-orientations. 
% with novel and difficult objects
% to track novel and even challenging interactions involving complex object movements with difficult, subtle, and detailed in-hand manipulations, 
% novel and even challenging interactions with
% The neural tracking control for dexterous manipulations aims to leverage human hands manipulating object trajectories, which have abundant data sources covering the internet videos and motion synthesis models, to learn a versatile and generalizable neural tracking controller. Given a dataset containing diverse human-object interaction trajectories, the controller is optimized aiming to track every manipulation trajectory in the dataset. Specifically, with the kinematics-only human object manipulation trajectory as input, the tracking controller aims to output an action trajectory that can drive a dexterous robotic hand to manipulate the object with the resulting hand trajectory and the object sequence closely mimicking their corresponding kinematic references. 
% % mimic the kinematic trajectory -- when letting a dexterous robot hand execute the output action trajectory, the resulting hand states and object states should be close to their corresponding kinematic trajectories in the input sequence. 
% A versatile and generalizable tracking controller ought to be able to generalize to novel and even challenging interactions with new and difficult objects. At the test time, given a manipulation sequence where both the hand motion and the object movements and the object geometry are unseen during the training, the controller is expected to precisely track the manipulation trajectory. 
% to give high-quality action outputs d
% that can drive the dexterous robot hand to precisely control the object so that the resulting hand sequence and the object sequences are close to the input reference. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% . When executing the action sequence 
% or each manipulation sequence, the tracking controller aims at output 
% In the test time, the optimized controller 
% to produce proper actions at each timestep aiming to track 
% to track every manipulating trajectory in the dataset. 
% At the train time, the controller is optimized to track every 
% human hands manipulating objects 
% learning a versatile and generalizable tracing controller from
% is to leverage reference motions of human hands manipulating objects, \textit{e.g.}, from videos or from motion synthesis methods. When available, these data can be tracked via a controller, allowing dexterous hands to quickly perform very diverse manipulation skills.
% preventing it from generalizing to new objects and skills. 
% in dexterous skill acquisition mainly resort to model-free reinforcement learning techniques and model-based trajectory optimizatons
% 1) the intricate dynamics involved in the manipulation resulting from the complex object motions including difficult and subtle in-hand re-orientations and the frequent rich hand-object variations which even frequently challenge the single trajectory tracking problem~\citep{pang2021convex,pang2023global,liu2024quasisim,Jin2024ComplementarityFreeMM}, 2) the requirement of controlling a high DoF dexterous hand to densely track each frame in the demonstration,  3) the wish for a general controller that generalizes well to control the hand to manipulate new objects to track new manipulation references. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Given a set of kinematics-only human hand-object interaction trajectories, taken from MoCap datasets~\citep{fan2023arctic,taheri2020grab,liu2024taco} or obtained via reconstructions from videos~\citep{Wu2024ReconstructingHO}, the goal of dexterous tracking control is to develop a single, general controller capable of mimicking a diverse range of manipulation sequences with both the resulting hand and object trajectories close to their corresponding reference sequences. 
% % trajectory and the object sequence close to those in
% % executing diverse manipulations specified by kinematic reference commands.
% This controller should generalize to unseen motion trajectories, adapt to novel object geometries, and exhibit high robustness towards large noise in the kinematic motions such as unreasonable states, severe penetrations, as well as out-of-distribution objects and interactions. 
% % such as those from MoCap dataset
% % hand-object interaction dataset from a simulated dexterous hand, such as those obtained via retargeting from human HOI datasets~\citep{fan2023arctic,taheri2020grab,liu2024taco} or reconstructed from videos~\citep{Wu2024ReconstructingHO}, the goal of 
% % with strong recovery behavior. 
% Solving this problem poses several significant challenges: 1) the intricate dynamics involved in the manipulation resulting from the complex object motions including difficult and subtle in-hand re-orientations and the frequent rich hand-object variations which even frequently challenge the single trajectory tracking problem~\citep{pang2021convex,pang2023global,liu2024quasisim,Jin2024ComplementarityFreeMM}, 2) the requirement of controlling a high DoF dexterous hand to densely track each frame in the demonstration,  3) the wish for a general controller that generalizes well to control the hand to manipulate new objects to track new manipulation references. 
% Previous works largely focus on solving per-trajectory tracking problems or learning task-specific skills, such as pouring, relocating~\citep{rajeswaran2017learning,qin2022dexmv,christen2022d,zhang2023artigrasp}, in-hand re-orientation, flipping, and spinning~\citep{chen2023visual,andrychowicz2020learning} with a fixed-base robot hand. Other works demonstrate versatility only in relatively simple tasks such as trajectory following~\citep{Luo2024GraspingDO} and dexterous grasping~\citep{xu2023unidexgrasp,wan2023unidexgrasp2}. Recent advances in humanoid tracking control suggest the potential of leveraging reinforcement learning (RL) to develop versatile tracking policies by carefully designing rewards and training strategies~\citep{Luo2023PerpetualHC,Luo2023UniversalHM}. However, dexterous manipulation poses additional difficulties. Training policies to handle various manipulations remains challenging.
% % Training policies to handle various manipulations, even with carefully crafted reward functions, remains challenging. 
% % This may stem from the unstructured and heterogeneous nature of reference motions, which further expose RL’s limitations in multi-task learning. 
% Model-based techniques that assume known system dynamics face significant challenges as well due to the difficulty in accurate system modeling in the dexterous manipulation scenario. 
% The correct path toward developing a universal tracking controller remains elusive, with few attempts documented in the literature.
% % simpler tasks, such as trajectory following~\citep{Luo2024GraspingDO} and dexterous grasping~\citep{xu2023unidexgrasp,wan2023unidexgrasp2}.



% specific task-oriented 


% 1) The intricate dynamics of manipulation, characterized by complex object motions, subtle in-hand re-orientations, and frequent variations in hand-object interactions, which can be difficult even for single-trajectory tracking~\citep{liu2024quasisim,Jin2024ComplementarityFreeMM}.
% 2) The need to control a high-DoF dexterous hand to densely track each frame in the reference demonstration.
% 3) The desire for a general controller that can adapt to new objects and manipulation tasks beyond those in the training data.





% general dexterous manipulation tracking aims at optimizing for a single controller (a ``tracker'' ) that 1) can control the hand to accomplish manipulations as demonstrated in each given kinematic motions and 2) can generalize to track novel manipulation trajectories involving novel interaction trajectories and unobserved object geometries. Solving this problem poses several significant challenges: 1) the intricate dynamics involved in the manipulation 
% Given the kinematic-only hand-object interaction dataset of a simulated dexterous hand, \emph{e.g.,} acquired via retargeting from human HOI datasets~\citep{fan2023arctic,taheri2020grab,liu2024taco} or lifting from videos~\citep{Wu2024ReconstructingHO}, dexterous tracking control problem aims at learning a single yet general tracking controller that can control the robot hand accomplish versatile manipulations specified by the kinematic reference commands. The tracking controller is expected to generalize well to unseen motion trajectories, and novel object geometries, and exhibit high robustness and recovery behaviors. Solving this problem poses several significant challenges: 1) the intricate dynamics involved in the manipulation resulting from the complex object motions including difficult and subtle in-hand re-orientations and the frequent rich hand-object variations which even frequently challenge the single trajectory tracking problem~\citep{liu2024quasisim,Jin2024ComplementarityFreeMM}, 2) the requirement of controlling a high DoF dexterous hand to densely track each frame in the demonstration,  3) the wish for a general controller that generalizes well to control the hand to manipulate new objects to track new manipulation references. Previous works mainly focus on solving per-trajectory tracking problems, learning specific goal-driven task skills such as pouring and re-locating~\citep{rajeswaran2017learning,qin2022dexmv,christen2022d,zhang2023artigrasp}, in-hand re-orientation, flipping and spinning~\citep{chen2023visual,andrychowicz2020learning} with a fixed-root robot hand, or only demonstrates the versatility in relatively simple tasks such as trajectory following~\citep{Luo2024GraspingDO} and dexterous grasping~\citep{xu2023unidexgrasp,wan2023unidexgrasp2}. Recent sucssess in humanoid tracking control has demonstrated the potential of leveraging advanced reinforcement learning (RL) to learn a versatile tracking policy by carefully design rewards and the training strategy~\citep{Luo2023PerpetualHC,Luo2023UniversalHM}. However, manipulation tracking control exhibits increasing difficulties. Directly training a policy to track various manipulations, even with dedicatedly designed rewards, can hardly work, perhaps due to unstructured heterogeneous reference motions that put RL which is notoriously in short of the multi-task ability, further into a difficult situation. What's the correct way to a universal tracking controller remains extremely unclear and difficult with very rare attempts in the literature. 


% Directly adapting previous methods to solve our problem,  such as the delicately designing rewards and leveraging advanced reinforcement learning (RL) with carefully designed training scheme to train a policy aiming to track every manipulation trajectory in the dataset, though proved effective in training humanoid locomotion controller~\citep{Luo2023PerpetualHC}, can hardly work in our problem scope, 

% Model-free reinforcement learning (RL), with its no assumption on the dynamic system and the strong optimization capability, has been widely appreciated and proved effective in previous literature~\citep{qin2022dexmv,christen2022d,zhang2023artigrasp,Luo2024GraspingDO,Luo2023PerpetualHC}. 
% Reinforcement learning (RL) is a widely appreciated in previous literature 
% which does not assume prior knowledge about the dynamic system, 
% In the current situation where optimizing for an effective single trajectory tracker still has no mature solutions, what's the correct way to a universal tracking controller is extremely unclear and difficult with very rare attempts in the literature. 
% In this work, 
% well to novel manipulations and new object geometrices. 
% the wish for a universal controller that can well track every manipulation demonstrations other than over-fitting to the single trajectory, and 3) the expectation in generalizing to unseen manipulations including novel hand-object trajectories and unobserved object geometries. 


% \todo{need to mention previous works in the universal humanoid tracking?}

% What's the correct way to a universal tracking controller is extremely unclear and lacking 
% How to optimize for 
% Obtaining single trajectory tracker is already very challenging and time-consuming~\citep{liu2024quasisim}, letting alone a universal tracking controller. 
% due to the difficult dynamics that are unfriendly for an optimizer. 
% or only demonstrates the effectiveness in relatively easy interact
% Most previous works focus on single trajectory tracking, where the optimized controller is only expected to be effective for one single trajectory~\citep{pang2023global,zhang2023artigrasp,liu2024quasisim,Jin2024ComplementarityFreeMM}, or is only effective in relatively easy interactions such as trajectory following~\citep{Luo2024GraspingDO}, goal-driven manipulations such as pouring and re-locating~\citep{rajeswaran2017learning,qin2022dexmv,christen2022d,zhang2023artigrasp}, in-hand re-orientation, flipping and spinning~\citep{chen2023visual,andrychowicz2020learning} with a fixed-root robot hand, and dexterous grasping~\citep{xu2023unidexgrasp,wan2023unidexgrasp2}. In this work, we take one step further and wish for a universal controller that can effectively track every manipulation involving expressive and difficult interactions with complex and challenging object movements, and frequent contact variations, and can also generalize to novel manipulations.\todo{rewrite this} 


% \eric{4. What are your key observations and/or high-level ideas
% \begin{itemize}
%     \item Learning is essential to handle reference noises and transfer data priors to novel cases.
%     \item Imitating from large amount of high-quality tracking results can make learning especially powerful as evidenced by data-scaling law in CV and NLP. % can make the learning essential powerful as evidenced by datascaling law 
%     \item Obtaining useful data could be tricky, but we can leverage data flywheel to improve the tracking controller and the amount of high-quality data in a bootstrapping manner.
% \end{itemize}
% }


To tackle challenges in developing a versatile tracking controller, our key observations lie in three aspects: 1) Compared to model-based approaches which primarily leverage trajectory optimization to develop the controller, learning plays a crucial role in handling reference motion noises and transferring data prior to novel cases to achieve robust and generalizable tracking control. 2) Learning from a large amount of high-quality imitation-ready data with paired data containing both the kinematic reference and the action sequence is a promising approach to make the neural controller essentially powerful as evidenced by the data-scaling law in CV and NLP spaces~\citep{Achiam2023GPT4TR,Brown2020LanguageMA}. 3) Due to the inherent difficulty in solving dexterous manipulation tracking control problems, obtaining useful imitation-ready data for tracking control could be very tricky. However, we can leverage the data flywheel~\citep{Chiang2024ChatbotAA,Bai2023QwenTR,Ouyang2022TrainingLM} to improve the tracking controller and the amount of high-quality data in a bootstrapping manner. 


% Obtaining high-quality imitation-ready data for dexterous manipulation tracking control could be very tricky. 
% generalizable and 
% strong generalizations
% generalizable and 
% traditional trajectory optimization, learning plays a crucial role in handling reference motion noises and transferring data prior to novel cases. Training a neural controller is a more promising technique for us to get to a universal and generalizable tracking controller capable of handling various situations. 2) Learning from a large amount of high-quality tracking results can make the neural controller essentially powerful as evidenced by the data-scaling law in CV and NLP. 3) Obtaining useful data could be tricky, but we can leverage the data flywheel to improve the neural tracking controller and the amount of high-quality data in a bootstrapping manner.
% A learning based neutral controller is 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Inspired by the data scaling law in the vision and NLP space~\citep{Brown2020LanguageMA,Achiam2023GPT4TR}, we envision a large number of imitation-ready data with reference and tracking result pairs could facilitate the learning of a general tracking controller. However, obtaining imitation-ready data itself is challenging since even tracking a single manipulation sequence is both costly and difficult~\citep{christen2022d,zhang2023artigrasp,pang2021convex,pang2023global,liu2024quasisim,Jin2024ComplementarityFreeMM}. In the general tracking problem scope, we envision the possibility of letting per-trajectory tracking benefit from the tracking data prior and the tracking task structure prior, which tells us cross-task relations that we can leverage to improve single task solving via the homotopy optimization. 
% % With the general tracking controller, we envision the possibility of letting the per-trajectory tracking benefit from general data prior in tracking encoded in the tracking controller and the task structure prior where the 
% % and also let the model 
% % one way that could let the per-trajectory tracking benefit from general data prior from the tracking controller and also l
% % We envision one way where we can let per-trajectory tracking benefit from tracking prior encoded in hte
% Therefore, we propose to grow the imitation-ready data and the tracking controller together in a bootstrapping manner. Starting from a small amount of imitation-ready data with action-labeled manipulation trajectories, we learn a tracking controller by letting the policy explore and evolve via RL and imitate high-quality action sequences; and also construct the tracking task structure encoding beneficial optimization paths which we can leverage to solve difficult tracking problems in a homotopy optimization manner. After that, we could leverage the data prior from the tracking controller and optimization paths proposed by the tracking task structure prior to enhance  per-trajectory tracking optimization. With these above considerations, we propose an iterative approach to gradually improve each side and finally arrive at a strong general tracking controller. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% the tracking task structure prio
% the data prior encoded in the learned tracking controller and the inference time structure prior 
% After that, we could leverage the data prior encoded in the learned tracking controller and the inference time structure prior to planning a correct optimization path which can finally ease the difficulty of per-trajectory optimization. Considering the inter-dependencies between the tracking controller optimization and per-trajectory trackers, we then propose an iterative approach to solve the ``chicken-and-egg'' puzzle where we gradually improve each side and finally arrive at a strong general tracking controller. 
% facilitate difficult
% where we can facilitate difficult task sol
% prior indicating how the per-trajectory tracking task could benefit from solving the other tracking tasks in a homotopy optimization manner. 
% the labeled data with high-quality action trajectories; 
% letting the policy explore and 
% trajectory in generic manipulation cases could be both costly and difficult -> 
% % Our key observation is that although RL would fall short in training a general tracking controller, it can indeed benefit from the guidance provided by successful trajectories with high-quality action sequences. 
% % successfully tracking high-quality trajectories, which also aligns with observations from the success of foundation models~\citep{Brown2020LanguageMA,Achiam2023GPT4TR}. \todo{add more refs} 
% However, how to effectively acquire a large amount of high-quality action-labeled manipulation trajectories itself is an unsolved problem. Existing methods for single trajectory tracking either fall short in quality or an unaffordable time requirement. Difficult trajectories involving challenging dynamics and tough object geometries are even harder to mimic. Optimizing a large scale of action-labeled trajectories and leveraging them to improve the general tracking controller's performance is not feasible. Restricted to a limited number of successful trajectories to provide guidance would potentially bias the tracking controller overfit to easy trajectories, hindering the capability and the generalization ability. How to improve the diversity and the quality of action-labeled trajectories is itself an urgent question. Observing the ability to leverage foundation models to solve specific tasks, we naturally seek the opportunity to improve per-trajectory tracking quality via borrowing tracking priros encoded in the general tracking controller. However, the tracking controller is learned from successfully optimized trajectories. Therefore, leveraging its tracking prior to resolve difficult problems may not be sufficient to solve very difficult problems.  Inspired by the recent advances in leveraging curriculum learning to solve difficult tasks~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}, we propose to find correct tracking curricula to improve the per-trajectory tracking. Identifying correct curriculum for each trajectory, which may require trail-and-error, is very time-consuming. This naturally lets us consider learning a curriculum scheduler that can schedule correct curricula to finally track difficult trajectories. The requirement of optimizing action-labeled datasets for training the general tracking controller and mining useful curricula for learning the curriculum scheduler further poses us with a ``chicken-and-egg'' puzzle. We consider an interactive approach where we can progressively improve the quality and diversity of action-labeled trajectories and train stronger tracking controller.
% To solve difficult per-trajectory
% better solve difficult per-trajectory tracking problems, where the tracking controller can hardly give us correct prior due to the limited coverage in its labeled training data, we further think about finding correct curricula to improve per-trajectory tracking, inspired by the recent advances in leveraging curriculum learning to solve difficult tasks~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}. 
% speed up and improve the per-trajectory tracking via tracking priors encoded in the general tracking controller. 
% or efficiency. 

% Therefore, to improve the diversity, coverage and quality of the action labeled trajectories, we naturally ask for the opportunity to improve the single-trajectory tracking via learned tracking policy priors as well as smartly design other techniques to speed up per-trajectory trackers' optimization as well as improve their performance. Observing the potential of leveraging general tracking knowldge encoded in the tracking controller and utilizing cross-task synergies for improving per-tracking trackers, we propose an interactive optimization scheme where we progressively improve the tracking controller via actionlabeled data and leveraging the tracking controller and cross-task synergies. 
% in one-shot 



% the general tracking knowledge encoded in the tracking controller that would be potentially beneficial for per-trajectory tracking and the 
% By exploring the possibilities of improving per-trajectories trackers 
% With key insights in 
% improving single per-trajectory tracking via 


% This naturally leads to a question: can we improve the single-trajectory tracking via learned tracking policy priors as well as smartly design other techniques to speed up per-trajectory trackers' optimization as well improve their performance? 
% Observing the role or curriculum in solving difficult control problems~\citep{Zhuang2023RobotPL,Luo2023PerpetualHC,liu2024quasisim,zhang2023learning}, we wish 
% % Recent advances in robotics and RL have witness the role 
% This naturally leads to a question: can we improve the single-trajectory tracking via the 
% either fall short in the efficiency or the tracking quality and can hardly equip us with lots of successful trajectories in a short 
% letting the tracking controller benefit from knowledge from per-trajectory tracking outcomes is a ``chitchen-and-egg'' problem in nature. 

% instead of model-free 
% Our key insight is iteratively letting the general controller optimization benefit from the guidance provided by trajectory-specific experts and improving each single trajectory tracking specialist via explicit and implicit cross-task transferrable knowledge. Instead of optimizing the general controller alone, where even the most advanced RL would be frequently challenged considering the requirement to jointly track every manipulation with distinct hand-object motion and object geometries, we wish to start from the relatively easy-to-solve single trajectory-specific controller optimization and propose an effective strategy that can let the general controller benefit from them. However, considering the inherent difficulties of dexterous manipulation tracking, single trajectory tracking specialists are hard to optimize to a satisfactory extent, especially for challenging interaction trajectories, and might require a long time. We therefore consider benefiting from single trajectory tracking from cross-task universal knowledge by modeling cross-task relations explicitly and exploring a structural task space that models cross-task relations. By iteratively solving the general tracker optimization and refining the trajectory-specific policies, we can finally arrive at a powerful general tracker via this ``specialist-generalist-specialist'' paradigm. 
% \todo{rewrite this --- should not assume that the single trajectory tracking is a solved problem --- especially the efficient single trajectory tracking} 
% % even the single trajectory tracking is difficult to optimize to a satisfactory extent. 

% is optimizing for the general controller that can properly benefit from the guidance provided by trajectory-specific trackers. 

% \eric{5. Explain your methods briefly
% \begin{itemize}
%     \item An overall pipeline explanation like the following. At train time, given a collection of human hand object manipulation trajectories, we first retarget human hands to robotic dexterous hands in the data preparation stage, resulting in a reference motion set. Our method then alternates between mining useful imitation-ready data from the reference motion set and training the tracking controller with the mined data. We have three key designs to enable the data flywheel to function effectively. 
%     \item First, we leverage an imitation-augmented reinforcement learning scheme to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance. ...
%     \item Second, we develop a per-trajectory tracking scheme which can leverage the general tracking controller to produce better imitation-ready data. ...
%     \item Third, we design a homotopy path generator, mimicking the chain of thought, to better leverage the general tracking controller for mining imitation-ready data from challenging manipulation skills. ...
% \end{itemize}
% }


We propose \modelnamenspace, a learning-based neural tracking controller designed for dexterous manipulations guided by human references. The key idea is to combine the reinforcement learning and imitation learning to train a robust and generalizable tracking controller  utilizing abundant high-quality imitation-ready data, while employing the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner. 
% employing a data flywheel to continually curate and enhance the dataset, thereby improving the tracking controller in a bootstrapping manner. 
% train a robust and generalizable tracking controller through a combination of reinforcement learning and imitation learning, utilizing abundant high-quality imitation-ready data while employing a data flywheel to continually curate and enhance the dataset, thereby improving the tracking controller in a bootstrapping manner. 
Given a collection of human hand-object manipulation trajectories, we first retarget human hand trajectories to robotic dexterous hand sequences in the data preparation stage. 
% In the data preparation stage, we begin by retargeting human hand-object manipulation trajectories into robotic dexterous hand sequences. 
% Our approach alternates between mining useful imitation-ready data from the reference motion set and training the tracking controller with this mined data. 
Our method then alternates between mining useful imitation-ready data from the reference motion set and training the tracking controller with the mined data. 
We propose two key designs to enable the data flywheel to function effectively. 
% We introduce two key designs to ensure the effective operation of the data flywheel. 
First, we learn the neural tracking controller by carefully integrating reinforcement learning and imitation learning techniques. 
By training the tracking controller to imitate a wealth of tracking results, we enhance its versatility in mastering a wide range of manipulation skills and generalization ability to novel interactions. At the same time, by employing the power of reinforcement learning to handle abnormal situations effectively, we can effectively improve the controller's robustness towards unexpected states and noise. 
% By combining the strengths of these approaches, we enable the tracking controller to imitate a wealth of tracking results, thereby enhancing its versatility in mastering a wide range of manipulation skills and generalization ability to novel interactions. 
% generalization ability and 
% we achieve a controller with high generalization ability and versatility. This enables the tracking controller to imitate a wealth of tracking results while also enhancing its robustness to unexpected states and noise, leveraging the power of reinforcement learning to handle abnormal situations effectively.
Second, we develop a per-trajectory tracking scheme that utilizes the neural tracking controller to mine higher-quality and more diverse imitation-ready data through a homotopy optimization scheme. To prepare this imitation-ready data, a basic solution is obtaining paired action sequences for kinematic reference trajectories via tracking trajectory-specific tracking policies to accurately follow the kinematic reference motions. 
However, the quality and diversity of the data can be limited since RL may face challenges when addressing difficult per-trajectory tracking problems. 
% due to the challenges that reinforcement learning (RL) faces when addressing difficult per-trajectory tracking problems. 
However, data quality and diversity can be limited due to the difficulty of RL in solving very challenging per-trajectory tracking problems. To enhance the effectiveness of per-trajectory tracking and ensure the data flywheel operates efficiently, we propose two techniques: 1) transferring tracking data from the tracking controller to the per-trajectory tracker to aid in solving complex problems; and 2) developing an innovative homotopy path generator that mimics a chain of thought, allowing us to plan beneficial optimization paths to address previously unsolvable per-trajectory tracking challenges through a homotopy optimization method. 

% However, this strategy frequently falls short in tracking difficult trajectories. Therefore, we propose two techniques to improve the quality of per-trajectory tracking results so that the data flywheel can work effectively: 1) transferring tracking data prior from the tracking controller to the per-trajectory tracker to facilitate difficult problem-solving; and 2) learning an innovative homotopy path generator, mimicking chain of thought, which can plan a beneficial homotopy optimization path that we can leverage to tackle previously unsolvable per-trajectory tracking problem via a homotopy method. 
% With the above designs, we propose an iterative optimization scheme where we alternately train the tracking controller and mine useful imitation-ready data, arriving us at a powerful tracking controller finally. 



% With these designs, we propose an iterative optimization scheme that alternates between: 1) training the tracking controller using high-quality imitation-ready data, and 2) mining higher-quality and more diverse data with the tracking controller via a homotopy optimization process.

% where we alternately 1) train the tracking controller via high-quality imitation-ready data, and 2) mine higher-quality and more diverse data using the tracking controller through a homotopy optimization scheme. 

% Therefore we propose to employ the power of tracking controller 
% for a kinematic reference trajectory involves training a trajectory-specific tracking policy to accurately follow the kinematic reference motions.
% Preparing the imitation-ready data by using RL to train per-trajectory tracking policies would fall 
% To prepare this imitation-ready data, our primary strategy for obtaining paired action sequences for a kinematic reference trajectory involves training a trajectory-specific tracking policy to accurately follow the kinematic reference motions.

% We propose \modelnamenspace, a learning-based neural tracking controller for dexterous manipulations from human references. The key idea lies in training a robust and generalizable tracking controller via reinforcement learning and imitation learning leveraging high-quality abundant imitation-ready data and leveraging the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner. Given a collection of human hand-object manipulation trajectories, we first retarget human hand trajectories to robotic dexterous hand sequences in the data preparation stage. 
% Our method then alternates between mining useful imitation-ready data from the reference motion set and training the tracking controller with the mined data. We propose two key designs to enable the data flywheel to function effectively. 
% First, we learn a neural tracking controller by carefully combining reinforcement learning and imitation learning techniques. Taking the best worlds of such two techniques, we can ensure the tracking controller have high generalization ability and versatility, taking advantage of imitating abundant tracking results, and also empowering it with high robustness towards unexpected states and noise, leveraging the power of reinforcement learning in handling abnormal situations. 
% Second, we develop a per-trajectory tracking scheme that can leverage the neural tracking controller to mine higher-quality and more diverse imitation-ready data through a homotopy optimization scheme. 
% To prepare imitation-ready data, our basic strategy to obtain the paired action sequence for a kinematic reference trajectory lies in training a trajectory-specific tracking policy to track the kinematic reference motions. 
% % At train time, given a collection of human hand-object manipulation trajectories, we first retarget human hands to robotic dexterous hands in the data preparation stage, resulting in a reference manipulation set containing retargeted hand trajectories and the original object pose sequences. 
% % To using model-free 
% % lies in training a trajectory-specific tracking policy for each trajectory. 
% % is using model-free RL to train a per-trajectory tracking policy for each trajectory.
% % However, the data quality and diversity would be restricted. 
% However, the data quality and diversity would be restricted. Therefore, we propose two techniques to improve the quality of per-trajectory tracking results so that the data flywheel can work effectively: 1) transferring tracking data prior from the tracking controller to the per-trajectory tracker to facilitate difficult problems solving; and 2) learning an innovative homotopy path generator, mimicking chain of thought, which can plan a beneficial homotopy optimization path that we can leverage to tackle previously unsolvable per-trajectory tracking problem via a homotopy method. 
% With the above designs, we propose an iterative optimization scheme where we alternately 1) train the tracking controller via high-quality imitation-ready data, and 2) mine higher-quality and more diverse data using the tracking controller through a homotopy optimization scheme. 


% high generalization ability and versatility 
% the tracking controller 
% let the tracking controller benefit from imitation-ready data, obtaining high generalization ability
% to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We have three key designs to enable the data flywheel to function effectively. 
% neural tracking controller via reinforcement learning the imitation 
% leveraging high-quality abundant imitation-ready data to train a tracking controller jointly with RL and tackling the difficulties in acquiring such data by leveraging the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner. At train time, given a collection of human hand object manipulation trajectories, we first retarget human hands to robotic dexterous hands in the data preparation stage, resulting in a reference manipulation set containing retargeted hand trajectories and the original object pose sequences.  Our method then alternates between mining useful imitation-ready data from the reference motion set and training the tracking controller with the mined data. We have three key designs to enable the data flywheel to function effectively. 
% First, we learn a neural tracking controller by carefully combining reinforcement learning and imitation learning techniques to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance. 
% % leverage both imitation learning and reinforcement learning techniques to train the neural tracking controller to 
% To combine the advantages from both sides, we devise an RL-based method for solving the general dexterous manipulation tracking problem. We then introduce an action supervision loss which encourages the policy to imitate high-quality imitation-ready data with action sequences. 
% Second, we develop a per-trajectory tracking scheme that can leverage the neural tracking controller to mine higher-quality and more diverse imitation-ready data through a homotopy optimization scheme. 
% % imitation-ready data. 
% % high-quality imitation-ready data. 
% % leverage the general tracking controller to produce better imitation-ready data.
% To prepare imitation-ready data, our basic strategy is using model-free RL to train a per-trajectory tracking policy for each trajectory. However, the data quality and diversity would be restricted due to the limited capability of reinforcement learning in solving difficult tracking problems. Therefore, we propose two techniques to improve the quality of per-trajectory tracking results to ensure the data flywheel works effectively: 1) transferring tracking data prior from the tracking controller to the per-trajectory tracker to facilitate difficult problems solving; and 2) learning an innovative homotopy path generator, mimicking chain of thought, which can plan a beneficial homotopy optimization path that we can leverage to tackle previously unsolvable per-trajectory tracking problem via a homotopy method. 
% With the above designs, we propose an iterative optimization scheme where we alternately 1) train the tracking controller via high-quality imitation-ready data, and 2) mine higher-quality and more diverse data using the tracking controller through a homotopy optimization scheme. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% for a difficult-to-track trajectory, 
% plans a homotopy optimization path, consisting of a series of tracking tasks, 
% We solve the per-trajectory tracking problem to prepare data via three techniques. 
% To obtain high-quality imitation data with action trajectories that can successfully drive the dexterous robotic hand to track the correspondence hand and object sequence, we leverage the popular model-free RL-based method by training a per-trajectory tracking policy using RL and use the tracking result as the optimized imitation-ready data. Despite no expectation in the versatility and generalization ability in the per-trajectory tracker, tracking difficult tracking problem is still very challenging. to improve the data quality and include more diverse imitation-ready data into the training of tracking controller, we propose to leverage the general tracking prior encoded in the tracking controller to improve the per-trajectory tracker optimization. Third, we design a homotopy path generator, mimicking the chain of thought, to better leverage the general tracking controller for mining imitation-ready data from challenging manipulation skills. Soley relying on tracking prior encoded in the tracking controller to improve the per-trajectory tracker is still not enough to solve a very difficult per-trajectory tracking problem. It is because that the hard-to-track trajectories are too out-of-distribution to the data prior encoded in the tracking controller, trained with imitation-ready data that has been successfully tracked. Thus such trajectory problems can hardly benefit from the tracking prior from the current tracking controller. To resolve these challenges, we propose to solve these problems in a homotopy method. Specifically, instead of solving the difficult per-trajectory tracking problem directly, we start from tracking a different trajectory to obtain its tracking result. After that we design a technique which allows us to let the difficult per-trajectory tracking problem benefit from the tracking result. In this way we are able to solve the difficult tracking task by starting from an easy task and gradually solve a series of tsks with the tracking results transferred to the next one. Finding such beneficial optimization paths, however, is very time-consuming. To further improve the efficiency, we propose to learn a tracking task structure prior model, which, in the inference time, can efficiently propose beneficial optimization paths for a tough single trajectory tracking problem. With the above three designs, we alternately 1) train the tracking controller and learn the tracking task structure prior model with high-quality imitation-ready data and 2) improve the data via the tracking controller and the tracking task structure prior model. The data flywheel can then function well, making it possible for us to train a strong tracking controller finally. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% solving the manipulation 
% , with delicately designed action space, observations, and rewards, for solving the manipulation tracking problem. 
% Second, we develop a per-trajectory tracking scheme which can 
% to train the tracking controller with
% a learning from demonstration sch
% leverage both the reinforcement learning and the imitation learning to learn  
% both reinforcement learning and imitation learning to optimize the tracking 
% imitation learning 
% leverage an imitation-augmented reinforcement learning scheme to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance. We devise a basic RL-based method to train the tracking controller with delicately designed action space, observations, and rewards for the general manipulation tracking problem. To let the policy benefit from the imitation-ready data, we add an additional supervised loss which, at each time, encourages the policy to imitate the action of the corresponding timestep in the trajectory.  Second, we develop a per-trajectory tracking 
% to first mine useful optimization paths from the training dataset and 
% to transfer the tracking result 
% propose to find an optimization path, 
% With the power of tracking prior 
% Per-trajectory tracking problem where the trackin
% encourage the policy t


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% To realize this vision, our method consists of three key designs: 1) an imitation augmented reinforcement learning technique that can effectively leverage high-quality action labeled trajectories to improve the tracking controller, 2) a homotopy method which effectively resolves the difficulty in challenging per-trajectory tracking problems, an tracking task structure prior model which encodes beneficial homotopy optimization paths, and 3) an iterative approach where per-trajectory trackers are improved via the tracking data prior and the task structure prior, together with the tracking controller getting stronger. 
% % tracking data prior from the tracking controller and the task structure prior 
% % automatic tracking task structure construction 
% % leveraging beneficial optimization paths
% % leveraging cross-tracking task relations, an automatic tracking task structure construction strategy where we identify cross-task structural relations in homotopy optimization, and a tracking task structure model for describing such relations to plan correct optimization paths for better solving per-trajectory tracking problem, and 3) an interactive optimization approach where per-trajectory trackers are gradually improved via tracking prior from the general tracking controller and effective optimization path scheduling, together with the tracking controller progressively getting stronger. 
% The imitation-augmented RL effectively leverages high-quality imitation-ready data with successful action trajectories to ease the training. Considering the difficulty in solving challenging single trajectory tracking problems, we propose two techniques to improve the single trajectory tracking optimization. The first one is a homotopy method that improves single trajectory tracking problem's solving via gradually solving each tracking problem in an optimization path. Finding correct optimization paths is very time-consuming. Therefore, we propose to learn a tracking task structure prior model that encodes beneficial optimization paths. During the inference, the structure prior model can propose beneficial optimization paths directly. Secondly, we consider leveraging general tracking prior encoded in the tracking controller to facilitate per-trajectory trackers' optimization. In more detail, we initialize the per-trajectory tracking policy via the action sequence proposed  by the tracking controller, followed by re-optimizing the per-trajectory tracker. 
% % transfer general tracking data prior encoded in the tracking 
% % To efficiently find correct o
% % in exploring the tracking task structure 
% % and improve single trajectory optimizing via correct optimization paths. Specifically, for a trajectory $A$ which is hard to track, we propose to leverage the homotopy optimization to finally solve it by gradually solving each tracking problem in an optimization path. Searching for correct optimization paths for each trajectory, however, is very expensive. Therefore, we propose to learn a model that can encode such structural tracking problem relations and use it as a structure prior to provide us with correct optimization paths. 
% % Secondly, we transfer general tracking prior to encoding in the tracking controller to speed up and enhance the per-trajectory trackers' optimization. 
% With the above designs, our method leverages an iterative approach that alternately 1) solves the per-trajectory tracking problem with the help of the tracking controller and the task structure prior model, and 2) trains a stronger tracking controller via supervision from imitation-ready data with high-quality action sequences. Specifically, in the beginning, we first sample a batch of samples, \emph{i.e.,} one hundred, to optimize for their per-trajectory tracking controllers. After that, the successful tracking results are collected to construct the first version of the action-labeled dataset. We then train the general controller via supervision provided by these action sequences. In the second stage, we sample another batch of trajectories from those that the current general policy cannot perform well. By optimizing their per-trajectory trackers using the initialization from the tracking controller, we obtain the second version of the action-label dataset. We then re-train the general tracking policy via guidance provided by the labeled dataset. In this stage, we find beneficial homotopy optimization paths via a heuristic-guided breadth-first searching strategy. The searched results can improve per-trajectory tracking results and can serve as the training from which we construct our tracking task structure prior model. In the third stage, we resample trajectories to grow the imitation-ready action-labeled trajectory dataset. We conduct per-trajectory tracking and try to improve previous tracking results via the guidance from the tracking data prior encoded in the tracking controller and the homotopy method leveraging optimization paths proposed by the tracking task structure prior model.  After that, we then re-train the general controller via these successful tracking results. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% high-quality labeled trajectories. 
% the third part of trajectories which are tracked via RL under the guidance of the tracking controller and curricula proposed by the learned curriculum scheduler.
% mine task curricula for improving difficult trajectories' tracking and learn the curriculum scheduler to model the curriculum prior. 
% rollout trajectories of such initial samples 
% 
% progressively improve the capability of the tracking controller. In the beginning, we 
% which gradually 
% solve a series of per-trajectory tracking optimization problem 
% tracking curriculum which can effectively solve difficult per-trajectory tracking problems, an automatic curricula mining strategy, and curriculum scheduler that models tracking curricula for efficient curriculum scheduling, and 3) an interactive optimization approach where per-trajectory trackers are gradually improved via tracking prior from the general tracking controller and effective curriculum scheduling, together with the tracking controller progressively getting stronger. 


% Moreover, the tracking prior encoded in the 
% Considering the limitations of the current advanced RL in solving single trajectory tracking problems, we design two strategies to improve per-trajectory trackers and optimize for raising the quality and diversity of the action-labeled dataset. The 
% % action-labeled trajectories produced by per-trajectory trackers to ease the training. 
% Considering the limitations of the current advanced RL in solving single trajectory tracking problems, we design two strategies to improve per-trajectory trackers and optimize for raising the quality and diversity of the action-labeled dataset. The first one lies in transferring general tracking prior to encoding in the tracking controller to speed up and enhance the per-trajectory trackers' optimization. Instead of optimizing the single trajectory tracker directly, we propose to use the data prior provided by the tracking controller which can offer us with a rough action trajectory to initialize the per-trajectory tracking optimization. 
% Secondly, instead of tracking each single trajectory along, we try to let the tracking task structural prior to plan optimization paths for solving tough single-trajectory tracking problems. 
% % and the inference time prior from the tracking task structural prior model to provide us with correct optimization paths to solve tough tasks finally. 
% % % use the action trajectory rollout from the tracking controller to initialize the policy so that the per-trajectory tracker can benefit from the general tracking prior, avoiding getting stuck into local optima and with the potential to converge faster. Secondly, instead of tracking each single trajectory along, we try to explore the potential of benefiting the single trajectory tracking problem, which is difficult to solve, from the tracking results of a different trajectory, formulating a tracking-curriculum where we start from simple problems and gradually solve the tough task finally. 
% Specifically, for a trajectory $A$ which is hard to optimize, the tracking curriculum tries to transfer the optimized action trajectory for task $B$ to initialize its policy to solve trajectory $A$'s tracking problem better finally. Since not every trajectory would benefit the tracking of trajectory $A$, leveraging this approach without to improve the per-trajectory tracking requires trail-and-errors for each trajectory, if without any prior guidance. Therefore, we further propose to learn a curriculum scheduler that can automatically plan a task curriculum to solve a difficult tracking problem. In more detail, we first mine such task curricula via testing such task relations from a small amount of data. After that, we train a model to describe such relations. 
% With the above designs, our method leverages an iterative approach that progressively improve the capability of the tracking controller. In the beginning, we first sample a batch of samples, \emph{i.e.,} one hundred, to optimize for their per-trajectory tracking controllers. After that, the successful rollout trajectories of such initial samples are collected to construct the first version of the action-labeled dataset. We then train the general controller via supervision provided by this dataset. In the second stage, we sample another batch of trajectories from those that the current general policy cannot perform well. By optimizing their per-trajectory trackers using the initialization from the tracking controller, we obtain the second version of the action-label dataset. We then re-train the general tracking policy via guidance provided by the labeled dataset. In this stage, we mine task curricula for improving difficult trajectories' tracking and learn the curriculum scheduler to model the curriculum prior. In the third stage, we resample for the third part of trajectories which are tracked via RL under the guidance of the tracking controller and curricula proposed by the learned curriculum scheduler. After that, we then re-train the general controller via all high-quality labeled trajectories. 


% where the per-trajectory trackers are efficiently and effectively improved together with a tracking controller that gradually become stronger taking advantage of tracking prior from the tracking controller and the curriculum scheduler. 
% an automatic curricula mining strategy that 
% breadth-first-searching that effecitlvye mines cross-task synergy relations and a curriculum schduler that models such relations for efficient curriculum schedule for improving per-trajectory trackers, and 3) an interactive approach where the per-trajectory trackers are efficiently and effectively improved together with a tracking controller that gradually become stronger taking advantage of tracking prior from the tracking controller and the curriculum scheduler. 
% a curriculum scheduler that models 
% an imitation augmented RL for improving the general tacker's performance with guidance from action-labeled trajectories produced by well-optimized single trajectory tracking specialists and a structural task relation space modeling as well as a task curriculum based on the molded task relations for improving single trajectory specialist controllers.
% from well-optimized trajectory-specific controllers  
% single trajectory tracking controllers to 

% current general tracking policy and the the structural cross-task relational model. 
% we search for cross-task relations, construct the structural task space and also distill them into a trajectory transformation model. 
% we try to transfer the optimization result from task $B$ to initialize its policy 
% Similar to the way of transferring tracking prior to improve the single trajectory tracking, for 
% Considering the difficulty and challenges in the dexterous manipulation tracking problem, single trajectory tracking controller optimization may still pose a significant challenges even for the current advanced RL algorithms, especially for very difficult manipulations. Therefore, to solve the manipulation tracking problem in such extremely challenging trajectories and to continuously improve the quality of specialist controllers, we propose to explore cross-task synergies in the manipulation tracking problem and improve each single trajectory tracker's performance leveraging cross-task synergies. Specifically, for each current task $A$, we wish to explore its ``parent tasks'' $\mathcal{P}_A$, so that task $A$'s optimization can benefit from the optimization result of its parent task $B\in \mathcal{P}_A$. By exploring such cross-task relations via bread-first-search, we can construct a structural task relation space from the given dataset. Each task pair is connected by a direct edge indicating which one can benefit from the other one and to what extent. We further propose to distill such searched cross-task relations into a trajectory transformation model, realized by a conditional diffusion model. This model can be further used to transform one given hard-to-optimize task to its ``parent task'', formulating a task curriculum to solve the current difficult task. We therefore train the general tracking controller by iteratively solving a single trajectory tracking problem for constructing a better action-labeled dataset and training the general tracker via the imitation augmented RL to let it benefit from such labeled guidance. Balancing the efficiency and the quantity as well as the quality of the action labeled dataset, our method for training the general tracking policy comprises three stages. At the beginning, we first sample a batch of samples, \emph{i.e.,} one hundred, to optimize for their trajectory-specific specialist tracking policies. After that, the successful rollout trajectories of such initial samples are collected to construct the first version of the action-labeled dataset. We then train the general tracking policy together via the imitation augmented RL via the labeled dataset. In the second stage, we sample another batch of trajectories from those that the current general policy cannot perform well. By conducting the trajectory-specific optimization on those trajectories, we obtain the second version of the action-label dataset. We then re-train the general tracking policy via guidance provided by the labeled dataset. In this stage, we search for cross-task relations, construct the structural task space and also distill them into a trajectory transformation model. In the third stage, we resample for the third part of trajectories which are tracked via RL under the guidance of the current general tracking policy and the the structural cross-task relational model. After that, we then re-train the general controller via all high-quality labeled trajectories till now. 

% demonstrate 

We demonstrate the superiority of our method and compare it with previous methods on challenging manipulation tracking tasks in two datasets, describing expressive hand-object interactions in daily and functional tool-using scenarios, involving complex object movements, difficult and subtle in-hand re-orientations, interactions with thin objects, and frequent hand-object rich contact variations. We conduct experiments in both the simulator, \emph{i.e.,} Isaac Gym~\citep{makoviychuk2021isaac},  and the real world to demonstrate the efficacy, generalization ability, and robustness of our general tracker to accomplish a wide range of manipulation tracking tasks and even excellently track novel manipulation trajectories (Figure~\ref{fig_intro_teaser}). We can track difficult manipulations involving expressive and complex object movements, detailed and subtle in-hand re-orientations, and frequent rich hand-object contact variations. Our approach successfully surpasses the previous methods both quantitatively and qualitatively, achieving more than 10\% success rate than the previous best-performed method. Besides, we conduct further analysis and demonstrate the various recovery behaviors of our controller, demonstrating its robustness to unexpected situations. Thorough ablations are conducted to validate the efficacy of our designs.

Our contributions are three-fold:
\begin{itemize}
    \item A scheme that combines reinforcement learning and imitation learning to effectively train a generalizable, versatile, and robust tracking controller, utilizing abundant high-quality imitation-ready data.
    % \item 
    % for effectively learning a generalizable, versatile, and robust tracking controller by leveraging reinforcement learning and imitation learning, utilizing abundant high-quality imitation-ready data.
    \item A per-trajectory optimization scheme for addressing challenging tracking problems using the tracking controller within a homotopy optimization framework.
    \item A homotopy optimization method for effectively solving difficult single trajectory tracking problems, an automatic homotopy optimization path exploration strategy, and a homotopy path generator that efficiently proposes beneficial optimization paths during inference.
    % \item A scheme for effectively learning a generalizable, versatile, and robust tracking controller taking advantage of reinfrmcemetn learning and imitation learning, leveraging abundant high-quality of imitation-ready data. 
    % \item A per-trajectory optimization scheme for solving difficult tracking problems using the tracking controller through a homotopy optimization paradigm. 
    % \item A homotopy method for solving very challenging single trajectory tracking problems effectively, an automatic homotopy optimization path exploration strategy, and a homotopy path generator that can efficiently propose beneficial optimization paths in the inference time. 
    % imitation-augmented RL technique that effectively facilitates tracking controller optimization via supervision from labeled trajectories with high-quality action sequences; 
    % eases the optimization difficulty of the tracking controller via supervision provided by high-quality action-labeled trajectories; 
    % A homotopy method for solving difficult tracking problems, an automatic tracking task optimization path searching strategy and a tracking task structure prior  model that can efficiently propose optimization paths for solving challenging optimization problems efficiently; 
    % An automatic 
    % tracking-curricula mining strategy and the design of a curriculum scheduler that expressively models the curriculum priors; 
    % An iterative approach that effectively improves per-trajectory trackers with the help from the tracking controller and the task structure prior model and gradually train stronger tracking controller. 
    % via tracking prior from the general tracking controller and the homotopy optimization path from the tracking task structure prior to solve challenging problems. 
    % the curriculum proposed by the curriculum scheduler. 
    % progressively improves the tracking controller via gradually enlarged and improved action-labeled data. 
\end{itemize}


% our tracker exhibits various recovery behaviours, 
% we also demonstrate its 
% Besides, optimizing through the physics curriculum can significantly enhance the performance of previously under-performed RL-based methods, almost completing the tracking problem from failure, as demonstrated in Fig.~\ref{fig_intro_teaser}. This indicates the universality of our approach to embodied AI through optimization via a physics curriculum. Thorough ablations are conducted to validate the efficacy of our designs.
% best-performed method 
% such as large rotations and complicated tool-using such as using a spoon to bring the water back and forth. Our approach successfully surpasses the previous best-performed method both quantitatively and qualitatively, achieving more than 11\% success rate than the previous best-performed method. Besides, optimizing through the physics curriculum can significantly enhance the performance of previously under-performed RL-based methods, almost completing the tracking problem from failure, as demonstrated in Fig.~\ref{fig_intro_teaser}. This indicates the universality of our approach to embodied AI through optimization via a physics curriculum. Thorough ablations are conducted to validate the efficacy of our designs.




% To be more specific, our method for training the general control policy compresises three stages. In the f
% % from which we can transfer the corresponding optimization results 


% expressive and difficult interactions 
% general controller that can universally track every mnaipulation trajectories in the dataset and can well generalize to unseen manipulations. \todo{rewrite this} 
% and grasping~\cite{xu2023unidexgrasp,wan2023unidexgrasp2}. 
% In this work we wish for a general controller 
% The task is inherently difficult 

% Some existing works rely on high-fidelity black-box simulators, where a small difference in robot control can result in dramatically different manipulation outcomes due to abrupt contact changes, making the tracking objective highly non-smooth and hard to optimize~\cite{qin2022dexmv,chen2023visual,christen2022d,rajeswaran2017learning,andrychowicz2020learning}. In this way, their tasks are restricted to relatively simple goal-driven manipulations such as pouring and re-locating~\cite{rajeswaran2017learning,qin2022dexmv,christen2022d,zhang2023artigrasp}, in-hand re-orientation, flipping and spinning~\cite{chen2023visual,andrychowicz2020learning} with a fixed-root robot hand, or manipulating objects with simple geometry such as balls~\cite{mordatch2012contact}. 



% focusing on a wide range of manipulation tasks -- dexterous manipulations tracking, we aim to explore
% we aim to explore the possibility of training a dexterous manipulation general policy. 

% Advancing an embodied agent's capacity to interact with the world represents a significant stride toward achieving general artificial intelligence. Due to the substantial costs and potential hazards of setting up real robots to do trial and error, the standard approach for developing embodied algorithms involves learning in physical simulators~\cite{coumans2016pybullet,makoviychuk2021isaac,todorov2012mujoco,wang2019redmax,hwangbo2018per,freeman2021brax,howell2022dojo} before transitioning to real-world deployment. In most cases, physical simulators are treated as black boxes, and extensive efforts have been devoted to developing learning and optimization methods for embodied skills within these black boxes. Despite the considerable progress~\cite{rajeswaran2017learning,chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,yao2022controlvae,fussell2021supertrack,grandia2023doc,peng2018deepmimic,wang2023physhoi,mordatch2012contact}, the question like whether the simulators used are the most suitable ones is rarely discussed.
% In this work, we investigate this issue and illustrate how optimizing the simulator concurrently with skill acquisition can benefit a popular yet challenging task in robot manipulation -- dexterous manipulation transfer.





==> articles/method.tex <==

% \section{Generalizable Dexterous Manipulation Tracking}
% \section{Dexterous Manipulation Tracking Control}
% \section{Generalizable Neural Tracking Control for Dexterous Manipulation}
\section{Method}

\vspace{-5pt}

% \todo{add the retargeting part}
 

\begin{figure}[h]
  \centering
  \vspace{-10pt}
  \includegraphics[width=\textwidth]{figs/method_19.pdf}
  \vspace{-20pt}
  \caption{\footnotesize
  % cks the potential for tr
  % Generalizable Dexterous Manipulation Tracking with Imitation Augmented RL and Structural Task Space Modeling. 
  % Dexterous Manipulation Tracking Control.
  % Iterative optimization to train a universal dexterous manipulation tracking controller. 
  % By augmenting RL with guidance from high-quality action-labeled data, \modelname unleashes the possibility of training a universal manipulation controller from human references. With the curriculum proposed by a curriculum scheduler that models the tracking curricula and the tracking prior provided by the tracking controller, we can in turn improve the quality of action-labeled trajectories. We adopt an interactive approach which finally offers us a universal tracking controller. 
  % \modelname unleashes the possibility of training a universal manipulation controller from human references by iteratively optimizing high-quality action-labeled trajectories and training the tracking controller via imitation-augmented RL with supervision from the labeled trajectories. Guiding RL with additional supervision from high-quality action-labeled data, \modelname effectively eases the difficulty in learning a universal tracking controller. Leveraging the tracking prior from the controller as well as the tracking curriculum proposed by a learned curriculum scheduler, we can effectively improve the quality and diversity of the action-labeled trajectories. 
  % \eric{The figure is not quite intuitive so far at the tracking prior part and the homotopy optimization part. I would suggest using a flow chart instead. I do not like the way how we visualize learning a neural network with PPO since it is not common and can not be understood immediately. We should consider checking other papers and borrowing their ways of illustration.}
  \href{https://projectwebsite7.github.io/gene-dex-manip/}{\modelname}learns a generalizable neural tracking controller for dexterous manipulation from human references. It alternates between training the tracking controller using abundant and high-quality robot tracking demonstrations, and improving the data
  % the data diversity and quality
  via the tracking controller through a homotopy optimization scheme.
  % By gradually optimizing the tracking controller and curating high-quality demonstration data in a bootstrapping manner, we can get a versatile, generalizable, and robust tracking controller finally. 
  % imitation-ready data 
  % unlocks the potential for training a universal manipulation controller from human references by iteratively curating high-quality, action-labeled trajectories and training the tracking controller through imitation-augmented reinforcement learning (RL) with supervision from these labeled trajectories. By guiding RL with supervision from the action-labeled data, we significantly reduce the challenges associated with learning a universal tracking controller. Utilizing the tracking prior from the controller and a tracking curriculum designed by a learned curriculum scheduler, we effectively enhance the quality and diversity of the action-labeled trajectories, driving improved performance.
  % The \textbf{parameterized quasi-physical simulator} relaxes the articulated multi rigid body dynamics as the \textit{parameterized point set dynamics}, 
  % controls the contact behavior via an unconstrained \textit{parameterized spring-damper contact model},
  % and compensates for unmodeled effects via \textit{parameterized residual physics networks}. 
  % We tackle the difficult dexterous manipulation transfer problem via \textbf{a physics curriculum}. 
  }
  \vspace{-15pt}
  \label{fig_method_pipeline}
\end{figure}

% \todo{change t to n}

% \todo{robot hand-obj kinematics dataset}

% (\emph{e.g.,} Allegro, LEAP, Shadow hand, etc.)

% The dexterous manipulation tracking control problem wishes to learn a tracking controller for a dexterous robot hand from human hand-object manipulation references. Given a manipulation sequence $(\mathbf{H}, \mathbf{O})$ describing the dexterous robot hand interacting with an object, \emph{e.g.,} obtained by kinematic retargeting from a human-object manipulation sequence, we expect the controller to robustly control the robot hand to manipulate the object so that both the resulting hand poses $\hat{\mathbf{H}}$ and the object poses $\hat{\mathbf{O}}$ can properly mimic their corresponding reference motions. We expect the controller to be able to track novel reference motions with unseen yet still challenging manipulation sequences and new objects. Such an ambitious vision is challenged by 1) the inherent difficulty underlying the tracking control problem resulting from intricate dynamics coming from frequently varying rich hand-object contacts and the complicated object movements, 2) the challenges in controlling a high-DoF dexterous robot hand to densely follow references, 3) the wish for a general tracking controller that can universally track every reference manipulations covering extremely challenging cases, and 4) the wish in high robustness and generalization ability side so that the controller can adapted to mimic unobserved references. 
% 

% The generalizable neural tracking control for dexterous manipulations from human references aims to leverage abundant and high-quality human-object interaction data to learn a generalizable manipulation tracking controller to equip a dexterous robot hand with versatile dexterous manipulation ability. Given a human-object interaction dataset containing, the tracking controller learns to track every manipulation sequence. At the test time, the tracking controller ought to generalize well to track novel, challenging human manipulation sequences with new objects, unseen hand, and object reference trajectories. Both advanced model-free RL based techniques and the model-based trajectory optimization would usually face significant challenges from the wish in the versatility and the generalization ability, the complex system, and the intricate dynamics from dynamic, rich contacts. 


% The problem is inherently difficult due to 1) the intricate dynamics involved in the dexterous manipulation that frequently challenges the optimization, 2) the high expectation in the versatility, high generalization ability, and the robustness of the controller. 

Given a collection of kinematic human-object manipulation trajectories, we wish to learn a generalizable and robust neural tracking controller for a dexterous robotic hand. 
% versatile, 
% from these references.
We expect the controller to equip the robot hand with a wide range of manipulation skills and also generalize well to robustly track novel and challenging manipulation tasks.
% a wide range of manipulation skills and also generalize well to robustly track novel and challenging manipulation tasks.
% tackle  novel and challenging manipulation tasks.
% track novel and challenging manipulations. 
% track 
% novel manipulation sequences with unseen object geometries and challenging, subtle in-hand manipulations. 
% to be able to 
The problem is inherently difficult because: 1) the complex dynamics of dexterous manipulation challenge precise control, which is crucial for delicate motions; 2) there are high expectations for the controller's adaptability, generalizability, and robustness.
% diverse 

% given a collection %


% \todo{exisitng methods?}
% dyanmcis 
% The problem is challenged by the 
% Either previous model-free techniques or model-based approaches 
% various novel manipulation 
% should be able to track 
% We expect the controller can not only track every manipulation sequence in the c
% with the aim to equipping a dexterous robot hand with versatile dexterous manipulation skills. We expect the tracking controller 
% generalizable neural tracking control 
% human-object interaction dataset c


% To overcome these challenges, the key of our method lies in 
% Our method 

% We propose a method that combines reinforcement learning (RL) with imitation learning (IL) to train a generalizable tracking controller using robot tracking demonstrations. Since acquiring high-quality demonstrations with paired kinematics and action sequences is challenging, we introduce a per-trajectory tracking scheme that enhances demonstration quality and diversity via homotopy optimization. By alternating between training the controller with high-quality data and generating improved demonstrations in a bootstrapping process, we develop an effective tracking controller. Detailed explanations of these steps are provided in Sections~\ref{sec:method_il_rl},~\ref{sec:method_data}, and~\ref{sec:method_iteration}.


To address these challenges, we propose to combine reinforcement learning (RL) and imitation learning (IL) to train a generalizable tracking controller using robot tracking demonstrations. Since acquiring high-quality demonstrations with paired kinematics and action sequences is challenging, we introduce a per-trajectory tracking scheme that enhances demonstration quality and diversity via the tracking controller through a homotopy optimization scheme. 
By alternating between training the controller with high-quality data and generating improved demonstrations in a bootstrapping process, we develop an effective tracking controller.
We will explain how we learn the neural tracking controller from demonstrations in Section~\ref{sec:method_il_rl}, how we mine high-quality demonstrations in Section~\ref{sec:method_data}, and how we iterate between learning controller and mining demonstrations in Section~\ref{sec:method_iteration}. 
% we propose to learn from a large number of robot tracking demonstrations and combine reinforcement learning (RL) with imitation learning (IL) to effectively train the tracking controller.

% a method that combines 
% in detail 
% homotopy optimization.
% Since obtaining high-quality dexterous manipulation tracking demonstrations with paired kinematics references and action sequences is difficult, we devise a per-trajectory tracking scheme where we improve the quality and diversity of demonstration data via the tracking controller through a homotopy optimization scheme. 
% We then alternate between training the tracking controller using high-quality demonstrations and curating more diverse and higher-quality demonstrations in a bootstrapping manner, ultimately developing an effective and generalizable tracking controller. We will explain in detail how we learn the neural tracking controller from demonstrations in Section~\ref{sec:method_il_rl}, how we mine high-quality demonstrations in Section~\ref{sec:method_data}, and how we iterate between learning controller and mining demonstrations in Section~\ref{sec:method_iteration}. 
% of a generalizable, versatile, and robust neural tracking controller with a wide range of high-quality robot tracking demonstrations. 

% due to inherent challenges in dexterous manipulation tracking,

% the demonstration data
% that can benefit from a tracking controller while effectively tackling the tracking challenge via homotopy optimization.
% to ensure the data flywheel functions well.

% imitation ready data 
% high-quality imitation-ready data 
% imitation-ready data. 
% which combines the 
% Our method tackles these challenges by training a tracking controller jointly using reinforcement learning and imitation learning to empower the controller with high generalization ability and versatility by learning abundant and high-quality imitation-ready data and also maintaining robustness towards unexpected situations taking advantage of interactions with the environment via trial-and-errors. However, acquiring a large number of imitation-ready data itself is costly and difficult due to challenges in the optimization side for single trajectory tracking. Therefore, to make sure the data flywheel functions properly, we alternate between training the tracking controller and mining more diverse and higher-quality imitation-ready data leveraging the tracking controller. 
% , using the tracking controller. 
% we wish to leverage high-quality and abundant imitation-ready data to train a tracking controller jointly with RL to let the tracking controller benefit from these successful to improve the versatility and the generalization ability. Due to the inherent difficulty in dexterous manipulation, we propose an iterative optimization approach where we alternately train the tracking controller and improve the quality and diversity of the imitation-ready data so that the data flywheel can function properly. 
% Our method wishes to 

% Our method consists of two key designs to realize this vision: 1) A learning-from-demonstration strategy that trains the tracking controller jointly via imitation learning and reinforcement learning, leveraging a large number of high-quality robot tracking demonstrations; 2) A per-trajectory tracking scheme that can effectively solve difficult single trajectory tracking tasks using a tracking controller through a homotopy optimization scheme, continuously providing tracking demonstrations.
% and a homotopy path generator, by transferring tracking prior in a homotopy manner. 
% imitation-ready data; 
% 
% which gradually mines 
% imitation-augmented reinforcement learning scheme to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance; 2) a per-trajectory tracking scheme that can leverage the general tracking controller to produce better imitation-ready data; and 3) a homotopy method and a homotopy generator that can better leverage the tracking controller to solve difficult per-trajectory tracking problem for mining imitation-ready data from challenging manipulation skills. 
% to overcome these challenges: 
% that can better leverage the general tracking controller to solve 
% effective for solving difficult per-trajectory tracking problem 
% mimicking the chain of thought, to better leverage the general tracking controller for mining imitation-ready data from challenging manipulation skills. 


% We devise a basic RL-based method to train the tracking controller with delicately design action space, observations, and rewards for the general manipulation tracking problem. To let the policy benefit from the imitation-ready data, we add an additional supervised loss which, at each time, 


% First, we leverage an imitation-augmented reinforcement learning scheme to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance. We devise a basic RL-based method to train the tracking controller with delicately design action space, observations, and rewards for the general manipulation tracking problem. To let the policy benefit from the imitation-ready data, we add an additional supervised loss which, at each time, encourages the policy to imitate the action of the corresponding timestep in the trajectory.  
% Second, we develop a per-trajectory tracking scheme which can leverage the general tracking controller to produce better imitation-ready data. To obtain high-quality imitation data with action trajectories that can successfully drive the dexterous robotic hand to track the correspondence hand and object sequence, we leverage the popular modle-free RL-based method by training a per-trjaectory tracking policy using RL and use the tracking result as the optimized imitation-ready data. Desptie no expectation in the versatility and generalization ability in the per-trajectory tracker, tracking difficult tracking problem is still very challenging. to improve the data quality and include more diverse imitation-ready data into the training of tracking controller, we propose to leverage the general tracking prior encoded in the tracking controller to improve the per-trajectory tracker optimization. Third, we design a homotopy path generator, mimicking the chain of thought, to better leverage the general tracking controller for mining imitation-ready data from challenging manipulation skills. Soley relying on tracking prior encoded in the tracking controller to improve the per-trajectory tracker is still not enough to solve very difficult per-trajecotyr tracking problem. It is because that the hard-to-track trajectories are too out-of-distribution to the data prior encoded in the tracking controller, trained with mitation-ready data that has been successfully tracked. Thus such trajectory problems can hardly benefit from the tracking prior from the current tracking controller. To resolve these challenges, we propose to solve these problems in a homotopy method. Specifically, instraed of solving the difficult per-trajectyr tracking problem directly, we start from tracking a different trajectory to obtain its tracking result. After that we design a technique which allows us to let the difficult per-trajectory tracking problem benefit from the tracking result. In this way we are able to solve the difficult tracking task by starting from an easy task and gradually solve a series of tsks with the tracking results transferred to the next one. Finding such beneficial optimization paths, however, is very time-consuming. To further improve the efficiency, we propose to learn a tracking task structure prior model, which, in the inference time, can efficiently propose beneficial optimization paths for a tough single trajectory tracking problem. With the above three designs, we alternately 1) train the tracking controller and learn the tracking task structure prior model with high-quality imitation-ready data and 2) improve the data via the tracking controller and the tracking task structure prior model. The data flywheel can then function well, making it possible for us to train a strong tracking controller finally. 




% we propose to alternately train strong tracking controller and improve the imitation ready data 
% as well as the intriacat dynamics from dynamic and rich conta

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% The key idea idea lies in leveraging high-qualtiy abutndaten imitation-ready data to train a tracking controller jointly with RL and tackling the difficulties in acquiring such data by leveraging the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner. At train time, given a collection of human hand object manipulation trajectories, we first retarget human hands to robotic dexterous hands in the data preparation stage, resulting in a reference manipulation  set containing retareted hand trajecotires and the original object pose sequences.  Our method then alternates between mining useful imitation-ready data from the reference motion set and training the tracking controller with the mined data. W
% e have three key designs to enable the data flywheel to function effectively. First, we leverage an imitation-augmented reinforcement learning scheme to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance. We devise a basic RL-based method to train the tracking controller with delicately design action space, observations, and rewards for the general manipulation tracking problem. To let the policy benefit from the imitation-ready data, we add an additional supervised loss which, at each time, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The wish in the generalization ability and versatility a
% adn versatility usually challenge popular advanced RL approaches which often requires task-specificd reward designs
% The problem is inherently chall
% The learned neural tracking controller is expected to be able to 
% At the train time, the tracking controller is optimized to track every manipulation trajectory in the training 
% Given a datset containing 
% The neural tracking control for dexterous manipulations aims at leverage human hands manipulating objects trajectories, which have abundant data sources covering the internet videos and motion synthesis models, to learn a versatile and generalizable tracking controller. Given a dataset containing diverse human-object interaction trajecotires, the controller is optimized aiming to track every manipulation trajectory in the dataset. Specifically, with the kinematics only human object manipulation trajectory as input, the tracking controller aims at output an action trajectory that can mimic the kinematic trajectory -- when letting a dexterous robot hand execute the output action trajectory, the resulting hand states and object states should be close to their corresponding kinematic trajecotires in the input sequence. A versatile and genralizable tracking controller ought be able to generalize to novel and enve challenging interactions wit new and difficult objects. At the test time, given an manipulation sequence where both the hand motion adn the object movements and the object geometry are usnee during the training, the controller is epxcted to give proper action outputs that can drive the dexterous roobt hand to precisely control the object so that the resulting hand sequence adn the object sequences are close to the input reference. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The problem of dexterous manipulation tracking control aims to develop a tracking controller for a dexterous robot hand based on human hand-object manipulation references. Given a manipulation sequence $(\mathbf{H}, \mathbf{O})$, we expect the controller to robustly control the robot hand to manipulate the object to mimic the reference motions closely. Specifically, the resulting hand poses $\hat{\mathbf{H}}$ and the object poses $\hat{\mathbf{O}}$ should accurately follow their respective reference motions. Furthermore, the controller should be capable of tracking novel reference motions involving unseen, complex manipulation sequences and new objects. This ambitious vision is challenged by several difficulties: 1) The inherent difficulty of the tracking control problem, coming from the intricate dynamics arising from frequently changing hand-object contacts and complex object movements; 2) The challenge of controlling a high-degree-of-freedom (DoF) robot hand to accurately follow dense reference points; 3) The need for a general tracking controller that can universally track diverse and highly challenging manipulation cases; 4) The requirement for high robustness and generalization, enabling the controller to adapt and accurately mimic previously unobserved reference motions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% due to the intricate dynamics arising from 
% \(\hat{\mathbf{H}}\) and object poses \(\hat{\mathbf{O}}\) 

% so that the resulting hand and object trajectories could closely mimic the reference motions. 
% in a way that closely mimics the reference motions.
% which describes the interaction between the robot hand and an object (\textit{e.g.}, obtained via kinematic retargeting from a human-object manipulation sequence), the goal is for the controller to robustly manage the robot hand to manipulate the object in a way that closely mimics the reference motions. 

% hindered by several challenges: 
% 1. The inherent difficulty of the tracking control problem due to the intricate dynamics arising from frequently changing hand-object contacts and complex object movements.
% 2. The challenge of controlling a high-degree-of-freedom (DoF) robot hand to accurately follow dense reference points.
% 3. The need for a general tracking controller that can universally track diverse and highly challenging manipulation cases.
% 4. The requirement for high robustness and generalization, enabling the controller to adapt and accurately mimic previously unobserved reference motions.

% The manipulation sequence may contain novel manipulation sequences and new object geometries that the controller is never aware of. We still expect the controller to be able to deal with such novel tracking targets. 

% inherent difficulty of controlling a dexterous hand to densely track a manipulation trajectory with complex object motions, the intricate dynamics resulting from the rich and changing contacts between the hand and the object, the difficulty of controlling a high DoF dexterous hand, and the morphology difference, 2) the vision of learning a single policy that can universally track all trajectories, and 3) the wish of the high generalization ability to unseen and difficult manipulations for the policy. 

% Given a set of human hand-object manipulation demonstrations $\mathcal{S}=\{ ( \mathbf{H}, \mathbf{O} ) \}$, the dexterous manipulation tracking control problem aims at learning a single tracking controller that can control a dexterous robot hand to manipulate the object so that both resulting hand poses and the object poses can accurately follow their corresponding references in the kinematic demonstration. Given new manipulations involving novel interactions and unseen object geometries, we expect the controller to generalize well and robustly track those unobserved manipulations. 
% % the generalizable dexterous manipulation tracking aims at learn a single general tracking policy that 1) can successfully track each trajectory in the dataset and 2) can generalize well to novel manipulation trajectories unseen during training.
% Formally, given a multi-fingered dexterous robot hand (\emph{e.g.,} Allegro, LEAP, Shadow hand, etc.) we wish to learn a tracking controller $\mathbf{\pi}(\cdot\vert \cdot)$ from the given kinematic-only human-object interaction demonstrations $\mathcal{S}$. 
% For each manipulation trajectory $(\mathbf{H}, \mathbf{O})$, $\mathbf{\pi}(\cdot\vert \cdot)$ should be able to output a physically plausible control sequence $\mathbf{A}$ that is able to drive the dexterous robot hand to manipulate the object so that the resulting hand trajectory $\hat{\mathbf{H}}$ and the object trajectory $\hat{\mathbf{O}}$ are close to the reference motion $(\mathbf{H}, \mathbf{O})$. 
% % the object according to the kinematic demonstration $(\mathbf{H}, \mathbf{O})$, where both the resulting hand sequence and the object sequence should be close to their corresponding target trajectories. 
% Besides, given a novel manipulation trajectory unseen during the training, we wish $\mathbf{\pi}(\cdot\vert \cdot)$ can generalize well and output a reasonable manipulation trajectory that can physically track the demonstration accordingly. The vision of learning a generalizable tracker is challenged by 1) the inherent difficulty of controlling a dexterous hand to densely track a manipulation trajectory with complex object motions, the intricate dynamics resulting from the rich and changing contacts between the hand and the object, the difficulty of controlling a high DoF dexterous hand, and the morphology difference, 2) the vision of learning a single policy that can universally track all trajectories, and 3) the wish of the high generalization ability to unseen and difficult manipulations for the policy. 

% primarily in the locomotion domain, % 
% Considering the above huge challenges, directly training a policy aiming to track each manipulation trajectory would challenge both current advanced model-based and model-free techniques. Inspired by the data scaling law in other spaces, we propose to leverage a large number of imitation-ready data with both demonstrations and action sequences that can correctly drive the hand to precisely mimic the reference trajectory to train a general tracking controller. However, optimizing a large number of high-quality imitation-ready data itself is very challenging. Therefore, we propose to facilitate and enhance the per-trajectory tracking optimization via data prior from the tracking controller and the task structure. Specifically, instead of solving each tracking problem alone, we propose to solve difficult tasks via a homotopy method. It tries to solve a difficult problem by gradually solving each task in the optimization path and transferring results to the next. To efficiently find correct optimization paths, we further propose to encode such structural relations into a model, which is leveraged to propose optimization paths directly during the inference. We then present an iterative optimization strategy that gradually improves each side and finally lets us arrive at a general tracking controller. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% could let us arrive at a general tracking controller finally. 
% Letting the model propoe correct optimization paths could spare us lots of time cost in the trail and error in finding optimization paths. We then present an iterative optimization strategy that could let us arrive at a general tracking controller finally. 
% through an optimization path. This path contains a series of per-trajectory tracking problems. A good path can let us solve the final problem better by solving each problem and transferring results to the next task one-by-one. 

% interactive strategy that could let us arrive at a general 
% Consideirng the dependencies between the tracking controller, tracking task structural prior, 

% To improve the efficiency of finding correct optimization paths, we further propose to search such beneficial optimization paths 
% The task structural prior 
% The homotopy method optimizes a tracking task of interest 
% tracking task structure prior. The tracking task structure encodes cross-task relations 
% The tracking task structural prior 
% Specifically, we leverage RL to train per-trajectory tracking policies. 
% We further propose to use tracking prior from the tracking controller 
% to solve difficult pre-trajectory tracking problem and impro
% is not feasible 
% We adopt a model-free approach to solve the problem considering the recent success achieved by model-free RL in developing strong and even universal controllers~\citep{Luo2024GraspingDO,xu2023unidexgrasp,wan2023unidexgrasp2,Luo2023PerpetualHC,Luo2023UniversalHM}. However, despite the strong capability of RL demonstrated in other tasks, directly training a policy aiming to track each manipulation trajectory is not feasible due to the above huge challenges. Compared to using a universal tracking controller, single trajectory tracking is an easier problem to solve. Observing recent trials and success in combining expert demonstrations or policies with RL, \todo{add refs}, we explore the possibility of learning a tracking controller with the joint effort of RL and guidance from high-quality action-labeled data. However, despite the eased difficulty in training per-trajectory trackers, advanced solutions would still fall short in resolving very difficult tracking problems or are extremely time-consuming~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}. This makes optimizing for abundant and high-quality action-labeled trajectories itself a very difficult problem. Observing the power of the foundation model in solving downstream tasks effectively and inspired by the recent success in leveraging curriculum learning to tackle difficult tasks~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}, we propose to improve the quality and diversity of action-labeled dataset via tracking prior from the tracking controller and correct tracking curriculum. Since finding correct curricula will cost a lot of time and requires trial and error, we present an automatic tracking curricula mining strategy and propose to learn a curriculum scheduler, which can be used to propose good curricula, from the mined valid curricula. The dependencies between high-quality per-trajectory trackers and the general tracking controller as well as the curriculum scheduler pose us a ``chicken-and-egg''  puzzle. We therefore propose an iterative approach that progressively enhances each side and finally lets us arrive at a universal tracking controller. 


% We adopt a model-free approach to tackle this problem, motivated by the recent success of model-free reinforcement learning (RL) in developing robust and even universal controllers~\citep{Luo2024GraspingDO,xu2023unidexgrasp,wan2023unidexgrasp2,Luo2023PerpetualHC,Luo2023UniversalHM}. However, despite the demonstrated strength of RL in other tasks, directly training a policy to track individual manipulation trajectories is not feasible due to the significant challenges outlined earlier. While using a universal tracking controller is highly complex, tracking a single trajectory presents a more manageable problem. 
% Recent advancements combining expert demonstrations or policies with RL have shown promise in addressing these challenges \todo{add refs}. Building on this, we explore the potential of developing a tracking controller by integrating RL with high-quality, action-labeled data. Although training per-trajectory trackers is more straightforward, even advanced solutions often fall short when faced with exceptionally difficult tracking problems, or they become prohibitively time-consuming~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}. As a result, optimizing a large, high-quality action-labeled dataset remains a complex task.
% Inspired by the power of foundation models to solve downstream tasks effectively, and drawing from recent successes in curriculum learning for tackling difficult challenges~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}, we propose enhancing the quality and diversity of the action-labeled dataset by leveraging a tracking prior from the controller and applying a refined tracking curriculum. Given the trial-and-error nature and time costs associated with identifying the correct curricula, we introduce an automatic tracking curriculum mining strategy. Additionally, we propose learning a curriculum scheduler that can suggest effective curricula based on the mined valid ones.
% The interdependencies between high-quality per-trajectory trackers, the general tracking controller, and the curriculum scheduler create a “chicken-and-egg” problem. To address this, we propose an iterative approach that progressively improves both components, ultimately leading to the development of a universal tracking controller.


% to effecitly improving the quality and diversity of action-labeld trajecotries taking advantage the joint power of per-trajectory tracking policy optimization, 
% due to the inherent difficulty in the manipulation tracking problem and the vision of tackling multiple and heterogeneous trajectory tracking problems at once.
% Considering the recent success achieved by model-free reinforcement learning in developing strong and even universal controllers~\citep{Luo2024GraspingDO,xu2023unidexgrasp,wan2023unidexgrasp2,Luo2023PerpetualHC,Luo2023UniversalHM}, and the little assumption in the known system dynamics, which may be very difficult to model to model for dexterous manipulations, we adopt a model-free approach and wish to leverage the reinforcement learning to learn a tracking policy for solving the problem. Directly training a policy aiming to track each manipulation trajectory in the dataset is not a feasible solution due to the inherent difficulty in the manipulation tracking problem and the vision of tackling multiple and heterogeneous trajectory tracking problems at once.
% where 
% \todo{some descriptions w.r.t. the distinctions and heter. within trajs?} 
% Based on the key observation in the benefit brought by the supervision provided by successful tracking trajectories\todo{rewrite this}, we pursue a strategy that can leverage the power of action-labeled manipulation trajectories to ease the difficulty in learning a universal tracking controller\todo{rewrite this -- unleash the power of data in xxx}. This further leads us to the problem of efficiently acquiring abundant high-quality action-label trajectories in an affordable time budget. Recent advances in model-free or model-based strategies to optimize an action trajectory that can successfully track a single trajectory either fall short in quality or is highly inefficient~\citep{christen2022d,zhang2023artigrasp,liu2024quasisim}. Successful trials in curriculum learning to solve difficult problems~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim} let us explore what's good structural relations we can explore in this problem that is beneficial to improve single trajectory tracking. However, despite the effectiveness, curriculum learning itself is time-expensive with additional requirements in the trial-and-error to find correct curricula. With the observation of the general knowledge encoded in the foundation model to zero-shot solving specific problems, we wonder about the possibility of leveraging the tracking knowledge learned by the tracking controller to help single trajectory tracking. This further led us to wonder if can we learn a curriculum scheduler from cross-trajectory relations encoding cross-task optimization synergies so that the scheduler can efficiently plan a task curriculum for us to solve each difficult tracking problems? The dependencies between high-quality per-trajectory trackers and the general tracking controller as well as the curriculum scheduler pose us a ``chicken-and-egg''  puzzle. We therefore propose an iterative approach that progressively enhances each side and finally lets us arrive at a universal tracking controller. 

% However we face a ``chicken-and-egg'' puzzle since acquiring  high-quality abundant action-labeled data efficiently is itself not feasible due to restrictions of current techniques.  Therefore, 
% However, despite the recent achievements, 
% Optimizing for an effective policy that can track a single manipulation trajectory is already extremely challenging considering the difficulties of the non-smooth dynamics and frequent rich contact variations. Training a generalist policy that can solve such a tough manipulation tracking problem is even more difficult. Training a single controller capable of tracking diverse motions often challenges advanced RL techniques. However, optimizing out a reasonable control trajectory for each not-too-difficult single manipulation sequence is feasible under the support of current techniques. Therefore, a natural question is can we design a strategy that can resolve difficulties in single trajectory tracking and manage to get a specialist policy and then leverage such optimized specialist policies to train the generalist policy? However, acquiring such as generalist for each single trajectory is too expensive and almost unaffordable due to the heavy time cost. Moreover, optimizing each trajectory independently may still struggle with solving extremely challenging problems. This naturally leads us to find cross-tracking task synergies to enhance each single task's performance. With the above considerations, we propose a specialist-generalist-specialist training scheme and a task curriculum, powered by a heuristic-guided task relational space exploration and modeling, for iteratively improving the capability of the generalist policy and enhancing the single manipulation trajectory tracking performance. 
% \todo{rewrite this paragraph.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method comprises three key designs: 1) an imitation augmented RL algorithm that can effectively optimize a tracking controller taking the joint effort from RL and guidance from action-labeled trajectories (Sec.~\ref{sec:method_il_rl}), 2) a homotopy optimization scheme for solving difficult per-trajectory tracking problem, an optimization path searching strategy, and a tracking task structure prior model that encode optimization paths (Sec.~\ref{sec:method_task_space_modeling}), and 3) an iterative optimization scheme which alternately improve the imitation-ready data and train the tracking controller for optimizing a powerful tracking controller finally (Sec.~\ref{sec:method_sgs}).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% a tracking task structure modeling strategy, and tracking task structure prior model that can efficiently propose correct optimization paths in the inference time to solve difficult problems via a homotopy method (Sec.~\ref{sec:method_task_space_modeling}), and 3) an iterative optimization scheme which alternately improve the imitation-ready data and train the tracking controller for optimizing a powerful tracking controller finally (Sec.~\ref{sec:method_sgs}).
% n automatic tracking curriculum searching strategy and a curriculum scheduler that models valid tracking curricula, which can be used to propose correct curricula for tracking very difficult trajectories  (Sec.~\ref{sec:method_task_space_modeling}), 3) an interactive optimization approach that progressive 1) improve the universal tracking controller, and 2) enalarge and improve the action-labeled dataset via tracking prior from the tracking controller as well as the curriculum scheduling (Sec.~\ref{sec:method_sgs}).
% such relations via a conditional diffusion model
% could benef
% general tracking controller's training from abundant high-quality action-labeled data 

% ``specialist-generalist-specialist'' training strategy which iteratively optimizing out better specialists, leveraging the cross-task synergies from the task relational model and the generalist policy, and improving the generalist performance by training with more and better specialists 
% task relational space modeling scheme with a heuristic-guided searching algorithm for constructing the task relational space and a conditional diffusion model for describing such relations 
% that could leverage action-labeled data to 
% enhance the performance of the generalist policy 
% % cross-task synergy modeling scheme 

% effectively let the generalist policy benefit from more and better action-labeled single trajectory manipulation's optimization result and 
% a heuristic-guided searching method for building the structural task relational space, which summarizes the cross-task optimization synergies in the manipulation tracking problem, 
% 2) an effective optimization scheme that 

% as well as an offline action trajectory and then leveraging such 
% that can manage to optimize for a reasonable control sequence for each manipulation trajectory 
% Directly leveraging davnaced RL techniques to train a single tracker capable of tracking diverse motions 

% \textcolor{red}{(TODO: explain why we employ a generalist-specialist-generalist approach, why we start from the specialist training; Explain the overall high level motivations at first and then continue with the key designs)}
% Our method comprises two key designs to tackle these challenges: 1) an imitation augmented RL algorithm that could leverage action-labeled data to learn a general tracking policy, 2) an effective optimization scheme for solving difficult tracking problems with an automatically explored hierarchical trajectory space, a distilled task translation model, and a task curriculum, and 3) an interactive model training and action-labeled data acquisition and improvement scheme leveraging the universal policy and the distilled task translation model. 
% \textcolor{red}{(TODO: Add section labels)}
% \textcolor{red}{(TODO: may be swap 1 and 2)}

% \todo{action labeled dataset for training the tracking controller}

% \todo{curriculum scheduler}

% \todo{using the above two tools to improve per-trajectory trackers}


% Consider %

% specialist formulation
% specialist formulation --- 
% d

% \todo{add some explanations on the kinematic retargeting}

% \todo{though the retargeted trajectories have noise, actually we would not be restricted by such noise}

% \todo{add the residual policy --- actually it is somewhat interesting and would not restrict us into adjacent part of the original kinematic trajectory}



% \subsection{Generalist Training via Imitation Augmented RL} \label{sec:method_il_rl}
% \subsection{Tracking Controller Training via Imitation Augmented RL} \label{sec:method_il_rl} 
% \subsection{Tracking Controller Training via Imitation Augmented RL} \label{sec:method_il_rl} 

\vspace{-5pt}
\subsection{Learning a Neural Tracking Controller from Demonstrations} \label{sec:method_il_rl} 
\vspace{-5pt}
% \eric{Imitation-augmented RL refers to a pretty broad range of methods and there are already a lot of similar algorithms in the literature. We don't necessarily need to come up with a name for this algorithm since it is probably not a very big deal. We could simply use ``learning a neural tracking controller from demonstrations'' as the subsection title. We could first motivate the usage of RL and IL together since RL is better at coping with dynamic state disturbance while IL can benefit from a large number of demonstrations. Then describe the RL part. Later, incorporate the IL part. Finally, conceptually analyze the framework a bit. see below.}

% \eric{We should conceptually compare with the old DAPG paper (Learning Complex Dexterous Manipulation with
% Deep Reinforcement Learning and Demonstrations) and also add ablations in the experiment section to motivate the necessity of coming up with the current approach. 
% For me, the difference sounds to be that we are doing tracking so even using RL the explored states will not deviate from the given trajectory too much, making the current design possible. In the current design, from RL's perspective, the imitation loss biases RL policy's action toward the imitation source to improve sampling efficiency. From IL's perspective, RL is injecting noises into the states to make learning more robust similar to DART.}

% We could first motivate the usage of RL and IL together since RL is better at coping with dynamic state disturbance while IL can benefit from a large number of demonstrations. Then describe the RL part. Later, incorporate the IL part. Finally, conceptually analyze the framework a bit. see below.

% \eric{Imitation-augmented RL refers to a pretty broad range of methods and there are already a lot of similar algorithms in the literature. We don't necessarily need to come up with a name for this algorithm since it is probably not a very big deal. We could simply use ``learning a neural tracking controller from demonstrations'' as the subsection title. We could first motivate the usage of RL and IL together since RL is better at coping with dynamic state disturbance while IL can benefit from a large number of demonstrations. Then describe the RL part. Later, incorporate the IL part. Finally, conceptually analyze the framework a bit. see below.}

% To train a tracking controller that can benefit from a large number of imitation-ready data and also be robust to dynamic state disturbances, we leverage reinforcement learning and imitation learning to train a tracking controller. Specifically, we propose an RL-based training strategy with carefully designed action apace, observations and rewards for the manipulation tracking problem. We further present an additional imitation loss so that we can train the tracking controller with additional supervision from the imitation-ready data with high-quality action sequences. 

% Given a collection of human-object manipulation trajectories and a set of high-quality robot tracking demonstrations, we wish to learn an effective and generalizable neural tracking controller. 
% In the beginning, we retarget human hand-object manipulation to a robotic hand as a data pre-processing step. 
% We combine RL and IL to develop a generalizable and robust neural tracking controller. 
% Taking advantage of imitating diverse and high-quality robot tracking demonstrations, we can effectively let the tracking controller master diverse manipulation skills and also equip it with high generalization ability. Jointly leveraging the power of RL, the controller would not get overfit to imitating successful tracking results covering a narrow distribution, maintaining strong robustness to dynamic state disturbances. Specifically, we design an RL-based learning scheme for training the tracking controller, including the carefully-designed action space, observations, and the reward tailored for the manipulation tracking task. We also introduce an IL-based strategy that lets the tracking controller benefit from imitating high-quality demonstration data. 
% By integrating these two approaches, we effectively address the complex problem of generalizable tracking control.


Given a collection of human-object manipulation trajectories and a set of high-quality robot tracking demonstrations, our goal is to learn an effective and generalizable neural tracking controller. 
In the beginning, we retarget human hand-object manipulation to a robotic hand as a data preprocessing step. We combine RL and IL to develop a generalizable and robust neural tracking controller. 
Taking advantage of imitating diverse and high-quality robot tracking demonstrations, we can effectively let the tracking controller master diverse manipulation skills and also equip it with high generalization ability. 
% Jointly leveraging the power of RL, the controller would not get overfit to imitating successful tracking results covering a narrow distribution, therefore maintaining strong robustness to dynamic state disturbances. 
Jointly leveraging the power of RL, the controller avoids overfitting to successful tracking results limited to a narrow distribution, thereby maintaining robust performance in the face of dynamic state disturbances.
Specifically, we design an RL-based learning scheme for training the tracking controller, including the carefully-designed action space, observations, and the reward tailored for the manipulation tracking task. We also introduce an IL-based strategy that lets the tracking controller benefit from imitating high-quality demonstration data. 
By integrating these two approaches, we effectively address the complex problem of generalizable tracking control.


% Combining the best of the two worlds, we finally succeed in the complex generalizable tracking control problem. 
% from the trajectories. 

% Then, in our formulation, the neural tracking controller is an agent that interacts with the environment according to a tracking policy $\pi$. At each timestep $n$, the policy observes the state $\hat{\mathbf{s}}_n$, consisting of the current state of the robotic dexterous hand and the object state, and the next goal $\mathbf{s}_{n+1}$, commanded as the next state of the robotic hand in the retargeted sequence and the next goal object state. Then the agent then samples an action $\mathbf{a}_n$ from the policy $\mathbf{a}_n\sim \pi(\cdot \vert \mathbf{s}_n, \mathbf{s}_{n+1})$. After applying action to the robotic dexterous hand, the hand transits and physically interacts with the object. The resulting hand state and the object state should be close to their corresponding nextstep state in the reference trajectory. 
% tracking policy $\pi_{\theta}$. At 
% We then combine reinforcement learning (RL) and imitation learning (IL) to develop a generalizable, versatile~\eric{we are using versatile a lot from the very beginning but it is not quite clear what it indeed refers to.}, and robust neural tracking controller. 

% reinforcement learning (RL) and imitation learning (IL) 
% leveraging knowledge learned 
% from the abundant data. 
% imitation-ready data, 
% Jointly leveraging the power of the reinforcement learning, we 
% equip the tracking controller with 
% we let the tracking controller 
% so that it can benefit from abundant imitation-ready data while maintaining robustness to dynamic state disturbances. 

% a well-defined action space, observations, and the reward 
% We design an RL-based strategy for solving the tracking controller problem, including a well-defined action space, observation framework, and reward structure tailored for the manipulation tracking task. 
% We begin by motivating the integration of RL, which excels in handling dynamic challenges, with IL, which benefits from extensive demonstration data. 
% Our RL-based strategy includes a well-defined action space, observation framework, and reward structure tailored for the manipulation tracking task. 

% let the 
% To guide the learning of the tracking controller, we introduce an imitation learning scheme to jointly train the controller with RL. 

% imitation loss 
% exploration of the RL's agent, we introduce an
% and to let us succeed in the generalizable tracking control problem, we 

% We will illustrate details as follows. 
% benefit the tracking controller 
% to enhance training by adding additional supervision from high-quality demonstration data. 
% with high-quality action sequences from the demonstration data, allowing for additional supervision. Finally, we will conceptually analyze this framework to highlight its effectiveness in training a neural tracking controller from demonstrations.
% which adds additional supervision 
% as an additional super


% To develop a generalizable and versatile neural tracking controller that can benefit from abundant imitation-ready data while maintaining robustness to dynamic state disturbances, we combine reinforcement learning (RL) and imitation learning (IL). 
% benefiting from abundant imitation-ready data while 
% that is versatile 
% utilizes abundant imitation-ready data 

% consider an approach where

% We design an imitation augmented RL algorithm to train the tracking controller. It is composed of a basic tracking policy and an action supervised loss. Given an action-labeled dataset composed of trajectories with high-quality action sequences, we can overcome the difficulty of training the general controller solely via RL leveraging the additional supervision provided by the action-labeled trajectories. 
% can benefit the tracking controller's learning via this strategy. 
% Optimizing the tracking controller aiming to solve multiple tracking problems is difficult considering the inherent poor multi-task ability of RL. \todo{add refs}
% Directly using advanced RL to train a tracking controller is an extremely challenging problem considering the inherent difficulty of dexterous manipulations and the high demand for generalization ability, versatility, and robustness. In comparison, single trajectory tracking, expecting no generalization ability or versatility, is an easier problem. Inspired by recent exploration and achievements on introducing supervision, either from the offline dataset, online trajectory optimization, or experts, into RL~\citep{rajeswaran2017learning,Liu2023BlendingIA}, we design an imitation augmented RL algorithm, composed of a basic tracking policy and an action supervised loss. Given an action-labeled dataset composed of trajectories with  high-quality action sequences, we can benefit the tracking controller's learning via this strategy. 
% with dedicated   to train the tacking controller, composed of a basic tracking 
% Single trajectory tracking is an 
% Inspired by 
% % Training a general tracking controller with the expectation of tracking all trajectories directly always turns out to be a problem that is too difficult to solve by current reinforcement learning techniques. 
% Therefore, instead of optimizing the general tracker directly,  we propose to augment the training with supervision from the action-labeled dataset to ease the training~\citep{Jenelten2023DTCDT,rajeswaran2017learning,Liu2023BlendingIA}. We delicately design the observations and rewards so that by leveraging advanced RL as the base approach we can solve many single trajectory tracking problems. With high-quality action-labeled trajectories rollout by their optimized per-trajectory trackers, we then propose an imitation augmented RL training scheme to ease the training and improve the general tracking controller. 
% How to leverage experts or offline datasets to improve RL training is still an active research topic currently. 
% Despite previous successful trials in other scenarios~\citep{Jenelten2023DTCDT,rajeswaran2017learning,Liu2023BlendingIA}, how to unleash the power of this trend of methods for dexterous manipulation tracking generalist poses many unique challenges. 
% Instead of directly training a generalist policy aiming to track all trajectories directly, which always turns out to be a problem that is too difficult to solve by current RL techniques, we propose to augment the training with the supervision from action labeled dataset for ease and speed up the policy learning. \todo{some references w.r.t. this approach} 
% \todo{rewrite the next sentence}
% To fulfill this vision, we need to curate action-labeled trajectories. Therefore, we again propose to leverage RL to train a trajectory-specific tracking policy to infer actions for the trajectory. 

\noindent\textbf{Neural tracking controller.} 
% In our formulation, the neural tracking controller is an agent that interacts with the environment according to a tracking policy $\pi$. At each timestep $n$, the policy observes the observation $\mathbf{o}_n$. $\mathbf{o}_n$ is computed based upon the current state $\mathbf{s}_n$, the next goal $\hat{\mathbf{s}}_{n+1}$ which is commanded as the next goal state of the robotic hand and the next goal object state, and the object geometry.
% Then, the agent samples an action $\mathbf{a}_n$ from the policy $\mathbf{a}_n\sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})$. After applying action to the robotic dexterous hand, the hand moves and physically interacts with the object. After that, both the hand and the object transit into the next state according to the environment dynamics, \emph{i.e.,} ${\mathbf{s}}_{n+1} \sim p(\cdot \vert {\mathbf{s}}_n, \mathbf{a}_n)$. 
% The resulting hand state and object state should closely match their respective next goal states.
In our formulation, the neural tracking controller acts as an agent that interacts with the environment according to a tracking policy \(\pi\). At each timestep \(n\), the policy observes the observation \(\mathbf{o}_n\) and the next goal \(\hat{\mathbf{s}}_{n+1}\) (designated as the target state for the robotic hand and the object). The policy then computes the distribution of the action. Then the agent sample an action $\mathbf{a}_n$ from the policy, \emph{i.e.,} \(\mathbf{a}_n \sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})\). The observation $\mathbf{o}_n$ primarily contains the current state $\mathbf{s}_n$ and the object geometry. 
% which is primarily computed based on the current state \(\mathbf{s}_n\) and the next goal \(\hat{\mathbf{s}}_{n+1}\) (designated as the target state for the robotic hand and the object). The policy then computes the distribution of the action. Then the agent sample an action $\mathbf{a}_n$ from the policy, \emph{i.e.,} \(\mathbf{a}_n \sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})\). The observation $\mathbf{o}_n$ primarily contains the current state $\mathbf{s}_n$ and the object geometry. 
% Then the agent 
% and the object geometry. 
% computed based on the current state \(\mathbf{s}_n\), the next goal \(\hat{\mathbf{s}}_{n+1}\) (designated as the target state for the robotic hand and the object), and the object geometry.
% The agent then samples an action \(\mathbf{a}_n\) from the policy, \emph{i.e.,} \(\mathbf{a}_n \sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})\). 
Upon executing the action with the robotic dexterous hand, the hand physically interacts with the object, leading both the hand and the object to transition into the next state according to the environment dynamics, represented as \(\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)\). 
% An effective tracking controller should let the resulting hand and object states should closely align with their respective next goal states.
An effective tracking controller should ensure that the resulting hand and object states closely align with their respective next goal states.
% The resulting hand and object states should closely align with their respective next goal states.

% which is computed based upon the current state $\mathbf{s}_n$, the next goal $\hat{\mathbf{s}}_{n+1}$, commanded as the next state of the robotic hand in the retargeted sequence and the next goal object state, and the object geometry.
% ~\eric{the writing is a bit confusing here. Does $\mathbf{o}_n$ include $\hat{\mathbf{s}}_{n+1}$ and the object geometry or it only includes $\mathbf{s}_n$? Why the object geometry is not a part of the policy input in the next formula?} % state-goal pair $(\mathbf{s}_n, \hat{\mathbf{s}}_{n+1})$ 
% primarily encodes the current hand and object state, object geometry, 
% the policy observes the state ${\mathbf{s}}_n$, consisting of the current state of the robotic dexterous hand and the object state, 
% and the next goal $\hat{\mathbf{s}}_{n+1}$, 
% commanded as the next state of the robotic hand in the retargeted sequence and the next goal object state. 

% The resulting hand state and the object state should be close to their corresponding next goal state. 
% nextstep state in the reference trajectory. 




% \todo{adapt to the tracking controller}
% \noindent\textbf{Per-trajectory tracker training.} 
% \noindent\textbf{Tracking controller optimization via RL.} 
% \noindent\textbf{Basic RL for training the tracking controller.} 
% \noindent\textbf{Training the tracking controller via RL.} 
\noindent\textbf{Reinforcement learning.}  
% Our single trajectory specialist training scheme leverages PPO to optimize for a tracking policy $\mathbf{\pi}(\cdot\vert \cdot)$. 
% Given a kinematic manipulation trajectory $(\mathbf{H}, \mathbf{O})$, we aim at optimizing a tracking policy $\mathbf{\pi}(\cdot\vert\cdot )$ that can control a dexterous robot hand to track the reference kinematic trajectory. 
% We use PD control to drive the hand. % links and joints %
% We carefully design the action space, and observation space as well as the reward and develop an RL-based optimization scheme for learning a tracking policy. Considering the poor sample efficiency of RL, instead of letting the tracking policy learn absolute positional target $\mathbf{a}_n$ at each timestep $n$, we assume there exists a basic trajectory, which is usually set to the kinematic reference trajectory, and let RL learn residual relative target $\Delta \mathbf{a}_n$ at each timestep $n$. For each timestep $n$, denote the hand state in the basic trajectory as $\mathbf{h}_n^b$, we calculate the final positional target as follows: 
% \begin{align}
%     \mathbf{a}_n = \mathbf{h}_n^b + \sum_{k=1}^n \Delta \mathbf{a}_k. 
% \end{align}
% In addition to the possibility in speeding up the training, the basic trajectory $\mathbf{H}^b=\{ \mathbf{h}_n^b \}$ gives us an additional dimension for optimizing the single trajectory tracking policy. For instance, we can initialize the basic trajectory as the tracking result of a different tracking task and re-optimize the residual policy to try to improve the single trajectory tracking. 
% \eric{The explanation should be more logical. We should start from introducing the state space, and then explain the common action space, e.g., joint positional targets, followed by mentioning our residual design. Finally rewards. I like how the \href{https://research.nvidia.com/labs/par/maskedmimic/assets/SIGGRAPHAsia2024_MaskedMimic.pdf}{MaskedMimic} paper introduces these.}
% We design 
% leverage 
% reinforcement learning scheme to 
% In the RL-based training scheme, the agent receives a reward $r_{n} = r({\mathbf{s}}_n, \mathbf{a}_n, \hat{\mathbf{s}}_{n+1}, \mathbf{s}_{n+1})$ after each transition. The training objective is maximizing the discounted cumulative reward: 
% \begin{align}
%     J = \mathbb{E}_{p(\tau\vert \pi)} \left[  \sum_{n=0}^{N} \gamma^{n}r_n  \right],
% \end{align}
% where $p(\tau\vert \pi) = p({\mathbf{s}}_0) \Pi_{n=0}^{N-1}p(\mathbf{s}_{n+1}\vert \mathbf{o}_n, \mathbf{a}_n)\pi(\mathbf{a}_n\vert \mathbf{s}_n,\hat{\mathbf{s}}_{n+1})$ is the likelihood of a transition trajectory of the agent $\tau = (\mathbf{s}_0,\mathbf{a}_0,r_0,...,\mathbf{s}_{N-1},\mathbf{a}_{N-1},r_{N-1}, \mathbf{s}_N)$. The discount factor $\gamma \in [0,1)$ determines the effective horizon length of the policy. 
% In the tracking control problem, the next goal state $\hat{\mathbf{s}}_{n+1}$ usually consists of the next step hand state and the object state in the kinematic reference sequence. 
% We control the robotic hand via a proportional derivative (PD) controller, following previous literature~\citep{Luo2024GraspingDO,Luo2023PerpetualHC,christen2022d,zhang2023artigrasp}. The action $\mathbf{a}_n$ then contains the target position commands of all hand joints. To improve the sample efficiency of RL, instead of letting the tracking policy learn the absolute positional target, we introduce a residual action space. Specifically, we introduce a baseline hand trajectory and train the policy to learn the residual relative target  $\Delta\mathbf{a}_n$ in each timestep. 
% The baseline trajectory is always available for the tracking problem -- one can trivially set it to the kinematic reference trajectory. 
% In each timestep $n$, we compute the position target via $\mathbf{a}_n = \mathbf{s}_n^{b} + \sum_{k=0}^{n}\Delta \mathbf{a}_k$, where $\mathbf{s}_n^{b}$ is the $n$-th step hand state in the baseline trajectory. 
% The observation at each timestep $n$ encodes the current hand and object state, the next goal state, baseline trajectory, actions, velocities, and the object geometry: 
% \begin{align}
%     \mathbf{o}_n = \{ \mathbf{s}_n, \dot{\mathbf{s}}_n, \hat{\mathbf{s}}_{n+1}, \mathbf{s}^b_n, \mathbf{a}_n, \text{feat}_{\text{obj}}, \text{aux}_n \}, \label{eq_obs}
% \end{align}
% where $\text{feat}_{\text{obj}}$ is the object feature produced by a pre-trained object point cloud encoder. We additionally introduce an auxiliary feature $\text{aux}_n$, computed based upon available states, to expose the agent with more informative information. We will explain in detail in Appendix~\ref{sec:supp_method}. 
% Our reward for manipulation tracking encourages the transited hand state and the object state to be close to their corresponding reference states and the hand-object affinity: 
% \begin{align}
%     r = w_{o, p} r_{o, p} + w_{o, q} r_{o, q} + w_{\text{wrist}} r_{\text{wrist}} + w_{\text{finger}} r_{\text{finger}} + w_{\text{affinity}} r_{\text{affinity}}, \label{eq_rew}
% \end{align}
% where $r_{o,p},r_{o, q},r_{\text{wrist}},r_{\text{finger}},r_{\text{affinity}}$ are rewards for object position, object orientation, hand wrist, hand fingers, and hand-object affinity, $w_{o, p},  w_{o, q}, w_{\text{wrist}}, w_{\text{finger}},  w_{\text{affinity}}$ are their weights. Details of the reward computation are deferred to the Appendix~\ref{sec:supp_method}. 
In the RL-based training scheme, the agent receives a reward \(r_{n} = r({\mathbf{s}}_n, \mathbf{a}_n, \hat{\mathbf{s}}_{n+1}, \mathbf{s}_{n+1})\) after each transition. The training objective is to maximize the discounted cumulative reward:
\begin{align}
    J = \mathbb{E}_{p(\tau\vert \pi)} \left[  \sum_{n=0}^{N-1} \gamma^{n}r_n  \right],
\end{align}
where \(p(\tau\vert \pi) = p({\mathbf{s}}_0) \prod_{n=0}^{N-1} p(\mathbf{s}_{n+1}\vert \mathbf{o}_n, \mathbf{a}_n)\pi(\mathbf{a}_n\vert \mathbf{s}_n,\hat{\mathbf{s}}_{n+1})\) is the likelihood of a transition trajectory of the agent \(\tau = (\mathbf{s}_0,\mathbf{a}_0,r_0,...,\mathbf{s}_{N-1},\mathbf{a}_{N-1},r_{N-1}, \mathbf{s}_N)\). The discount factor \(\gamma \in [0,1)\) determines the effective horizon length of the policy.
In the tracking control problem, the next goal state \(\hat{\mathbf{s}}_{n+1}\) typically comprises the subsequent hand state and the object state from the kinematic reference sequence. We control the robotic hand using a proportional derivative (PD) controller, following previous literature~\citep{Luo2024GraspingDO,Luo2023PerpetualHC,christen2022d,zhang2023artigrasp}. The action \(\mathbf{a}_n\) contains the target position commands for all hand joints. 
To enhance the sample efficiency of RL, rather than allowing the tracking policy to learn the absolute positional targets, we introduce a residual action space. Specifically, we introduce a baseline hand trajectory and train the policy to learn the residual relative target \(\Delta\mathbf{a}_n\) at each timestep. The baseline trajectory is consistently available for the tracking problem and can be trivially set to the kinematic reference trajectory. 
In each timestep $n$, we compute the position target via $\mathbf{a}_n = \mathbf{s}_n^{b} + \sum_{k=0}^{n}\Delta \mathbf{a}_k$, where $\mathbf{s}_n^{b}$ is the $n$-th step hand state in the baseline trajectory. 
% The observation at each timestep \(n\) encodes the current hand and object states, the next goal state, the baseline trajectory, actions, velocities, and the object geometry:
The observation at each timestep $n$ encodes the current hand and object state, the baseline trajectory, actions, velocities, and the object geometry:
% the next goal state, 
% baseline trajectory, actions, velocities, and the object geometry: 
\begin{align}
    % \mathbf{o}_n = \{ \mathbf{s}_n, \dot{\mathbf{s}}_n, \hat{\mathbf{s}}_{n+1}, \mathbf{s}^b_n, \mathbf{a}_n, \text{feat}_{\text{obj}}, \text{aux}_n \}, \label{eq_obs}
    \mathbf{o}_n = \{ \mathbf{s}_n, \dot{\mathbf{s}}_n, \mathbf{s}^b_n, \mathbf{a}_n, \text{feat}_{\text{obj}}, \text{aux}_n \}, \label{eq_obs}
\end{align}
where \(\text{feat}_{\text{obj}}\) is the object feature generated by a pre-trained object point cloud encoder. We also introduce an auxiliary feature \(\text{aux}_n\), computed based on available states, to provide the agent with more informative context. Further details will be explained in Appendix~\ref{sec:supp_method}.
Our reward for manipulation tracking encourages the transited hand state and the object state to closely match their respective reference states, as well as promoting hand-object affinity:
\begin{align}
    r = w_{o, p} r_{o, p} + w_{o, q} r_{o, q} + w_{\text{wrist}} r_{\text{wrist}} + w_{\text{finger}} r_{\text{finger}} + w_{\text{affinity}} r_{\text{affinity}}, \label{eq_rew}
\end{align}
where \(r_{o,p}, r_{o, q}, r_{\text{wrist}}, r_{\text{finger}}, r_{\text{affinity}}\) represent rewards for object position, object orientation, hand wrist, hand fingers, and hand-object affinity, respectively, while \(w_{o, p}, w_{o, q}, w_{\text{wrist}}, w_{\text{finger}}, w_{\text{affinity}}\) are their corresponding weights. Details regarding the reward computation are deferred to Appendix~\ref{sec:supp_method}.



% ~\eric{should be ``trivially''. Please use Grammarly to carefully check the whole paper to avoid grammar errors.} 
% $\mathbf{b}_n$ 

% , $\text{aux}_n$ is the auxiliary features, computed based upon available states~\eric{at least we should explain the purpose of including some auxiliary features?}, which we will explain in detail in Appendix~\ref{sec:supp_method}. 

% Our reward for manipulating tracking comprises three components: the hand reward $r_{h}$, the object reward $r_o$, and the hand-object affinity reward $r_d$. The object reward encourage the transited object position and the orientation close to their kinematic references: $r_o = w_p r_{o,p} + w_q r_{o,q}$. 
% The object reward includes both position and orientation rewards, defined as: 
% \begin{align}
%     r_o = w_p(0.9 - \Vert \mathbf{s}_n^p - \hat{\mathbf{o}}_n^p \Vert_2 ) + w_q(\text{np.pi} - \text{Diff\_Angle}(\mathbf{o}_n^q - \hat{\mathbf{o}}_n^q )), \label{eq:rew_obj}
% \end{align}
% where $w_p$ and $w_q$ are the weights for position and orientation rewards, respectively, and $\text{Diff\_Angle}(\cdot, \cdot)$  computes the rotation angle difference between two quaternions. The hand reward is calculated as the negative weighted sum of the current hand joint positions and the reference positions:
% \begin{align}
%     r_h = -(w_{\text{trans}} \Vert \mathbf{h}_n[:3] - \hat{\mathbf{h}}_n[:3] \Vert_1 + w_{\text{ornt}} \Vert \mathbf{h}_n[3:6] - \hat{\mathbf{h}}_n[3:6] \Vert_1 + w_{\text{finger}} \Vert \mathbf{h}_n[6:] - \hat{\mathbf{h}}_n[6:] \Vert_1  ), \label{eq:rew_hand}
% \end{align}
% % we include in the observation, 
% % The tracking controller for manipulation should be aware of the geometry of the object. So we include the object feature, produced by a pre-trainedd object point cloud encoder, into the state. The final state contains 

%%%%%%%%%%%%%%%%%%%%%% baseline trajs %%%%%%%%%%%%%%%%%%%%%%
% This approach benefits us from two ways. First, the RL exploration needs to explore around the baseline trajectory only, thereby accelerating the convergence. Second, it offers us an additional dimension for optimizing the tracking policy -- 
% needs to explore around a baseline hand trajectory. 
% it can accelerate the training 
% we introduce a baseline hand trajectory
% The action $\mathbf{a}_n$ contains the joint torque commands applied to all hand joints. We follow the literature and adopt 
% contains the positional target of each hand joint. 
% is the positional target of each hand joint
% in the kinematic reference sequence
% aims at optimizing $\pi$ 
% Our RL-based scheme for training the tracking controller aims at optimizing the tracking policy $\pi$ with the objective to maximize the discounted cumulative reward: 
% \begin{align}
%     J = \mathbb{E}_{p(\tau\vert )}
% \end{align}
% We carefully design the action space, observation space, and reward to develop an RL-based optimization scheme for learning a tracking controller. To address the poor sample efficiency of RL, instead of letting the tracking policy learn the absolute positional target $\mathbf{a}_n$ at each timestep $n$, we introduce a basic trajectory~\eric{base trajectory or basic trajectory? I would suggest the former. Please make sure we modify all terms together.}, commonly the kinematic reference trajectory, and allow RL to learn the residual relative target $\Delta \mathbf{a}_n$ at each timestep. For each timestep $n$, denote the hand state in the basic trajectory as $\mathbf{h}_n^b$, we compute the final positional target as follows: 
% % we denote the hand state in the basic trajectory as $\mathbf{h}_n^b$ and compute the final positional target as follows:
% \begin{align}
%     \mathbf{a}_n = \mathbf{h}_n^b + \sum_{k=1}^n \Delta \mathbf{a}_k. 
% \end{align}
% This approach not only accelerates training but also provides an additional dimension for optimizing the single trajectory tracking policy. For instance, we can initialize the basic trajectory using the tracking results from a different task and then re-optimize the residual policy to enhance the single trajectory tracking performance.
%%%%%%%%%%%%%%%%%%%%%% baseline trajs %%%%%%%%%%%%%%%%%%%%%%


% using the action trajectory sampled 
% In our method, we try to improve the single trajectory tracking by varying the basic trajectory from its own kinematic reference motion to the rollout action trajectory produced by a well-trained expert for a different task or from the general tracking policy, followed by re-optimizing the residual policy. 

%%%%%%%%%%%%%%%%%%%%%% observation space %%%%%%%%%%%%%%%%%%%%%%
% At each timestep $n$, the observation includes information about the current hand and object states, the next frame tracking target, the current cumulated residual targets, the next step hand state in the basic trajectory, and the pre-processed object feature $\text{feat}_{\text{obj}}$. The $n$-th step observation, denoted as $\mathbf{o}\mathbf{b}\mathbf{s}_n$, is calculated as follows:
% \begin{align}
%     \mathbf{o}\mathbf{b}\mathbf{s}_n = \{ \hat{\mathbf{h}}_n, \hat{\mathbf{o}}_n,  \hat{\dot{\mathbf{h}}}_n, \hat{\dot{\mathbf{o}}}_n, \mathbf{f}_n,  \mathbf{h}_{n+1}, \mathbf{o}_{n+1}, \mathbf{h}_{n+1} - \hat{\mathbf{h}}_n, \mathbf{o}_{n+1} \ominus \hat{\mathbf{o}}_n, \sum_{k=1}^n\Delta\mathbf{a}_k, \mathbf{h}_{n+1}^b, \text{feat}_{\text{obj}}   \}, \label{eq:observations}
% \end{align}
% where $\hat{\mathbf{h}}_n$ and $\hat{\mathbf{o}}_n$ represent the observed positions of hand joints and object orientation at timestep $n$, $\hat{\dot{\mathbf{h}}}_n$ and $\hat{\dot{\mathbf{o}}}_n$ denote the velocities of hand joints and object linear and angular velocities, respectively, $\mathbf{f}_n$ indicates the hand finger positions in the world space.
%%%%%%%%%%%%%%%%%%%%%% observation space %%%%%%%%%%%%%%%%%%%%%%






% At each timestep $n$, the observation comprises the current hand and object state information, the next frame tracking target, the current cumulated residual targets, the next step basic hand state, and the pre-processed object feature $\text{feat}_{\text{obj}}$ as input and output the hand action for the hand to achieve the next state. Specifically, at each timestep $n$, we calculate the observation $\mathbf{o}\mathbf{b}\mathbf{s}_n$ as follows: 
% \begin{align}
%     \mathbf{o}\mathbf{b}\mathbf{s}_n = \{ \hat{\mathbf{h}}_n, \hat{\mathbf{o}}_n,  \hat{\dot{\mathbf{h}}}_n, \hat{\dot{\mathbf{o}}}_n, \mathbf{f}_n,  \mathbf{h}_{n+1}, \mathbf{o}_{n+1}, \mathbf{h}_{n+1} - \hat{\mathbf{h}}_n, \mathbf{o}_{n+!} \ominus \hat{\mathbf{o}}_n, \sum_{k=1}^n\Delta\mathbf{a}_k, \mathbf{h}_{n+1}^b, \text{feat}_{\text{obj}}   \}, \label{eq:observations}
% \end{align}
% where $\hat{\mathbf{h}}_n$ and $\hat{\mathbf{o}}_n$ are observed hand joint DoF positions and the object orientation as well as positions at the timestep $t$, $\hat{\dot{\mathbf{h}}}_n$ and $\hat{\dot{\mathbf{o}}}_n$ are hand DoF velocities and object linear as well as angular velocities respectively, $\mathbf{f}_n$ denotes the hand finger positions in the world space. 

% $\mathbf{h}_{n+1}$ and $\mathbf{o}_{n+1}$ are the kinematic targets of the hand DoF positions and the object state in the next timestep. 

% The reward consists a hand tracking reward $r_{h}$, object tracking reward $r_o$, and the hand-object affinity reward $r_d$. Specifically, the object reward contains the object position reward and the orientation reward: 
% \begin{align}
%     r_o = w_p(0.9 - \Vert \mathbf{o}_n^p - \hat{\mathbf{o}}_n^p \Vert_2 ) + w_q(\text{np.pi} - \text{Diff\_Angle}(\mathbf{o}_n^q - \hat{\mathbf{o}}_n^q )), \label{eq:rew_obj}
% \end{align}
% where $w_p$ and $w_q$ are weights of the position reward and the orientation reward respectively, $\text{Diff\_Angle}(\cdot, \cdot)$ calculates the rotation angle difference of two rotations represented as quaternions. The hand reward is the negative of the weighted sum of the current hand DoF positions and the reference positions: 
% \begin{align}
%     r_h = -(w_{\text{trans}} \Vert \mathbf{h}_n[:3] - \hat{\mathbf{h}}_n[:3] \Vert_1 + w_{\text{ornt}} \Vert \mathbf{h}_n[3:6] - \hat{\mathbf{h}}_n[3:6] \Vert_1 + w_{\text{finger}} \Vert \mathbf{h}_n[6:] - \hat{\mathbf{h}}_n[6:] \Vert_1  ), \label{eq:rew_hand}
% \end{align}
% where $w_{\text{trans}}, w_{\text{ornt}}$, and $w_{\text{finger}}$ are weights. The hand-object affinity reward encourages the hand palm and fingers to get close to the object: 
% \begin{align}
%     r_d = -(w_{\text{palm}} \Vert \mathbf{p}_n^{\text{palm}} - \hat{\mathbf{o}}_n^p \Vert + w_{\text{finger}} \sum_{i=1}^{n_f} \Vert \mathbf{f}_{n,i} - \hat{\mathbf{o}}_n^p \Vert),  \label{eq:rew_affinity}
% \end{align}
% where $w_{\text{palm}}$ and $w_{\text{finger}}$ are weights of the palm-object and finger-object affinities respectively, $n_f$ denotes the number of fingers, $\mathbf{f}_{n,i}$ represents the position of the $i$-th finger in the current frame $n$. 
% Finally, the overall reward is composed as the sum of these three components: $r = r_h + r_o + r_d$. 
% We leverage PPO~\citep{Schulman2017ProximalPO} implemented in rl\_games~\citep{rlgames2021} to train our policy. 


%%%%%%%%%%%%%%%%%%%%%% reward function %%%%%%%%%%%%%%%%%%%%%%
% The reward function comprises three components: the hand-tracking reward $r_{h}$, the object-tracking reward $r_o$, and the hand-object affinity reward $r_d$. The object reward includes both position and orientation rewards, defined as:
% \begin{align}
%     r_o = w_p(0.9 - \Vert \mathbf{o}_n^p - \hat{\mathbf{o}}_n^p \Vert_2 ) + w_q(\text{np.pi} - \text{Diff\_Angle}(\mathbf{o}_n^q - \hat{\mathbf{o}}_n^q )), \label{eq:rew_obj}
% \end{align}
% where $w_p$ and $w_q$ are the weights for position and orientation rewards, respectively, and $\text{Diff\_Angle}(\cdot, \cdot)$  computes the rotation angle difference between two quaternions. The hand reward is calculated as the negative weighted sum of the current hand joint positions and the reference positions:
% \begin{align}
%     r_h = -(w_{\text{trans}} \Vert \mathbf{h}_n[:3] - \hat{\mathbf{h}}_n[:3] \Vert_1 + w_{\text{ornt}} \Vert \mathbf{h}_n[3:6] - \hat{\mathbf{h}}_n[3:6] \Vert_1 + w_{\text{finger}} \Vert \mathbf{h}_n[6:] - \hat{\mathbf{h}}_n[6:] \Vert_1  ), \label{eq:rew_hand}
% \end{align}
% % degrees of freedom (DoF) 
% % \[
% % r_h = -\left(w_{\text{trans}} \|\mathbf{h}_n[:3] - \hat{\mathbf{h}}_n[:3]\|_1 + w_{\text{ornt}} \|\mathbf{h}_n[3:6] - \hat{\mathbf{h}}_n[3:6]\|_1 + w_{\text{finger}} \|\mathbf{h}_n[6:] - \hat{\mathbf{h}}_n[6:]\|_1\right), \label{eq:rew_hand}
% % \]
% with weights $w_{\text{trans}}, w_{\text{ornt}}$, and $w_{\text{finger}}$. The hand-object affinity reward encourages proximity between the hand palm and fingers and the object:
% \begin{align}
%     r_d = -(w_{\text{palm}} \Vert \mathbf{p}_n^{\text{palm}} - \hat{\mathbf{o}}_n^p \Vert + w_{\text{finger}} \sum_{i=1}^{n_f} \Vert \mathbf{f}_{n,i} - \hat{\mathbf{o}}_n^p \Vert),  \label{eq:rew_affinity}
% \end{align}
% % \[
% % r_d = -\left(w_{\text{palm}} \|\mathbf{p}_n^{\text{palm}} - \hat{\mathbf{o}}_n^p\| + w_{\text{finger}} \sum_{i=1}^{n_f} \|\mathbf{f}_{n,i} - \hat{\mathbf{o}}_n^p\|\right), \label{eq:rew_affinity}
% % \]
% where $w_{\text{palm}}$ and $w_{\text{finger}}$ are the weights for the palm-object and finger-object affinities, respectively, $n_f$ is the number of fingers, and $\mathbf{f}_{n,i}$ denotes the position of the $i$-th finger at timestep $n$. The overall reward is then computed as the sum of these three components: $r = r_h + r_o + r_d$.  
% % We utilize PPO~\citep{Schulman2017ProximalPO} as implemented in rl\_games~\citep{rlgames2021} to train our policy.
%%%%%%%%%%%%%%%%%%%%%% reward function %%%%%%%%%%%%%%%%%%%%%%


% \todo{bonus reward? }

% \textcolor{red}{(TODO: add the reward design here)}
% \textcolor{red}{(TODO: add the residual policy here --- it is important since we need to justify the task curriculum here)}

% By re-optimizng the residual policy, we can possibly arrive at a better 
% For instance, by setting the base trajectory to an action trajectory produced by an expert trained for a different trajectory, 
% It opens the opportunity to transfer 
% This strategy natrualy afford us an additional dimension in optimizing the single trajectory tracking policy. 
% we train the tracker to output a residual relative target $\Delta \mathbf{a}_n$. 
% letting the policy learn absolute positional targets $\mathbf{a}_n$, we 
% residual policies whose outputs are treated as residual positional targets added to a base trajectory. Formally, 
% given a base trajectory containing the hand DoF positos at each  timestep, \emph{i.e.,} $\mathbf{H}^b = \{ \mathbf{h}_n^b \}_{n=1}^N$, we let the policy to learn a residual positional 
% To further improve the RL's sample efficiency, instead of letting the policy to output abs

% \todo{residual policy here!!!}

% \noindent\textbf{Single manipulation trajectory specialist tracking policy.}  Given a kinematic manipulation trajectory $(\mathbf{H}, \mathbf{O})$, training a specialist policy aims at optimizing a tracking policy $\mathbf{\pi}(\cdot\vert\cdot )$ that can control a dexterous robot hand to track the reference kinematic trajectory. 
% We train a specialist policy leveraging RL to solve the problem. 
% Considering the intricate dynamics involved in the dexterous manipulation resulting from the high DoF of a dexterous hand and the rich and changing hand-object contacts, we resort to model free approaches and leverage RL to optimize the manipulation tracking policy. 
% \noindent\textbf{Trajectory specific specialist policy.} Given a kinematic manipulation trajectory $(\mathbf{H}, \mathbf{O})$, training a specialist policy aims at optimizing a tracking policy $\mathbf{\pi}(\cdot\vert\cdot )$ that can control a dexterous robot hand to track the reference kinematic trajectory. 
% Assuming the physical model is unknown and non-differentiable, we leverage reinforcement learning to optimize the policy. 

% \noindent\textbf{Imitation augmented RL for learning a general tracking controller.} 
% \noindent\textbf{Imitation augmented RL.} 

% \noindent\textbf{Additional Imitation Loss.}  

% \noindent\textbf{Imitation loss.}
% \noindent\textbf{Learning from tracking demonstration.} 
\noindent\textbf{Imitation learning.} 
% To let the tracking controller benefit from a large number of robot tracking demonstration data, we train 
% of imitation-ready data, we train the actor to imitate successful tracking results, aiming at distill ``tracking knowledge'' from these trajectories into the tracking controller. 
% Leveraging the powe
% Relying on RL solely can hardly let us train a strong tracking controller due to its restriction 
% The RL-based learning scheme, restricted by sample inefficiency and the incapability to master multiple tracking problems, can hardly solve the generalizable tracking control problem, as evidenced by our early experiments. Therefore, we propose an IL-based strategy and try to distill successful, abundant, and diverse ``tracking knowledge'' to the tracking controller. Specifically, we train the tracking agent to imitate a large number of high-quality robot tracking demonstrations. 
% In this way, we can effectively guide the agent to produce ``expert actions'' that can successfully track the reference state. Besides, by imitating diverse tracking demonstrations, the agent can avoid repeatedly experiencing low rewards in difficult tracking scenarios, while also preventing over-exploitation of easier tracking tasks. 
% Formally, a robot tracking demonstration of length $N$ contains a kinematic reference sequence $(\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_{N})$, and an expert's state-action trajectory $(\mathbf{s}_0^L, \mathbf{a}_0^L, ..., \mathbf{s}_{N-1}^L, \mathbf{a}_{N-1}^L, \mathbf{s}_N^L)$.
% In addition to the actor loss, we add an action supervision loss to bias the policy's prediction at each timestep towards its corresponding expert action in the demonstration: 
% \begin{align}
%     \mathcal{L}_a = \mathbb{E}_{\mathbf{a}_n\sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})} \Vert \mathbf{a_n} - \mathbf{a}^L_{n}  \Vert. 
% \end{align}
% In this way, we can guide the policy’s exploration via these demonstrations, ultimately speeding up convergence and improving the performance in the complex problem.  From the IL's perspective, the RL exploration adds noise to the states to make the imitation more robust to noise in a similar flavor to DART~\citep{laskey2017dart}. 
% Since the agent should not and will not explore states too far from the reference states in the tracking control task, it is possible to optimize the policy via both the imitation loss and RL reward simultaneously.
The RL-based learning scheme, hindered by sample inefficiency and its inability to handle multiple tracking problems, struggles to solve the generalizable tracking control problem, as demonstrated by our early experiments. Therefore, we propose an IL-based strategy to distill successful, abundant, and diverse ``tracking knowledge'' into the tracking controller. Specifically, we train the tracking agent to imitate a large number of high-quality robot tracking demonstrations. 
This approach effectively guides the agent to produce ``expert actions'' that can successfully track the reference state. Additionally, by imitating diverse tracking demonstrations, the agent can avoid repeatedly encountering low rewards in challenging tracking scenarios, while also preventing over-exploitation of easier tasks.
Formally, a robot tracking demonstration of length \(N\) consists of a kinematic reference sequence \((\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_{N})\) and an expert's state-action trajectory \((\mathbf{s}_0^L, \mathbf{a}_0^L, ..., \mathbf{s}_{N-1}^L, \mathbf{a}_{N-1}^L, \mathbf{s}_N^L)\). 
In addition to the actor loss, we incorporate an action supervision loss to bias the policy's predictions at each timestep towards the corresponding expert action in the demonstration:
\begin{align}
    \mathcal{L}_a = \mathbb{E}_{\mathbf{a}_n\sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})} \Vert \mathbf{a_n} - \mathbf{a}^L_{n}  \Vert. 
\end{align}
This guidance allows the policy’s exploration to be informed by these demonstrations, ultimately speeding up convergence and enhancing performance in complex problems. From the perspective of IL, the RL exploration introduces noise into the states, making the imitation more robust, in a similar flavor to DART~\citep{laskey2017dart}. 
Since the agent should not and will not explore states too far from the reference states in the tracking control task, it is feasible to optimize the policy using both the imitation loss and RL reward simultaneously.


% the agent can avoid continuously experiencing low rewards in hard tracking cases, thereby free of exploiting easy tracking problems. 
% getting stuck in exploiting easy tracking problems due to low positive reward from hard tracking cases.
% ~\eric{due to low positive reward from hard tracking cases?}. 

% ~\eric{In addition to the actor loss,} 

% action prediction for the state-goal pair $(\mathbf{s}_n, \hat{\mathbf{s}}_{n+1})$ towards its corresponding expert action in the demonstration: 

% encourage the policy predict 
% when training the agent to solve the tracking problem with a kinematic sequence $(\hat{\mathbf{s}}_0, .., \hat{\mathbf{s}}_N)$ and the expert action trajectory $(\mathbf{a}^L_0, ..., \mathbf{a}^L_{N-1})$ from the demonstration, we add an action supervision loss to the policy's predicted action $\mathbf{a}_n$ at each timestep: 
% \begin{align}
%     \mathcal{L}_a = \sum_{n=0}^{N-1} \mathbb{E}_{\mathbf{a}_n\sim \pi(\cdot\vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})} \Vert \mathbf{a_n} - \mathbf{a}^L_{n}  \Vert.  
% \end{align}

% making it possible to optimize with both the imitation loss and RL reward simultaneously.
% In the tracking control task, where the RL should not and will not explore states too far from the reference states, making it possible to optimize with both the imitation loss and RL reward simultaneously.
% the demonstrations can guide 
% The demonstrations bias the policy toward the supervision data. It can thereby 

% for each tracking demonstration containing the expert action sequence $(\mathbf{a}^L_0, ..., \mathbf{a}^L_{N-1})$ for tracking the kinematic sequence $(\hat{\mathbf{s}}_0, .., \hat{\mathbf{s}}_N)$, we add an action supervision loss to the policy's predicted action $\mathbf{a}_n$ at each timestep
% hardly offer us a strong tracking controller. 
% can hardly let us get a strong tracking controller. 
% To facilitate the learning of the tracking controller, we propose to distill successful ``tracking knowledge'' from high-quality robot tracking demonstrations. 
% % Specifically, we propose to train the  tracking controller to imitate high-quality robot tracking demonstrations. 
% % propose to leverage the joint power of RL and IL and train the tracking 
% Specifically, instead of relying on the RL-based training scheme solely, we additionally train the tracking controller to imitate high-quality robot tracking demonstrations. 
% % in addition to the RL-based training scheme, 
% Formally, for each trajectory with the action sequence $(\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L)$, we incorporate the following action supervision loss into the policy's prediction at each timestep \((\mathbf{\mu}_n, \mathbf{\sigma}_n)\) to  encourage the actor to mimic this trajectory: 
% % encourage the actor to mimic this trajectory at each timestep by incorporating the following action supervision loss into the policy's prediction at each timestep \((\mathbf{\mu}_n, \mathbf{\sigma}_n)\):
% \begin{align}
%     \mathcal{L}_a = \Vert \mathbf{\mu}_n -  \mathbf{a}_n \Vert, 
% \end{align} 
% where \(\mathbf{a}_n\) denotes the action taken at the \(n\)-th timestep from the action trajectory $\mathbf{A}_L$.


% This strategy aims to align the action trajectory produced by the current policy with the optimized successful action sequence from the dataset, resembling the approach used in DART~\citep{laskey2017dart}~\eric{from RL's perspective, the demonstrations bias the policy toward the supervision data. from IL's perspective, the RL exploration adds noise to the states to make the imitation more robust to noise in a similar flavor to DART}.~\eric{Also mention that since this is the tracking task, the RL policy should not and will not explore states too far from the reference states, making it possible to optimize with both the imitation loss and RL reward simultaneously.}


% s at each timestep \((\mathbf{\mu}_n, \mathbf{\sigma}_n)\):
% an imitation loss to the 
% Given a dataset containing paired kinematic trajectories and action sequences $\mathcal{S}_L=\{ (\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L) \}$, we introduce an additional action supervision loss to the actor loss, aimed at distilling successful ``tracking knowledge'' from these trajectories into the tracking controller. 

% Formally, for each labeled trajectory \((\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L)\), we incorporate the following action supervision loss into the policy's predictions at each timestep \((\mathbf{\mu}_n, \mathbf{\sigma}_n)\):
% \begin{align}
%     \mathcal{L}_a = \Vert \mathbf{\mu}_n -  \mathbf{a}_n \Vert, 
% \end{align}
% where \(\mathbf{a}_n\) denotes the action taken at the \(n\)-th timestep from the optimized action trajectory. This strategy aims to align the current trajectory with the optimized successful trajectory from the dataset, resembling the approach used in DART~\citep{laskey2017dart}.

% \noindent\textbf{Additional imitation loss.} 
% Given a dataset containing paired kinematic trajectories and action sequences $\mathcal{S}_L=\{ (\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L) \}$, we add an additional action supervision loss to the actor loss to distill successful ``tracking knowledge'' from these trajectories to the tracking controller. 
% Formally, for each labeled trajectory $(\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L)$, the following action supervised loss is additionally added on the policy's prediction in each timestep $(\mathbf{\mu}_n, \mathbf{\sigma}_n))$ to train the policy:
% \begin{align}
%     \mathcal{L}_a = \Vert \mathbf{\mu}_n -  \mathbf{a}_n \Vert, 
% \end{align}
% where $\mathbf{a}_n$ denotes $n$-th step action taken from the optimized action trajectory. This strategy tries to bias the current trajectory towards the optimized successful trajectory in the dataset, in a similar flavor to DART~\citep{laskey2017dart}. 


% With the carefully designed specialist policy training strategy and the task relational space exploration and modeling scheme, it is possible for us to optimize for a satisfactory result for each single manipulation trajectory tracking task. However, it is still not enough to acquire a generalist that can not only achieve good performance in each sequence but even generalize to unseen trajectories. Simply following the above RL scheme and training a single policy on multiple tasks is not feasible as demonstrated in our early experiments. As the number of training tasks increases, the RL would even struggle with effectively optimizing a strong policy that can solve every training task, letting alone generalize to unseen trajectories and resolve the novel manipulation sequence tracking challenge. We suppose such pool fitting phenomenon comes from the inherent deficiency of RL in solving multiple tasks. We therefore propose to introduce labeled single trajectory optimization results into the training process of RL, \textit{i.e.,} providing additional action labels as the supervision signals to train the policy together with RL. Specifically, 
% n action-labeled dataset 

% wthe imitation augmented RL involves adding an additional action supervision loss to the actor loss to distill successful ``tracking knowledge'' from these trajectories to the tracking controller. 
% where each trajectory $(\mathbf{H}_L, \mathbf{O}_L)$ is augmented with an additional action sequence $\mathbf{A}_L$, 
% we add an action supervision loss to the actor loss. 
% produced by well-trained per-trajectory trackers,
% Intuitively, this strategy tries to distill knowledge form the action-labeled trajectories to the tracking controller. 
% optimized knowledge in per-trajectory trackers to the general tracking controller. 

% $(\mathbf{\mu}_n, \mathbf{\sigma}_n) = \mathbf{\pi}(\cdot \vert \hat{\mathbf{s}}_n)$ to train the policy:

% to train the policy $\mathbf{\pi}(\cdot\vert \cdot)$  


% \todo{need to say we usthe same model-free tacking algo as that for the tracking controller}
\vspace{-5pt}
\subsection{Mining High-Quality Robot Tracking Demonstrations Using Neural Controller through a Homotopy Optimization Scheme} 
\label{sec:method_data}
\vspace{-5pt}
% To prepare demonstrations to train the tracking controller, we need to infer action sequences from kinematic-only trajectories to create paired data with kinematic references and the action sequence. We primarily leverage model-free reinforcement learning techniques to train the tracking policy for each single trajectory to acquire its corresponding action sequence.~\eric{we should briefly explain the naive way of doing per-trajectory tracking. No one knows its relation with the controller at this moment and we should not assume that is straightforward to understand.} Though this straightforward solution can successfully track lots of trajectories~\eric{I think we should mention that a lot of trajectories can not be tracked by this naive method instead of emphasizing that it is already quite successful?}, relying solely on optimizing per-trajectory tracking policy independently presents challenges for complex tracking scenarios. To resolve difficulties in tracking challenging trajectories to improve the diversity and the quality of tracking demonstrations, we then explore the possibility of~\eric{this expression sounds weak} using the tracking controller through a homotopy optimization scheme to improve per-trajectory tracking by 1) transferring tracking prior from the tracking controller and 2) learning a homotopy path generator which can propose useful homotopy paths that we can leverage to track previously difficult-to-track trajectories through a homotopy optimization method. 
% % directly training a policy leveraging RL with the above designs 

% Preparing demonstrations to train the training controller

% Preparing demonstrations to train the tracking controller requires us to infer the action 
% To prepare a demonstration to train the tracking controller, we need to infer the action sequence $(\mathbf{a}^L_0,...,\mathbf{a}^L_{N-1})$ that can successfully track the kinematic reference trajectory $(\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)$. A naive way is leveraging RL to train a single trajectory tracking policy $\pi$ and take its resulting action sequence as the demonstration. However, leveraging this strategy alone can hardly provide us with a diverse and high-quality tracking demonstration dataset because RL would be challenged by the inherent difficulties in dexterous manipulation. To improve the diversity and the quality of robot tracking demonstrations, we propose to leverage the tracking controller and a homotopy optimization scheme to improve the per-trajectory tracking results. 

To prepare a demonstration from a kinematic reference trajectory \((\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)\) for training the tracking controller, we need to infer the action sequence \((\mathbf{a}^L_0, ..., \mathbf{a}^L_{N-1})\) that successfully tracks the reference sequence.  
% trajectory \((\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)\). 
A straightforward approach is to leverage RL to train a single-trajectory tracking policy \(\pi\) and use its resulting action sequence directly. 
% as the demonstration. 
However, relying solely on this strategy often fails to provide a diverse and high-quality dataset of tracking demonstrations, as RL struggles with the inherent challenges of dexterous manipulation.
To enhance both the diversity and quality of robot tracking demonstrations, we propose utilizing the tracking controller in conjunction with a homotopy optimization scheme to improve the per-trajectory tracking results.

% We first think present a naive solution 

% ~\eric{train a single policy or train a per-trajectory tracking policy?
% }

% of the inherent difficulty of dexterous manipulation tracking that would 
% which will challenge the optimization of RL, especially in difficult manipulation tracking problems.

% this strategy can hardly provide 
% Specifically, we can formulate is as a single trajectory tracking problem. Given the kinematic references, we aim at optimizing a tracking policy $\pi$ that can track the reference trajectory. In each tiemstep, $\pi$ observes the current state $\mathbf{s}_n$ and the next goal state $\hat{\mathbf{s}}_{n+1}$; and predict the distribution of the current action $\mathbf{a}_n$. $\pi$ is optimized to minimize the difference between the transited state $\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)$ in each timestep $n$ is close to the goal state $\hat{\mathbf{s}}_{n+1}$. 
% By sampling from the $\pi$ in each step and transiting to the next state, we can  
% However, this way of doing per-trajectory tracking cannot provide us with 

\noindent\textbf{RL-based single trajectory tracking.} 
% A basic solution to acquire the demonstration is leveraging RL to solve the per-trajectory tracking problem and taking the resulting action sequence as the demonstration. Given a kinematic reference trajectory, we aim at optimizing a tracking policy $\pi$ that can track the reference trajectory. In each timestep, $\pi$ observes the current state $\mathbf{s}_n$ and the next goal state $\hat{\mathbf{s}}_{n+1}$. It then predicts the distribution of the current action $\mathbf{a}_n$. 
% The policy $\pi$ is optimized to minimize the difference between the transited state $\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)$ at each timestep $n$ and the goal state $\hat{\mathbf{s}}_{n+1}$. Similar to our design for the RL-based learning scheme for the tracking controller, we adopt a residual action space. We introduce a baseline trajectory $(\mathbf{s}^b_0,...,\mathbf{s}^b_N)$ for each tracking task, while only leveraging RL to learn a residual policy. Observations and reward are the same to our design for tracking controller (see Eq.~\ref{eq_obs}~\ref{eq_rew}). Once $\pi$ has been optimized, we can sample the action $\mathbf{a}_n$ from $\pi$ in each timestep. By iteratively transferring to the next state using the predicted action and querying the policy $\pi$ to generate a new action, we can get the expert action sequence $(\mathbf{a}_0^L, ..., \mathbf{a}_{N-1}^L)$ for the input kinematic reference trajectory. 
A basic approach to acquiring demonstrations is to leverage RL to address the per-trajectory tracking problem, using the resulting action sequence as the demonstration. Given a kinematic reference trajectory, our goal is to optimize a tracking policy \(\pi\) that can accurately track this reference trajectory. At each timestep, \(\pi\) observes the current state \(\mathbf{s}_n\) and the next goal state \(\hat{\mathbf{s}}_{n+1}\), and it predicts the distribution of the current action \(\mathbf{a}_n\).
The policy \(\pi\) is optimized to minimize the difference between the transited state \(\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)\) at each timestep \(n\) and the goal state \(\hat{\mathbf{s}}_{n+1}\). Similar to our design for the RL-based learning scheme for the tracking controller, we adopt a residual action space. For each tracking task, we introduce a baseline trajectory \((\mathbf{s}^b_0, ..., \mathbf{s}^b_N)\) and only learn a residual policy using RL. The observations and rewards follow the same design as for the tracking controller (see Eq.~\ref{eq_obs} and Eq.~\ref{eq_rew}).
Once \(\pi\) has been optimized, we can sample the action \(\mathbf{a}_n\) from \(\pi\) at each timestep. By iteratively transitioning to the next state using the predicted action and querying the policy \(\pi\) to generate a new action, we can obtain the expert action sequence \((\mathbf{a}_0^L, ..., \mathbf{a}_{N-1}^L)\) for the input kinematic reference trajectory.


% $\pi$ is optimized to minimize the difference between the transited state $\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)$ in each timestep $n$ is close to the goal state $\hat{\mathbf{s}}_{n+1}$.~\eric{this sentence is grammarly incorrect.}

% with those designed for the tracking controller (see Eq.~\ref{eq_obs}~\ref{eq_rew}). 
% each kinematic trajectory, while 



% naive per-trajectory tracking 

\noindent\textbf{Transferring tracking prior.} 
% To improve the quality and diversity of the demonstrations, we devise a strategy that utilizes the general ``tracking knowledge'' encoded in the universal tracking controller to improve trajectory-specific tracking policies. Specifically, to track a kinematic reference trajectory $(\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)$, we first track it via the tracking controller with the baseline trajectory set to the kinematic reference. We then set the baseline trajectory to the resulting action sequence and re-optimize the residual policy leveraging the RL-based single trajectory tracking method. The tracking controller can help us find a better baseline trajectory, which eases policy learning and improves the single trajectory tracking result. 
To enhance the quality and diversity of demonstrations, we devise a strategy that leverages the general ``tracking knowledge'' encoded in the universal tracking controller to improve trajectory-specific tracking policies. Specifically, to track a kinematic reference trajectory \((\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)\), we first utilize the tracking controller to track the trajectory, with the baseline trajectory set to the kinematic reference sequence. We then adjust the baseline trajectory to the resulting action sequence and re-optimize the residual policy using the RL-based single trajectory tracking method. This approach can help us find a better baseline trajectory, facilitating single-trajectory tracking policy learning and improving the per-trajectory tracking results.
% the result. 
% the single trajectory tracking result. 
% allows the tracking controller to find a better baseline trajectory, facilitating policy learning and improving the single trajectory tracking result. 

% ~\eric{it might confuse the reader here since the tracking policy refers to a per-trajectory tracker while the tracking controller refers to the general tracker. I think it would be better if we could use a more distinctive term to differentiate in this whole section. Maybe trajectory-specific tracking policy v.s. universal tracking controller?} 

% per-trajectory tracking. 

% The tracking controller can help us find a better baseline trajectory that would ease the policy learning, thereby facilitating the per-trajectory tracking. 

% per-trajectory tracking.
% Then we set the baseline trajectory as the
% use the tracking controller to track 
% to track a 
% % for a 
% kinematic reference trajectory $(\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)$, we first query the tracking controller to generate an action sequence $(\mathbf{a}^{\text{prior}}_0, ..., \mathbf{a}^{\text{prior}}_{N-1})$. After that, we set the baseline trajectory as the sampled actions and optimize the residual policy leveraging the RL-based per-trajectory tracking scheme. The tracking controller can help us find a better baseline trajectory that would ease the policy learning, thereby facilitating the per-trajectory tracking. 
% If the action sequence we've sampled from the tracking controller proved to serve as a better baseline trajectory for the single trajectory tracking policy, we then take the new tracking result as its action sequence and improve the demonstration. 
% Since the tracking controller 
% Once the residual policy have been optimized, we can get its tracking results. If we can better track the kinematic references in this way than adopting the original approach, 
% without transferring the tracking prior, 
% the resulting action 
% If the action sequence 

% can get a better tracking result. 
% baseline trajectory that we've sampled from the tracking controller proves to serve asa 
% transfer the general knowledge encoded in the tracking controller to improve the per
% Considering the 
% the limitations of leveraging RL to solve the per-trajectory tracking 
% With the tracking controller, which has already been optimized to be able to track lots of manipulation trajectories, we devise a method that can let the single trajectory tracking benefit from the tracking controller. Specifically, for a tracking task $T$ that is difficult to solve, we first query the tracking controller for an action sequence $\mathbf{A}$. After that, we initialize $\mathbf{A}$ as the basic trajectory in the single trajectory tracking policy~\eric{since we did not explain how to do the per-trajectory tracking above, it is weird here to talk about the base trajectory.}. We then optimize the residual policy aiming to track the trajectory $T$.  Taking advantage of the general tracking prior encoded in the tracking controller, we can potentially~\eric{do not use these very vague term} get better tracking results than directly tracking $T$ with the kinematic sequence as the basic trajectory. 
% After that, we optimize the residual policy aiming to track the trajectory $T$.



% \noindent\textbf{Learning a homotopy path generator and tracking via a homotopy method.} 

% \noindent\textbf{Solving difficult tracking problem via a homotopy optimization scheme.} 
\noindent\textbf{A homotopy optimization scheme.}
% The tracking controller's training relies on the results from previously successfully tracked trajectories, which would limit its ability.~\eric{this sentence seems redundant. maybe remove it and just keep the next sentence.} 
Training the controller with data mined from itself can introduce biases and reduce diversity, hindering its generalization capabilities. To address this issue, we propose a homotopy optimization scheme to improve the per-trajectory tracking performance and to tackle previously unsolvable single-trajectory tracking problems. For the tracking problem $T_0$, instead of solving it directly, the homotopy optimization iteratively solves each tracking task in an optimization path, \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$, and finally solves $T_0$, in a similar flavor to ``chain-of-thought''~\citep{Wei2022ChainOT}. In the beginning, we leverage the RL-based tracking method to solve $T_K$. After that, we solve each task $T_m$ via the RL-based tracking method with the baseline trajectory set to the tracking result of $T_{m+1}$. This transfer of tracking results from other tasks helps us establish better baseline trajectories, ultimately yielding higher-quality tracking outcomes.
% solves it via iteratively solving each tracking task in an optimization path, \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$, 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Transferring the tracking results of other tasks can help us find better baseline trajectories, thereby offering us better tracking results with improved quality. 
% an optimization path,  \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$. 
% Instead of tracking a trajectory directly, the homotopy optimization 
% solving each single-trajectory tracking problem directly, 
% % a strategy that utilizes RL and transfers tracking knowledge to tackle previously unsolvable single-trajectory tracking problems. 
% Instead of addressing each single-trajectory problem directly, we employ a homotopy optimization method, inspired by the "chain-of-thought" approach~\citep{Wei2022ChainOT}, to enhance tracking results. Specifically, the homotopy optimization addresses the tracking problem for task \(T_0\) through an optimization path, \((T_K, T_{K-1}, ..., T_0)\). Initially, we use RL to solve for \(T_K\). Subsequently, we address each task \(T_m\) by applying the RL-based tracking method, using the tracking result of \(T_{m+1}\) as the baseline trajectory. This transfer of tracking results from other tasks enables us to establish better baseline trajectories, ultimately yielding higher-quality tracking outcomes.

% Considering the fact that the tracking controller is trained with the supervision from the tracking results of the already successfully tracked trajectories, its ability would be restricted.  Using data mined by the controller to train the controller could suffer from data biases and diversity issues, which may hinder the generalization ability of the tracking controller. To mitigate this issue, we need a strategy that can solve previously unsolvable single trajectory tracking problems by leveraging RL and even transferring the tracking prior. Therefore, instead of solving each single-trajectory tracking problem directly, we propose to leverage a homotopy optimization method, mimicking ``chain-of-thought''~\citep{Wei2022ChainOT}, to improve the tracking results. Specifically, the homotopy optimization solves the racking problem of task $T_0$ via an optimization path,  \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$. At the beginning, we leverage the RL to solve $T_K$. After that, we solve each task $T_m$ via the RL-based tracking method with the baseline trajectory set to the tracking result of $T_{m+1}$. Transferring the tracking results of other tasks can help us find better baseline trajectories, thereby offering us better tracking results with improved quality. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% may be restricted in the ability to solve 
% relatively simple tracking problems.
% Therefore, using the data mined 
% that can effectively improve the diversity and quality 
% ~\eric{Need to mention that the using the data mined by the controller to train the controller could suffer from data biases and diversity issues, which could hinder the generalizability of the controller to novel and challenging cases. Therefore we need bias mitigation techniques.} Solving very difficult single trajectory tracking problems would still pose lots of challenges. 

% optimizing the per-trajectory tracker alone, we propose to leverage a 

% to improve the tracking results of very difficult trajectories~\eric{very difficult trajectories sound like just a very small portion of the data? it is better to give the feeling that the method is generally helpful}.

% higher-quality
% by the controller to train the controller could suffer from data biases and diversity issues, which may hinder the generalization ability of the tracking controller. To mitigate this issue, we need a strategy that can solve previously unsolvable single trajectory tracking problems by leveraging RL and even transferring the tracking prior. 
% by transferring the tracking result of $T_{m+1}$ as the baseline trajectory. x

% In this way, we leverage the tracking knowled
% If the tracking result of $T_0$ can achieve can achieve better tracking performance
% Iteratively solving each problem 
% transfer the tracking results of $T_{m+1}$ as the baseline trajectory of the tracking task $T_m$  
% solve the per-
% for a tracking task $T_0$, 
% $T_0$ that is hard to solve, we propose to solve $T_0$ via a homotopy path, \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$. Starting from solving the first task $T_K$, we transfer the tracking result obtained in the current task to initialize the basic trajectory of the next tracking task. By gradually transferring tracking results from the previous task and solving each problem gradually in this manner, we could potentially~\eric{again, this is a very weak term and should be avoided} get better tracking results of task $T_0$. 

\noindent\textbf{Finding effective homotopy optimization paths.}
% Although leveraging the homotopy optimization scheme to solve previously unsolvable tracking problems proves to be an effective strategy for many tracking tasks, it relies on effective optimization paths. A naive way to find an effective homotopy path is brute-force searching. Specifically, given a collection of kinematic references, we optimize their per-trajectory tracking results at first. We also identify neighbors for each tracking task, \emph{e.g.,} based upon the similarity between every two kinematic reference trajectories. After that, we iteratively transfer the optimization results from neighbors and re-optimize the residual policy for each tracking task. We record the neighbor that can give the current tracking task a better baseline trajectory than its kinematic reference sequence as an effective ``parent task''. After we've reached the maximum number of iterations, \emph{i.e.,} $K$, to find effective homotopy paths for the tracking task $T_0$, we can start from $T_0$ and backtrace effective ``parent tasks''. We regard $(T_{K}, ..., T_0)$ as an effective homotopy path of $T_0$ if for each $0\le m \le K$, $T_{m+1}$ is an effective parent task of $T_m$. 
While leveraging the homotopy optimization scheme to solve previously unsolvable problems has proven effective for many tasks, it depends on identifying effective optimization paths. A straightforward approach is brute-force searching. Specifically, given a set of kinematic references, we first optimize their per-trajectory tracking outcomes. We then identify neighbors for each task based on the similarity between pairs of kinematic reference trajectories. Next, we iteratively transfer optimization results from neighboring tasks and re-optimize the residual policy for each tracking task. For a specific task, we consider a neighbor that provides a better baseline trajectory than its kinematic trajectory as an effective ``parent task''.
% We consider a neighbor that provides a better baseline trajectory than the original kinematic reference as an effective ``parent task''. 
After reaching the maximum number of iterations, $K$, we can find effective homotopy paths for a task, \emph{i.e.,} $T_0$, by starting from $T_0$ and backtracing
% begin from the target task to optimize $T_0$ and backtrace 
% the
effective ``parent tasks''. We define $(T_{K}, ..., T_0)$ as an effective homotopy path for $T_0$ if, for each $0 \leq m \leq K$, $T_{m+1}$ is 
% serves as 
an effective parent task for $T_m$.


% In each iteration, for each tracking task, we try to transfer the tracking result of each of its neighbors as its baseline trajectory and re-optimize the residual tracking policy. 

% suppose we wish to 
% several iterations, 

% the best initialization as the best ``parent task''. After several iterations, \emph{i.e.,} $K$, if we can solve the current target tracking task successfully (\emph{i.e.,} achieving the tracking error smaller than a success threshold), we then start from the current tracking task and backtrace to find an effective homotopy optimization path. In more detail, starting from the task $T_0$, we can find its best ``parent task'' $T_1$. Then for each $1\le m\le K-1$, we find its best ``parent task'' $T_{m+1}$. Finally, we get an effective optimization path $(T_{K}, ..., T_0)$ for the task $T_0$. 

% If we can get better tracking result, we record the 
% every tracking task, we try to transfer th 


% \noindent\textbf{Learning a homotopy generator by encoding effective optimization paths.} 
\noindent\textbf{Learning a homotopy generator for efficient homotopy path planning.} 
% Leveraging the homotopy optimization scheme to 
% Since finding effective homotopy optimization paths is costly, which is unaffordable during the inference time 
% Finding effective homotopy optimization paths for tracking each trajectory is extremely costly and unaffordable during inference time. Therefore, we propose to learn a homotopy path generator $\mathcal{M}$ from a small set. Then, we can use the homotopy generator to propose effective homotopy paths for a tracking task efficiently. The most critical part of finding a homotopy path is finding effective ``parent tasks''. We re-formulate the homotopy path generator learning problem as a tracking task transformation problem. For each tracking task $T_0$, we wish the generator $\mathcal{M}$ to give us a distribution of its effective ``parent tasks'': $\mathcal{M}(\cdot\vert T_0)$, considering the fact that a single tracking task may have multiple effective ``parent tasks''. Once $\mathcal{M}$ has been trained, for $T_0$, we can iteratively query $\mathcal{M}$ to generate a homotopy path: $(T_K, ..., T_0)$, where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m), \forall 0\le m\le K-1$. 
% We propose to learn a conditional diffusion model as the tracking task transformer, taking advantage of its strong distribution modeling ability. Given a collection of tracking tasks, described using the kinematic reference trajectories of the hand and the object, and the object geometry, we first train a diffusion model to describe the distribution of tracking tasks. 
% To prepare data to fine-tune the diffusion model into a conditional diffusion model, we first search effective homotopy paths from the tracking task collection. 
% Having completed the search, we can obtain a set of paired data of (tracking task $T_c$, effective ``parent task'' $T_p$). 
% We then use these data to tune the diffusion model into a conditional diffusion model, \emph{i.e.,} $T_p \sim \mathcal{M}(\cdot\vert T_c)$. A well-trained $\mathcal{M}$ can propose an effective ``homotopy path'' by recursively finding the parent: $(T_K,...,T_0)$, where $T_{m+1}\sim \mathcal{M}(\cdot \vert \mathcal{T}_m),\forall 0\le m\le K-1$.
Finding effective homotopy optimization paths for tracking each trajectory is computationally expensive and impractical during inference. To address this, we propose learning a homotopy path generator $\mathcal{M}$ from a small dataset, enabling efficient generation of effective homotopy paths for other tracking tasks. The key problem in identifying homotopy paths lies in finding  effective ``parent tasks''. We reformulate this problem as a tracking task transformation problem,
% , 
aiming for a generator $\mathcal{M}$ that provides a distribution of effective ``parent tasks'' for each tracking task $T_0$: $\mathcal{M}(\cdot \vert T_0)$, considering the fact that a single tracking task may have multiple effective ``parent tasks''.
Once $\mathcal{M}$ is trained, we can find a homotopy path by iteratively finding parent tasks.
% iteratively query it to generate a homotopy path for a tracking task. 
% for $T_0$: $(T_K, ..., T_0)$, where $T_{m+1} \sim \mathcal{M}(\cdot \vert T_m)$ for all $0 \le m \le K-1$.
We propose training a conditional diffusion model as the tracking task transformer, leveraging its strong distribution modeling capability. Given a set of tracking tasks, characterized by the kinematic reference trajectories of the hand and object, as well as object geometry, we first train a diffusion model to capture the distribution of tracking tasks.
To fine-tune this diffusion model into a conditional model, we first search for effective homotopy paths within the tracking task dataset. This yields a set of paired data of the tracking task $T_c$ and their corresponding effective ``parent task'' $T_p$. We then use this data to tune the diffusion model into a conditional diffusion model, such that $T_p \sim \mathcal{M}(\cdot \vert T_c)$. A well-trained $\mathcal{M}$ can efficiently propose an effective homotopy path for a tracking task, \emph{i.e.,} $T_0$, by starting from $T_0$ and recursively finding the parent task, resulting in  $(T_K, ..., T_0)$, where $T_{m+1} \sim \mathcal{M}(\cdot \vert T_m)$ for all $0 \le m \le K-1$.
% propose an effective homotopy path by recursively finding parent tasks: $(T_K, ..., T_0)$, where $T_{m+1} \sim \mathcal{M}(\cdot \vert T_m)$ for all $0 \le m \le K-1$.


% that can efficiently generate an effective homotopy path $(T_K, ...., T_0)$ for a tracking task $T_0$. 
% With the learned generator $\mathcal{M}$, we can leverage it to efficiently
% With the learned generator $\mathcal{M}$, 
% Then we can transfer the knowledge of ``homotopy paths'' encoded in $\mathcal{M}$ to more diverse trajectories and plan effective homotopy paths for them using $\mathcal{M}$ in an efficient manner. 

% apply the homotopy generator 
% effectively transfer the 
% Since t


% With a well-trained $\mathcal{M}$, we can recursively find 
% ~\eric{Need a summary sentence describing the inference time behavior?} 

% the collection of tracking tasks. 
% a collection of 
% We first train a diffusion model to describe the distribution of 
% To prepare data, we first search effective homotopy paths from a collection of tracking tasks. Having completed the search, we can obtain a set of paired data of (tracking task, effective ``parent task''). 
% After the search 
% Each searched path can give us a collection of paried tracking 

% can be leveraged to propose effective homotopy optimization paths efficiently during the inference. 



% Taking the tracking task $T_0$ as the example, in each iteration, we try to transfer the optimization result of each  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \noindent\textbf{Learning a homotopy generator by encoding beneficial optimization paths.} 
% \noindent\textbf{Learning a homotopy generator by encoding beneficial optimization paths.} 
% Solving each difficult tracking task in this fashion~\eric{what fashion? make sure every time when you use pronoun, it is clear}, though proved to enough effective, relies on correct~\eric{effective or correct? there does not seem to be a only correct answer for homotopy path} homotopy paths.~\eric{need to explain the naive way to build these paths first (the basic trial and error stuff) before you comment on the cost below.} Searching for correct paths for each difficult-to-track trajectory from scratch, however, is very costly. Therefore, we propose to learn a homotopy generator that can directly propose beneficial homotopy paths at the inference time.~\eric{comment on its connection of chain of though}
% Learning a homotopy generator requires valid optimization paths.~\eric{it is not clear since people dont know you are learning in a supervised manner. You assume too much context here.} Thus we first design an automatic tracking task structure exploration strategy for finding beneficial homotopy paths. We then train a homotopy generator to encode the mined paths~\eric{for efficient inference}.

% Specifically, we try to explore beneficial homotopy optimization paths from the trajectories in the training dataset via a breadth-first-searching strategy. 
% % Specifically, we iteratively explore beneficial cross-tracking task relations from a set of kinematic trajectories
% % We iteratively explore  beneficial cross-.
% % We explore beneficial homotopy paths from the trajectories in the training dataset via a 
% In each searching iteration, we iteratively explore beneficial cross-tracking task relations~\eric{this term is weird and not intuitive. An easier way to introduce what you what to do is to define the term first and then use it. It seems we are using terms first and deine later...Here for every two trajectories, we can evaluate whether their tracking results can benefit the tracking process of each other and we use directional edges to encode such relations.} from a set of kinematic trajectories. For each trajectory, we first identify its neighborhood from other kinematic trajectories via the similarity between two kinematic sequences. After that, we first run the per-trajectory tracking optimization to get their tracking results. Then we try to construct cross-tracking task relations via an iterative BFS approach. 
% In each iteration, for each tracking task $T$, we try to transfer the tracking result of its neighbour $T_p$ to initialize its basic trajectory and re-train the residual policy. If we can get better tracking results using the initialization from $T_p$, we say $T_p\rightarrow T$ a beneficial cross-task relation. We regard $T_p$ as the ``parent trajectory'' of $T$. We record the best tracking result for each trajectory obtained at this iteration.
% After severe iterations, we have obtained a beneficial cross-task relation set $\mathcal{C} = \{ (T_p\rightarrow T) \}$ which contains each beneficial cross-task relation. With $\mathcal{C}$, we regard $(T_{K}, T_{K-1}, ..., T_0)$ is a valid homotopy path if $T_{m+!}$ is the parent task of $T_m$ for each $0\le m \le K - 1$. 



% We propose to train a model that transforms each trajectory $T_c$ to the parent trajectory $T_p$ to model the tracking task structure.~\eric{need to talk about the motivation. the previous mined relationship is only a small set due to the heavy computation cost and we need to use the model to cover more diverse trajectories} 
% Considering the fact that a single child trajectory $T_c$ may have multiple different parent trajectories $T_p$, we formulate it as a conditional trajectory generation problem where the goal is to generate the parent trajectories conditioned on the child $T_c$. Therefore, we train a conditional diffusion model to accomplish this vision. Specifically, we first train a trajectory diffusion model $\mathcal{M}$ which models the distribution of all kinematic trajectories. After that, we fine-tune it to a conditional generative model that describes the distribution of the parent trajectory of each child trajectory. By sampling from the conditional generative model, we transform each tracking task to its parent tracking task, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. We can construct a homotopy path by iteratively querying the conditional generative model to sample the parent tasks, \emph{i.e.,} $(T_K, T_{K-1}, ..., T_0)$ where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m)$, $0\le m \le  K - 1$. 

% At the inference time, we let the homotopy generator propose a homotopy path for a hard-to-solve task $T$.~\eric{when to stop?} We gradually solve each tracking task in the path and transfer tracking results to the next task to solve the problem finally. 


% These tracking results are regarded as 
% For each trajectory, we first identify a neighborhood for it from other kinematic trajectories via the similarity between two kinematic trajectories. We first run the per-trajectory tracking optimization to get their individual tracking results. Then we try to construct cross-task relations using an iterative BFS approach. 
% % \todo{all trajs with the initially optimized results} \todo{at first jwe identify ja neighborhood set } 
% In each iteration, for each 





% homotopy path exploration strategy for 
% automatic tracking task structure exploration strategy for finding beneficial homotopy paths. Then we train a homotopy generator to encode the mined paths.


% previous tracking task to initialize the basic trajectory of the next tracking task. By gradually solving each problem in this manner in the series, we could potentially get better results in the task $T$, taking advantage of the basic trajectory initialized from other tracking tasks. 

% % to explore the tracking task
% % explore the tracking task structure and leverage a homotopy method to resolve these challenges by borrowing knowledge from other problems. 
% % Specifically, for a tracking task 
% % to explore


% The homotopy method, though proved to enough effective in resolving challenges in very difficult tracking tasks, relies on correct homotopy paths. 




\vspace{-5pt}
\subsection{Improving the Tracking Controller via Iterative Optimization}
\label{sec:method_iteration}
\vspace{-5pt}

% We employ an iterative approach that alternates between training the tracking controller using abundant robot tracking demonstrations and curating more diverse and higher-quality tracking demonstrations using the controller. Our method consists of three stages. 
% In the first stage, we sample a small set of tracking tasks and generate a demonstration set by applying reinforcement learning (RL) to obtain single trajectory tracking results for each task.  With these demonstrations, we train a tracking controller using RL and IL. We do not learn the homotopy path generator at this stage because the generalization ability of the learned model will be restricted by the number of effective homotopy paths used for training. 
% In the second stage, we sample a trajectory dataset from the remaining tasks, weighted by the tracking error of the controller. We use RL, with attempts to transfer tracking prior, to obtain per-trajectory tracking results, search for homotopy paths, and learn a homotopy generator based on these results. The best tracking results of all successfully tracked trajectories are then curated into a new demonstration set, which we use to re-train the tracking controller.

We adopt an iterative approach that alternates between training the tracking controller with abundant robot tracking demonstrations and curating more diverse, higher-quality demonstrations using the controller. Our method is divided into three stages.
In the first stage, we sample a small set of tracking tasks and generate an initial demonstration set by applying RL to obtain single-trajectory tracking results for each task. Using these demonstrations, we train the tracking controller with both RL and IL. At this stage, we do not train the homotopy path generator, as the model's generalization ability would be limited by the small number of effective homotopy paths available for training.
In the second stage, we sample a dataset of trajectories from the remaining tasks, weighted according to the controller's tracking error. We then use RL, incorporating tracking priors, to optimize per-trajectory tracking, search for homotopy paths, and train a homotopy path generator based on the resulting data. The best tracking results from all successfully tracked trajectories are curated into a new demonstration set, which is used to re-train the tracking controller.
In the third stage, we resample tracking tasks from the remaining set and leverage RL, the tracking controller, and the homotopy generator to curate another set of tracking demonstrations. This final set is used to optimize the tracking controller, resulting in our final model.

% With the above designs, we then adopt an iterative approach where we alternate between 1) training the tracking controller using abundant robot tracking demonstrations and 2) curating a large number of tracking demonstrations using the tracking controller. 
% To balance between the effectiveness of the tracking controller and the time cost in its training, our method consists of three stages as detailed as follows. In the first stage, we sample a small amount of tracking tasks $\mathcal{S}_1$ from all training tasks. 
% Since we do not have the tracking controller or the homotopy generator at the beginning, we create a robot tracking demonstration set by directly leveraging RL to obtain the single trajectory tracking result for each tracking task in $\mathcal{S}_1$. With these demonstrations, we train a tracking controller using RL and IL. The homotopy path generator is not learned at this stage because the generalizaton ability of the learned model will berestricted by the number of effective homotopy paths used for training. 
% In the second stage, we additionally sample a trajectory dataset from the remaining training tracking tasks, with weight positively proportional to the tracking error of the tracking controller. We then jointly leverage RL and the tracking controller to obtain per-trajectory tracking results. We also search the homotopy paths and learn a homotopy generator using searched results. We then curate a demonstration set from the best per-trajectory tracking results we've obtained. 
% With these demonstrations, we re-train a tracking controller.  
% In the third stage, we re-sample tracking tasks from the remaining set. Jointly leveraging RL, the tracking controller, and the homotopy generator, we curate a new robot tracking demonstration set. We then re-train the tracking controller with the supervision provided by these demonstrations. We take it as the final optimized tracking controller. 
% Specifically, 

% data from the whole training dataset. 


% Denote the total tracking task set sampled till now as $\mathcal{S}_2$, 




% We then try to get the per-trajectory tracking results taking the joint effort of per-trajectory tracking optimization, tracking data prior from the tracking controller and the homotopy generator. Having obtained current action-labeled trajectories, we re-train the tracking controller with the supervision provided by those trajectories. We then take it as the final optimized tracking controller.~\eric{Here we only introduce what we do but do not explain the rationality. Why only homotopy in the third stage but not the second stage? Why only three stages in total but not more? At least we should comment a bit on this since with high chance reviewers will ask about it as well. It is better to say something before the others ask.}

% To learn a homotopy generator, we search effective homotopy optimization paths and j
% to get single trajectory tracking result for each 
% We then try~\eric{avoid using these weak terms} to get the per-trajectory tracking result for each trajectory in both the re-sampled dataset and the original dataset taking the joint effort of both the per-trajectory tracking optimization and the tracking data prior provided by the tracking controller. After that, we obtained the second version of the demonstration data. We then re-train the trajectory controller with the supervision from action sequences in the dataset. In this stage, we construct the tracking task structure by searching homotopy optimization paths from trajectories in the dataset. We train a homotopy generator that encodes the searched optimization paths. In the third stage, we re-train the tracking controller via labeled trajectories obtained till now. In the third stage, 
% By optimizing the per-trajectory tracker for each trajectory in the dataset, we get the first version of demonstration data containing trajectories with high-quality action sequences. After that, the labeled dataset is leveraged to train the tracking controller. Then in the second stage, 

% and the tracking task structure prior provided by the tracking task structure prior model. 
% a tracking task structure prior model which encodes the optimization paths. 
% via the imitation-augmented RL. 
% is composed of three stages. 
% e then adopt an interactive approach to gradually get a strong tracking controller. 











% Considering the fact that the tracking controller is trained with the supervision from the tracking results of the already successfully tracked trajectories, it may be restricted in the ability to solve relatively simple tracking problems. Solving very difficult single trajectory tracking problems would still pose lots of challenges. Therefore, instead of optimizing the per-trajectory tracker alone, we propose to explore the tracking task structure and leverage a homotopy method to resolve these challenges by borrowing knowledge from other problems. 
% Specifically, for a tracking task $T$ that is hard to solve, we propose to solve $T$ via a homotopy path, \emph{e.g.,} $(T_A, T_B, ..., T)$. Starting from solving the first task $T_A$, we transfer the tracking result obtained in the previous tracking task to initialize the basic trajectory of the next tracking task. By gradually solving each problem in this manner in the series, we could potentially get better results in the task $T$, taking advantage of the basic trajectory initialized from other tracking tasks. 


% for difficult-to-solve problems 
% to facilitate the per-trajectory tracking problem solving, and 2) 
% introduce two techniques to improve the per-trajectory tracking policy
% with the  tracking controller, we try to 
% With the tracking controller, we try

% th successful action sequences, we need to infer action 
% we need to infer action sequences for kinematics
% We devise a per-trajectory tracking scheme to extract a large volume of high-quality imitation-ready data from kinematic-only trajectories. Initially, single trajectory tracking simplifies the problem by not requiring versatility or generalization, making it more manageable than training a general tracking controller. For various straightforward manipulation trajectories, per-trajectory tracking can effectively leverage the basic RL-based training scheme outlined earlier. However, relying solely on RL to track each trajectory independently presents challenges for more complex tracking scenarios. To address this, we introduce two techniques that enable single trajectory tracking to benefit from the neural controller and the structure of the tracking tasks. The first technique involves transferring tracking data to the controller to enhance single trajectory performance. The second explores the tracking task structure, employing a homotopy method to mitigate the difficulties associated with challenging single trajectory tracking problems.
% % We devise a per-trajectory tracking scheme to mine a large number of high-quality imitation-ready data from kinematic-only trajectories. First, single trajectory tracking, without the demand on versatility or the generalization ability, reduced to a simpler problem than training a general tracking controller. For various manipulation trajectories that are not very difficult, per-trajectory tracking is a solvable problem leveraging the basic RL-based training scheme detailed above. However, solely relying on tracking every single trajectory independently via RL would still face challenges in resolving very difficult tracking problems. Therefore, we propose two techniques to let the single trajectory tracking benefit from the neural controller and the tracking task structure. The first one involves transferring the tracking data prior to the tracking controller to facilitate the single trajectory tracking. The second one tries to explore the tracking task structure and leverage a homotopy method to ease the difficulty in challenging single trajectory tracking problems. 
% % if leveraging advanced model-free RL techniques. 
% % By leveraging the RL to train a single trajectory tracking policy, leveraging the above designed action space, observations, and the reward, we can already get high-quality tracking results for lots of manipulation trajectoreis. 


% \noindent\textbf{Improving per-trajectory tracking via tracking data prior.} With the tracking controller, which has already been optimized to be able to track lots of manipulation trajectories, we devise a method that can let the single trajectory tracking benefit from the tracking controller's tracking capability. Specifically, for a tracking task $T$ that is difficult to solve, we first query the tracking controller for a reasonable action sequence $\mathbf{A}$. After that, we initialize $\mathbf{A}$ as the basic trajectory in the single trajectory tracking policy. After that, we optimize the residual policy aiming to track the trajectory $T$. Taking advantage of the general tracking prior encoded in the tracking controller, we can potentially get better tracking results than directly tracking $T$ with the kinematic sequence as the basic trajectory. 

% \noindent\textbf{A homotopy method for solving difficult per-trajectory tracking.} Considering the fact that the tracking controller is trained with the supervision from the tracking results of the already successfully tracked trajectories, it may be restricted in the ability to solve relatively simple tracking problems. Solving very difficult single trajectory tracking problems would still pose lots of challenges. Therefore, instead of optimizing the per-trajectory tracker alone, we propose to explore the tracking task structure and leverage a homotopy method to resolve these challenges by borrowing knowledge from other problems. 
% Specifically, for a tracking task $T$ that is hard to solve, we propose to solve $T$ via a homotopy path, \emph{e.g.,} $(T_A, T_B, ..., T)$. Starting from solving the first task $T_A$, we transfer the tracking result obtained in the previous tracking task to initialize the basic trajectory of the next tracking task. By gradually solving each problem in this manner in the series, we could potentially get better results in the task $T$, taking advantage of the basic trajectory initialized from other tracking tasks. 

% \noindent\textbf{Learning a homotopy generator by mining beneficial optimization paths.} The homotopy method, though proved to enough effective in resolving challenges in very difficult tracking tasks, relies on correct homotopy paths. Searching for correct paths for each difficult-to-track trajectory from scratch, however, is very costly. Therefore, we propose to learn a homotopy generator that can directly propose beneficial homotopy paths at the inference time. 
% Learning a homotopy generator requires valid homotopy paths. Thus we first design an automatic tracking task structure exploration strategy for finding beneficial homotopy paths. Then we train a homotopy generator to encode the mined paths.

% We explore beneficial homotopy paths from the trajectories in the training dataset via a breadth-first-searching strategy. Specifically, we iteratively explore beneficial cross-tracking task relations from a set of kinematic trajectories.
% For each trajectory, we first identify a neighborhood for it from other kinematic trajectories via the similarity between two kinematic trajectories. We first run the per-trajectory tracking optimization to get their individual tracking results. Then we try to construct cross-task relations using an iterative BFS approach. 
% % \todo{all trajs with the initially optimized results} \todo{at first jwe identify ja neighborhood set } 
% In each iteration, for each tracking task $T$, we try to transfer the tracking result of its neighboring tracking task $T_p$ to initialize its basic trajectory and re-train the residual policy. If we can get better tracking results in this manner, we say $T_p\rightarrow T$ a beneficial cross-task relation. We regard $T_p$ as the ``parent trajectory'' of $T$. We record the best tracking result for each trajectory obtained at this iteration After severe iterations, we have obtained a beneficial cross-task relation set $\mathcal{C} = \{ (T_p\rightarrow T) \}$ which contains each beneficial cross-task relation. With $\mathcal{C}$, we regard $(T_{K}, T_{K-1}, ..., T_0)$ is a valid homotopy path if $T_{m+!}$ is the parent task of $T_m$ for each $0\le m \le K - 1$. 

% We propose to train a model that transforms each trajectory $T_c$ to the parent trajectory $T_p$ to model the tracking task structure. 
% Considering the fact that a single child trajectory $T_c$ may have multiple different parent trajectories $T_p$, we formulate it as a conditional trajectory generation problem where the goal is to generate the parent trajectories conditioned on the child $T_c$. Therefore, we train a conditional diffusion model to accomplish this vision. Specifically, we first train a trajectory diffusion model $\mathcal{M}$ which models the distribution of all kinematic trajectories. After that, we fine-tune it to a conditional generative model that describes the distribution of the parent trajectory of each child trajectory. By sampling from the conditional generative model, we transform each tracking task to its parent tracking task, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. We can construct a homotopy path by iteratively querying the conditional generative model to sample the parent tasks, \emph{i.e.,} $(T_1, T_2, ..., T_k)$ where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m)$, $1\le m \le k-1$. 

% At the inference time, we let the homotopy generator propose a homotopy path for a hard-to-solve task $T$. We gradually solve each tracking task in the path and transfer tracking results to the next task to solve the problem finally. 



% \noindent\textbf{Iterative optimization for progressively improving the tracking controller. } We then adopt an interactive approach to gradually get a strong tracking controller. Specifically, our method is composed of three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing the per-trajectory tracker for each trajectory in the dataset, we get the first version of imitation-ready data containing trajectories with high-quality action sequences. After that, the labeled dataset is leveraged to train the tracking controller via the imitation-augmented RL. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories with weight positively proportional to the tracking error of the first version controller. We then try to get the per-trajectory tracking result for each trajectory in both the re-sampled dataset and the original dataset taking the joint effort of both the per-trajectory tracking optimization and the tracking data prior provided by the tracking controller. After that, we obtained the second version of the imitation-ready data. We then re-train the trajectory controller with the supervision from action sequences in the dataset. In this stage, we construct the tracking task structure by searching homotopy optimization paths from trajectories in the dataset. We train a tracking task structure prior model which encodes the optimization paths. In the thrid stage, we re-train the tracking controller via labeled trajectories obtained till now. In the third stage, we re-sample a subste from the remaining trajectories. We then try to get the per-trajectory tracking results taking the joint effort of per-trajectory tracking optimization, tracking data prior from the tracking controller, and the tracking task structure prior provided by the tracking task structure prior model. Having obtained current action-labeled trajectories, we re-train the tracking controller with the supervision provided by those trajectories. We then take it as the final optimized tracking controller. 


% e further propose a homotopy method to resolve challenges in those problems. 
% propose to tackle difficult
% tackle difficult per-trajectory trac
% it may still be very hard for us to get good results in
% % Leveraging advanced RL with our dedicated designs for tracking, we can solve lots of per-trajectory tracking problems to a satisfactory extent. However, this strategy still struggles to solve very difficult tracking problems considering the inherent challenges of manipulation tracking. 
% % restrictions of RL. 
% Therefore, we propose to tackle difficult per-trajectory tracking problems via a homotopy method. 
% % a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% % Therefore, we propose a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% Specifically, for the trajectory $A=(\mathbf{H}_A, \mathbf{O}_A)$ that is difficult to track directly, instead of directly tracking the trajectory $A$, we propose to find an optimization path consisting of a series of tracking tasks that can help us solve the tracking problem of $A$. We then try to track $A$ by tracking each trajectory in the path and transfer results to the next in a one-by-one manner. If in this way we can get better tracking results for $A$ than directly solving $A$, we regard it as a good optimization path for $A$. We then further propose to encode such tracking task structure into a model so that it can propose useful optimization paths during the inference time efficiently. To fulfill this vision, we propose to first mine useful optimization paths from trajectories in the training dataset. We then encode the searched optimization paths into a model so that it can provide us with good optimization paths during the inference period efficiently. 



% to benefit single trajectory tracking from 
% the demand on the tracking
% resuded as a simpler problem than training a general racking controller, 
% To acquire a large number of high-quality tracking results, we devise a per-trajectory tracking scheme
% acquire high-quality per-trajectory tracking results 
% Training a high quality tracking controller requires 
% Training the tracking controller requires a large j
% Single tracjectoyr tracking control, tho
% Solving the per-trajectory tracking problem directly would still make it hard to address the challenge in tracking very difficult trajectories. To improve tracking results in these so that we can get more diverse imitation ready data with high quality action sequences in more tracking cases, we design a strategy where we can leverage the general tracking controller and the tracking task structure prior to better solve per-trajectory tracking problem. With the tracking controller, we devise two strategies to improve per-trajectory tracking performance. First, we try to leverage the general tracking prior encoded in the tracking controller to facilitate difficult per-trajectory tracking problem solving. The tracking controller trained to track lots of manipulation trajectories, with the supervision from high-quality imitation-ready data, already has the capability to give reasonable tracking results for various manipulation trajectories. So we design a strategy where we can let difficult per-trajectory tracking benefit from such tracking prior from the tracking controller. Second, instead of solving the per-trajectory tracking problem alone, we propose a homotopy method whih can effectively solve a difficult tracking problem by solving the task via an optimization path, and a homotopy generator which can propose beneficial homotopy optimization paths efficiently for a problem that is difficult to solve. We will detail them as follows. 


% \noindent\textbf{}



% % \noindent\textbf{Improving per-trajectory trackers via tracking prior and curriculum scheduling.} 
% \noindent\textbf{Improving per-trajectory trackers via tracking data prior and task structure prior.} The general tracking controller and the tracking task structure prior offer us two ways to improve the per-trajectory tracking result of a specific trajectory that is difficult to track, denoted as $A$. Firstly, we sample the action sequence from the general tracking controller for the current tracking task. We then initialize the basic trajectory as the sampled action sequence and re-train the residual policy to try to get better tracking results. Secondly, we let the tracking task structure prior model propose an optimization path consisting of a series of tracking tasks. After that, we solve the tracking problem of $A$ by gradually solving each task in the optimization path and transferring the results to the next one. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\textbf{A homotopy method for solving difficult per-trajectory tracking problem.} 
% % We propose 
% Leveraging advanced RL with our dedicated designs for tracking, we can solve lots of per-trajectory tracking problems to a satisfactory extent. However, this strategy still struggles to solve very difficult tracking problems considering the inherent challenges of manipulation tracking. 
% % restrictions of RL. 
% Therefore, we propose to tackle difficult per-trajectory tracking problems via a homotopy method. 
% % a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% % Therefore, we propose a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% Specifically, for the trajectory $A=(\mathbf{H}_A, \mathbf{O}_A)$ that is difficult to track directly, instead of directly tracking the trajectory $A$, we propose to find an optimization path consisting of a series of tracking tasks that can help us solve the tracking problem of $A$. We then try to track $A$ by tracking each trajectory in the path and transfer results to the next in a one-by-one manner. If in this way we can get better tracking results for $A$ than directly solving $A$, we regard it as a good optimization path for $A$. We then further propose to encode such tracking task structure into a model so that it can propose useful optimization paths during the inference time efficiently. To fulfill this vision, we propose to first mine useful optimization paths from trajectories in the training dataset. We then encode the searched optimization paths into a model so that it can provide us with good optimization paths during the inference period efficiently. 


% \noindent\textbf{Learning a homotopy generator by mining beneficial optimization paths. } 
% Given a trajectory set containing $K$ trajectories, we find useful tracking task optimization paths via breadth-first search. For each trajectory, we first identify its potential parent set via cross-trajectory similarity. Then in each searching iteration, for each task $A$, we try to use the best-tracked action trajectory of each of its parent task $B$ to initialize its tracking policy and see whether the policy optimization could benefit from the initialization. If the tracking result of trajectory $B$ can help us track the trajectory $A$, we regard $B$ as a beneficial parent tracking task of $A$. After several iterations, we identify a set of optimization paths $\mathcal{C} = \{ (T_n, ..., T_1) \} $, where for each  $1\le k \le n-1$, $T_{k+1}$ is the parent task of $T_k$.  

% Having obtained the optimization path set $\mathcal{C}$, we propose to train a model that transform each trajectory $T_c$ to the parent trajectory $T_p$ to model the tracking task structure. 
% % to model the tracking task structure. 
% Considering the fact that a single child trajectory $T_c$ may have multiple different parent trajectories $T_p$, we formulate it as a conditional trajectory generation problem where the goal is to generate the parent trajectories conditioned on the child $T_c$. Therefore, we train a conditional diffusion model to accomplish this vision. Specifically, we first train a trajectory diffusion model $\mathcal{M}$ which models the distribution of all kinematic trajectories. After that, we fine-tune it to a conditional generative model that describes the distribution of the parent trajectory of each child trajectory. By sampling from the conditional generative model, we transform each tracking task to its parent tracking task, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. We can construct an optimization path by iteratively querying the conditional generative model to sample the parent tasks, \emph{i.e.,} $(T_1, T_2, ..., T_k)$ where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m)$, $1\le m \le k-1$. 


% % \noindent\textbf{Planning the homotopy paths for solving difficult problems. } 


% \noindent\textbf{Iterative optimization for progressively improving the tracking controller. } We then adopt an interactive approach to gradually get a strong tracking controller. Specifically, our method is composed of three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing the per-trajectory tracker for each trajectory in the dataset, we get the first version of imitation-ready data containing trajectories with high-quality action sequences. After that, the labeled dataset is leveraged to train the tracking controller via the imitation-augmented RL. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories with weight positively proportional to the tracking error of the first version controller. We then try to get the per-trajectory tracking result for each trajectory in both the re-sampled dataset and the original dataset taking the joint effort of both the per-trajectory tracking optimization and the tracking data prior provided by the tracking controller. After that, we obtained the second version of the imitation-ready data. We then re-train the trajectory controller with the supervision from action sequences in the dataset. In this stage, we construct the tracking task structure by searching homotopy optimization paths from trajectories in the dataset. We train a tracking task structure prior model which encodes the optimization paths. In the thrid stage, we re-train the tracking controller via labeled trajectories obtained till now. In the third stage, we re-sample a subste from the remaining trajectories. We then try to get per-trajectory tracking result taking the joint effort of per-trajectory tracking optimization, tracking data prior from the tracking controller, and the tracking task structure prior provided by the tracking task structure prior model. Having obtained current action-labeled trajectories, we re-train the tracking controller with the supervision provided by those trajectories. We then take it as the final optimized tracking controller. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% propose to build the tracking task structure
% lots of imitation-ready data 
% the tracking controller is trained to mimic 
% with the tracking controller which already has the ability to track various manipulation 
% transfer tracking data prior encoded in the tracking controller to better solve per-trajectory tracking problem. Specifically, to solve the problem of tracking the trajectory $A$, we first try to query the trajectory controller to obtain the tracking result, an action sequence, of $A$. After that, we try to use the sampled action sequence to initialize the per-trajectory tracking 
% can leverage the tracking prior encoded in the tracking 


% \subsection{Per-Trajectory Tracking via Tracking Data Prior}
% \todo{todo} % 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Solving per-trajectory tracking directly would still make it hard to address the challenge in tracking very difficult trajectories. To improve tracking results in these difficult cases so that we can get more diverse imitation ready data with high quality action sequences in more tracking cases, we design a strategy where we can transfer tracking data prior encoded in the tracking controller to better solve per-trajectory tracking problem. Specifically, to solve the problem of tracking the trajectory $A$, we first try to query the trajectory controller to obtain the tracking result, an action sequence, of $A$. After that, we try to use the sampled action sequence to initialize the per-trajectory tracking 
% can leverage the tracking prior encoded in the tracking 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% % \subsection{Homotopy Path Generator Learning} 

% % tracking task structural modeling 

% % % \subsection{Structural Cross-Task Synergy Modeling}
% % \subsection{Structural Task Relational Space Modeling} \label{sec:method_task_space_modeling}
% % \subsection{Curriculum Scheduler Modeling via Mining and Modeling Cross-Trajectory Relations} \label{sec:method_task_space_modeling}
% % \subsection{Curriculum Scheduler Modeling} \label{sec:method_task_space_modeling}
% % \subsection{Learning Curriculum Scheduler via Modeling Tracking Curricula} \label{sec:method_task_space_modeling}
% % \subsection{Modeling Tracking Task Structure via Encoding Beneficial Optimization Paths} \label{sec:method_task_space_modeling}
% \subsection{Tracking Task Structure Modeling via Encoding Homotopy Optimization Paths} \label{sec:method_task_space_modeling}
% Leveraging advanced RL with our dedicated designs for tracking, we can solve lots of per-trajectory tracking problems to a satisfactory extent. However, this strategy still struggles to solve very difficult tracking problems considering the inherent challenges of manipulation tracking. 
% % restrictions of RL. 
% Therefore, we propose to tackle difficult per-trajectory tracking problems via a homotopy method. 
% % a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% % Therefore, we propose a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% Specifically, for the trajectory $A=(\mathbf{H}_A, \mathbf{O}_A)$ that is difficult to track directly, instead of directly tracking the trajectory $A$, we propose to find an optimization path consisting of a series of tracking tasks that can help us solve the tracking problem of $A$. We then try to track $A$ by tracking each trajectory in the path and transfer results to the next in a one-by-one manner. If in this way we can get better tracking results for $A$ than directly solving $A$, we regard it as a good optimization path for $A$. We then further propose to encode such tracking task structure into a model so that it can propose useful optimization paths during the inference time efficiently. To fulfill this vision, we propose to first mine useful optimization paths from trajectories in the training dataset. We then encode the searched optimization paths into a model so that it can provide us with good optimization paths during the inference period efficiently. 
% % inference-time tracking task prior 
% % tracking task structure into a model so that it can provide us with inference-time tracking task structure prior efficiently. 
% % useful optimization paths into a model so that it 

% % and  and track $A$ by 
% % propose to track $A$ 
% % to solve the problem by solving each tracking 
% % the tracking curriculum tries to transfer the optimized action trajectory of a different tracking task, \emph{e.g.,} $B=(\mathbf{H}_B, \mathbf{O}_B)$ to initialize the tracking policy of $A$. If the re-optimized tracker can achieve better results than the original one, such a trail ($B\rightarrow A$) is regarded as a good curriculum. We say trajectory $B$ is the ``parent'' trajectory of $A$. Although the tracking curriculum is provided highly effective in our experiments, finding a good curriculum for solving each hard-to-track problem requires lots of trial and error and is thus very time-inefficient. Therefore, we propose to use a curriculum scheduler to expressively model tracking curricula so that that scheduler can be leveraged to propose tracking curricula efficiently. To fulfill this vision, we propose to first mine such tracking curricula from a batch of data, followed by learning a curriculum scheduler to model such tested effective curricula. 
% % rollout by a successful tracker 
% % We propose a tracking curriculum to tackle difficult per-trajectory tracking problems that continuously challenge RL when being optimized alone. 

% % \noindent\textbf{Constructing the tracking task structure.} 
% \noindent\textbf{Searching optimization paths.}
% Given a trajectory set containing $K$ trajectories, we find useful tracking task optimization paths via breadth-first search. For each trajectory, we first identify its potential parent set via cross-trajectory similarity. Then in each searching iteration, for each task $A$, we try to use the best-tracked action trajectory of each of its parent task $B$ to initialize its tracking policy and see whether the policy optimization could benefit from the initialization. If the tracking result of trajectory $B$ can help us track the trajectory $A$, we regard $B$ as a beneficial parent tracking task of $A$. After several iterations, we identify a set of optimization paths $\mathcal{C} = \{ (T_n, ..., T_1) \} $, where for each  $1\le k \le n-1$, $T_{k+1}$ is the parent task of $T_k$.  
% % we identify a set of parent tasks for each task, which further construct our tracking task structure. 
% % Such relations then form our tracking task structure. 
% % we regard $B\rightarrow A$ 
% % as a valid curriculum. After several iterations, two times in our experiments, we can identify a set of valid tracking curricula $\mathcal{C} = \{ T_p \rightarrow T_c \}$, where $T_p$ denotes the parent trajectory and $T_c$ represents the child trajectory. 
% % we find tracking curricula via breadth-first search. For each trajectory, we first identify its potential parent set via 

% % \noindent\textbf{Searching tracking curricula.} 

% \noindent\textbf{Modeling tracking task structure.}  Having obtained the optimization path set $\mathcal{C}$, we propose to train a model that transform each trajectory $T_c$ to the parent trajectory $T_p$ to model the tracking task structure. 
% % to model the tracking task structure. 
% Considering the fact that a single child trajectory $T_c$ may have multiple different parent trajectories $T_p$, we formulate it as a conditional trajectory generation problem where the goal is to generate the parent trajectories conditioned on the child $T_c$. Therefore, we train a conditional diffusion model to accomplish this vision. Specifically, we first train a trajectory diffusion model $\mathcal{M}$ which models the distribution of all kinematic trajectories. After that, we fine-tune it to a conditional generative model that describes the distribution of the parent trajectory of each child trajectory. By sampling from the conditional generative model, we transform each tracking task to its parent tracking task, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. We can construct an optimization path by iteratively querying the conditional generative model to sample the parent tasks, \emph{i.e.,} $(T_1, T_2, ..., T_k)$ where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m)$, $1\le m \le k-1$. 
% % we then complete the trajectory transformation 
% % complete the trajectory transformation problem, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. 
% % % \noindent\textbf{Learning curriculum scheduler via modeling tracking curricula.}
% % $\mathcal{M}_{\mathcal{C}}: T_c $


% % With our carefully designed reward and observation space, the PPO can effectively optimize a specialist policy that achieves satisfactory performance on easy or medium manipulation tracking tasks. However, it would still struggle with achieving a reasonable solution for very difficult tasks involving intricate hand-object interactions such as subtle in-hand re-orientations and frequent contact shifting. Therefore, to further enhance the single trajectory tracking performance for providing better supervision for the tracking controller's training, we propose to explore trajectory curricula to better solve difficult tracking problems. Specifically, if we can transfer the optimized action sequence from tracking problem $A=(\mathbf{H}_A, \mathbf{O}_A)$ to $B=(\mathbf{H}_B, \mathbf{O}_B)$ as the start point of the task $B$'s optimization (\emph{i.e.,} setting the action sequence $\mathbf{A}_B$ that can successfully solve $B$ as the basic trajectory of $A$ and re-optimize the residual policy), which we also observe can achieve better performance than directly tracking $B$, we regard the problem of tracking $B$ can be benefit from tracking $A$, \emph{i.e.,} saying task $A$ is the ``parent'' trajectory of $B$. We then aim to leverage such cross-trajectory relations to construct a curriculum for each trajectory that is hard to optimize. To efficiently and effectively find such relations, we wish to learn a model that can tell us what's the most suitable ``parents'' for the current trajectory. It is hard to heuristically define a rule-based criterion such as based on the kinematic similarities or object geometry affinities, that exactly refect such relations. Therefore, we formulate this problem as a trajectory transformation and aim at learning  model $\mathcal{M}_{\mathcal{S}}$ from the trajectory dataset $\mathcal{S}$ to solve it. In detail, given a difficult-to-track trajectory $(\mathbf{H}, \mathbf{O})$, we want the model $\mathcal{M}_{\mathcal{S}}$ to transform it to its ``parent'' $(\mathbf{H}^p, \mathbf{O}^p)$. Considering the fact that there may be multiple instances that can serve as the ``parent'' for a single trajectory, the trajectory transformation ought to be a stochastic process where $\mathcal{M}_{\mathcal{S}}$ models the distribution of the parent, \textit{i.e.,} $(\mathbf{H}^p, \mathbf{O}^p) \sim \mathcal{M}_{\mathcal{S}}(\cdot\vert (\mathbf{H}, \mathbf{O}))$.

% % cross-task synergies to improve the training of a difficult task. 

% % To fulfill this vision, we further formulate the learning problem of the model $\mathcal{M}_{\mathcal{S}}$ as a conditional generative model training problem. Specifically, $\mathcal{M}_{\mathcal{S}}$ takes a trajectory $(\mathbf{H}, \mathbf{O})$ as the input and generates its parent trajectory. Therefore, we first train a diffusion model to describe the distribution of all kinematic trajectories contained in the dataset $\mathcal{S}$. After that, to acquire data for tuning it to a conditional generative model for the task transformation purpose, we propose a BFS approach to mine such ``parent-child'' paired data from the dataset. Detailed steps regarding the curriculum searching and the curriculum scheduler's training are deferred to Appendix~\ref{}. 


% %%%%%%%%%%%%%%%% move to appendix %%%%%%%%%%%%%%%
% % The BFS-based approach for constructing the task relational space and the conditional diffusion model training are detailed as follows. 

% % \todo{ add a picture for this structural space construction}

% % \todo{add the retargeted motions such as same trajectory different objects}

% % \todo{details w.r.t. how we identify the cross task affinities? }

% % \todo{extended task set?}

% % \noindent\textbf{Heuristic guided BFS for structural task relational space construction.} Given all manipulation trajectories from the training dataset $\mathcal{S}$, we first construct an expanded task set by augmenting each single task $(\mathbf{H}_A, \mathbf{O}_A, m_A)$ into $(\mathbf{H}_C, \mathbf{O}_A, m_A)$ and $(\mathbf{H}_A, \mathbf{O}_A, m_C)$. The structural task relational space wants to quantify the cross-task relations for each two different tasks in the expanded task set. One can imagine a most ideal way that is trying to test each pair of two manipulation trajectories $(A, B)$ to test whether one task, for instance task $B$ can benefit from task $A$. However, such a strategy is too expensive with the time complexity $\vert \mathcal{S}\vert^2$. If we wish not to be restricted to the first order cross-task relations only and also want to explore the high-order relations, for instance, the current task $C$ can benefit from the optimization result of task $B$ with the initialization of task $A$, the brute-force searching would cost $K\vert \mathcal{S}\vert^2$. Therefore, we adopt a heuristic guided searching strategy to reduce the time consumption to an affordable amount. 

% % Specifically, we first identify potential neighbours for each task via trajectory similarities and object geometry similarities. Having restricted the number of potential neighbours to a reasonable value, \emph{i.e.,} $K_{\text{nei}}$, we only conduct the affinity test between each potential neighbours. With this strategy, we can reduce the timeconsumption to $K K_{\text{nei}} \vert \mathcal{S}\vert$. By tuning $K$ and $K_{\text{nei}}$, we can balance the accuracy and the efficiency of the task relation space construction process. Please refer to the Supp. for more details. 
% % % Besides, it may overlook the high-order task relations, where the current task $C$ can benefit from the optimization result of task $B$ with the initialization of task $A$.  

% % % Specifically, \textcolor{red}{(TODO: add the description for the BFS part)}

% % \noindent\textbf{Conditional diffusion model for task relation modeling.} 
% % \todo{how we obtain the pairs to train the diffusion model -- both the high order and the first order} 
% % \todo{how to train the model}

% % \todo{re-check this part}
% %%%%%%%%%%%%%%%% move to appendix %%%%%%%%%%%%%%%

% % \todo{details w.r.t. how to improve per-trajectory tracker via tracking prior and the curriculum scheduler}


% % \textcolor{red}{(TODO: pharse it into a specialist-generalist-specialist iteration? )}
% % \noindent\textbf{Progressive generalist model training and labeled dataset improvement.}
% % \subsection{Progressive Generalist Model Training via ``Specialist-Generalist-Specialist'' Iterations} \label{sec:method_sgs}

% % \subsection{Progressively Improving the Tracking Controller via Iterative Optimization} \label{sec:method_sgs}

% \subsection{Iterative Optimization for Progressively Improving Tracking Controller} \label{sec:method_sgs}
% Based on the above designs, we then propose an iterative approach where the tracking controller is progressively improved by alternately executing the following two steps: 1) improving per-trajectory trackers with the joint effort of per-trajectory tracking optimization, data prior from the tracking controller, and the homotopy optimization path from the tracking task structure prior model; 2) training better tracking controller with the supervision from the improved imitation-ready data with action sequences. 
% % improving the action-labeled dataset by training better per-trajectory trackers on more trajectories leveraging the power of tracking prior provided by the general tracking controller and the optimization path from the tracking task structure prior; 2) training better tracking controller via supervision from the improved action-labeled dataset. 
% % the trajectory curriculum proposed by the curriculum scheduler; 

% % \noindent\textbf{Improving per-trajectory trackers via tracking prior and curriculum scheduling.} 
% \noindent\textbf{Improving per-trajectory trackers via tracking data prior and task structure prior.} The general tracking controller and the tracking task structure prior offer us two ways to improve the per-trajectory tracking result of a specific trajectory that is difficult to track, denoted as $A$. Firstly, we sample the action sequence from the general tracking controller for the current tracking task. We then initialize the basic trajectory as the sampled action sequence and re-train the residual policy to try to get better tracking results. Secondly, we let the tracking task structure prior model propose an optimization path consisting of a series of tracking tasks. After that, we solve the tracking problem of $A$ by gradually solving each task in the optimization path and transferring the results to the next one. 
% % tracker of a specific trajectory. Firstly, we can sample 
% % The sampled action sequence is init %
% % % , \emph{e.g.,} $A$. 
% % Firstly, we can use the action trajectory sampled from the general tracking controller on the current trajectory as the basic trajectory in its policy. By re-optimizing the residual policy, we may get better results than the original optimization. Secondly, by transforming trajectory $A$ into its parent trajectory $B$ via the curriculum scheduler and using the successful rollout action trajectory on the trajectory $B$ as the basic trajectory of $A$'s tracking policy, we re-optimize the residual policy for $A$ to try to get a better tracker for $A$. 
% % the curriculum scheduler
% % curriculum scheduler %

% \noindent\textbf{Iteratively improving tracking controller and the action-labeled dataset.} We then adopt an interactive approach to gradually get a strong tracking controller. Specifically, our method is composed of three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing the per-trajectory tracker for each trajectory in the dataset, we get the first version of imitation-ready data containing trajectories with high-quality action sequences. After that, the labeled dataset is leveraged to train the tracking controller via the imitation-augmented RL. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories with weight positively proportional to the tracking error of the first version controller. We then try to get the per-trajectory tracking result for each trajectory in both the re-sampled dataset and the original dataset taking the joint effort of both the per-trajectory tracking optimization and the tracking data prior provided by the tracking controller. After that, we have obtained the second version of the imitation ready data. We then re-train the trajectory controller with the supervision from action sequences in the dataset. In this stage, we construct the tracking task structure by searching homotopy optimization paths from trajectories in the dataset. We train a tracking task structure prior model which encodes the optimization paths. In the thrid stage, we re-train the tracking controller via labeled trajectories obtained till now. In the third stage, we re-sample a subste from the remaining trajectories. We then try to get per-trajectory tracking result taking the joint effort of per-trajectory tracking optimization, tracking data prior from the tracking controller, and the tracking task structure prior provided by the tracking task structure prior model. Having obtained current action-labeled trajectories, we re-train the tracking controller with the supervision provided by those trajectories. We then take it as the final optimized tracking controller. 
% % The tracking controller 
% % by encoding such optimization paths. 
% % The resampled dataset is leveraged the action-labeled dataset, \emph{i.e.,} $\mathcal{A}_1$. After that, the labeled dataset is leveraged to train the tracking controller. With the trained general controller, we evaluate it on all training tasks. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories where the weight is positively proportional to the tracking error of the first version controller. The resampled dataset is then labeled by optimizing their per-trajectory trackers. 
% % Combining these optimized trajectories and labeled trajectories in the first stage, we obtain the second version of the labeled dataset $\mathcal{A}_2$. The tracking controller is then trained via the supervision provided by $\mathcal{A}_2$. We mine trajectory curricula to improve tracking results of the currently selected trajectory. With the resulting tracking curricula, we then train a curriculum scheduler. In the third stage, we re-sample a subset from the remaining trajectories and use the tracking controller as well as the curriculum scheduler to label them, resulting in the third version of labeled dataset $\mathcal{A}_3$. After that, we re-train the tracking controller with supervision provided by $\mathcal{A}_3$. 
% % In the third stage, 
% % with the re-trained controller, we then construct the 
% % task relations space and try to improve the single trajectory optimization results leveraging the task relations space and the knowledge encoded in the generlaist model. Denote the improved labeled dataset as $\mathcal{A}_3$, the final controller is then trained with the supervision guidance from $\mathcal{A}_3$. 
% % % a specialist policy for each single trajectory in the initially sampled small dataset, we obtain the first version of the labeled dataset $\mathcal{A}_1$. 


% % \begin{itemize}
% %     \item 
% % \end{itemize}

% % Despite the effectiveness of the above single trajectory specialist policy optimization strategy leveraging RL and the task curriculum, it is infeasible for us to optimizing out a tracking policy for each individual trajectory in the training dataset considering the unaffordable computation and time consumption. Moreover, the task relation modeling may fail to explore valuable cross-trajectory relations when we only have a limited number of labeled data. Therefore the single trajectory optimization may still not that perfect due to the under-explored task relations. To leverage high-quality labeled data for training the tracking controller and to balance the amount of the labeled data with the time consumption, we propose a progressive policy training and labeled data improvement strategy. Specifically, the model is gradually trained via three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing a specialist policy for each single trajectory in the initially sampled small dataset, we obtain the first version of the labeled dataset $\mathcal{A}_1$. After that, the labeled dataset is leveraged to train the tracking controller via the above imitation augmented RL training strategy. With the trained tracking controller, we evaluate it on all training tasks. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories where the weight is positively proportional to the tracking error of the first version policy. The resampled dataset is then labeled via the specialist training. Combining theses optimized trajectories and labeled trajectories in the first stage, we obtain the second version of the labeled dataset $\mathcal{A}_2$. The tracking controller is then trained via the additional supervision provided by $\mathcal{A}_2$. In the third stage, with the re-trained controller, we then construct the task relations space and try to improve the single trajectory optimization results leveraging the task relations space and the knowledge encoded in the generlaist model. Denote the improved labeled dataset as $\mathcal{A}_3$, the final controller is then trained with the supervision guidance from $\mathcal{A}_3$. 




% % \subsection{Structural Cross-Task Synergy Modeling}







% % Following the above specialist policy training strategy, we can optimize a trajectory specific policy the inferred action sequence for each single manipulation trajectory. With such action-labeled trajectories $\mathcal{A}$, we train the generalist policy together with the imitation supervision provided by the action labeled trajectories and the RL. 

% % for each single manipulation trajectory


% % To efficiently optimizing single action-labeled trajectory with minimal hand tuning effort, we wish for a single suit of reward and observation design with which we can effectively optimize for a specialist policy for each single single trajectory. 
% % However, considering the inherent difficulties underlying the dexterous manipulation tracking, the RL algorithm may struggle with tracking some very difficult manipulation trajectories, \textit{e.g.,} with difficult object movements such as subtle re-orientations or involving grasping extremely thin objects. Therefore, we propose to ease the difficult single trajectory optimization problem by transferring knowledge from other trajectories. Specifically, we propose to explore cross-trajectory relations. That is, for each single trajectory that is hard to track, we aim to find its ``parent tasks'' whose optimization results can benefit its optimization. 
% % % employ model-free approach 


% % \textcolor{red}{(TODO: in this paragraph, the focus is how to train the specialist policy -- we can directly use the specialist policy (exactly the term) here )}

% % \subsection{Dexterous Manipulation Tracking via RL and Automatic Task Curriculum}

% % \textcolor{red}{(TODO: move the MDP and the model-free approach training and learning --- the model-free approach, the model unknown assumption, the MDP formulation to the beginning of the paragraph)}
% % % Automatic task
% % Considering the intricate dynamics involved in the dexterous manipulation resulting from the high DoF of a dexterous hand and the rich and changing hand-object contacts, we employ a model-free approach for tackle the problem. 
% % \textcolor{red}{(TODO: add the MDP formulation that frequently appear in other papers)}
% % Given a single kinematic manipulation trajectory $(\mathbf{H}, \mathbf{O})$, the trajectory specific specialist training aims at optimizing a tracking policy $\mathbf{\pi}(\cdot\vert\cdot )$ that can control a dexterous robot hand to track the reference kinematic trajectory. Assuming the physical model is unknown and non-differentiable, we leverage reinforcement learning to optimize the policy. To efficiently optimizing single action-labeled trajectory with minimal hand tuning effort, we wish for a single suit of reward and observation design with which we can effectively optimize for a specialist policy for each single single trajectory. However, considering the inherent difficulties underlying the dexterous manipulation tracking, the RL algorithm may struggle with tracking some very difficult manipulation trajectories, \textit{e.g.,} with difficult object movements such as subtle re-orientations or involving grasping extremely thin objects. Therefore, we propose to ease the difficult single trajectory optimization problem by transferring knowledge from other trajectories. Specifically, we propose to explore cross-trajectory relations. That is, for each single trajectory that is hard to track, we aim to find its ``parent tasks'' whose optimization results can benefit its optimization. \textcolor{red}{(TODO: rephrase this sentence, given xxx , we aim at xxx )}
% % Specifically, we propose a BFS based searching strategy that can automatically explore the trajectory relational space, quantifying relations between each trajectory pair from the datasets. After acquiring cross-trajectory relations, we propose to distill the explored trajectory relational space into a trajectory relational model. The trajectory relational model can then serve as a task relational prior model for providing knowledge w.r.t. cross-trajectory affinities. Then for each hard to track trajectory, we can leverage this model to transform it into a different trajectory, saying  the ``parent trajectory''. By first tracking the ``parent trajectory'' and then optimizing based on the tracked sequence of the parent trajectory, we can better track the original difficult trajectory finally. 



% % \noindent\textbf{Specialist policy training.} Our single trajectory specialist training scheme leverages PPO to optimize for a tracking policy $\mathbf{\pi}(\cdot\vert \cdot)$. The policy takes the current observation, comprising the current hand and object state information and the next frame tracking target as input and output the hand action for the hand to achieve the next state. Specifically, at each timestep $t$, we calculate the observation $\mathbf{o}\mathbf{b}\mathbf{s}_t$ as follows: 
% % \begin{align}
% %     \mathbf{o}\mathbf{b}\mathbf{s}_t = \{ \hat{\mathbf{h}}_t, \hat{\mathbf{o}}_t, \hat{\dot{\mathbf{h}}}_t, \hat{\dot{\mathbf{o}}}_t, \mathbf{f}_t,  \mathbf{h}_{t+1}, \mathbf{o}_{t+1}, \mathbf{h}_{t+1} - \hat{\mathbf{h}}_t, \mathbf{o}_{t+!} \ominus \hat{\mathbf{o}}_t   \}, 
% % \end{align}
% % where $\hat{\mathbf{h}}_t$ and $\hat{\mathbf{o}}_t$ are observed hand joint DoF positions and the object orientation as well as positions at the timestep $t$, $\hat{\dot{\mathbf{h}}}_t$ and $\hat{\dot{\mathbf{o}}}_t$ are hand DoF velocities and object linear as well as angular velocities respectively, $\mathbf{f}_t$ denotes the hand finger positions in the world space, $\mathbf{h}_{t+1}$ and $\mathbf{o}_{t+1}$ are the kinematic targets of the hand DoF positions and the object state in the next timestep. 

% % The reward consists a hand tracking reward $r_{h}$, object tracking reward $r_o$, and the hand-object affinity reward $r_d$. Specifically, xxx 
% % \textcolor{red}{(TODO: add the reward design here)}
% % \textcolor{red}{(TODO: add the residual policy here --- it is important since we need to justify the task curriculum here)}
    
% % % the observation $\mathbf{o}_t$ 


% % % \noindent\textbf{Trajectory relational space exploration via BFS.} 
% % \noindent\textbf{Trajectory relational space exploration and modeling.} 
% % We propose an automatic task curriculum to tackle difficult manipulation trajectories that are hard to track directly. Treating each single trajectory tracking problem as a task, for a tough task, the task curriculum tries to find its affinity tasks and transferring the optimized control trajectories for these tasks as the initialization for the current task to improve the tracking performance. \textcolor{red}{(TODO: add details here)} Such an approach requires us to find affinity tasks, which act as ``parent tasks'' for the current hard to solve problem. The current difficult task should be able to benefit from the optimization results of the ``parent tasks''. It is hard to heuristically define a rule-based criterion such as based on the kinematic similarities or object geometry affinities, that exactly refect such relations. Therefore, we formulate this problem as a trajectory transformation and aim at learning  model $\mathcal{M}_{\mathcal{S}}$ from the trajectory dataset $\mathcal{S}$ to solve it. In detail, given a difficult task, described as a kinematic trajectory $(\mathbf{H}, \mathbf{O})$, we want the model $\mathcal{M}_{\mathcal{S}}$ to transform it to its ``parent task'', described via a kinematic trajectory $(\mathbf{H}^p, \mathbf{O}^p)$ as well. Considering the fact that there may be multiple tasks that can serve as the ``parent task'' for a single difficult task, the trajectory transformation ought to be a stochastic process where $\mathcal{M}_{\mathcal{S}}$ models the distribution of the parent, \textit{i.e.,} $(\mathbf{H}^p, \mathbf{O}^p) \sim \mathcal{M}_{\mathcal{S}}(\cdot\vert (\mathbf{H}, \mathbf{O}))$.

% % To fulfill this vision, we further formulate the learning problem of the model $\mathcal{M}_{\mathcal{S}}$ as a conditional generative model training problem. Specifically, $\mathcal{M}_{\mathcal{S}}$ takes a trajectory $(\mathbf{H}, \mathbf{O})$ as the input and generates its parent tasks. Therefore, we first train a diffusion model to describe the distribution of all kinematic trajectories contained in the dataset $\mathcal{S}$. After that, to acquire data for tuning it to a conditional generative model for the task transformation purpose, we propose a BFS approach to mine such ``parent-child'' paired data from the dataset. Specifically, \textcolor{red}{(TODO: add the description for the BFS part)}




% % % Given a tracking task $(\mathbf{H}, \mathbf{O})$, 
% % % model outhgt to model a distribution of the parent.
% % % we aim at learning a model $\mathcal{M}_{\mathcal{S}}$ from the trajectory dataset $\mathcal{S}$ 
% % % We therefore propose a BFS based approach for mining cross-task relations for constructing the task relational space from the given trajectory dataset $\mathcal{S}$. 
% % % BFS based approach for mining cross-task relations 

% % % the task curriculum tries to fi


% % % \noindent\textbf{Trajectory relation modeling via conditional diffusion.}  

% % % aiming to find ``parent tasks'' 
% % % with difficult object movements such as subtle re-orientations or involving grasping thin objects, 
% % % Considering the vision to efficiently optimizing single action-labeled trajectory with minimal hand tuning effort, we wish for a single suit of reward and observation design for each trajectory. 

% % % For each manipulation reference trajectory, we wish to d


% % % Given the unknown model assumption, we leverage reinforcement learning to optimize the policy. 


% % % For single trajectory specific specialist policy training, 


% % \subsection{General Tracking Policy via Imitation Augmented RL}
% % With the carefully designed specialist policy training strategy and the task relational space exploration and modeling scheme, it is possible for us to optimize for a satisfactory result for each single manipulation trajectory tracking task. However, it is still not enough to acquire a generalist that can not only achieve good performance in each sequence but even generalize to unseen trajectories. Simply following the above RL scheme and training a single policy on multiple tasks is not feasible as demonstrated in our early experiments. As the number of training tasks increases, the RL would even struggle with effectively optimizing a strong policy that can solve every training task, letting alone generalize to unseen trajectories and resolve the novel manipulation sequence tracking challenge. We suppose such pool fitting phenomenon comes from the inherent deficiency of RL in solving multiple tasks. We therefore propose to introduce labeled single trajectory optimization results into the training process of RL, \textit{i.e.,} providing additional action labels as the supervision signals to train the policy together with RL. Specifically, given an action-labeled  dataset $\mathcal{S}_L=\{ (\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L) \}$, where each trajectory is augmented with an additional action sequence $\mathbf{A}$, we add an additional action supervision loss to train the policy together with RL, trying to distill optimized knowledge to the policy. Formally, for each labeled trajectory $(\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L)$, the following action supervised loss is additionally added on the policy's prediction in each timestep $(\mathbf{\mu}_t, \mathbf{\sigma}_t) = \mathbf{\pi}(\cdot \vert \hat{\mathbf{s}}_t)$ to train the policy:
% % % to train the policy $\mathbf{\pi}(\cdot\vert \cdot)$  
% % \begin{align}
% %     \mathcal{L}_a = \Vert \mathbf{\mu}_t -  \mathbf{a}_t \Vert, 
% % \end{align}
% % where $\mathbf{a}_t$ denotes $t-$th step action taken from the optimized action trajectory. This strategy tries to bias the current trajectory towards the optimized successful trajectory in the dataset, in a similar flavor to DART~\citep{laskey2017dart}. 
% % % the action superv ised loss -- 



% % \textcolor{red}{(TODO: pharse it into a specialist-generalist-specialist iteration? )}
% % \noindent\textbf{Progressive generalist model training and labeled dataset improvement.}
% % Despite the effectiveness of the above single trajectory specialist policy optimization strategy leveraging RL and the task curriculum, it is infeasible for us to optimizing out a tracking policy for each individual trajectory in the training dataset considering the unaffordable computation and time consumption. Moreover, the task relation modeling may fail to explore valuable cross trajectory relations when we only have a limited number of labeled data. Therefore the single trajectory optimization may still not that perfect due to the under-explored task relations. To leverage high-quality labeled data for training the generalist policy and to balance the amount of the labeled data with the time consumption, we propose a progressive policy training and labeled data improvement strategy. Specifically, the model is gradually trained via three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing a specialist policy for each single trajectory in the initially sampled small dataset, we obtain the first version of the labeled dataset $\mathcal{A}_1$. After that, the labeled dataset is leveraged to train the generalist policy via the above imitation augmented RL training strategy. With the trained generalist, we evaluate it on all training tasks. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories where the weight is positively proportional to the tracking error of the first version policy. The resampled dataset is then labeled via the specialist training. Combining theses optimized trajectories and labeled trajectories in the first stage, we obtain the second version of the labeled dataset $\mathcal{A}_2$. The generalist is then trained via the additional supervision provided by $\mathcal{A}_2$. In the third stage, with the re-trained generalist, we then construct the task relations space and try to improve the single trajectory optimization results leveraging the task relations space and the knowledge encoded in the generlaist model. Denote the improved labeled dataset as $\mathcal{A}_3$, the final generalist model is then trained with the supervision guidance from $\mathcal{A}_3$. 




% % % maximize the potential benefit of the labeled data for training the generalist tracking policy and to 
% % % To tackle theses issues and 
% % % o fully exploit the potential of leveraging labeled 
% % % have a limited number of labeled dataset
% % % task relation modeling may fail to explore valuable trajectory 




% % % The RL would even struggle to optimize an effective policy that can solve every task when the size of the training task set
% % % us to obtain good result in each single trajectory tracking 


% % % for enhancing the multi-task performance of RL to learn a universal 

% % % each manipulation trajectory 
% % % that can output a physically plausible control sequence $\mathbf{A}$ for each manipulation trajectory $(\mathbf{H}, \mathbf{O})$ which is able to drive a dexterous robot 



==> articles/related.tex <==

% \usepa

\vspace{-10pt}

\section{Related Work}

\vspace{-5pt}

% \noindent\textbf{Dexterous manipulation skill acquisition.} 

Equipping robots with human-level dexterous manipulation skills is crucial for future advancements. Previous approaches either rely on model-based trajectory optimization or model-free reinforcement learning (RL). Model-based methods face challenges due to the complexity of dynamics, often requiring approximations~\citep{pang2023global,Jin2024ComplementarityFreeMM,pang2021convex}. Model-free approaches, using RL~\citep{rajeswaran2017learning,chen2023visual,chen2021system,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact}, focus on goal-driven tasks with task-specific rewards, limiting their generalization across diverse tasks.
% limiting generalization to diverse tasks.
Our work explores a general controller for dexterous manipulations. Besides, learning via mimicking kinematic trajectories has recently become a popular train to equip the agent with various expressive skills~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC,Luo2023UniversalHM}. DTC~\citep{Jenelten2023DTCDT} proposes a strategy that can combine the power of model-based motion planning and RL to overcome the sample inefficiency of RL. 
% overcome the deficiency of the sample inefficiency of RL. 
In the humanoid motion tracking space, PHC~\citep{Luo2023PerpetualHC} proposes an effective RL-based training strategy to develop a general humanoid motion tracker. Recently, OmniGrasp~\citep{Luo2024GraspingDO} proposes to train a universal grasping and trajectory following policy. The policy can generalize to unseen objects as well as track novel motions. However, their considered motions are still restricted in grasping and trajectory following, leaving the problem of tracking more interesting and difficult trajectories such as those with subtle in-hand manipulations largely not explored. In this paper, we focus on these difficult and challenging manipulations. Moreover, we are also related to recent trials on combining RL with imitation learning. To overcome the sample inefficiency problem of RL and to facilitate the convergence, various approaches have been developed aiming to augment RL training with demonstrations~\citep{Sun2018TruncatedHP,Hester2017DeepQF,Booher2024CIMRLCI,Liu2023BlendingIA}. In our work, we wish to leverage high-quality demonstrations to guide the agent's explorations. Unlike previous work where demonstrations are readily available, acquiring a sufficient amount of high-quality robot tracking demonstrations remains a significant challenge in our task.
% Different from previous literature where demonstrations are assumed available, how to acquire abundant high-quality robot tracking demonstrations is a challenging problem in our task. 





% , however, struggle with the complexity of dynamics and often require approximations
% Equipping robots with human-level dexterous manipulation skills is critical for advancing robotics. Previous approaches largely rely on either model-based trajectory optimization or model-free reinforcement learning (RL). Model-based methods face challenges due to the complexity of dynamics, often requiring approximations~\citep{pang2023global,Jin2024ComplementarityFreeMM,pang2021convex}. On the other hand, model-free methods, using RL~\citep{rajeswaran2017learning,chen2023visual,chen2021system,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact}, focus on task-specific rewards, limiting their generalization across diverse tasks. In our work, we aim to develop an agent with versatile manipulation skills. Recently, learning by mimicking kinematic trajectories has gained popularity as a way to equip robots with a wider range of expressive skills~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC,Luo2023UniversalHM}. For instance, DTC~\citep{Jenelten2023DTCDT} presents a hybrid strategy that combines model-based motion planning with RL, addressing RL's sample inefficiency. In humanoid motion tracking, PHC~\citep{Luo2023PerpetualHC} introduces an effective RL-based training approach to develop a generalized humanoid motion tracker. Recently, OmniGrasp~\citep{Luo2024GraspingDO} has trained a universal policy for grasping and trajectory tracking that generalizes to unseen objects and novel motions. However, the motions considered are limited to grasping and trajectory following, with more complex tasks remaining largely unexplored. Our paper focuses on these challenging manipulation tasks. Additionally, we explore the integration of RL with IL to overcome the sample inefficiency problem and enhance convergence. Several methods have been developed to augment RL with demonstrations~\citep{Sun2018TruncatedHP,Hester2017DeepQF,Booher2024CIMRLCI,Liu2023BlendingIA}. Unlike previous work where demonstrations are readily available, acquiring a sufficient amount of high-quality robot tracking demonstrations remains a significant challenge in our task.
% remains a significant challenge


% Recent methods combining RL with motion imitation~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC} enhance expressiveness, yet they focus on simpler motions like grasping. In contrast, we target complex manipulations involving subtle in-hand re-orientations. To improve RL efficiency, imitation learning with demonstrations~\citep{Sun2018TruncatedHP,Liu2023BlendingIA} has been explored, but obtaining high-quality robot tracking demonstrations remains a challenge in our task.

% Equipping an embodied agent with dexterous manipulation skills is a vital step towards a future robot. Previous methods either adopt a model-based trajectory optimization approach or resort to a model-free method aiming to train a policy without assumptions on prior knowledge about the system. Developing a model-based method to solve dexterous manipulation is extremely challenging due to the complexity of the underlying dynamics. Therefore, previous methods would typically develop an approximated model~\citep{pang2023global,Jin2024ComplementarityFreeMM,pang2021convex}. A more popular approach is assuming the system dynamics is unknown and training a policy using advanced reinforcement learning~\citep{rajeswaran2017learning,chen2023visual,chen2021system,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact}. Despite recent promising advances that have been demonstrated in the literature, they typically focus on learning goal-driven skills and require task-specific reward designs~\citep{chen2023visual,chen2021system,rajeswaran2017learning,christen2022d,zhang2023artigrasp,qin2022dexmv}, preventing them from generalizing to a wide range of diverse and novel tasks. In this work, we take a step further and explore the problem of learning a general controller for dexterous manipulations. Besides, learning a controller via mimicking kinematic trajectories has recently become a popular train to equip the controller with various expressive skills~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC,Luo2023UniversalHM}. DTC~\citep{Jenelten2023DTCDT} proposes a strategy that can combine the power of model-based motion planning and RL to overcome the deficiency of the sample inefficiency of RL. In the humanoid motion tracking space, PHC~\citep{Luo2023PerpetualHC} proposes an effective RL-based training strategy to develop a general humanoid motion tracker. Recently, OmniGrasp~\citep{Luo2024GraspingDO} proposes to train a universal grasping and trajectory following policy. The policy can generalize to unseen objects as well as track novel motions. However, their considered motions are still restricted in grasping and trajectory following, leaving the problem of tracking more interesting and difficult trajectories such as those with subtle in-hand re-orientations largely not explored. In this paper, we focus on these difficult and challenging manipulations. Moreover, we are also related to recent trials on combining RL with imitation learning. To overcome the sample inefficiency problem of RL and to facilitate the convergence, various approaches have been developed aiming to augment RL training with demonstrations~\citep{Sun2018TruncatedHP,Hester2017DeepQF,Booher2024CIMRLCI,Liu2023BlendingIA}. In our work, we wish to leverage high-quality demonstrations to guide the agent's explorations. Different from previous literature where demonstrations are assumed available, how to acquire abundant high-quality robot tracking demonstrations is a challenging problem in our task. 
% such as in-hand re-orientation using the hand with a fixed base~\citep{chen2023visual,chen2021system}~\citep{chen2023visual,chen2021system}, grasping, re-locating, relatively simple tool-using~\citep{rajeswaran2017learning,christen2022d,zhang2023artigrasp,qin2022dexmv}, or single manipulation trajectory mimicking~\citep{liu2024quasisim}. 
% Recent trials only learning general skills are still restricted to relatively simple tasks such as grasping~\citep{xu2023unidexgrasp,wan2023unidexgrasp2}. 

% want to take a step further and explore the possibility of learning a general tracking controller that can accomplish a wide range of challenging manipulation tasks. 

% via using planned motions to give dense rewards, and also at the same time keep the robustness of RL in the final controller.

% where RL is leveraged to train a tracking policy with hard mining strategies. 

% action-labeled data is itself a difficult question in our problem. 
% in training a general tracking controller using RL. 
% such as complex tool-using with non-trivial object motions and subtle manipulations using fingers. 
% even the MoCap trajectories that are never seen during the training. 
% Leveraing 
% Training a general tracking 
% Our method is also related 
% \todo{learning from humans? }
% mimicking a diverse range of challenging 
% Although there are recent trails that try to learn general controller, they are still restricted to 
% Althrough there are recent trails on learning general controllers 
% is leveraging a model-free 
% Despite impressive achievements they have demonstrated, 
% a simplified model such as using a relaxed soft contact model~\citep{pang2023global,drake,Jin2024ComplementarityFreeMM}.

% \noindent\textbf{Tracking control.} Learning a controller via mimicking kinematic trajectories has recently become a popular train to equipe the controller with various expressive skills~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC,Luo2023UniversalHM}. DTC~\citep{Jenelten2023DTCDT} proposes a strategy that can combine the power of model-based motion planning and RL to overcome the deficiency of the sample inefficiency of RL via using planned motions to give dense rewards, and also at the same time keep the robustness of RL in the final controller. In the humanoid motion tracking space, PHC~\cite{Luo2023PerpetualHC} proposes an effective training strategy where RL is leveraged to train a tracking policy with hard mining strategies. Recently, OmniGrasp~\citep{Luo2024GraspingDO} proposes to train a universal grasping and trajectory following policy. The policy can generalize to unseen objects as well as track novel motions, even the MoCap trajectories that are never seen during the training. However, the difficulty of their considered motion is still restricted in grasping and trajectory following, leaving the problem of tracking more interesting and difficult trajectories such as those with complex object movements with subtle in-hand re-orientations largely not explored. In this paper, we focus on difficult and challenging manipulations such as complex tool-using with non-trivial object motions and subtle manipulations using fingers. 

% \noindent\textbf{Reinforcement learning with imitation learning.} 
% How to combine RL with imitation learning has attracted lots of attention. To overcome the sample inefficiency problem of RL and to facilitate the convergence, various approaches are developed aiming to augment RL training with demonstrations~\citep{Sun2018TruncatedHP,Hester2017DeepQF,Booher2024CIMRLCI,Liu2023BlendingIA}. In our work, we wish to leverage high-quality offline data to ease the difficulty in training a general tracking controller using RL. Different from previous literature where the labeled dataset is assumed available, how to acquire enough and high-quality action-labeled data is itself a difficult question in our problem. \todo{reifne this para.}
% the training difficulty of RL in solving the 
% the difficulty of training a general tracking controller 
% Despite their achievements, what's a proper way to combine the power of both sides in the dexterous manipulation space remains largely unexplored. Moreover, 

\vspace{-5pt}

==> articles/repro_state.tex <==
\section{Reproducibility Statement}

\noindent \textbf{Novel Models and Algorithms.}
Our method is composed of two novel designs: 
1) The tracking controller training strategy which combines RL and IL. We have provided detailed explanations of the algorithm in Section~\ref{sec:method_il_rl} and Appendix~\ref{sec:supp_method}. Besides, we have included the source code in the Supplementary Materials, where the implementations of the algorithm are contained. Please refer to \emph{Key Implementations} section in the file \emph{DexTrack-Code/README.md} in our Supplementary Materials. 
% The \rep representation. We have provided detailed explanations of the representation in Section~\ref{sec:geneoh} and Appendix~\ref{sec_appen_rep_design}. Besides, we have included the source code in the Supplementary Materials, where the implementations of \rep are contained. Please refer to \emph{Key Implementations} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 
2) The homotopy optimization scheme, the homotopy path searching strategy as well as the homotopy path generator. 
% tracking curriculum and the tracking curricula mining strategy as well as the curriculum scheduler. 
We have provided detailed explanations in Section~\ref{sec:method_data} and Appendix~\ref{sec:supp_method}. Besides, we have included the source code in the Supplementary Materials. Please refer to the \emph{Key Implementations} section in the file \emph{DexTrack-Code/README.md} in our Supplementary Materials. 
3) The iterative optimization approach. We have provided detailed explanations in Section~\ref{sec:method_iteration} and Appendix~\ref{sec:supp_method}.  Besides, we have included the source code in the Supplementary Materials. Please refer to the \emph{Key Implementations} section and \emph{Usage} section in the file \emph{DexTrack-Code/README.md} in our Supplementary Materials. 
% The progressive HOI denoising method. We have provided detailed explanations of the denoising method in Section~\ref{sec:diffusion} and Appendix~\ref{sec_genenoh_diffusion_details}. Model, training, and evaluation details are included in Appendix~\ref{sec_appen_model_details} and~\ref{sec_appen_training_details}. Besides, we have included the source code in the Supplementary Materials. Please refer to the \emph{Key Implementations} section and \emph{Usage} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 

% \noindent \textbf{Theoretical Results.}
% Please refer to section~\ref{sec_appen_rep_design} in the Appendix for the proof of the property of leveraging the stage-wise denoising can clean the noisy input where each stage would not comprise the naturalness achieved after previous denoising stages. 

% \noindent \textbf{Datasets.}
% Please refer to Section~\ref{sec_exp_settings} and Appendix~\ref{sec_appen_datasets} for a detailed explanation of the datasets used. The data preprocessing part can be found in the \emph{Data Preprocessing} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 

\noindent \textbf{Experiments.} 
For experiments, we provide 1) Source code.
Please refer to the folder \emph{DexTrack-Code} in our Supplementary Materials for details. 
2) Experimental details of our method and compared baselines. Please refer to the Section~\ref{sec:exp_setting} and in the Appendix~\ref{sec:supp_exp_details} for details. 
We also provide related information and instructions in the \emph{DexTrack-Code/README.md} file. 


==> articles/teaser_figure.tex <==
\begin{figure}[htbp]
  % \includegraphics[width=\textwidth]{figs/teaser_8.pdf}
  % \includegraphics[width=\textwidth]{figs/teaser_15.pdf}
  \includegraphics[width=\textwidth]{figs/teaser_19.pdf}
  \vspace{-20pt}
  \caption{ \footnotesize
  % By only Training on limited data, 
 %  \href{https://projectwebsite7.github.io/gene-dex-manip/}{
 % \eric{It is very hard to see the teaser figure clearly even after zooming in. The text in the figure should be at least as large as the caption text size. The images are so small and the highlight can hardly be seen even after zooming in by 200\%. The captions should also highlight the key: our neural tracking controller can track diverse and novel human hand object manipulation references once trained.} \modelname}
 % \eric{The figure font size is still much smaller than the caption font size. Please adjust and increase the font size. Also, I think for kinematic references, maybe it is better to show the original human motion? The red circles are highlighting something invisible... We should reduce the number of figures to increase the size of each figure. Please make sure the figure is still visible when printed out using A4 paper.}
 \href{https://projectwebsite7.github.io/gene-dex-manip/}{\modelname} learns a generalizable neural tracking controller for dexterous manipulation from human references. Our neural controller can adeptly generalize to track novel manipulation trajectories with unseen objects, involving difficult interactions with thin objects (\emph{Fig. (a)}), intricate tool-using with intriguing re-orientations (\emph{Fig. (b)}),  exhibits high robustness towards large kinematics noise, and is valuable in real-world applications (\emph{Fig. (c)}). Figures in \textcolor{orange}{orange rectangles} with \textcolor{orange}{orange background} illustrate kinematic references.
 % ~\eric{should use more bold color instead of gray. it is very hard to see the gray rectangles or background.} 
 % with complex movements and 
 % The controller can 
 % various and novel manipulation trajectories involving difficult manipulations with thin objects (\emph{Fig. (a)}), intricate tool-using with complex movements and subtle in-hand re-orientations (\emph{Fig. (b)}),  exhibits high robustness towards large kinematics noise, and is valuable in real-world applications (\emph{Fig. (c)}). Figures in \textcolor{gray}{gray rectangles} with \textcolor{gray}{gray background} illustrate kinematic references. 
 % and out-of-domain (OOD) interactions involving objects from a brand new category (\emph{Fig. (c)}) 
 % The controller can adeptly control a dexterous robot hand to accomplish various challenging manipulations involving novel and difficult manipulations with complex object movements and intricate in-hand re-orientations (\emph{Fig. (a)}), new and challenging object geometries (\emph{Fig. (b)}),  and is robust to large kinematics noise and out-of-domain (OOD) interactions involving objects from a brand new category (\emph{Fig. (c)}). 
 % dexterous manipulation tracking controller from human manipulation references. 
  }
  \vspace{-1pt}
  \label{fig_intro_teaser}
\end{figure}

==> articles_final/exp.tex <==

\vspace{-5pt}
\section{Experiments} \label{sec:exp}
\vspace{-5pt}
% TODO: overview part




% and adaptability 
% We conduct extensive experiments to demonstrate the effectiveness, generalization ability, and robustness, of our tracking controller. We evaluate our method on two HOI datasets containing complex functional daily manipulation featured by difficult trajectories with non-trivial object movements and subtle in-hand re-orientations, challenging object geometries, as well as rich and changing contacts. 
% We train our model in the Isaac Gym environment and conduct evaluations both in the simulator and the real world (see Section~\ref{sec:exp_setting}). We compare strong baselines with dedicated designs for dexterous manipulations to demonstrate the superiority of our method. Our tracking controller can track diverse, difficult, and novel hand-object interactions involving challenging and functional movements, extremely thin objects, as well as rich and changing contacts (see Section~\ref{sec:exp_results}).  However, previous approaches either fail to generalize or behave unsatisfactorily in challenging cases. On average, we can boost the tracking success rate by 10\% from the previously best-performed method. We make further analysis of our method on its robustness and the generalization ability to out-of-distribution test cases (see Section~\ref{sec:exp_analysis}) to illustrate its capability and utility (see Section~\ref{sec:exp_analysis}).  

% We conduct extensive experiments to evaluate the effectiveness, generalization ability, and robustness of our tracking controller. Our method is tested on two HOI datasets featuring complex, functional, daily manipulation tasks. We conduct both through experiments both in the simulation and evaluations in the real world (see Section~\ref{sec:exp_setting}). We compare our method against strong baselines to demonstrate its superiority. Our tracking controller successfully handles novel, difficult, and intriguing manipulations, including those involving intricate functional movements, extremely thin objects, and dynamic contacts (see Section~\ref{sec:exp_results}). In contrast, previous approaches fail to generalize well. On average, our method improves the tracking success rate by more than 10\% over the best prior methods across both datasets. We further analyze our controller's robustness towards significant kinematic noise such as unrealistic states and large penetrations (see Section~\ref{sec:exp_analysis}). 
We conduct extensive experiments to evaluate the effectiveness, generalizability, and robustness of our tracking controller. Tested on two HOI datasets featuring complex daily manipulation tasks, our method is assessed through both simulation and real-world evaluations (see Sec.~\ref{sec:exp_setting}). We compare our approach to strong baselines, showing its superiority. Our controller successfully handles novel manipulations, including intricate movements, thin objects, and dynamic contacts (see Sec.~\ref{sec:exp_results}), while previous methods fail to generalize well. On average, our method improves the tracking success rate by over 10\% compared to the best prior methods. Additionally, we analyze its robustness to significant kinematic noise, such as unrealistic states and large penetrations (see Sec.~\ref{sec:exp_analysis}).
% showcasing its versatility and practical utility.
% , as well as the generalization capabilities towards out-of-distribution test cases (see Section~\ref{sec:exp_analysis}), 
% , specifically designed for dexterous manipulations, 
% Empowered by our proposed training pipeline, we demonstrate that our tracking controller can effectively generalize to novel and challenging interaction trajectories involving unseen object geometry and unobserved manipulations. 
% , demonstrating strong capability and robustness. 


% , which are crucial properties that we expect for a general controller, to demonstrate its capability and utility (see Section~\ref{sec:exp_analysis}). 
% With a single policy, we 





% \textcolor{red}{TODO: track some interesting and long motions?}

\vspace{-10pt}
\subsection{Experimental Settings} \label{sec:exp_setting}
\vspace{-5pt}


% \todo{add the retargeting to the appendix} 

\noindent\textbf{Datasets.}
We test our method on two public human-object interaction  datasets:
% Our dexterous robot hand-object manipulation dataset is built by retargeting two public human-object interaction datasets: 
GRAB~\citep{taheri2020grab}, featuring daily interactions, and 
% single-hand interaction and 
TACO~\citep{liu2024taco}, containing functional tool-use interactions. 
% (single-hand interactions) and TACO~\citep{liu2024taco} (functional tool-use interactions). 
In simulation, we use the Allegro hand, with URDF adapted from IsaacGymEnvs~\citep{makoviychuk2021isaac}, and in real-world experiments, the LEAP hand~\citep{Shaw2023LEAPHL}, due to hardware constraints. Human-object interaction trajectories are retargeted to create robot hand-object sequences using PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. We fully retargeted the GRAB and TACO datasets, producing 1,269 and 2,316 robot hand manipulation sequences, respectively. The evaluation on GRAB focus on testing the model’s generalization to unseen interaction sequences. 
Specifically, we use sequences from subject \texttt{s1} (197 sequences) as the test data while the remaining trajectories as the training set. 
% sequences from subject \texttt{s1} (197 sequences) are used as the test dataset. 
% while the training dataset includes the remaining sequences from other subjects. 
For the TACO dataset, we follow the generalization evaluating setting suggested by the authors~\citep{liu2024taco} and split the dataset into a training set with 1,565 trajectories and four distinct test sets at different difficulty levels. The primary quantitative results are reported on the first-level set. More details are provided in Appendix~\ref{sec:supp_exp_details}. 
% and results are provided in Appendix~\ref{sec:supp_exp_details}. 
% More details on the dataset splitting and our results on remaining test sets are provided in Appendix~\ref{sec:supp_exp_details}. 
% to assess generalization at different levels. 
% evaluation setting suggested by the authors~\citep{liu2024taco}. The dataset is split into a training set with 

% GRAB focuses on testing generalization to unseen sequences, while TACO evaluates generalization across four distinct test sets. More details on dataset splitting and results are provided in Appendix~\ref{sec:supp_exp_details}.

% Our dexterous robot hand-object manipulation dataset is constructed by retargeting two public human-object interaction datasets: GRAB~\citep{taheri2020grab}, which focuses on single-hand interactions with everyday objects, and TACO~\citep{liu2024taco}, which features functional tool-use interactions. For simulation experiments, we use the Allegro hand, while in real-world experiments, the LEAP hand~\citep{Shaw2023LEAPHL} is employed due to constraints in the hardware resources. In simulation, the URDF file for the Allegro hand is adapted from IsaacGymEnvs~\citep{makoviychuk2021isaac}, while the LEAP hand URDF is adapted from dex\_urdf~\citep{bunnyvisionpro}. We retarget human-object interaction (HOI) trajectories to simulated robot hand to create the robot hand-object interaction sequences. We use the forward kinematics implemented in PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024} in the retargeting method. Further details are provided in Appendix~\ref{sec:supp_method}. We fully retargeted the GRAB and released TACO datasets, yielding 1,269 and 2,316 robot hand manipulation sequences, respectively. The GRAB dataset evaluation focuses on testing the model’s generalization to unseen interaction sequences, given the large variations in object geometries. Specifically, sequences from subject \texttt{s1} (197 sequences) are used as the test dataset, while the training dataset includes the remaining sequences from other subjects. For the TACO dataset, we follow the generalization evaluation setting suggested by the authors~\citep{liu2024taco}. The dataset is split into a training set with 1,565 trajectories and four distinct test sets to assess generalization at different levels. The primary quantitative results are reported on the first-level test set. More details on the dataset splitting and our results on remaining test sets are provided in Appendix~\ref{sec:supp_exp_details}. 

% The forward kinematics algorithm in  the retargeting method is
% We describe these hands in simulation using URDF files from dex\_urdf~\citep{bunnyvisionpro} and retarget human-object interaction (HOI) trajectories to both hands, generating corresponding kinematic trajectories through PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. 

% the test set S0. More details on the dataset splitting and visualizations are provided in Appendix~\ref{sec:supp_exp_details}. 
% : 1) S0: Both the tool object geometries and interaction triplets are seen during training; 2) S1: Novel tool geometries, but the interaction triplets are seen during training; 3) S2: Novel interaction triplets, but familiar object categories and geometries; 4) S3: Both object geometries and interaction triplets are novel. The primary quantitative results are reported on the test set S0. More details on the dataset splitting and visualizations are provided in Appendix~\ref{sec:supp_exp_details}. 

% Our dexterous robot hand-object manipulation dataset is created by retargeting two public human-object datasets, namely GRAB~\citep{taheri2020grab}, containing single-hand interactions with daily objects, and TACO~\citep{liu2024taco}, featured by functional tool using interactions. We use simulated Allegro hand in our simulation experiments while LEAP hand~\citep{Shaw2023LEAPHL} in the real world experiments due to the hardware constraints. We use URDF files from dex\_urdf~\citep{bunnyvisionpro} as their descriptions in the simulation. We retarget HOI trajectories to these two hands to create their corresponding kinematic trajectories leveraging PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. 
% For details of the retargeting method that we leverage in our method, please refer to Appendix~\ref{sec:supp_method}. 
% We retarget the full GRAB dataset and the full released TACO dataset, obtaining 1269 and 2316 robot hand manipulation sequences respectively. The evaluation on GRAB mainly aims at testing the model's generalization ability toward unseen interaction sequences considering the large distinctions between their object geometries. Specifically, we use sequences of subject \texttt{s1}, with  197 sequences in total, as the test dataset.  The training dataset is constructed by remaining sequences from other subjects. 
% For the TACO dataset, we create one training set with four distinct test sets with different generalization levels for a detailed evaluation of the model's generalization performance, as suggested by authors~\citep{liu2024taco}. Specifically, the whole dataset is split into a training dataset, containing 1565 trajectories, and the test set S0 where both the tool object geometries and the interaction triplets are seen during training, the test set S1 where the tool geometry is novel but the interaction triplets are seen during training, the test set S2 with novel interaction triplets but seen object categories and geometries, and the test set S4 with new object geometries and interaction triplets. Main quantitative results are reported on the test set S0.  Details w.r.t. the dataset splitting and visualizations are deferred to Appendix~\ref{sec:supp_exp_details}. 
% robot hand manipulation sequences and 2316 sequences
% obtaining 1269 manipulation sequences in total, and the full released TACO data which contains 2316 sequences in total. 
% For TACO dataset, to balance the time consumption and the final data amount, we randomly select 1800 sequences from 2316 sequences in total for retargeting.


% create four different test sets to evaluate the generalization 
% For GRAB, we mainly evaluate the model's generalization ability towards novel interaction sequences considering the large distinctions between their object geometries. For 
% To evaluate the model's generalization capability towards novel manipulation trajectories, we further split them into train and test splits. For the GRAB dataset, we use sequences of the \texttt{subject s1}, with 197 sequences in total, as the test dataset. The train dataset is constructed by remaining sequences from other subjects. For the TACO dataset, we 190 trajectories randomly selected from 1800 sequences for test, while the remaining trajectories as the training data. 
% \todo{unboserved objects? a different splitting method for TACO that considers the object category?}  For evaluating the model's generalization ability towards unseen geometry, we additionally construct a subset from the TACO's training dataset and a subset from TACO's test dataset as a new test split. \todo{details about that}
% For the GRAB datset, although there are existing previous splitting routines~\citep{Zhou2022TOCHSO,Liu2024GeneOHDT}, they mainly focus on cross object generalization. 








% so many todos 
\vspace{-5pt}
\noindent\textbf{Metrics.} 
We introduce five metrics to evaluate the tracking accuracy and task success: 1) Per-frame average object rotation error: \( R_{\text{err}} = \frac{1}{N+1} \sum_{n=0}^N \text{Diff\_Angle}(\mathbf{q}_n, \hat{\mathbf{q}}_n) \), where \( \hat{\mathbf{q}}_n \) and  \( \mathbf{q}_n \)  are reference and tracked orientation.
2) Per-frame average object translation error: \( T_{\text{err}} = \frac{1}{N+1} \sum_{n=0}^N \Vert \mathbf{t}_n - \hat{\mathbf{t}}_n \Vert \), where \( \mathbf{t}_n \) and \( \hat{\mathbf{t}}_n \) are the tracked and reference translations. 3) Per-frame average wrist position and rotation error: \( E_{\text{wrist}} = \frac{1}{N+1} \sum_{n=0}^N \left( 0.5 \, \text{Diff\_Angle}(\mathbf{q}_n^{\text{wrist}}, \hat{\mathbf{q}}_n^{\text{wrist}}) + 0.5 \Vert \mathbf{t}_n^{\text{wrist}} - \hat{\mathbf{t}}_n^{\text{wrist}} \Vert \right) \), where \( \mathbf{q}_n^{\text{wrist}} \) and \( \hat{\mathbf{q}}_n^{\text{wrist}} \) are wrist orientations, and \( \mathbf{t}_n^{\text{wrist}} \) and \( \hat{\mathbf{t}}_n^{\text{wrist}} \) are translations. 4) Per-frame per-joint average position error: \( E_{\text{finger}} = \frac{1}{N+1} \sum_{n=0}^N \left( \frac{1}{d} \Vert \mathbf{\theta}_n^{\text{finger}} - \hat{\mathbf{\theta}}_n^{\text{finger}} \Vert_1 \right) \), where $\mathbf{\theta}$ denotes finger joint positions, \( d \) is the degrees of freedom.
% (16 for both Allegro and LEAP hands).  
% and \( \Vert \cdot \Vert_1 \) denotes the 1-norm. 
5) Success rate: A tracking attempt is successful if \( T_{\text{err}} \), \( R_{\text{err}} \), and \( 0.5E_{\text{wrist}} + 0.5E_{\text{finger}} \) are all below the thresholds. Success is calculated with two thresholds: \( 10\text{cm} \)-\(20^\circ\)-\(0.8\) and \( 10\text{cm} \)-\(40^\circ\)-\(1.2\).
% object tracking quality, hand tracking accuracy, and 
% We introduce five metrics to evaluate the quality of object tracking, hand tracking accuracy, and overall success in the tracking task: 
% 1) Per-frame average object rotation error: $R_{\text{err}} = \frac{1}{N} \sum_{n=1}^N \text{Diff\_Angle}(\mathbf{q}_n, \hat{\mathbf{q}}_n) $, where $\mathbf{q}_n$ is the ground-truth orientation, $\hat{\mathbf{q}}_n$ is the tracked result, represented in quaternion, $\text{Diff\_Angle}(\cdot, \cdot)$ computes the angular difference between two quaternions.
% 2) Per-frame average object translation error: $T_{\text{err}} = \frac{1}{N} \sum_{n=1}^N \Vert \mathbf{t}_n - \hat{\mathbf{t}}_n \Vert$, where $\mathbf{t}_n$ and $\hat{\mathbf{t}}_n$  represent the ground-truth and tracked translations, respectively.
% 3) Per-frame average wrist position and rotation error: $E_{\text{wrist}}=\frac{1}{N}  \sum_{n=1}^N (0.5 \text{Diff\_Angle}(\mathbf{q}_n^{\text{wrist}}, \hat{\mathbf{q}}_n^{\text{wrist}})  + 0.5 \Vert \mathbf{t}_n^{\text{wrist}} - \hat{\mathbf{t}}_n^{\text{wrist}} \Vert )$, where $\mathbf{q}_n^{\text{wrist}}$ and $\hat{\mathbf{q}}_n^{\text{wrist}}$ represent the orientation of the wrist in the reference motion and the tracking result, respectively, while $\mathbf{t}^{\text{wrist}}_n $ and $\hat{\mathbf{t}}_n^{\text{wrist}}$ denote the wrist translation in the reference trajectory and the tracking result, respectively. 
% 4) Per-frame per-joint average position error: 
% $E_{\text{finger}}= \frac{1}{N}  \sum_{n=1}^N (\frac{1}{d} \Vert \mathbf{\theta}_n^{\text{finger}} - \hat{\mathbf{\theta}}_n^{\text{finger}} \Vert_1 )$, where $d$ is the number of degree-of-freedom (DoF) of the dexterous robot hand, \emph{i.e.,} 16 for Allegro hand and the LEAP hand used in our experiments, $\Vert \cdot \Vert_1$ denote the $1$-norm of the vector. 
% 5) Success rate: A tracking attempt is deemed successful if the object translation error $T_{\text{err}}$, object rotation error $R_{\text{err}}$, and the hand tracking error $0.5E_{\text{wrist}} + 0.5E_{\text{finger}}$ are all below their specified thresholds. Success rates are calculated using two thresholds: $10\text{cm}$-$20^\circ$-$0.8$, $10\text{cm}$-$40^\circ$-$1.2$. 

% are smaller than their corresponding threshold. Three success rates are calculated using two different thresholds, namely $10\text{cm}-20^\circ-0.8$, $10\text{cm}-40^\circ-1.2$. 
% a tracking is regarded as successful if the object rotation error object translation error 
% $15\text{cm}-40^\circ-1.6$.


\vspace{-5pt}
\noindent\textbf{Baselines.} 
To our knowledge, no prior model-based methods have directly tackled tracking control for dexterous manipulation. Most existing approaches focus on single goal-driven trajectory optimization with simplified dynamics models~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex}, limiting their adaptability for our framework's generalizable tracking controller. Thus, we primarily compare our method with model-free approaches: 1) DGrasp~\citep{christen2022d}: Adapted to track by dividing sequences into subsequences of 10 frames, with each subsequence solved incrementally. 2) PPO (OmniGrasp rew.): We re-implemented OmniGrasp's reward~\citep{Luo2024GraspingDO} to train a policy for tracking object trajectories. 3) PPO (w/o sup., tracking rew.): We trained a policy using PPO with our proposed tracking reward and observation design.
% To the best of our knowledge, no prior model-based methods have specifically addressed tasks identical or comparable to the tracking control for dexterous manipulation. 
% Most existing approaches are constrained to single goal-driven trajectory optimization~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex} with a simplified dynamics model, making them difficult to adapt for optimizing a versatile tracking controller as required by our framework.
% Therefore, we primarily compare our method against model-free approaches: 1) DGrasp~\citep{christen2022d}: We adapt DGrasp to address the tracking problem by dividing the entire sequence into several subsequences, each consisting of 10 frames. The last frame of each subsequence is defined as its reference frame. This transforms each subsequence tracking task into a solvable problem for DGrasp. We then train a policy to incrementally solve each subproblem. 2) PPO (OmniGrasp rew.): OmniGrasp proposes a universal controller for grasping objects from a table and following the given object trajectory. Since the original implementation has not been open-sourced, we re-implemented the reward as described in the paper~\citep{Luo2024GraspingDO}. Using this reward and PPO, we train a policy aimed at tracking each training trajectory. 3) PPO (w/o sup., tracking rew.): We directly train a policy using PPO and our proposed tracking reward, along with our observation design (see Section~\ref{sec:method_il_rl}). 
% To our best knowledge, there is no previous model-based methods aiming to solve the task same or similar to our dexterous manipulation tracking control. Most of them are restricted in single goal-driven trajectory optimization~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex} which is hard to be adapted to align with our goal of  optimizing a tracking controller.
% which does not and can hardly be adapted to align with our goal in optimizing a tracking controller. 

% Therefore, we mainly compare model-free approaches: 1) DGrasp~\citep{christen2022d}. We adapt DGrasp to solve the tracking problem. We divide the whole sequence into several subsequences with a length of 10 frames. We then define the last frame of each subsequence as its reference frame. After that, each subsequence tracking becomes a problem that DGrasp can solve. We then train a policy to solve each subproblem gradually. 2) PPO (OmniGrasp rew.). OmniGrasp proposes a universal controller for grasping objects from the table and following the given object trajectory. Since it has not been open-sourced yet, we re-implement the reward as described in the paper~\citep{Luo2024GraspingDO}. We then train a policy using the reward and PPO, with the goal of tracking each trajectory in the training dataset. 3) PPO (w/o sup., tracking rew.). We directly train a policy using PPO and our proposed tracking reward as well as the observation design (see Equation~\ref{eq:observations}~\ref{eq:rew_obj}~\ref{eq:rew_hand}~\ref{eq:rew_affinity}). 

% Since in the tracking phase, 

% We re-implement the reward as described in the paper~\citep{Luo2024GraspingDO}. A PPO is trained 
% divide the whole sequence into several subsequences, each of which has 10 frames, and define the end frame of the subsequence as the reference frame. Then the grasping policy is used to guide the hand and gradually track the object according to the hand and the object pose of each reference frame. 
% We compare our method with previous model-free approaches. 
% omni grasp reward o not considerthe 


\vspace{-5pt}
\noindent\textbf{Training and evaluation settings.} 
% The training process involves three stages, each using different tracking demonstrations. 
We use PPO~\citep{Schulman2017ProximalPO}, implemented in {rl\_games}~\citep{rlgames2021}, with Isaac Gym~\citep{makoviychuk2021isaac} for simulation. Training is performed with 8192 parallel environments for both the per-trajectory tracker and the tracking controller. For the dexterous hand, the position gain and damping coefficient are set to 20 and 1 per finger joint. Evaluation results are averaged across 1000 parallel environments, and for real-world evaluations, we use LEAP~\citep{Shaw2023LEAPHL} with a Franka arm and FoundationPose~\citep{Wen2023FoundationPoseU6} for object state estimation. Additional details are provided in Appendix~\ref{sec:supp_exp_details}.
% for the tracking controller 
% without transferring weights between models.
% The training process for the tracking controller consists of three stages, as outlined in the method section. In each stage, we retrain the model using different labeled datasets, without transferring weights from the previous model.  We use PPO~\citep{Schulman2017ProximalPO}, implemented in {rl\_games}~\citep{rlgames2021}, as our reinforcement learning algorithm. Isaac Gym~\citep{makoviychuk2021isaac}, a widely-used simulated physical environment, is utilized for training. We employ 8192 parallel environments to train both the per-trajectory tracker and the tracking controller. For the articulated dexterous hand, the position gain and damping coefficient are set to 20 and 1, respectively, for each finger joint. During the evaluation phase, we average evaluation results obtained in 1000 parallel execution environments as the final result.  For real-world evaluations, we use LEAP~\citep{Shaw2023LEAPHL} with Franka arm. We use FoundationPose~\citep{Wen2023FoundationPoseU6} to estimate the object states. 
% Further details, such as the simulation environment and the real setup, are provided in Appendix~\ref{sec:supp_exp_details}. 
% During the evaluation phase, we sample the policy 1000 times across 1000 parallel execution environments and average the metrics to obtain the evaluation result for the current trajectory. 

% such as the simulation  setup, are provided in Appendix~\ref{sec:supp_exp_details}. 
% including the simulation environment setup, 
% This is because we found that transferring weights makes the model more difficult to train, rather than speeding up the training process.
% The tracking controller training is composed of three stages as we detailed in the method section. In each stage, we re-train the model with different labeled datasets without transferring weights from the previously trained model. It is because we observe that weight transferring would make the model even harder to train, other than accelerating the training process. We leverage PPO~\citep{Schulman2017ProximalPO} implemented in {rl\_games}~\citep{rlgames2021} as our RL algorithm. We use the widely appreciated Isaac Gym~\citep{makoviychuk2021isaac} as the simulated physical environment. We use 8192 parallel environments to train both the per-trajectory tracker and the tracking controller. For articulated dexterous hands, the position gain and the damping coefficient are set to 20 and 1 respectively for each finger joint. During the evaluation phase, we sample from the policy 1000 times (using 1000 parallel execution environments) and average their metrics as the evaluation result of the current trajectory. More details such as the simulation environment setting are deferred to Appendix~\ref{sec:supp_exp_details}. 
% For both the per-trajectory tracker and the tracking controller, 
% the single trajectory specialist tracking policy training and the general tracking policy optimization, we use 8192 parallel environments to train RL. 






% take the widely appreciated Isaac Gym as our simulated environment where we train our 


% rich and changing contacts, j
\vspace{-5pt}
% \subsection{Generalizable Dexterous Manipulation Tracking Control } \label{sec:exp_results}
\subsection{Generalizable Tracking Control for Dexteroous Manipulation } \label{sec:exp_results}
\vspace{-5pt}


% \todo{add the time consumption}

\begin{figure}[ht]
  \centering
  \vspace{-10pt}
  \includegraphics[width=\textwidth]{figs/robustness_noise.pdf}
  \vspace{-20pt}
  \caption{\footnotesize
  \textbf{Robustness w.r.t. unreasonable states. }
  Please check \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{video}}}} for animated results.
  % ~\eric{the subsection title has been occluded by the figure... please adjust.}
  }
  \label{fig_res_robustness}
  \vspace{-10pt}
\end{figure}

% \todo{change the w/o prior, w/o curri. to w/o data, w/o structure}

\begin{figure}[ht]
  \centering
  % \vspace{-10pt}
  % \includegraphics[width=\textwidth]{figs/res_5.pdf}
  \includegraphics[width=\textwidth]{figs/eval_res_all_v2_compressed.pdf}
  % \vspace{-20pt}
  \caption{\footnotesize
  \textbf{Qualitative comparisons. }
  Please check \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
  }
  \label{fig_res}
  \vspace{-10pt}
\end{figure}




% \begin{table*}[t]
%     \centering
%     \caption{ 
%     \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
%     } 
%     % \vspace{-10pt}
%     \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{@{\;}llccccc@{\;}}
%         \toprule
%         %         
%         Dataset & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

        
%         \cmidrule(l{0pt}r{1pt}){1-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}

%         % \multirow{5}{*}{ GRAB } & ControlVAE & - & -  & -  & - 
%         % \\ 
%         % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         % \\ 
%         % % \cmidrule(l{15pt}r{17pt}){3-9}

%         % % \cmidrule(l{15pt}r{17pt}){3-9}
%         % \cmidrule(l{1pt}r{1pt}){2-3}
%         % % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         \multirow{2}{*}{ GRAB } & DGrasp & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (w/o sup., tracking rew.)  & 0.3945 & 6.11  & 0.1076 & 0.5899 & 38.78/55.05/60.58 
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){2-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}
        
        
%         % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         % \\ 
%         ~ & \model~(w/ sup.)  & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         \\ 
%         ~ & \model~(w/ sup., w/ curriculum)  & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         \\ 
%         ~ & \model  & \bred{0.3303} & \bred{4.53} & {0.1118} & \bred{0.5048} & \bred{47.12}/\bred{65.52}/\bred{72.41}
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){1-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}


%         % \multirow{5}{*}{ TACO } & ControlVAE & - & -  & -  & - 
%         % \\ 
%         % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         % \\ 
%         % % \cmidrule(l{15pt}r{17pt}){3-9}

%         % % \cmidrule(l{15pt}r{17pt}){3-9}
%         % \cmidrule(l{1pt}r{1pt}){2-3}
%         % % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
%         % \\ 

%         \multirow{2}{*}{ TACO } & DGrasp & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (Tracking rew.)  & 0.4815 & 7.82  & 0.1195  & 0.4682 & {35.13}/{47.69}/61.54
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){2-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}
%         % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
%         % \\ 
%         ~ & \model~(w/ sup.)  &  0.4444 & 2.33  & 0.1782  & 0.5438 & 47.97/67.12/73.66
%         \\ 
%         ~ & \model~(w/ sup., w/ curriculum)  & {0.4854} & {1.99} & { 0.1298} & {0.4772} & 54.90/72.55/79.74
%         \\ 
%         ~ & \model & {0.4953} &  {2.10} & {0.1510} & {0.4661} & \bred{49.02}/\bred{74.50}/\bred{81.05}
%         \\ 

%         \bottomrule
 
%     \end{tabular}
%     }
%     \vspace{-10pt}
%     \label{tb_exp_main}
% \end{table*} 




% \todo{change the w/o prior, w/o curri. to w/o data, w/o structure}
\begin{table*}[t]
    \centering
    \caption{ 
    \footnotesize
    \textcolor{myblue}{\textbf{Quantitative evaluations.}}  \bred{Bold red} and \iblue{italic blue} \textcolor{myblue}{values for best and the second best-performed ones respectively}. 
    \textcolor{myblue}{``Ours (w/o) data'' and ``Ours (w/o data, w/o homotopy)'' are two ablated versions w.r.t. quality of robot tracking demonstrations used in imitation learning (see Section~\ref{sec:ablation_studies} for details). }
    % Demonstrations used in ``Ours (w/o) data'' are not improved by 
    % ``Ours (w/o) data'' uses demonstrations that are not improved by transferring ``tracking prior'', while ``Ours (w/o data, w/o homotopy)'' uses demonstrations neither improved by transferring tracking prior nor via the homotopy optimization scheme.
    % is the ablated version where demonstrations are curated without transferring ``tracking prior'', while ``Ours (w/o data, w/o homotopy)'' uses demonstrations neither improved by transferring tracking prior nor via the homotopy optimization scheme.}
    % numbers for best values and  for the second best-performed ones. 
    } 
    % \vspace{-10pt}
    \resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{\;}llccccc@{\;}}
        \toprule
        %         
        Dataset & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$) \\

        
        \cmidrule(l{0pt}r{1pt}){1-2}
        \cmidrule(l{2pt}r{2pt}){3-7}

        

        % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
        % \\ 
        \multirow{6}{*}{ GRAB } & DGrasp & 0.4493 & 6.75  & 0.1372  & 0.6039 & 34.52/52.79
        \\ 
        ~ & PPO (OmniGrasp rew.) & 0.4404 & 6.69  & 0.1722 & 0.6418  & 35.53/54.82
        \\ 
        ~ & PPO (w/o sup., tracking rew.)  & 0.3945 & 6.11  & \bred{0.1076} & 0.5899 & 38.58/54.82 % & 
        \\ 
        
        \cmidrule(l{0pt}r{1pt}){2-2}
        \cmidrule(l{2pt}r{2pt}){3-7}
        
        
        % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
        % \\ 
        % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
        % \\ 
        ~ & \model~(w/o data, w/o homotopy)  & {0.3443} & {7.81} & {0.1225} & \iblue{0.5218} & 39.59/57.87 
        \\ 
        ~ & \model~(w/o data)  & \iblue{0.3415} & \iblue{4.97} & { 0.1483} & {0.5264} & \iblue{43.15}/\iblue{62.44} % 
        \\ 
        ~ & \model  & \bred{0.3303} & \bred{4.53} & \iblue{0.1118} & \bred{0.5048} & \bred{46.70}/\bred{65.48} 
         \\ 
        
        \cmidrule(l{0pt}r{1pt}){1-2}
        \cmidrule(l{2pt}r{2pt}){3-7}


        % \multirow{5}{*}{ TACO } & ControlVAE & - & -  & -  & - 
        % \\ 
        % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
        % \\ 
        % % \cmidrule(l{15pt}r{17pt}){3-9}

        % % \cmidrule(l{15pt}r{17pt}){3-9}
        % \cmidrule(l{1pt}r{1pt}){2-3}
        % % \cmidrule(l{2pt}r{2pt}){8-12}


        % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
        % \\ 
        % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
        % \\ 
        % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
        % \\ 

        \multirow{6}{*}{ TACO } & DGrasp & 0.5021 & 5.04  & \bred{0.1129}  &  0.4737 & 38.42/47.78
        \\ 
        ~ & PPO (OmniGrasp rew.) & 0.5174 & 5.43  & 0.1279  & 0.4945 & 33.5/46.31
        \\ 
        ~ & PPO (w/o sup., tracking rew.)  & \iblue{0.4815} & 4.82  & \iblue{0.1195}  & \iblue{0.4682} & {34.98}/{57.64} 
        \\ 
        
        \cmidrule(l{0pt}r{1pt}){2-2}
        \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){8-12}
        % \cmidrule(l{2pt}r{2pt}){1-2}
        % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
        % \\ 
        % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
        % \\ 
        ~ & \model~(w/o data, w/o homotopy)  &  \bred{0.4444} & 2.33  & 0.1782  & 0.5438 & 44.83/67.00
        \\ 
        ~ & \model~(w/o data)  & {0.4854} & \iblue{2.21} & { 0.1698} & {0.4772} & \iblue{47.78}/\iblue{72.41}
        \\  
        ~ & \model & {0.4953} &  \bred{2.10} & {0.1510} & \bred{0.4661} & \bred{48.77}/\bred{74.38}
        \\ 

        \bottomrule
 
    \end{tabular}
    }
    \vspace{-10pt}
    \label{tb_exp_main}
\end{table*} 


% \todo{do not claim the efficiency and jmove the timeconsumption to the appendix}



% \begin{table*}[t]
%     \centering
%     \caption{ 
%     \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
%     } 
%     % \vspace{-10pt}
%     \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{@{\;}lllccccc@{\;}}
%         \toprule
%         %         
%         Dataset & ~ & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

        
%         \cmidrule(l{0pt}r{1pt}){1-3}
%         \cmidrule(l{2pt}r{2pt}){4-8}

%         \multirow{5}{*}{ GRAB } & \multirow{2}{*}{ \makecell[c]{Model \\ Based} } & ControlVAE & - & -  & -  & - 
%         \\ 
%         ~ & ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         \\ 
%         % \cmidrule(l{15pt}r{17pt}){3-9}

%         % \cmidrule(l{15pt}r{17pt}){3-9}
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         ~ & \multirow{2}{*}{ \makecell[c]{Model \\ Free} }  & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & ~ & PPO (Tracking rew.)  & 0.3945 & 6.11  & 0.1076 & 0.5899 & 38.78/55.05/60.58 
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}

%         % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         % \\ 
%         ~ & ~ & Ours  & \bred{0.3303} & \bred{4.53} & {0.1118} & \bred{0.5048} & \bred{47.12}/\bred{65.52}/\bred{72.41}
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){1-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}


%         \multirow{5}{*}{ TACO } & \multirow{2}{*}{ \makecell[c]{Model \\ Based} } & ControlVAE & - & -  & -  & - 
%         \\ 
%         ~ & ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         \\ 
%         % \cmidrule(l{15pt}r{17pt}){3-9}

%         % \cmidrule(l{15pt}r{17pt}){3-9}
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
%         % \\ 

%         ~ & \multirow{2}{*}{ \makecell[c]{Model \\ Free} }  & PPO (OmniGrasp rew.) & - & -  & -  & - 
%         \\ 
%         ~ & ~ & PPO (Tracking rew.)  & 0.4815 & 10.11  & 0.1195  & 0.4682 & {5.13}/{5.13}/61.54
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}
%         % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
%         % \\ 
%         ~ & ~ & Ours & {0.4953} &  {2.10} & {0.1510} & {0.4661} & \bred{49.02}/\bred{74.50}/\bred{81.05}
%         \\ 

%         \bottomrule
 
%     \end{tabular}
%     }
%     \vspace{-10pt}
%     \label{tb_exp_main}
% \end{table*} 




% \begin{figure}[h]
%   \centering
%   % \vspace{-10pt}
%   \includegraphics[width=\textwidth]{figs/res.pdf}
%   % \vspace{-20pt}
%   \caption{
%   \textbf{Qualitative comparisons. }
%   Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig_res_bak}
%   % \vspace{-10pt}
% \end{figure}




% \begin{wraptable}[6]{r}{0.5\textwidth}
% \vspace{-30pt}
%     \centering
%     \caption{ 
%     % \textbf{Ablation studies} on the GRAB dataset. 
%     Total training time consumption (GRAB dataset). 
%     } 
%     % \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccc@{\;}}
%         \toprule
%         ~ & \makecell[c]{PPO \\ (w/o sup)} & \makecell[c]{Ours \\ (w/ sup.)}  & \makecell[c]{Ours \\ (w/ sup., \\ w/ curri.)} & Ours   \\

%         \midrule % 

%         Time  &  $\sim$1 day & $\sim$4.5 days & $\sim$9 days & $\sim$5 days
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_exp_timeconsumption}
% \end{wraptable}





% decompose 

% \todo{which card and the hardware settings}

% We demonstrate the generalization ability of our tracking controller to unseen trajectories involving difficult manipulations and novel, thin objects. Our controller has no difficulty in dealing with very intricate motions involving thin objects, subtle in-hand re-orientations, and expressive functional manipulations. As presented in Table~\ref{tb_exp_main}, we can achieve significantly higher success rates calculated under two thresholds than the best-performed baseline in both two datasets. Figure~\ref{fig_res} illustrates qualitative examples and comparisons. Please check out our website and video for animated results. 
We demonstrate the generalization ability and robustness of our tracking controller on unseen trajectories involving challenging manipulations and novel, thin objects. Our controller has no difficulty in handling intricate motions, subtle in-hand re-orientations, and expressive functional manipulations, even when dealing with thin objects. 
As shown in Table~\ref{tb_exp_main}, we achieve significantly higher success rates, calculated under two different thresholds, compared to the best-performing baseline across both datasets. Figure~\ref{fig_res} provides qualitative examples and comparisons. We show the real-world effectiveness of our method and the superiority over best-performing baselines (Figure~\ref{fig_res},Table~\ref{tb_real_world_results}). For animated results, please visit our \href{https://projectwebsite7.github.io/gene-dex-manip/}{project website} and the \href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{accompanying video}.
% in two HOI datasets. Empowered by xxx, our policy can generalize well and robustly track challenging manipulations unseen during training. Most impressively and perhaps even surprising to us, our policy has no difficulty in dealing with very intricate motions involving thin objects, subtle in-hand re-orientations, and expressive functional manipulations. 



% \textcolor{red}{(TODO: cross-object generalization test? and that should be delivered in a small table)}


% \noindent\textbf{Expressive and functional motions with subtle in-hand re-orientations.} 

\noindent\textbf{Intriguing in-hand manipulations.}
% Expressive motions with s
% ubtle in-hand manipulations.} 
Our method effectively generalizes to novel, complex, and challenging functional manipulations, featured by subtle in-hand re-orientations, essential for precise tool-use tasks. For instance, in Figure~\ref{fig_res}a, the shovel is lifted, tilted, and reoriented with intricate finger movements to complete a {stirring} motion. Similarly, in Figure~\ref{fig_res}c, the small shovel is reoriented using minimal wrist adjustments. These results demonstrate the robustness and generalization of our controller, outperforming the PPO baseline, which struggles with basic lifting. 
% tasks like lifting thin tools.
% including
% complex object movements and 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method effectively generalizes to unseen, challenging manipulations that involve complex functional object movements and subtle in-hand re-orientations, which are crucial for achieving precise reorientations during tool-use tasks. For example, in Figure~\ref{fig_res}a, the shovel must first be lifted with the inner side facing down, then tilted so the inner part faces upward, while the fingers control the handle to complete a \texttt{stirring} motion. Our results nearly achieve this goal, despite the intricate finger movements required to re-orient the object.
% In Figure~\ref{fig_res}c, the trajectory demands that the small shovel be re-oriented to face right so it can be used to hold things. Although our method initially lifts the shovel with the inner side facing left (as shown in the third frame), it successfully re-orients the tool using detailed finger adjustments, with minimal change in wrist orientation (as shown in the fourth frame).
% These results highlight the robust performance and exceptional generalization ability of our controller. In contrast, the best-performing baseline, PPO (w/o sup.), which attempts to train a general controller using our designed rewards, struggles even with basic tasks like lifting thin tools from the table.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalizes well to unseen challenging manipulations involving complex functional object movements, and detailed and subtle in-hand re-orientations that are crucial to achieve correct orientations for accurately mimicking tool-using motions. In Figure~\ref{fig_res}a, the shovel should be lifted at first with the inner side facing towards and then tiled down with the inner part facing upwards and fingers controlling the handle to complete the \texttt{stirring} motion. Our results can almost fulfill the goal despite the need to use detailed finger movements to re-orient the object. As demonstrated in Figure~\ref{fig_res}c, the trajectory requires the hand to make the small shovel face towards the right side so that it can use it to hold things. Despite the fact that our method manage to lift the object up from the table with the object facing towards the left side (shown in the third frame), it can then successfully re-orient the small shovel so that it faces towards the right side mainly using fingers without varying the wrist orientation a lot (as shown in the forth frame). 
% These great performance convincingly demonstrate the strong capability and notable generalization ability of our controller. 
% In comparison to ours' adeptly tracking functional interactions, the best-performed baseline PPO (w/o sup.), which attempts to directly train a general controller using PPO with our carefully designed rewards but without additional guidance, even faces challenges in lifting such thin tools up from the table. 
% However xxx (baseline methods). \todo{baseline's performance}
% Such tool using method demonstrates the high generalizable dexterity enabled by our general tracker. 



% \begin{wraptable}[5]{r}{0.6\textwidth}
% \vspace{-23pt}
%     \centering
%     \caption{ 
%     % \textbf{Ablation studies} on the GRAB dataset. 
%     % \textbf{Generalization ability evaluations} on the TACO dataset. 
%     % \textbf{Gen} on the TACO dataset. 
%     \footnotesize
%     Generalizability evaluations on the TACO dataset. 
%     } 
%     \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{@{\;}lccccc@{\;}}
%         \toprule
%         Test set & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

%         % \\
%         \midrule % 


%         % \\
%         % \cmidrule(l{15pt}r{17pt}){2-4}
        
%         % \model (w/o SpatialDiff) & 2.94 & 3.45  & 31.67
%         % \\ 

%         % \model (w/o TemporalDiff) & \bred{1.72} & \bred{1.90} & 34.25 % 18.65 %
%         % \\

%         % \model (w/o Diffusion) & 3.16 & 3.83  & 18.65 

%         % S0 & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\
        
%         S1 & 0.5787 & {2.43} & {0.1481} & {0.4703} & 35.97/67.63
%         \\ 

%         % 
%         % \model (w/o Canon.) & {2.36} & {3.57} & \iblue{13.26}
%         S2 & {0.6026} & {2.46} & { 0.1455} & {0.4709} & 30.83/65.00
%         \\ 

%         S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % }
%     % \vspace{-16pt}
%     \label{tb_exp_taco_generalization_test}
% \end{wraptable}



\noindent\textbf{Intricate manipulations with thin objects. } 
Our method also generalizes well to challenging manipulations involving thin objects. In Figure~\ref{fig_res}b, despite the thin \texttt{shovel}'s complexity and missing CAD model parts, our method successfully lifts and controls it using a firm grasp with the second and third fingers. Similarly, in Figure~\ref{fig_res}e, our controller adeptly lifts and manipulates a thin \texttt{flute}, while the best-performing baseline struggles with the initial grasp. These results highlight the advantages of our approach in handling complex and delicate manipulations.
% that are difficult to grasp and control. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalizes effectively to unseen, challenging manipulations involving extremely thin objects that are both difficult to grasp and control. As shown in Figure~\ref{fig_res}b, the shovel is extremely thin, with some triangles missing from the CAD model, which adds to the complexity. Additionally, controlling such a long and thin object from the end further increases the difficulty. Despite these challenges, our method performs well, successfully lifting the object using the second and third fingers while maintaining a firm grip to follow the trajectory, even with this unconventional grasping pose.
% In the scenario depicted in Figure~\ref{fig_res}e, the task involves lifting a notably thin flute from the table and manipulating it. Our controller demonstrates remarkable proficiency in interacting with such objects. In contrast, the best-performing baseline struggles significantly during the initial grasping phase, highlighting the advantages of our approach in handling complex and delicate manipulations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalize well to unseen challenging manipulations involving extremely thin objects that are both difficult to grasp and control. As demonstrated in Figure~\ref{fig_res}b, the shovel is very thin here even with some triangles missing from the CAD model. Besides, controlling such a long and thin object from the end side further adds huge difficulties. Despite such challenges, our method can still generalize well and achieve good performance in this case. It manages to lift the object up using the second and the third fingers and control the hand to firmly hold the objects to follow its trajectory, using this unfriendly grasping pose. 
% In the case drawn in Figure~\ref{fig_res}f, the challenging task involves lifting an extremely thin flute from the table and playing with it. Our controller has no difficulty in interacting with this kind of object. 
% In comparison, the best-performed baseline faces significant challenges in the initial grasping stage. 
% Our controller can even perform robustly in this unfriendly grasping pose, controlling the hand to firmly hold the object and follow its trajectory. 

% complex object movements, extremely thin objects that are very difficult to grasp
% has no difficult in resolving challenging manipulation

% \begin{wrapfigure}[6]{r}{0.45\textwidth} % {0pt}
% \vspace{-4ex}
% \includegraphics[width = 0.45\textwidth]{./figs/real_eval_figs.pdf}
% \vspace{-24pt}
%     \caption{\footnotesize
%     Qualitative results in the real world.
%     }
%     \label{fig:fig_real_eval_figs}
% \vspace{-20pt}
% \end{wrapfigure}


% \todo{add this part}







\begin{table*}[t]
    \centering
    \caption{ \footnotesize
    \textbf{Real-world quantitative comparisons.}  \bred{Bold red} numbers for best values.
    % and \iblue{italic blue} values for the second best-performed ones. 
    } 
    % \vspace{-10pt}
        \resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{\;}lcccccccccc@{\;}}
        \toprule
       Method & \texttt{apple} & \texttt{banana} & \texttt{duck}  & \texttt{elephant} & \texttt{flashlight}    & \texttt{flute}   & \texttt{hammer}  & \texttt{hand}  & \texttt{phone}  & \texttt{waterbottle}     \\

        % \\
        \midrule % 

        PPO (w/o sup., tracking rew) & 0/0/0 & 25.0/25.0/0.0 & 50.0/25.0/0 & 50.0/0.0/0.0 & 50.0/0/0 & 0/0/0 & 25.0/0/0 & 66.7/33.3/0 & 25.0/0/0 & 33.3/33.3/0
        \\ 

        % 
        \model & \bred{25.0}/0/0 & \bred{50.0}/\bred{50.0}/\bred{25.0} & \bred{75.0}/\bred{50.0}/\bred{25.0} & \bred{75.0}/\bred{50.0}/\bred{50.0} & \bred{50.0}/\bred{25.0}/\bred{25.0}  & \bred{25.0}/\bred{25.0}/\bred{25.0} & \bred{50.0}/\bred{50.0}/\bred{50.0} & \bred{66.7}/\bred{33.3}/\bred{33.3} & \bred{50.0}/\bred{50.0}/\bred{25.0} & \bred{50.0}/\bred{33.3}/\bred{33.3} 
        \\ 

        % S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
        % \\ 
        
        \bottomrule
 
    \end{tabular}
    }
    \vspace{-20pt}
    \label{tb_real_world_results}
\end{table*} 

% % \begin{wraptable}[5]{r}{0.6\textwidth}
% \begin{table*}[t]
% \vspace{-23pt}
%     \centering
%     \caption{ 
%     \footnotesize
%     Generalizability evaluations on the TACO dataset. 
%     } 
%     \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccccccccc@{\;}}
%         \toprule
%        Method & apple & banana & duck  & elephant & flashlight    & flute   & hammer  & hand  & phone  & waterbottle     \\

%         % \\
%         \midrule % 

        
%         PPO (w/o sup., tracking rew) & 0.5787 & {2.43} & {0.1481} & {0.4703} & 35.97/67.63
%         \\ 

%         % 
%         % \model (w/o Canon.) & {2.36} & {3.57} & \iblue{13.26}
%         \model & {0.6026} & {2.46} & { 0.1455} & {0.4709} & 30.83/65.00
%         % \\ 

%         % S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
%         % \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_real_world_results}
% % \end{wraptable}
% \end{table*}


% \begin{figure}[ht]
%   \centering
%   \vspace{-10pt}
%   \includegraphics[width=0.8\textwidth]{figs/real_exp_cmp_3.pdf}
%   \vspace{-20pt}
%   \caption{\footnotesize
%   \textbf{Qualitative real-world evaluations and comparisons. }
%   % Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig:fig_real_eval_figs}
%   \vspace{-10pt}
% \end{figure}
% \vspace{-5pt}

\noindent\textbf{Real-world evaluations and comparisons.} 
% We transfer tracking results directly to the real world to assess tracking quality and also transfer the state-based controller to evaluate its robustness to noises in the state estimator. Success rates are measured under three thresholds and compared with the best baseline. Table~\ref{tb_real_world_results} summarizes per-object success rates averaged over their manipulation trajectories (transferred controller setting). Demonstrated in Figure~\ref{fig_res}f~\ref{fig_res}g, we enable the robot to track complex object movements in real-world scenarios. Further details are in Appendix~\ref{sec:supp_real_world}.
We directly transfer tracking results to the real world to assess tracking quality and evaluate the robustness of the state-based controller against noise in the state estimator. Success rates are measured under three thresholds and compared with the best baseline. Table~\ref{tb_real_world_results} summarizes the per-object success rates averaged over their manipulation trajectories in the transferred controller setting. As demonstrated in Figures~\ref{fig_res}f and \ref{fig_res}g, we enable the robot to track complex object movements and successfully lift a hard-to-grasp round apple in real-world scenarios. While the baseline fails. Further details can be found in Appendix~\ref{sec:supp_real_world}.

% We transfer tracking results directly to the real world to assess tracking quality and evaluate the robustness of the state-based tracker to noise in the state estimator. We measure success rates under three success thresholds for both settings and compare them with the best-performing baseline. Table~\ref{tb_real_world_results} summarizes the performance of the transferred tracker. We report per-object success rates averaged over their corresponding manipulation trajectories. As shown in Figure~\ref{fig_res}f,g, our method enables the robot to successfully track complex object movements in real-world scenarios. Additional details and results are provided in Appendix~\ref{sec:supp_real_world}.
% reports the 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We directly transfer tracking results to the real world to demonstrate the tracking quality and also transfer the state-based tracker to the real world to evaluate its robustness to noises in the state estimator. We evaluate the success rate under three types of success thresholds for both settings and compare it with the best-performed baseline method. Values reported in Table~\ref{tb_real_world_results} are the per-object success rate averaged over their corresponding manipulation trajectories, achieved via the transferred tracker. As shown in Figure~\ref{fig_res}f,g, our results executed in the real world can successfully let the robot track difficult manipulations with complex object movements. More details and results are deferred to the Appendix~\ref{sec:supp_real_world}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% success rate of each object averaged over the number of manipulation trajectories, 
% and evaluate the success rate. Moreover, we also transfer the state-based tracker to the real world to evaluate its robustness to noises in the state estimator. 




\vspace{-10pt}
\subsection{Further Analysis and Discussions} \label{sec:exp_analysis}
\vspace{-5pt}


\noindent\textbf{Robustness to noise in the kinematic reference motions.} 
% Our method is robust to significant kinematic noise. 
Despite severe hand-object penetrations in Figure~\ref{fig_res}c (frames 2 and 3) and Figure~\ref{fig_res}a (frame 2), the hand still interacts effectively with the object, highlighting the resilience of our tracking controller in challenging scenarios.
% Our method is robust to significant noise in the kinematic motions. For example, even with severe hand-object penetrations occurring in the motions depicted in Figure~\ref{fig_res}c (in the second and third frames) and Figure~\ref{fig_res}a (in the second frame), we can still effectively control the hand to interact correctly with the object. This resilience underscores the effectiveness of our tracking controller in handling challenging scenarios.
% We would not be affected by obvious noise in the kinematic motions. For instance, although there are severe hand-object penetrations in the motion shown in Figure~\ref{fig_res}c (the second and the third frame) and Figure~\ref{fig_res}a (the second frame), we can successfully control the hand to correctly interact with the object. 



% \begin{figure}[ht]
%   \centering
%   \vspace{-10pt}
%   \includegraphics[width=\textwidth]{figs/robustness_2.pdf}
%   \vspace{-20pt}
%   \caption{
%   \textbf{Robustness towards unreasonable references and novel object categories. }
%   Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig_res_robustness}
%   \vspace{-10pt}
% \end{figure}





\noindent\textbf{Robustness to unreasonable references. }
As shown in Figure~\ref{fig_res_robustness}, our method remains unaffected by significant noise in the kinematic references with unreasonable states.
% , even when they include unreasonable or unreachable states.
We effectively track the entire motion trajectory, demonstrating the controller's robustness in handling unexpected noise.
% As shown in Figure~\ref{fig_res_robustness}a, our method remains unaffected by significant noise in the kinematic references, even when they include unreasonable or unreachable states. We can effectively track the entire motion trajectory despite these challenges, demonstrating our controller's robustness in handling unexpected noise. 
% The kinematic reference trajectory is obtained by interpolating a different trajectory from the TACO dataset, demonstrating our controller's robustness in handling complex and noisy inputs.
% As demonstrated in Figure~\ref{fig_res_robustness}a, we would not be affected by the large noise in the kinematics references containing unreasonable and unreachable states and can still manage to track the whole motion trajectory. The kinematic reference trajectory is obtained by interpolating a different trajectory with a sequence from TACO. 
% \todo{xxx}




% \noindent\textbf{Further generalization ability evaluations.}
% We further evaluate the model's generalization ability across various test sets within the TACO dataset. As shown in Table~\ref{tb_exp_taco_generalization_test}, the controller performs well in the category-level generalization setting (S1), where object categories are known but manipulation trajectories and object geometries are novel. Performance on S2, involving novel interaction triplets, is satisfactory, demonstrating the controller's capacity to handle new manipulation sequences. However, results from S3 reveal challenges when dealing with new object categories and unseen interaction triplets. For instance, generalizing from interactions with shovels and spoons to using bowls for holding objects is particularly difficult. As shown in Figure~\ref{fig_res_robustness}b, despite unfamiliar objects and interactions, we successfully lift the knife and mimic the motion, though execution is imperfect, highlighting areas for improvement and adaptability in challenging scenarios.

% We further evaluate the model's generalization ability across different levels of test sets within the TACO dataset. As shown in Table~\ref{tb_exp_taco_generalization_test}, the controller performs well in the category-level generalization setting, where the object category is known during training, but the manipulation trajectories and object geometries are novel, as evidenced by its strong performance on test set S1.
% The performance on S2, which involves novel interaction triplets, remains relatively satisfactory, demonstrating the controller's capacity to generalize to new manipulation sequences. However, results from S3 highlight the challenges faced when dealing with novel object categories and unseen interaction triplets. For instance, generalizing from interactions that involve lifting and waving shovels and spoons to using bowls for holding objects proves to be too difficult for the current design. 
% As illustrated in Figure~\ref{fig_res_robustness}b, despite the unfamiliar object category and interaction triplet, we still manage to lift the knife and mimic the intended motion, although the execution is not perfect. This indicates potential areas for improvement while showcasing the model's adaptability in challenging scenarios.

% We further test the model's generalization ability on different levels of test sets on the TACO dataset. As indicated in Table~\ref{tb_exp_taco_generalization_test}, the controller can perform well in the category-level generalization setting, where the object category is observed during the training while the manipulation trajectories and the object geometry are novel, as indicated by its good performance in the test set S1. 
% The performance on S2 contains novel interaction triples is still relatively satisfactory, indicating its ability to generalize to control novel manipulation sequences. However, results on S3 indicate the model's being challenged by novel object categories and unseen interaction triplets. Generalizing from interactions demonstrating lifting and waving shovels and spoons to using bowls to hold things is still too challenging for the current design. As shown in Figure~\ref{fig_res_robustness}b, given the unobserved object category and the interaction triplet, though not perfect, we can still manage to lift the knife up and mimic the motion. 
% \todo{add the qualitative evals}
% The object position error is still kept to a small value, indicating 

% Specifically, the whole dataset is split into a training dataset, containing 1565 trajectories, and the test set S0 where both the tool object geometry and the interaction triplets are seen during training, the test set S1 where the tool geometry is novel but the interaction triplets are seen during training, the test set S2 with novel interaction triplets but seen object categories and geometries, and the test set S4 with new object geometries and interaction triplets. Details w.r.t. the dataset splitting and visualizations are deferred to Appendix~\ref{}. 

% \begin{wraptable}[6]{r}{0.5\textwidth}
% \vspace{-30pt}
%     \centering
%     \caption{ 
%     Total training time consumption (TACO dataset). 
%     } 
%     % \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccc@{\;}}
%         \toprule
%         ~ & \makecell[c]{PPO \\ (w/o sup)} & \makecell[c]{Ours \\ (w/ sup.)}  & \makecell[c]{Ours \\ (w/ sup., \\ w/ curri.)} & Ours   \\

%         \midrule % 

%         Time  &  $\sim$1 day & $\sim$5 days & $\sim$13 days & $\sim$4 days
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_exp_timeconsumption}
% \end{wraptable}


% \noindent\textbf{Time consumption.} Table~\ref{tb_exp_timeconsumption} summarizes the total time consumption of different methods on the TACO dataset. Directly training PPO without any supervision is the most efficient approach while the performance lagged behind due to no proper guidance. Exact curriculum learning for acquiring high-quality per-trajectory trackers, though as we observe in Table~\ref{tb_exp_main}, is an effective strategy, which also aligns with conclusions in previous approaches, is extremely time-consuming. For 400 trajectories that we finally select to optimize to produce an action-labeled dataset, searching the exact curriculum costs about 13 days to complete. However, our method requires only slightly more time than the version without tracking prior or curriculum scheduling (Ours w/ sup.). However we can achieve a much higher success rate than this version, taking advantage of the increased diversity and the quality of action-labeled data. 




\vspace{-10pt}
\section{Ablation Studies} \label{sec:ablation_studies}
\vspace{-5pt}


\noindent\textbf{Diversity and quality of robot tracking demonstrations.} 
We propose enhancing the diversity and quality of tracking demonstrations using the tracking controller and homotopy generator. We ablate these strategies by creating two variants: ``Ours (w/o data, w/o homotopy)'', where the dataset is built by optimizing each trajectory without prior knowledge, and ``Ours (w/o data)'', which uses only the homotopy optimization scheme to improve demonstrations. Despite using the same number of demonstrations, both variants produce lower-quality data. As shown in Table~\ref{tb_exp_main}, they underperform compared to our full method, underscoring the importance of data quality in training the controller.
% We propose to improve the diversity and the quality of the robot tracking demonstrations via the tracking controller and the homotopy generator. We ablate these two strategies by creating two variants: ``Ours (w/o data, w/o homotopy)'', where the dataset is built by directly optimizing each trajectory without prior knowledge, and ``Ours (w/o data)'', where we only leverage the homotopy optimization scheme to improve demonstrations. Both strategies, despite using the same amount of demonstrations, result in lower data quality. As shown in Table~\ref{tb_exp_main}, they underperform compared to our full method, highlighting the importance of data quality in training the controller.
% 
% where optimization combines trajectory-specific efforts with the controller's tracking prior.
% We propose transferring tracking knowledge from the controller and curriculum before optimization to handle more difficult and diverse trajectories in the dataset. We ablate these strategies 
% We propose to transfer general tracking knowledge encoded in the tracking controller and the curriculum prior to the optimization process for solving difficult-to-solve problems so that we can include more difficult and diverse labeled trajectories into the dataset. We've tried to ablate such two strategies and create ``Ours (w/o data, w/o structure)'' where the final labeled dataset is created by directly optimizing each trajectory without any prior from the tracking controller or the curriculum scheduler, and ``Ours (w/o data)'' where each trajectory is optimized under the joint effort of the per-trajectory tracking optimization and the tracking prior provided by the tracking controller. Such two strategies, though using the same amount of labeled data as our full method to provide supervision, may fall short in the data quality aspect. As shown in Table~\ref{tb_exp_main}, they would lag behind our full version, illustrating the role of data quality in training the tracking controller. 
% This approach can potentially let us get better per-trajectory tracker under expansive tracking curriculum trail-and-error. However, it is extremely time-consuming and unaffordable. As presented in Table~\ref{tb_exp_main}, Ours (w/ sup.), as restricted by the quality and the diversity of the action-labeled data, typically lags behind our full method on both the GRAB dataset and the TACO dataset. It validates the importance of data quality and coverage used to train the tracking controller. Ours (w/ sup., w/ curriculum) leverages the power of curriculum learning and the benefit of per-trajectory searched accurate curriculum, and can sometimes outperform out proposed strategy, which uses the tracking controller to provide tracking priors and the curriculum scheduler to propose the tracking schedule for tracking difficult trajectories. However, leveraging this approach is highly time-consuming, and would become extremely unaffordable when the number of data increases. Our proposed strategy can not only effectively improve the data quality, but smartly reduces the time consumption. 
% using per-trajectory tracking optimization and the tracking prior from the tracking controller. 
% optimized with per-trajectory searched curriculum, other than the curriculum planned by the scheduler. 
% This demonstrate the effectiveness of the tracking curriculum and the quality of our mined curricula. 
% typically lags behind our full method,
% \todo{xxxx} 
% \todo{for the curriculum, say that the trajectories between TACO is a little bit similar so we can observe the the one with exact curriculum can achieve better performance some times}


\begin{wrapfigure}[13]{r}{0.45\textwidth} % {0pt}
\vspace{-3ex}
\includegraphics[width = 0.45\textwidth]{./figs/scaling.pdf}
\vspace{-30pt}
    \caption{\footnotesize
    Scaling the amount of demonstrations.
    }
    \label{fig:fig_scaling}
% \vspace{-30pt}
\end{wrapfigure}

\vspace{-5pt}
\noindent\textbf{Scaling the number of demonstrations.} 
To investigate the relationship between the tracking controller's performance and the number of demonstrations, we vary the size of the demonstration dataset during training and tested performance on the TACO dataset. Specifically, in the final training iteration, we down-sampled the dataset to 0.1, 0.3, 0.5, and 0.9 of its original size and re-trained the model. As shown in Figure~\ref{fig:fig_scaling}, there is a clear correlation between the amount of demonstrations and model performance. Since the curve has not plateaued, we hypothesize that increasing the amount of high-quality data could further improve performance.
% general tracking controller's performance and the amount of labeled data, 
% To explore the relation between the performance of the general tracking controller and the number of labeled data, we try to vary the number of final labeled data to train the model and test the model's performance on the TACO dataset. To be more specific, in the last training iteration, we try to down-sample the \emph{final action-labeled dataset} into $0.1, 0.3, 0.5, 0.9$ of its original size and re-train the model. As summarized in Figure~\ref{fig:fig_scaling}, there exists an obvious relation between the amount of labeled data used for training and the model's performance. Besides, the curve has not yet reached a flat raising mode in our trails. So we hypothesize that our method's performance could still be enhanced if we can manage to create more high-quality data to train the general tracking controller. 
 
% \todo{a scaling law that demonstrate the role of the data } 

% \todo{time consumption and the time efficiency}


\vspace{-10pt}
% \todo{repro statement}



==> articles_revision/abstract.tex <==
\input{articles_revision/teaser_figure}


\begin{abstract}

We address the challenge of developing a generalizable neural tracking controller for dexterous manipulation from human references. This controller aims to manage a dexterous robot hand to manipulate diverse objects for various purposes defined by kinematic human-object interactions. Developing such a controller is complicated by the intricate contact dynamics of dexterous manipulation and the need for adaptivity, generalizability, and robustness. Current reinforcement learning and trajectory optimization methods often fall short due to their dependence on task-specific rewards or precise system models. We introduce an approach that curates large-scale successful robot tracking demonstrations, comprising pairs of human references and robot actions, to train a neural controller. Utilizing a data flywheel, we iteratively enhance the controller's performance, as well as the number and quality of successful tracking demonstrations. We exploit available tracking demonstrations and carefully integrate reinforcement learning and imitation learning to boost the controller's performance in dynamic environments. At the same time, to obtain high-quality tracking demonstrations, we individually optimize per-trajectory tracking by leveraging the learned tracking controller in a homotopy optimization method. The homotopy optimization, mimicking chain-of-thought, aids in solving challenging trajectory tracking problems to increase demonstration diversity. We showcase our success by training a generalizable neural controller and evaluating it in both simulation and real world. Our method achieves over a 10\% improvement in success rates compared to leading baselines. The project website with animated results is available at  \href{https://projectwebsite7.github.io/gene-dex-manip/}{DexTrack}.
% and the number and quality of successful tracking demonstrations. 


% % We explore the problem of obtaining a generic controller for dexterous robotic hands 
% % learning a generalizable neural tracking controller for dexterous manipulation from human references. 
% We explore the problem of learning a generalizable neural tracking controller for dexterous manipulation from human references.
% % The task wishes for a versatile controller that can control a dexterous robot hand to accomplish various, challenging and expressive manipulation tasks specified by kinematic human-object manipulations. 
% This task wishes for a versatile controller capable of managing a dexterous robot hand to execute various complex and expressive manipulation tasks, as defined by kinematic human-object interactions.
% It is inherently challenged by the optimization difficulty resulting from intricate dynamics involved in dexterous manipulation and the expectation in the versatility, generalization ability, and robustness of the tracking controller.
% % to various, novel, and challenging manipulation tasks. 
% Either advanced model-free reinforcement learning (RL)-based techniques or model-based trajectory optimization fall short in resolving such huge challenges due to the demand on task-specific reward designs that largely hinder the generalization capability and the difficulty in complex system modeling in the dexterous manipulation scenario.
% Our key idea lies in leveraging high-quality abundant imitation-ready data to train a tracking controller and tackling the difficulties in acquiring such data by leveraging the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner.
% % by carefully combining reinforcement learning and imitation learning, 
% % jointly with RL and tackling the difficulties in acquiring such data by leveraging the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner.
% % leverage abundant, high-quality, imitation-ready data to facilitate the learning of a generalizable tracking controller.
% We carefully combine reinforcement learning and imitation learning to train the neural tracking controller to enhance its versatility, generalization ability, and robustness towards dynamic environment variations. To curate abundant high-quality imitation-ready data, we devise a per-trajectory tracking strategy using the tracking controller and a homotopy path generator, mimicking chain-of-thought, that can propose beneficial homotopy optimization paths to help us solve difficult single trajectory tracking problems. We showcase our success in training a versatile neural tracking controller with high generalization ability and robustness. Through extensive experiments conducted in both simulation and real world, our method demonstrates an improvement in success rates of over 10\% compared to the best-performing baseline. The project website with animated results is available at \href{https://projectwebsite7.github.io/gene-dex-manip/}{DexTrack}.
% % We demonstrate our success in training a versatile neural tracking controller with high generalization ability and robustness. We conduct extensive experiments in both the simulator and the real world, demonstrating capability of our method in boosting the success rate by 10\%+ from the best-performed baseline. The project website is available at \href{https://projectwebsite7.github.io/gene-dex-manip/}{DexTrack}. 
% % We conduct extensive experiments in both the simulator the real world, demonstrating the versatility, generalization ability, and robustness of our tracking controller,  capability of boosting the success rate by 10\%+ from the best-performed baseline. The project website is available at \href{https://projectwebsite7.github.io/gene-dex-manip/}{DexTrack}.
% % Isaac Gym and 
% % that effectively improves single trajectory tracking results via the tracking controller and a homotopy path generator, mimicking chain-of-thought, that can propose beneficial homotopy optimization paths. 
% % We leverage imitation learning and reinforcement learning to train the neural tracking controller to let it benefit from a large number of high-quality data and also be able to cope with dynamic state disturbances. To curate abundant high-quality imitation-ready data, we devise a per-trajectory tracking scheme that effectively improves single trajectory tracking results via the tracking controller and a homotopy path generator, mimicking chain-of-thought, that can propose beneficial homotopy optimization paths. 
% % We successfully train a universal tracking controller that enables a dexterous robot hand to adeptly interact with diverse objects to accomplish a wide range of novel and expressive manipulation tasks. 
% % with dynamics, rich hand-object contacts. 

% % Previous approaches are typically restricted to task-specific manipulation skill acquisition or only demonstrate the versatility in relatively simple tasks such as grasping, leaving 
% % the general dexterous tracking control largely unsolved~\eric{``Dexterous tracking control'' is not a good term. Dexterous is used to describe manipulation other than tracking.}. 
% % are typically limited by the unsatisfactory capability and versatility, leaving the universal dexterous tracking control largely unsolved. 
% % unsatisfactory task difficulties or being restricted in single trajectory tracking, leaving the universal dexterous tracking control largely unsolved. 
% % We propose to leverage the joint effort of reinforcement learning (RL) and the diverse and high-quality action-labeled data to open the possibility of training general tracking control policy. 
% % We wish to learn a versatile and generalizable neural controller by imitating abundant, high-quality data with actions to obtain the generalization ability towards veraious situations, and leveraging reinforcement learning to maintain the robustness and unepxted situations. However, acquiring  a large number of imitation-ready data itself is tricky and challenging. 
% % We propose to leverage abundant, high-quality, imitation-ready data to facilitate the learning of a generalizable tracking controller.
% % Since acquiring a large amount of imitiation-ready data with hgih-quality action sequences itself is very challenging, we devise a strategy w
% % But acquiring a large amount of imitation-ready data itself is very challenging. We propose to learn a tracking task structure prior model which is further leveraged to plan optimization paths so that we can solve difficult tracking problems via a homotopy method. 
% % model tracking task structure 
% % by 
% % transferring tracking data prior and a homotopy method propose
% % with the optimization paths generated by a homotopy generator. 
% % We design an iterative way to improve the imitation-ready data by data prior from the tracking controller and the tracking task structure prior, and enhance the tracking controller in a bootstrapping manner. 
% % improve the tracking controller 
% % But acquiring high-quality data itself
% % data to facilitate the tracking 
% % We design an iterative approach where we 1) curate high-quality action-labeled data taking the joint power of tracking prior from the tracking controller and tracking curriculum proposed by a learned curriculum scheduler, and 2) train the tracking controller taking advantage of the guidance from the labeled data. 
% % a universal controller that can generalize to adeptly complete various novel and challenging manipulation tasks. 
% % challenged by inherent difficulties from 
% % We explore the problem of learning a universal tracking controller from human references. The task wishes for a versatile controller that can control a dexterous robot hand to accomplish various challenging and expressive manipulation tasks specified by kinematic motions. It is challenged by inherent difficulties from the complex and intricate dynamics involved in dexterous manipulation and the wish for a universal controller that can generalize to adeptly complete various novel and challenging manipulation tasks. Previous approaches are typically limited by unsatisfactory task difficulties or being restricted in single trajectory tracking, leaving the universal dexterous tracking control largely unsolved. We propose to leverage the joint effort of reinforcement learning (RL) and the diverse and high-quality action-labeled data to open the possibility of training genera tracking control policy. We design an iterative approach where we 1) curate high-quality action-labeled data taking the joint power of tracking prior from the tracking controller and tracking curriculum proposed by a learned curriculum scheduler, and 2) train the tracking controller taking advantage of the guidance from the labeled data. We successfully train a universal tracking controller that enables a dexterous robot hand to adeptly interact with diverse objects to accomplish a wide range of novel and expressive manipulation tasks. We conduct extensive experiments in both Isaac Gym and the real world, demonstrating the capability of boosting the success rate by xx\%+ from the best-performed baseline. 
\end{abstract}

==> articles_revision/conclusions.tex <==
\section{Conclusions and Limitations}

% In this work, we propose \modelname to tackle the challenge of developing a generalizable tracking controller for dexterous manipulation. By leveraging abundant high-quality robot tracking demonstrations and employing a pre-trajectory tracking scheme to mine imitation-ready data, we progressively refine the controller using a bootstrapping strategy. Extensive experiments validate the effectiveness of our approach, establishing it as a strong foundation for future advancements in generalizable tracking control. \noindent\textbf{Limitations.} The primary limitation of our method is the efficiency of acquiring high-quality demonstrations. Currently, searching for optimal homotopy optimization paths to improve demonstrations is time-consuming. Future research could focus on finding faster, approximate homotopy optimization methods to accelerate the training process.

\vspace{-5pt}

We propose \modelname to develop a generalizable tracking controller for dexterous manipulation. Leveraging high-quality tracking demonstrations and a pre-trajectory tracking scheme, we refine the controller through bootstrapping. Extensive experiments confirm its effectiveness, establishing a strong foundation for future advancements. \noindent\textbf{Limitations.} A key limitation is the time-consuming process of acquiring high-quality demonstrations. Future work could explore faster, approximate methods for homotopy optimization to speed up training.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% In this work, we propose \modelname to address the challenge of developing a generalizable tracking controller for dexterous manipulation. 
% By leveraging abundant high-quality robot tracking demonstrations to train the tracking controller and employing a pre-trajectory tracking scheme that effectively mines high-quality imitation-ready data, we gradually solve problems in each side and finally arrive at a strong tracking controller via a bootstrapping strategy. 
% Extensive experiments demonstrate the effectiveness of our method, evidencing it as a promising foundation for future developments in generalizable tracking control. 
% \noindent\textbf{Limitations.} The main limitation of our method lies in the efficiency of acquiring high-quality demonstrations. Currently, searching for good homotopy optimization paths to improve demonstrations is a little bit time-consuming. A meaningful future research direction is approximately finding beneficial homotopy optimization in a time-efficient way, therefore accelerating the homotopy generator's training. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The main limitation of our approach lies in the efficiency of acquiring high-quality action-labeled data. Currently, searching for good tracking curricula for training the curriculum scheduler is the most time-consuming part of our method. How to improve the efficiency such as using approximate curricula for training the scheduler is an interesting future research direction. 


% To address the difficulties in acquiring abundant and high-quality data 
% universal tracking controller for dexterous robot hand manipulation. By combining reinforcement learning with high-quality action-labeled data, we unleash the possibility of using RL to train a tracking controller for solving difficult manipulation problems. To address the ``chicken-and-egg'' problem by 1) training the controller using both RL and action-labeled datasets, and 2) optimizing for high-quality action-labeled data effectively in an acceptable time-budget, we design an interactive approach. 
% Leveraging the joint power of a learned tracking curriculum and data guidance, we can effectively improve the quality of the labeled dataset. We then progressively improve the capability of the tracking controller by curating data with higher quality. Extensive experiments demonstrate the effectiveness of our method, evidencing it as a promising foundation for future developments in universal tracking control.

% \noindent\textbf{Limitations.} The main limitation of our approach lies in the efficiency of acquiring high-quality action-labeled data. Currently, searching for good tracking curricula for training the curriculum scheduler is the most time-consuming part of our method. How to improve the efficiency such as using approximate curricula for training the scheduler is an interesting future research direction. 
% The process of curating this data is resource-intensive, requiring significant time and effort to generate diverse and accurate labels that effectively guide the training of the tracking controller. While our method achieves notable performance improvements, the dependence on large amounts of labeled data could hinder scalability, particularly when expanding to more complex tasks or environments. Future work could explore strategies to reduce the reliance on labeled data, such as incorporating self-supervised learning or more efficient data-generation techniques, to enhance both the practicality and scalability of the approach.
% we can create enough high-quality data in an acceptable time budget for training 
% demonstrates significant improvements in manipulation performance across a range of novel and expressive tasks. Extensive experiments, both in simulation and real-world environments, validate the effectiveness of our approach, with notable improvements in success rates over existing baselines. This research opens new avenues for advancing dexterous robot manipulation, providing a promising foundation for future developments in universal tracking control.

==> articles_revision/exp.tex <==

\vspace{-5pt}
\section{Experiments} \label{sec:exp}
\vspace{-5pt}
% TODO: overview part




% and adaptability 
% We conduct extensive experiments to demonstrate the effectiveness, generalization ability, and robustness, of our tracking controller. We evaluate our method on two HOI datasets containing complex functional daily manipulation featured by difficult trajectories with non-trivial object movements and subtle in-hand re-orientations, challenging object geometries, as well as rich and changing contacts. 
% We train our model in the Isaac Gym environment and conduct evaluations both in the simulator and the real world (see Section~\ref{sec:exp_setting}). We compare strong baselines with dedicated designs for dexterous manipulations to demonstrate the superiority of our method. Our tracking controller can track diverse, difficult, and novel hand-object interactions involving challenging and functional movements, extremely thin objects, as well as rich and changing contacts (see Section~\ref{sec:exp_results}).  However, previous approaches either fail to generalize or behave unsatisfactorily in challenging cases. On average, we can boost the tracking success rate by 10\% from the previously best-performed method. We make further analysis of our method on its robustness and the generalization ability to out-of-distribution test cases (see Section~\ref{sec:exp_analysis}) to illustrate its capability and utility (see Section~\ref{sec:exp_analysis}).  

% We conduct extensive experiments to evaluate the effectiveness, generalization ability, and robustness of our tracking controller. Our method is tested on two HOI datasets featuring complex, functional, daily manipulation tasks. We conduct both through experiments both in the simulation and evaluations in the real world (see Section~\ref{sec:exp_setting}). We compare our method against strong baselines to demonstrate its superiority. Our tracking controller successfully handles novel, difficult, and intriguing manipulations, including those involving intricate functional movements, extremely thin objects, and dynamic contacts (see Section~\ref{sec:exp_results}). In contrast, previous approaches fail to generalize well. On average, our method improves the tracking success rate by more than 10\% over the best prior methods across both datasets. We further analyze our controller's robustness towards significant kinematic noise such as unrealistic states and large penetrations (see Section~\ref{sec:exp_analysis}). 
We conduct extensive experiments to evaluate the effectiveness, generalizability, and robustness of our tracking controller. Tested on two HOI datasets featuring complex daily manipulation tasks, our method is assessed through both simulation and real-world evaluations (see Sec.~\ref{sec:exp_setting}). We compare our approach to strong baselines, showing its superiority. Our controller successfully handles novel manipulations, including intricate movements, thin objects, and dynamic contacts (see Sec.~\ref{sec:exp_results}), while previous methods fail to generalize well. On average, our method improves the tracking success rate by over 10\% compared to the best prior methods. Additionally, we analyze its robustness to significant kinematic noise, such as unrealistic states and large penetrations (see Sec.~\ref{sec:exp_analysis}).
% showcasing its versatility and practical utility.
% , as well as the generalization capabilities towards out-of-distribution test cases (see Section~\ref{sec:exp_analysis}), 
% , specifically designed for dexterous manipulations, 
% Empowered by our proposed training pipeline, we demonstrate that our tracking controller can effectively generalize to novel and challenging interaction trajectories involving unseen object geometry and unobserved manipulations. 
% , demonstrating strong capability and robustness. 


% , which are crucial properties that we expect for a general controller, to demonstrate its capability and utility (see Section~\ref{sec:exp_analysis}). 
% With a single policy, we 





% \textcolor{red}{TODO: track some interesting and long motions?}

\vspace{-10pt}
\subsection{Experimental Settings} \label{sec:exp_setting}
\vspace{-5pt}


% \todo{add the retargeting to the appendix} 

\noindent\textbf{Datasets.}
We test our method on two public human-object interaction  datasets:
% Our dexterous robot hand-object manipulation dataset is built by retargeting two public human-object interaction datasets: 
GRAB~\citep{taheri2020grab}, featuring daily interactions, and 
% single-hand interaction and 
TACO~\citep{liu2024taco}, containing functional tool-use interactions. 
% (single-hand interactions) and TACO~\citep{liu2024taco} (functional tool-use interactions). 
In simulation, we use the Allegro hand, with URDF adapted from IsaacGymEnvs~\citep{makoviychuk2021isaac}, and in real-world experiments, the LEAP hand~\citep{Shaw2023LEAPHL}, due to hardware constraints. Human-object interaction trajectories are retargeted to create robot hand-object sequences using PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. We fully retargeted the GRAB and TACO datasets, producing 1,269 and 2,316 robot hand manipulation sequences, respectively. The evaluation on GRAB focus on testing the model’s generalization to unseen interaction sequences. 
Specifically, we use sequences from subject \texttt{s1} (197 sequences) as the test data while the remaining trajectories as the training set. 
% sequences from subject \texttt{s1} (197 sequences) are used as the test dataset. 
% while the training dataset includes the remaining sequences from other subjects. 
For the TACO dataset, we follow the generalization evaluating setting suggested by the authors~\citep{liu2024taco} and split the dataset into a training set with 1,565 trajectories and four distinct test sets at different difficulty levels. The primary quantitative results are reported on the first-level set. More details are provided in Appendix~\ref{sec:supp_exp_details}. 
% and results are provided in Appendix~\ref{sec:supp_exp_details}. 
% More details on the dataset splitting and our results on remaining test sets are provided in Appendix~\ref{sec:supp_exp_details}. 
% to assess generalization at different levels. 
% evaluation setting suggested by the authors~\citep{liu2024taco}. The dataset is split into a training set with 

% GRAB focuses on testing generalization to unseen sequences, while TACO evaluates generalization across four distinct test sets. More details on dataset splitting and results are provided in Appendix~\ref{sec:supp_exp_details}.

% Our dexterous robot hand-object manipulation dataset is constructed by retargeting two public human-object interaction datasets: GRAB~\citep{taheri2020grab}, which focuses on single-hand interactions with everyday objects, and TACO~\citep{liu2024taco}, which features functional tool-use interactions. For simulation experiments, we use the Allegro hand, while in real-world experiments, the LEAP hand~\citep{Shaw2023LEAPHL} is employed due to constraints in the hardware resources. In simulation, the URDF file for the Allegro hand is adapted from IsaacGymEnvs~\citep{makoviychuk2021isaac}, while the LEAP hand URDF is adapted from dex\_urdf~\citep{bunnyvisionpro}. We retarget human-object interaction (HOI) trajectories to simulated robot hand to create the robot hand-object interaction sequences. We use the forward kinematics implemented in PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024} in the retargeting method. Further details are provided in Appendix~\ref{sec:supp_method}. We fully retargeted the GRAB and released TACO datasets, yielding 1,269 and 2,316 robot hand manipulation sequences, respectively. The GRAB dataset evaluation focuses on testing the model’s generalization to unseen interaction sequences, given the large variations in object geometries. Specifically, sequences from subject \texttt{s1} (197 sequences) are used as the test dataset, while the training dataset includes the remaining sequences from other subjects. For the TACO dataset, we follow the generalization evaluation setting suggested by the authors~\citep{liu2024taco}. The dataset is split into a training set with 1,565 trajectories and four distinct test sets to assess generalization at different levels. The primary quantitative results are reported on the first-level test set. More details on the dataset splitting and our results on remaining test sets are provided in Appendix~\ref{sec:supp_exp_details}. 

% The forward kinematics algorithm in  the retargeting method is
% We describe these hands in simulation using URDF files from dex\_urdf~\citep{bunnyvisionpro} and retarget human-object interaction (HOI) trajectories to both hands, generating corresponding kinematic trajectories through PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. 

% the test set S0. More details on the dataset splitting and visualizations are provided in Appendix~\ref{sec:supp_exp_details}. 
% : 1) S0: Both the tool object geometries and interaction triplets are seen during training; 2) S1: Novel tool geometries, but the interaction triplets are seen during training; 3) S2: Novel interaction triplets, but familiar object categories and geometries; 4) S3: Both object geometries and interaction triplets are novel. The primary quantitative results are reported on the test set S0. More details on the dataset splitting and visualizations are provided in Appendix~\ref{sec:supp_exp_details}. 

% Our dexterous robot hand-object manipulation dataset is created by retargeting two public human-object datasets, namely GRAB~\citep{taheri2020grab}, containing single-hand interactions with daily objects, and TACO~\citep{liu2024taco}, featured by functional tool using interactions. We use simulated Allegro hand in our simulation experiments while LEAP hand~\citep{Shaw2023LEAPHL} in the real world experiments due to the hardware constraints. We use URDF files from dex\_urdf~\citep{bunnyvisionpro} as their descriptions in the simulation. We retarget HOI trajectories to these two hands to create their corresponding kinematic trajectories leveraging PyTorch\_Kinematics~\citep{Zhong_PyTorch_Kinematics_2024}. 
% For details of the retargeting method that we leverage in our method, please refer to Appendix~\ref{sec:supp_method}. 
% We retarget the full GRAB dataset and the full released TACO dataset, obtaining 1269 and 2316 robot hand manipulation sequences respectively. The evaluation on GRAB mainly aims at testing the model's generalization ability toward unseen interaction sequences considering the large distinctions between their object geometries. Specifically, we use sequences of subject \texttt{s1}, with  197 sequences in total, as the test dataset.  The training dataset is constructed by remaining sequences from other subjects. 
% For the TACO dataset, we create one training set with four distinct test sets with different generalization levels for a detailed evaluation of the model's generalization performance, as suggested by authors~\citep{liu2024taco}. Specifically, the whole dataset is split into a training dataset, containing 1565 trajectories, and the test set S0 where both the tool object geometries and the interaction triplets are seen during training, the test set S1 where the tool geometry is novel but the interaction triplets are seen during training, the test set S2 with novel interaction triplets but seen object categories and geometries, and the test set S4 with new object geometries and interaction triplets. Main quantitative results are reported on the test set S0.  Details w.r.t. the dataset splitting and visualizations are deferred to Appendix~\ref{sec:supp_exp_details}. 
% robot hand manipulation sequences and 2316 sequences
% obtaining 1269 manipulation sequences in total, and the full released TACO data which contains 2316 sequences in total. 
% For TACO dataset, to balance the time consumption and the final data amount, we randomly select 1800 sequences from 2316 sequences in total for retargeting.


% create four different test sets to evaluate the generalization 
% For GRAB, we mainly evaluate the model's generalization ability towards novel interaction sequences considering the large distinctions between their object geometries. For 
% To evaluate the model's generalization capability towards novel manipulation trajectories, we further split them into train and test splits. For the GRAB dataset, we use sequences of the \texttt{subject s1}, with 197 sequences in total, as the test dataset. The train dataset is constructed by remaining sequences from other subjects. For the TACO dataset, we 190 trajectories randomly selected from 1800 sequences for test, while the remaining trajectories as the training data. 
% \todo{unboserved objects? a different splitting method for TACO that considers the object category?}  For evaluating the model's generalization ability towards unseen geometry, we additionally construct a subset from the TACO's training dataset and a subset from TACO's test dataset as a new test split. \todo{details about that}
% For the GRAB datset, although there are existing previous splitting routines~\citep{Zhou2022TOCHSO,Liu2024GeneOHDT}, they mainly focus on cross object generalization. 








% so many todos 
\vspace{-5pt}
\noindent\textbf{Metrics.} 
We introduce five metrics to evaluate the tracking accuracy and task success: 1) Per-frame average object rotation error: \( R_{\text{err}} = \frac{1}{N+1} \sum_{n=0}^N \text{Diff\_Angle}(\mathbf{q}_n, \hat{\mathbf{q}}_n) \), where \( \hat{\mathbf{q}}_n \) and  \( \mathbf{q}_n \)  are reference and tracked orientation.
2) Per-frame average object translation error: \( T_{\text{err}} = \frac{1}{N+1} \sum_{n=0}^N \Vert \mathbf{t}_n - \hat{\mathbf{t}}_n \Vert \), where \( \mathbf{t}_n \) and \( \hat{\mathbf{t}}_n \) are the tracked and reference translations. 3) Per-frame average wrist position and rotation error: \( E_{\text{wrist}} = \frac{1}{N+1} \sum_{n=0}^N \left( 0.5 \, \text{Diff\_Angle}(\mathbf{q}_n^{\text{wrist}}, \hat{\mathbf{q}}_n^{\text{wrist}}) + 0.5 \Vert \mathbf{t}_n^{\text{wrist}} - \hat{\mathbf{t}}_n^{\text{wrist}} \Vert \right) \), where \( \mathbf{q}_n^{\text{wrist}} \) and \( \hat{\mathbf{q}}_n^{\text{wrist}} \) are wrist orientations, and \( \mathbf{t}_n^{\text{wrist}} \) and \( \hat{\mathbf{t}}_n^{\text{wrist}} \) are translations. 4) Per-frame per-joint average position error: \( E_{\text{finger}} = \frac{1}{N+1} \sum_{n=0}^N \left( \frac{1}{d} \Vert \mathbf{\theta}_n^{\text{finger}} - \hat{\mathbf{\theta}}_n^{\text{finger}} \Vert_1 \right) \), where $\mathbf{\theta}$ denotes finger joint positions, \( d \) is the degrees of freedom.
% (16 for both Allegro and LEAP hands).  
% and \( \Vert \cdot \Vert_1 \) denotes the 1-norm. 
5) Success rate: A tracking attempt is successful if \( T_{\text{err}} \), \( R_{\text{err}} \), and \( 0.5E_{\text{wrist}} + 0.5E_{\text{finger}} \) are all below the thresholds. Success is calculated with two thresholds: \( 10\text{cm} \)-\(20^\circ\)-\(0.8\) and \( 10\text{cm} \)-\(40^\circ\)-\(1.2\).
% object tracking quality, hand tracking accuracy, and 
% We introduce five metrics to evaluate the quality of object tracking, hand tracking accuracy, and overall success in the tracking task: 
% 1) Per-frame average object rotation error: $R_{\text{err}} = \frac{1}{N} \sum_{n=1}^N \text{Diff\_Angle}(\mathbf{q}_n, \hat{\mathbf{q}}_n) $, where $\mathbf{q}_n$ is the ground-truth orientation, $\hat{\mathbf{q}}_n$ is the tracked result, represented in quaternion, $\text{Diff\_Angle}(\cdot, \cdot)$ computes the angular difference between two quaternions.
% 2) Per-frame average object translation error: $T_{\text{err}} = \frac{1}{N} \sum_{n=1}^N \Vert \mathbf{t}_n - \hat{\mathbf{t}}_n \Vert$, where $\mathbf{t}_n$ and $\hat{\mathbf{t}}_n$  represent the ground-truth and tracked translations, respectively.
% 3) Per-frame average wrist position and rotation error: $E_{\text{wrist}}=\frac{1}{N}  \sum_{n=1}^N (0.5 \text{Diff\_Angle}(\mathbf{q}_n^{\text{wrist}}, \hat{\mathbf{q}}_n^{\text{wrist}})  + 0.5 \Vert \mathbf{t}_n^{\text{wrist}} - \hat{\mathbf{t}}_n^{\text{wrist}} \Vert )$, where $\mathbf{q}_n^{\text{wrist}}$ and $\hat{\mathbf{q}}_n^{\text{wrist}}$ represent the orientation of the wrist in the reference motion and the tracking result, respectively, while $\mathbf{t}^{\text{wrist}}_n $ and $\hat{\mathbf{t}}_n^{\text{wrist}}$ denote the wrist translation in the reference trajectory and the tracking result, respectively. 
% 4) Per-frame per-joint average position error: 
% $E_{\text{finger}}= \frac{1}{N}  \sum_{n=1}^N (\frac{1}{d} \Vert \mathbf{\theta}_n^{\text{finger}} - \hat{\mathbf{\theta}}_n^{\text{finger}} \Vert_1 )$, where $d$ is the number of degree-of-freedom (DoF) of the dexterous robot hand, \emph{i.e.,} 16 for Allegro hand and the LEAP hand used in our experiments, $\Vert \cdot \Vert_1$ denote the $1$-norm of the vector. 
% 5) Success rate: A tracking attempt is deemed successful if the object translation error $T_{\text{err}}$, object rotation error $R_{\text{err}}$, and the hand tracking error $0.5E_{\text{wrist}} + 0.5E_{\text{finger}}$ are all below their specified thresholds. Success rates are calculated using two thresholds: $10\text{cm}$-$20^\circ$-$0.8$, $10\text{cm}$-$40^\circ$-$1.2$. 

% are smaller than their corresponding threshold. Three success rates are calculated using two different thresholds, namely $10\text{cm}-20^\circ-0.8$, $10\text{cm}-40^\circ-1.2$. 
% a tracking is regarded as successful if the object rotation error object translation error 
% $15\text{cm}-40^\circ-1.6$.


\vspace{-5pt}
\noindent\textbf{Baselines.} 
To our knowledge, no prior model-based methods have directly tackled tracking control for dexterous manipulation. Most existing approaches focus on single goal-driven trajectory optimization with simplified dynamics models~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex}, limiting their adaptability for our framework's generalizable tracking controller. Thus, we primarily compare our method with model-free approaches: 1) DGrasp~\citep{christen2022d}: Adapted to track by dividing sequences into subsequences of 10 frames, with each subsequence solved incrementally. 2) PPO (OmniGrasp rew.): We re-implemented OmniGrasp's reward~\citep{Luo2024GraspingDO} to train a policy for tracking object trajectories. 3) PPO (w/o sup., tracking rew.): We trained a policy using PPO with our proposed tracking reward and observation design.
% To the best of our knowledge, no prior model-based methods have specifically addressed tasks identical or comparable to the tracking control for dexterous manipulation. 
% Most existing approaches are constrained to single goal-driven trajectory optimization~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex} with a simplified dynamics model, making them difficult to adapt for optimizing a versatile tracking controller as required by our framework.
% Therefore, we primarily compare our method against model-free approaches: 1) DGrasp~\citep{christen2022d}: We adapt DGrasp to address the tracking problem by dividing the entire sequence into several subsequences, each consisting of 10 frames. The last frame of each subsequence is defined as its reference frame. This transforms each subsequence tracking task into a solvable problem for DGrasp. We then train a policy to incrementally solve each subproblem. 2) PPO (OmniGrasp rew.): OmniGrasp proposes a universal controller for grasping objects from a table and following the given object trajectory. Since the original implementation has not been open-sourced, we re-implemented the reward as described in the paper~\citep{Luo2024GraspingDO}. Using this reward and PPO, we train a policy aimed at tracking each training trajectory. 3) PPO (w/o sup., tracking rew.): We directly train a policy using PPO and our proposed tracking reward, along with our observation design (see Section~\ref{sec:method_il_rl}). 
% To our best knowledge, there is no previous model-based methods aiming to solve the task same or similar to our dexterous manipulation tracking control. Most of them are restricted in single goal-driven trajectory optimization~\citep{Jin2024ComplementarityFreeMM,pang2023global,pang2021convex} which is hard to be adapted to align with our goal of  optimizing a tracking controller.
% which does not and can hardly be adapted to align with our goal in optimizing a tracking controller. 

% Therefore, we mainly compare model-free approaches: 1) DGrasp~\citep{christen2022d}. We adapt DGrasp to solve the tracking problem. We divide the whole sequence into several subsequences with a length of 10 frames. We then define the last frame of each subsequence as its reference frame. After that, each subsequence tracking becomes a problem that DGrasp can solve. We then train a policy to solve each subproblem gradually. 2) PPO (OmniGrasp rew.). OmniGrasp proposes a universal controller for grasping objects from the table and following the given object trajectory. Since it has not been open-sourced yet, we re-implement the reward as described in the paper~\citep{Luo2024GraspingDO}. We then train a policy using the reward and PPO, with the goal of tracking each trajectory in the training dataset. 3) PPO (w/o sup., tracking rew.). We directly train a policy using PPO and our proposed tracking reward as well as the observation design (see Equation~\ref{eq:observations}~\ref{eq:rew_obj}~\ref{eq:rew_hand}~\ref{eq:rew_affinity}). 

% Since in the tracking phase, 

% We re-implement the reward as described in the paper~\citep{Luo2024GraspingDO}. A PPO is trained 
% divide the whole sequence into several subsequences, each of which has 10 frames, and define the end frame of the subsequence as the reference frame. Then the grasping policy is used to guide the hand and gradually track the object according to the hand and the object pose of each reference frame. 
% We compare our method with previous model-free approaches. 
% omni grasp reward o not considerthe 


\vspace{-5pt}
\noindent\textbf{Training and evaluation settings.} 
% The training process involves three stages, each using different tracking demonstrations. 
We use PPO~\citep{Schulman2017ProximalPO}, implemented in {rl\_games}~\citep{rlgames2021}, with Isaac Gym~\citep{makoviychuk2021isaac} for simulation. Training is performed with 8192 parallel environments for both the per-trajectory tracker and the tracking controller. For the dexterous hand, the position gain and damping coefficient are set to 20 and 1 per finger joint. Evaluation results are averaged across 1000 parallel environments, and for real-world evaluations, we use LEAP~\citep{Shaw2023LEAPHL} with a Franka arm and FoundationPose~\citep{Wen2023FoundationPoseU6} for object state estimation. Additional details are provided in Appendix~\ref{sec:supp_exp_details}.
% for the tracking controller 
% without transferring weights between models.
% The training process for the tracking controller consists of three stages, as outlined in the method section. In each stage, we retrain the model using different labeled datasets, without transferring weights from the previous model.  We use PPO~\citep{Schulman2017ProximalPO}, implemented in {rl\_games}~\citep{rlgames2021}, as our reinforcement learning algorithm. Isaac Gym~\citep{makoviychuk2021isaac}, a widely-used simulated physical environment, is utilized for training. We employ 8192 parallel environments to train both the per-trajectory tracker and the tracking controller. For the articulated dexterous hand, the position gain and damping coefficient are set to 20 and 1, respectively, for each finger joint. During the evaluation phase, we average evaluation results obtained in 1000 parallel execution environments as the final result.  For real-world evaluations, we use LEAP~\citep{Shaw2023LEAPHL} with Franka arm. We use FoundationPose~\citep{Wen2023FoundationPoseU6} to estimate the object states. 
% Further details, such as the simulation environment and the real setup, are provided in Appendix~\ref{sec:supp_exp_details}. 
% During the evaluation phase, we sample the policy 1000 times across 1000 parallel execution environments and average the metrics to obtain the evaluation result for the current trajectory. 

% such as the simulation  setup, are provided in Appendix~\ref{sec:supp_exp_details}. 
% including the simulation environment setup, 
% This is because we found that transferring weights makes the model more difficult to train, rather than speeding up the training process.
% The tracking controller training is composed of three stages as we detailed in the method section. In each stage, we re-train the model with different labeled datasets without transferring weights from the previously trained model. It is because we observe that weight transferring would make the model even harder to train, other than accelerating the training process. We leverage PPO~\citep{Schulman2017ProximalPO} implemented in {rl\_games}~\citep{rlgames2021} as our RL algorithm. We use the widely appreciated Isaac Gym~\citep{makoviychuk2021isaac} as the simulated physical environment. We use 8192 parallel environments to train both the per-trajectory tracker and the tracking controller. For articulated dexterous hands, the position gain and the damping coefficient are set to 20 and 1 respectively for each finger joint. During the evaluation phase, we sample from the policy 1000 times (using 1000 parallel execution environments) and average their metrics as the evaluation result of the current trajectory. More details such as the simulation environment setting are deferred to Appendix~\ref{sec:supp_exp_details}. 
% For both the per-trajectory tracker and the tracking controller, 
% the single trajectory specialist tracking policy training and the general tracking policy optimization, we use 8192 parallel environments to train RL. 






% take the widely appreciated Isaac Gym as our simulated environment where we train our 


% rich and changing contacts, j
\vspace{-5pt}
% \subsection{Generalizable Dexterous Manipulation Tracking Control } \label{sec:exp_results}
\subsection{Generalizable Tracking Control for Dexteroous Manipulation } \label{sec:exp_results}
\vspace{-5pt}


% \todo{add the time consumption}

\begin{figure}[ht]
  \centering
  \vspace{-10pt}
  \includegraphics[width=\textwidth]{figs/robustness_noise.pdf}
  \vspace{-20pt}
  \caption{\footnotesize
  \textbf{Robustness w.r.t. unreasonable states. }
  Please check \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{video}}}} for animated results.
  % ~\eric{the subsection title has been occluded by the figure... please adjust.}
  }
  \label{fig_res_robustness}
  \vspace{-10pt}
\end{figure}

% \todo{change the w/o prior, w/o curri. to w/o data, w/o structure}

\begin{figure}[ht]
  \centering
  % \vspace{-10pt}
  % \includegraphics[width=\textwidth]{figs/res_5.pdf}
  \includegraphics[width=\textwidth]{figs/eval_res_all_v2.pdf}
  % \vspace{-20pt}
  \caption{\footnotesize
  \textbf{Qualitative comparisons. }
  Please check \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
  }
  \label{fig_res}
  \vspace{-10pt}
\end{figure}




% \begin{table*}[t]
%     \centering
%     \caption{ 
%     \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
%     } 
%     % \vspace{-10pt}
%     \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{@{\;}llccccc@{\;}}
%         \toprule
%         %         
%         Dataset & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

        
%         \cmidrule(l{0pt}r{1pt}){1-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}

%         % \multirow{5}{*}{ GRAB } & ControlVAE & - & -  & -  & - 
%         % \\ 
%         % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         % \\ 
%         % % \cmidrule(l{15pt}r{17pt}){3-9}

%         % % \cmidrule(l{15pt}r{17pt}){3-9}
%         % \cmidrule(l{1pt}r{1pt}){2-3}
%         % % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         \multirow{2}{*}{ GRAB } & DGrasp & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (w/o sup., tracking rew.)  & 0.3945 & 6.11  & 0.1076 & 0.5899 & 38.78/55.05/60.58 
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){2-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}
        
        
%         % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         % \\ 
%         ~ & \model~(w/ sup.)  & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         \\ 
%         ~ & \model~(w/ sup., w/ curriculum)  & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         \\ 
%         ~ & \model  & \bred{0.3303} & \bred{4.53} & {0.1118} & \bred{0.5048} & \bred{47.12}/\bred{65.52}/\bred{72.41}
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){1-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}


%         % \multirow{5}{*}{ TACO } & ControlVAE & - & -  & -  & - 
%         % \\ 
%         % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         % \\ 
%         % % \cmidrule(l{15pt}r{17pt}){3-9}

%         % % \cmidrule(l{15pt}r{17pt}){3-9}
%         % \cmidrule(l{1pt}r{1pt}){2-3}
%         % % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
%         % \\ 

%         \multirow{2}{*}{ TACO } & DGrasp & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & PPO (Tracking rew.)  & 0.4815 & 7.82  & 0.1195  & 0.4682 & {35.13}/{47.69}/61.54
%         \\ 
        
%         \cmidrule(l{0pt}r{1pt}){2-2}
%         \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}
%         % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
%         % \\ 
%         ~ & \model~(w/ sup.)  &  0.4444 & 2.33  & 0.1782  & 0.5438 & 47.97/67.12/73.66
%         \\ 
%         ~ & \model~(w/ sup., w/ curriculum)  & {0.4854} & {1.99} & { 0.1298} & {0.4772} & 54.90/72.55/79.74
%         \\ 
%         ~ & \model & {0.4953} &  {2.10} & {0.1510} & {0.4661} & \bred{49.02}/\bred{74.50}/\bred{81.05}
%         \\ 

%         \bottomrule
 
%     \end{tabular}
%     }
%     \vspace{-10pt}
%     \label{tb_exp_main}
% \end{table*} 




% \todo{change the w/o prior, w/o curri. to w/o data, w/o structure}
\begin{table*}[t]
    \centering
    \caption{ 
    \footnotesize
    \textcolor{myblue}{\textbf{Quantitative evaluations.}}  \bred{Bold red} and \iblue{italic blue} \textcolor{myblue}{values for best and the second best-performed ones respectively}. 
    \textcolor{myblue}{``Ours (w/o) data'' and ``Ours (w/o data, w/o homotopy)'' are two ablated versions w.r.t. quality of robot tracking demonstrations used in imitation learning (see Section~\ref{sec:ablation_studies} for details). }
    % Demonstrations used in ``Ours (w/o) data'' are not improved by 
    % ``Ours (w/o) data'' uses demonstrations that are not improved by transferring ``tracking prior'', while ``Ours (w/o data, w/o homotopy)'' uses demonstrations neither improved by transferring tracking prior nor via the homotopy optimization scheme.
    % is the ablated version where demonstrations are curated without transferring ``tracking prior'', while ``Ours (w/o data, w/o homotopy)'' uses demonstrations neither improved by transferring tracking prior nor via the homotopy optimization scheme.}
    % numbers for best values and  for the second best-performed ones. 
    } 
    % \vspace{-10pt}
    \resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{\;}llccccc@{\;}}
        \toprule
        %         
        Dataset & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$) \\

        
        \cmidrule(l{0pt}r{1pt}){1-2}
        \cmidrule(l{2pt}r{2pt}){3-7}

        

        % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
        % \\ 
        \multirow{6}{*}{ GRAB } & DGrasp & 0.4493 & 6.75  & 0.1372  & 0.6039 & 34.52/52.79
        \\ 
        ~ & PPO (OmniGrasp rew.) & 0.4404 & 6.69  & 0.1722 & 0.6418  & 35.53/54.82
        \\ 
        ~ & PPO (w/o sup., tracking rew.)  & 0.3945 & 6.11  & \bred{0.1076} & 0.5899 & 38.58/54.82 % & 
        \\ 
        
        \cmidrule(l{0pt}r{1pt}){2-2}
        \cmidrule(l{2pt}r{2pt}){3-7}
        
        
        % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
        % \\ 
        % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
        % \\ 
        ~ & \model~(w/o data, w/o homotopy)  & {0.3443} & {7.81} & {0.1225} & \iblue{0.5218} & 39.59/57.87 
        \\ 
        ~ & \model~(w/o data)  & \iblue{0.3415} & \iblue{4.97} & { 0.1483} & {0.5264} & \iblue{43.15}/\iblue{62.44} % 
        \\ 
        ~ & \model  & \bred{0.3303} & \bred{4.53} & \iblue{0.1118} & \bred{0.5048} & \bred{46.70}/\bred{65.48} 
         \\ 
        
        \cmidrule(l{0pt}r{1pt}){1-2}
        \cmidrule(l{2pt}r{2pt}){3-7}


        % \multirow{5}{*}{ TACO } & ControlVAE & - & -  & -  & - 
        % \\ 
        % ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
        % \\ 
        % % \cmidrule(l{15pt}r{17pt}){3-9}

        % % \cmidrule(l{15pt}r{17pt}){3-9}
        % \cmidrule(l{1pt}r{1pt}){2-3}
        % % \cmidrule(l{2pt}r{2pt}){8-12}


        % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
        % \\ 
        % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
        % \\ 
        % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
        % \\ 

        \multirow{6}{*}{ TACO } & DGrasp & 0.5021 & 5.04  & \bred{0.1129}  &  0.4737 & 38.42/47.78
        \\ 
        ~ & PPO (OmniGrasp rew.) & 0.5174 & 5.43  & 0.1279  & 0.4945 & 33.5/46.31
        \\ 
        ~ & PPO (w/o sup., tracking rew.)  & \iblue{0.4815} & 4.82  & \iblue{0.1195}  & \iblue{0.4682} & {34.98}/{57.64} 
        \\ 
        
        \cmidrule(l{0pt}r{1pt}){2-2}
        \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){3-7}
        % \cmidrule(l{2pt}r{2pt}){8-12}
        % \cmidrule(l{2pt}r{2pt}){1-2}
        % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
        % \\ 
        % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
        % \\ 
        ~ & \model~(w/o data, w/o homotopy)  &  \bred{0.4444} & 2.33  & 0.1782  & 0.5438 & 44.83/67.00
        \\ 
        ~ & \model~(w/o data)  & {0.4854} & \iblue{2.21} & { 0.1698} & {0.4772} & \iblue{47.78}/\iblue{72.41}
        \\  
        ~ & \model & {0.4953} &  \bred{2.10} & {0.1510} & \bred{0.4661} & \bred{48.77}/\bred{74.38}
        \\ 

        \bottomrule
 
    \end{tabular}
    }
    \vspace{-10pt}
    \label{tb_exp_main}
\end{table*} 


% \todo{do not claim the efficiency and jmove the timeconsumption to the appendix}



% \begin{table*}[t]
%     \centering
%     \caption{ 
%     \textbf{Quantitative evaluations and comparisons to baselines.}  \bred{Bold red} numbers for best values and \iblue{italic blue} values for the second best-performed ones. 
%     } 
%     % \vspace{-10pt}
%     \resizebox{1.0\textwidth}{!}{%
% \begin{tabular}{@{\;}lllccccc@{\;}}
%         \toprule
%         %         
%         Dataset & ~ & Method & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

        
%         \cmidrule(l{0pt}r{1pt}){1-3}
%         \cmidrule(l{2pt}r{2pt}){4-8}

%         \multirow{5}{*}{ GRAB } & \multirow{2}{*}{ \makecell[c]{Model \\ Based} } & ControlVAE & - & -  & -  & - 
%         \\ 
%         ~ & ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         \\ 
%         % \cmidrule(l{15pt}r{17pt}){3-9}

%         % \cmidrule(l{15pt}r{17pt}){3-9}
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         ~ & \multirow{2}{*}{ \makecell[c]{Model \\ Free} }  & PPO (OmniGrasp rew.) & - & -  & -  & - & - 
%         \\ 
%         ~ & ~ & PPO (Tracking rew.)  & 0.3945 & 6.11  & 0.1076 & 0.5899 & 38.78/55.05/60.58 
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}

%         % ~ & ~ & Ours (Stage I) & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.3415} & {4.97} & { 0.1483} & {0.5264} & 43.25/58.13/68.51
%         % \\ 
%         ~ & ~ & Ours  & \bred{0.3303} & \bred{4.53} & {0.1118} & \bred{0.5048} & \bred{47.12}/\bred{65.52}/\bred{72.41}
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){1-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}


%         \multirow{5}{*}{ TACO } & \multirow{2}{*}{ \makecell[c]{Model \\ Based} } & ControlVAE & - & -  & -  & - 
%         \\ 
%         ~ & ~ & MPC (w/ QuasiSim Base) & - & -  & -  & - 
%         \\ 
%         % \cmidrule(l{15pt}r{17pt}){3-9}

%         % \cmidrule(l{15pt}r{17pt}){3-9}
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         % \cmidrule(l{2pt}r{2pt}){8-12}


%         % ~ & \multirow{3}{*}{ \makecell[c]{Model \\ Free} } & PPO & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & DGrasp-Tracking & - & -  & -  & - 
%         % \\ 
%         % ~ & ~ & \makecell[l]{OmniGrasp} & - & -  & -  & - 
%         % \\ 

%         ~ & \multirow{2}{*}{ \makecell[c]{Model \\ Free} }  & PPO (OmniGrasp rew.) & - & -  & -  & - 
%         \\ 
%         ~ & ~ & PPO (Tracking rew.)  & 0.4815 & 10.11  & 0.1195  & 0.4682 & {5.13}/{5.13}/61.54
%         \\ 
        
%         \cmidrule(l{1pt}r{1pt}){2-3}
%         \cmidrule(l{1pt}r{1pt}){4-8}
%         % \cmidrule(l{2pt}r{2pt}){3-7}
%         % \cmidrule(l{2pt}r{2pt}){8-12}
%         % \cmidrule(l{2pt}r{2pt}){1-2}
%         % ~ & ~ & Ours (Stage I) & \bred{ 0.5012} & \bred{4.10} & {0.2461} & {0.5771} & 5.12/5.12/61.53
%         % \\ 
%         % ~ & ~ & Ours (Stage II) & {0.4853} & {1.99} & \bred{ 0.1298} & \bred{0.4771} & 44.90/72.54/79.73
%         % \\ 
%         ~ & ~ & Ours & {0.4953} &  {2.10} & {0.1510} & {0.4661} & \bred{49.02}/\bred{74.50}/\bred{81.05}
%         \\ 

%         \bottomrule
 
%     \end{tabular}
%     }
%     \vspace{-10pt}
%     \label{tb_exp_main}
% \end{table*} 




% \begin{figure}[h]
%   \centering
%   % \vspace{-10pt}
%   \includegraphics[width=\textwidth]{figs/res.pdf}
%   % \vspace{-20pt}
%   \caption{
%   \textbf{Qualitative comparisons. }
%   Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig_res_bak}
%   % \vspace{-10pt}
% \end{figure}




% \begin{wraptable}[6]{r}{0.5\textwidth}
% \vspace{-30pt}
%     \centering
%     \caption{ 
%     % \textbf{Ablation studies} on the GRAB dataset. 
%     Total training time consumption (GRAB dataset). 
%     } 
%     % \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccc@{\;}}
%         \toprule
%         ~ & \makecell[c]{PPO \\ (w/o sup)} & \makecell[c]{Ours \\ (w/ sup.)}  & \makecell[c]{Ours \\ (w/ sup., \\ w/ curri.)} & Ours   \\

%         \midrule % 

%         Time  &  $\sim$1 day & $\sim$4.5 days & $\sim$9 days & $\sim$5 days
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_exp_timeconsumption}
% \end{wraptable}





% decompose 

% \todo{which card and the hardware settings}

% We demonstrate the generalization ability of our tracking controller to unseen trajectories involving difficult manipulations and novel, thin objects. Our controller has no difficulty in dealing with very intricate motions involving thin objects, subtle in-hand re-orientations, and expressive functional manipulations. As presented in Table~\ref{tb_exp_main}, we can achieve significantly higher success rates calculated under two thresholds than the best-performed baseline in both two datasets. Figure~\ref{fig_res} illustrates qualitative examples and comparisons. Please check out our website and video for animated results. 
We demonstrate the generalization ability and robustness of our tracking controller on unseen trajectories involving challenging manipulations and novel, thin objects. Our controller has no difficulty in handling intricate motions, subtle in-hand re-orientations, and expressive functional manipulations, even when dealing with thin objects. 
As shown in Table~\ref{tb_exp_main}, we achieve significantly higher success rates, calculated under two different thresholds, compared to the best-performing baseline across both datasets. Figure~\ref{fig_res} provides qualitative examples and comparisons. We show the real-world effectiveness of our method and the superiority over best-performing baselines (Figure~\ref{fig_res},Table~\ref{tb_real_world_results}). For animated results, please visit our \href{https://projectwebsite7.github.io/gene-dex-manip/}{project website} and the \href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{accompanying video}.
% in two HOI datasets. Empowered by xxx, our policy can generalize well and robustly track challenging manipulations unseen during training. Most impressively and perhaps even surprising to us, our policy has no difficulty in dealing with very intricate motions involving thin objects, subtle in-hand re-orientations, and expressive functional manipulations. 



% \textcolor{red}{(TODO: cross-object generalization test? and that should be delivered in a small table)}


% \noindent\textbf{Expressive and functional motions with subtle in-hand re-orientations.} 

\noindent\textbf{Intriguing in-hand manipulations.}
% Expressive motions with s
% ubtle in-hand manipulations.} 
Our method effectively generalizes to novel, complex, and challenging functional manipulations, featured by subtle in-hand re-orientations, essential for precise tool-use tasks. For instance, in Figure~\ref{fig_res}a, the shovel is lifted, tilted, and reoriented with intricate finger movements to complete a {stirring} motion. Similarly, in Figure~\ref{fig_res}c, the small shovel is reoriented using minimal wrist adjustments. These results demonstrate the robustness and generalization of our controller, outperforming the PPO baseline, which struggles with basic lifting. 
% tasks like lifting thin tools.
% including
% complex object movements and 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method effectively generalizes to unseen, challenging manipulations that involve complex functional object movements and subtle in-hand re-orientations, which are crucial for achieving precise reorientations during tool-use tasks. For example, in Figure~\ref{fig_res}a, the shovel must first be lifted with the inner side facing down, then tilted so the inner part faces upward, while the fingers control the handle to complete a \texttt{stirring} motion. Our results nearly achieve this goal, despite the intricate finger movements required to re-orient the object.
% In Figure~\ref{fig_res}c, the trajectory demands that the small shovel be re-oriented to face right so it can be used to hold things. Although our method initially lifts the shovel with the inner side facing left (as shown in the third frame), it successfully re-orients the tool using detailed finger adjustments, with minimal change in wrist orientation (as shown in the fourth frame).
% These results highlight the robust performance and exceptional generalization ability of our controller. In contrast, the best-performing baseline, PPO (w/o sup.), which attempts to train a general controller using our designed rewards, struggles even with basic tasks like lifting thin tools from the table.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalizes well to unseen challenging manipulations involving complex functional object movements, and detailed and subtle in-hand re-orientations that are crucial to achieve correct orientations for accurately mimicking tool-using motions. In Figure~\ref{fig_res}a, the shovel should be lifted at first with the inner side facing towards and then tiled down with the inner part facing upwards and fingers controlling the handle to complete the \texttt{stirring} motion. Our results can almost fulfill the goal despite the need to use detailed finger movements to re-orient the object. As demonstrated in Figure~\ref{fig_res}c, the trajectory requires the hand to make the small shovel face towards the right side so that it can use it to hold things. Despite the fact that our method manage to lift the object up from the table with the object facing towards the left side (shown in the third frame), it can then successfully re-orient the small shovel so that it faces towards the right side mainly using fingers without varying the wrist orientation a lot (as shown in the forth frame). 
% These great performance convincingly demonstrate the strong capability and notable generalization ability of our controller. 
% In comparison to ours' adeptly tracking functional interactions, the best-performed baseline PPO (w/o sup.), which attempts to directly train a general controller using PPO with our carefully designed rewards but without additional guidance, even faces challenges in lifting such thin tools up from the table. 
% However xxx (baseline methods). \todo{baseline's performance}
% Such tool using method demonstrates the high generalizable dexterity enabled by our general tracker. 



% \begin{wraptable}[5]{r}{0.6\textwidth}
% \vspace{-23pt}
%     \centering
%     \caption{ 
%     % \textbf{Ablation studies} on the GRAB dataset. 
%     % \textbf{Generalization ability evaluations} on the TACO dataset. 
%     % \textbf{Gen} on the TACO dataset. 
%     \footnotesize
%     Generalizability evaluations on the TACO dataset. 
%     } 
%     \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{@{\;}lccccc@{\;}}
%         \toprule
%         Test set & \makecell[c]{$R_{\text{err}}$ ($\text{rad}, \downarrow$)} & \makecell[c]{$T_{\text{err}}$ (${cm}, \downarrow$)}  &  $E_{\text{wrist}}$ ($ \downarrow$)  & $E_{\text{finger}}$ ($\text{rad}, \downarrow$) & Success Rate ($\%, \uparrow$)   \\

%         % \\
%         \midrule % 


%         % \\
%         % \cmidrule(l{15pt}r{17pt}){2-4}
        
%         % \model (w/o SpatialDiff) & 2.94 & 3.45  & 31.67
%         % \\ 

%         % \model (w/o TemporalDiff) & \bred{1.72} & \bred{1.90} & 34.25 % 18.65 %
%         % \\

%         % \model (w/o Diffusion) & 3.16 & 3.83  & 18.65 

%         % S0 & {0.3443} & {7.81} & {0.1225} & {0.5218} & 39.79/58.13/66.78
%         % \\
        
%         S1 & 0.5787 & {2.43} & {0.1481} & {0.4703} & 35.97/67.63
%         \\ 

%         % 
%         % \model (w/o Canon.) & {2.36} & {3.57} & \iblue{13.26}
%         S2 & {0.6026} & {2.46} & { 0.1455} & {0.4709} & 30.83/65.00
%         \\ 

%         S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % }
%     % \vspace{-16pt}
%     \label{tb_exp_taco_generalization_test}
% \end{wraptable}



\noindent\textbf{Intricate manipulations with thin objects. } 
Our method also generalizes well to challenging manipulations involving thin objects. In Figure~\ref{fig_res}b, despite the thin \texttt{shovel}'s complexity and missing CAD model parts, our method successfully lifts and controls it using a firm grasp with the second and third fingers. Similarly, in Figure~\ref{fig_res}e, our controller adeptly lifts and manipulates a thin \texttt{flute}, while the best-performing baseline struggles with the initial grasp. These results highlight the advantages of our approach in handling complex and delicate manipulations.
% that are difficult to grasp and control. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalizes effectively to unseen, challenging manipulations involving extremely thin objects that are both difficult to grasp and control. As shown in Figure~\ref{fig_res}b, the shovel is extremely thin, with some triangles missing from the CAD model, which adds to the complexity. Additionally, controlling such a long and thin object from the end further increases the difficulty. Despite these challenges, our method performs well, successfully lifting the object using the second and third fingers while maintaining a firm grip to follow the trajectory, even with this unconventional grasping pose.
% In the scenario depicted in Figure~\ref{fig_res}e, the task involves lifting a notably thin flute from the table and manipulating it. Our controller demonstrates remarkable proficiency in interacting with such objects. In contrast, the best-performing baseline struggles significantly during the initial grasping phase, highlighting the advantages of our approach in handling complex and delicate manipulations.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method generalize well to unseen challenging manipulations involving extremely thin objects that are both difficult to grasp and control. As demonstrated in Figure~\ref{fig_res}b, the shovel is very thin here even with some triangles missing from the CAD model. Besides, controlling such a long and thin object from the end side further adds huge difficulties. Despite such challenges, our method can still generalize well and achieve good performance in this case. It manages to lift the object up using the second and the third fingers and control the hand to firmly hold the objects to follow its trajectory, using this unfriendly grasping pose. 
% In the case drawn in Figure~\ref{fig_res}f, the challenging task involves lifting an extremely thin flute from the table and playing with it. Our controller has no difficulty in interacting with this kind of object. 
% In comparison, the best-performed baseline faces significant challenges in the initial grasping stage. 
% Our controller can even perform robustly in this unfriendly grasping pose, controlling the hand to firmly hold the object and follow its trajectory. 

% complex object movements, extremely thin objects that are very difficult to grasp
% has no difficult in resolving challenging manipulation

% \begin{wrapfigure}[6]{r}{0.45\textwidth} % {0pt}
% \vspace{-4ex}
% \includegraphics[width = 0.45\textwidth]{./figs/real_eval_figs.pdf}
% \vspace{-24pt}
%     \caption{\footnotesize
%     Qualitative results in the real world.
%     }
%     \label{fig:fig_real_eval_figs}
% \vspace{-20pt}
% \end{wrapfigure}


% \todo{add this part}







\begin{table*}[t]
    \centering
    \caption{ \footnotesize
    \textbf{Real-world quantitative comparisons.}  \bred{Bold red} numbers for best values.
    % and \iblue{italic blue} values for the second best-performed ones. 
    } 
    % \vspace{-10pt}
        \resizebox{1.0\textwidth}{!}{%
\begin{tabular}{@{\;}lcccccccccc@{\;}}
        \toprule
       Method & \texttt{apple} & \texttt{banana} & \texttt{duck}  & \texttt{elephant} & \texttt{flashlight}    & \texttt{flute}   & \texttt{hammer}  & \texttt{hand}  & \texttt{phone}  & \texttt{waterbottle}     \\

        % \\
        \midrule % 

        PPO (w/o sup., tracking rew) & 0/0/0 & 25.0/25.0/0.0 & 50.0/25.0/0 & 50.0/0.0/0.0 & 50.0/0/0 & 0/0/0 & 25.0/0/0 & 66.7/33.3/0 & 25.0/0/0 & 33.3/33.3/0
        \\ 

        % 
        \model & \bred{25.0}/0/0 & \bred{50.0}/\bred{50.0}/\bred{25.0} & \bred{75.0}/\bred{50.0}/\bred{25.0} & \bred{75.0}/\bred{50.0}/\bred{50.0} & \bred{50.0}/\bred{25.0}/\bred{25.0}  & \bred{25.0}/\bred{25.0}/\bred{25.0} & \bred{50.0}/\bred{50.0}/\bred{50.0} & \bred{66.7}/\bred{33.3}/\bred{33.3} & \bred{50.0}/\bred{50.0}/\bred{25.0} & \bred{50.0}/\bred{33.3}/\bred{33.3} 
        \\ 

        % S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
        % \\ 
        
        \bottomrule
 
    \end{tabular}
    }
    \vspace{-20pt}
    \label{tb_real_world_results}
\end{table*} 

% % \begin{wraptable}[5]{r}{0.6\textwidth}
% \begin{table*}[t]
% \vspace{-23pt}
%     \centering
%     \caption{ 
%     \footnotesize
%     Generalizability evaluations on the TACO dataset. 
%     } 
%     \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccccccccc@{\;}}
%         \toprule
%        Method & apple & banana & duck  & elephant & flashlight    & flute   & hammer  & hand  & phone  & waterbottle     \\

%         % \\
%         \midrule % 

        
%         PPO (w/o sup., tracking rew) & 0.5787 & {2.43} & {0.1481} & {0.4703} & 35.97/67.63
%         \\ 

%         % 
%         % \model (w/o Canon.) & {2.36} & {3.57} & \iblue{13.26}
%         \model & {0.6026} & {2.46} & { 0.1455} & {0.4709} & 30.83/65.00
%         % \\ 

%         % S3  & {0.6508} & {8.06} & {0.1513} & {0.4683} & 10.18/{46.32}
%         % \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_real_world_results}
% % \end{wraptable}
% \end{table*}


% \begin{figure}[ht]
%   \centering
%   \vspace{-10pt}
%   \includegraphics[width=0.8\textwidth]{figs/real_exp_cmp_3.pdf}
%   \vspace{-20pt}
%   \caption{\footnotesize
%   \textbf{Qualitative real-world evaluations and comparisons. }
%   % Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig:fig_real_eval_figs}
%   \vspace{-10pt}
% \end{figure}
% \vspace{-5pt}

\noindent\textbf{Real-world evaluations and comparisons.} 
% We transfer tracking results directly to the real world to assess tracking quality and also transfer the state-based controller to evaluate its robustness to noises in the state estimator. Success rates are measured under three thresholds and compared with the best baseline. Table~\ref{tb_real_world_results} summarizes per-object success rates averaged over their manipulation trajectories (transferred controller setting). Demonstrated in Figure~\ref{fig_res}f~\ref{fig_res}g, we enable the robot to track complex object movements in real-world scenarios. Further details are in Appendix~\ref{sec:supp_real_world}.
We directly transfer tracking results to the real world to assess tracking quality and evaluate the robustness of the state-based controller against noise in the state estimator. Success rates are measured under three thresholds and compared with the best baseline. Table~\ref{tb_real_world_results} summarizes the per-object success rates averaged over their manipulation trajectories in the transferred controller setting. As demonstrated in Figures~\ref{fig_res}f and \ref{fig_res}g, we enable the robot to track complex object movements and successfully lift a hard-to-grasp round apple in real-world scenarios. While the baseline fails. Further details can be found in Appendix~\ref{sec:supp_real_world}.

% We transfer tracking results directly to the real world to assess tracking quality and evaluate the robustness of the state-based tracker to noise in the state estimator. We measure success rates under three success thresholds for both settings and compare them with the best-performing baseline. Table~\ref{tb_real_world_results} summarizes the performance of the transferred tracker. We report per-object success rates averaged over their corresponding manipulation trajectories. As shown in Figure~\ref{fig_res}f,g, our method enables the robot to successfully track complex object movements in real-world scenarios. Additional details and results are provided in Appendix~\ref{sec:supp_real_world}.
% reports the 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% We directly transfer tracking results to the real world to demonstrate the tracking quality and also transfer the state-based tracker to the real world to evaluate its robustness to noises in the state estimator. We evaluate the success rate under three types of success thresholds for both settings and compare it with the best-performed baseline method. Values reported in Table~\ref{tb_real_world_results} are the per-object success rate averaged over their corresponding manipulation trajectories, achieved via the transferred tracker. As shown in Figure~\ref{fig_res}f,g, our results executed in the real world can successfully let the robot track difficult manipulations with complex object movements. More details and results are deferred to the Appendix~\ref{sec:supp_real_world}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% success rate of each object averaged over the number of manipulation trajectories, 
% and evaluate the success rate. Moreover, we also transfer the state-based tracker to the real world to evaluate its robustness to noises in the state estimator. 




\vspace{-10pt}
\subsection{Further Analysis and Discussions} \label{sec:exp_analysis}
\vspace{-5pt}


\noindent\textbf{Robustness to noise in the kinematic reference motions.} 
% Our method is robust to significant kinematic noise. 
Despite severe hand-object penetrations in Figure~\ref{fig_res}c (frames 2 and 3) and Figure~\ref{fig_res}a (frame 2), the hand still interacts effectively with the object, highlighting the resilience of our tracking controller in challenging scenarios.
% Our method is robust to significant noise in the kinematic motions. For example, even with severe hand-object penetrations occurring in the motions depicted in Figure~\ref{fig_res}c (in the second and third frames) and Figure~\ref{fig_res}a (in the second frame), we can still effectively control the hand to interact correctly with the object. This resilience underscores the effectiveness of our tracking controller in handling challenging scenarios.
% We would not be affected by obvious noise in the kinematic motions. For instance, although there are severe hand-object penetrations in the motion shown in Figure~\ref{fig_res}c (the second and the third frame) and Figure~\ref{fig_res}a (the second frame), we can successfully control the hand to correctly interact with the object. 



% \begin{figure}[ht]
%   \centering
%   \vspace{-10pt}
%   \includegraphics[width=\textwidth]{figs/robustness_2.pdf}
%   \vspace{-20pt}
%   \caption{
%   \textbf{Robustness towards unreasonable references and novel object categories. }
%   Please refer to \textbf{\href{https://projectwebsite7.github.io/gene-dex-manip/}{our website} and {\href{https://projectwebsite7.github.io/gene-dex-manip/static/videos-lowres/video_7.mp4}{\textcolor{orange}{the accompanying video}}}} for animated results.
%   }
%   \label{fig_res_robustness}
%   \vspace{-10pt}
% \end{figure}





\noindent\textbf{Robustness to unreasonable references. }
As shown in Figure~\ref{fig_res_robustness}, our method remains unaffected by significant noise in the kinematic references with unreasonable states.
% , even when they include unreasonable or unreachable states.
We effectively track the entire motion trajectory, demonstrating the controller's robustness in handling unexpected noise.
% As shown in Figure~\ref{fig_res_robustness}a, our method remains unaffected by significant noise in the kinematic references, even when they include unreasonable or unreachable states. We can effectively track the entire motion trajectory despite these challenges, demonstrating our controller's robustness in handling unexpected noise. 
% The kinematic reference trajectory is obtained by interpolating a different trajectory from the TACO dataset, demonstrating our controller's robustness in handling complex and noisy inputs.
% As demonstrated in Figure~\ref{fig_res_robustness}a, we would not be affected by the large noise in the kinematics references containing unreasonable and unreachable states and can still manage to track the whole motion trajectory. The kinematic reference trajectory is obtained by interpolating a different trajectory with a sequence from TACO. 
% \todo{xxx}




% \noindent\textbf{Further generalization ability evaluations.}
% We further evaluate the model's generalization ability across various test sets within the TACO dataset. As shown in Table~\ref{tb_exp_taco_generalization_test}, the controller performs well in the category-level generalization setting (S1), where object categories are known but manipulation trajectories and object geometries are novel. Performance on S2, involving novel interaction triplets, is satisfactory, demonstrating the controller's capacity to handle new manipulation sequences. However, results from S3 reveal challenges when dealing with new object categories and unseen interaction triplets. For instance, generalizing from interactions with shovels and spoons to using bowls for holding objects is particularly difficult. As shown in Figure~\ref{fig_res_robustness}b, despite unfamiliar objects and interactions, we successfully lift the knife and mimic the motion, though execution is imperfect, highlighting areas for improvement and adaptability in challenging scenarios.

% We further evaluate the model's generalization ability across different levels of test sets within the TACO dataset. As shown in Table~\ref{tb_exp_taco_generalization_test}, the controller performs well in the category-level generalization setting, where the object category is known during training, but the manipulation trajectories and object geometries are novel, as evidenced by its strong performance on test set S1.
% The performance on S2, which involves novel interaction triplets, remains relatively satisfactory, demonstrating the controller's capacity to generalize to new manipulation sequences. However, results from S3 highlight the challenges faced when dealing with novel object categories and unseen interaction triplets. For instance, generalizing from interactions that involve lifting and waving shovels and spoons to using bowls for holding objects proves to be too difficult for the current design. 
% As illustrated in Figure~\ref{fig_res_robustness}b, despite the unfamiliar object category and interaction triplet, we still manage to lift the knife and mimic the intended motion, although the execution is not perfect. This indicates potential areas for improvement while showcasing the model's adaptability in challenging scenarios.

% We further test the model's generalization ability on different levels of test sets on the TACO dataset. As indicated in Table~\ref{tb_exp_taco_generalization_test}, the controller can perform well in the category-level generalization setting, where the object category is observed during the training while the manipulation trajectories and the object geometry are novel, as indicated by its good performance in the test set S1. 
% The performance on S2 contains novel interaction triples is still relatively satisfactory, indicating its ability to generalize to control novel manipulation sequences. However, results on S3 indicate the model's being challenged by novel object categories and unseen interaction triplets. Generalizing from interactions demonstrating lifting and waving shovels and spoons to using bowls to hold things is still too challenging for the current design. As shown in Figure~\ref{fig_res_robustness}b, given the unobserved object category and the interaction triplet, though not perfect, we can still manage to lift the knife up and mimic the motion. 
% \todo{add the qualitative evals}
% The object position error is still kept to a small value, indicating 

% Specifically, the whole dataset is split into a training dataset, containing 1565 trajectories, and the test set S0 where both the tool object geometry and the interaction triplets are seen during training, the test set S1 where the tool geometry is novel but the interaction triplets are seen during training, the test set S2 with novel interaction triplets but seen object categories and geometries, and the test set S4 with new object geometries and interaction triplets. Details w.r.t. the dataset splitting and visualizations are deferred to Appendix~\ref{}. 

% \begin{wraptable}[6]{r}{0.5\textwidth}
% \vspace{-30pt}
%     \centering
%     \caption{ 
%     Total training time consumption (TACO dataset). 
%     } 
%     % \vspace{5pt}
% 	% \resizebox{\linewidth}{!}{%
%     \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{@{\;}lcccc@{\;}}
%         \toprule
%         ~ & \makecell[c]{PPO \\ (w/o sup)} & \makecell[c]{Ours \\ (w/ sup.)}  & \makecell[c]{Ours \\ (w/ sup., \\ w/ curri.)} & Ours   \\

%         \midrule % 

%         Time  &  $\sim$1 day & $\sim$5 days & $\sim$13 days & $\sim$4 days
%         \\ 
        
%         \bottomrule
 
%     \end{tabular}
%     }
%     % \vspace{-16pt}
%     \label{tb_exp_timeconsumption}
% \end{wraptable}


% \noindent\textbf{Time consumption.} Table~\ref{tb_exp_timeconsumption} summarizes the total time consumption of different methods on the TACO dataset. Directly training PPO without any supervision is the most efficient approach while the performance lagged behind due to no proper guidance. Exact curriculum learning for acquiring high-quality per-trajectory trackers, though as we observe in Table~\ref{tb_exp_main}, is an effective strategy, which also aligns with conclusions in previous approaches, is extremely time-consuming. For 400 trajectories that we finally select to optimize to produce an action-labeled dataset, searching the exact curriculum costs about 13 days to complete. However, our method requires only slightly more time than the version without tracking prior or curriculum scheduling (Ours w/ sup.). However we can achieve a much higher success rate than this version, taking advantage of the increased diversity and the quality of action-labeled data. 




\vspace{-10pt}
\section{Ablation Studies} \label{sec:ablation_studies}
\vspace{-5pt}


\noindent\textbf{Diversity and quality of robot tracking demonstrations.} 
We propose enhancing the diversity and quality of tracking demonstrations using the tracking controller and homotopy generator. We ablate these strategies by creating two variants: ``Ours (w/o data, w/o homotopy)'', where the dataset is built by optimizing each trajectory without prior knowledge, and ``Ours (w/o data)'', which uses only the homotopy optimization scheme to improve demonstrations. Despite using the same number of demonstrations, both variants produce lower-quality data. As shown in Table~\ref{tb_exp_main}, they underperform compared to our full method, underscoring the importance of data quality in training the controller.
% We propose to improve the diversity and the quality of the robot tracking demonstrations via the tracking controller and the homotopy generator. We ablate these two strategies by creating two variants: ``Ours (w/o data, w/o homotopy)'', where the dataset is built by directly optimizing each trajectory without prior knowledge, and ``Ours (w/o data)'', where we only leverage the homotopy optimization scheme to improve demonstrations. Both strategies, despite using the same amount of demonstrations, result in lower data quality. As shown in Table~\ref{tb_exp_main}, they underperform compared to our full method, highlighting the importance of data quality in training the controller.
% 
% where optimization combines trajectory-specific efforts with the controller's tracking prior.
% We propose transferring tracking knowledge from the controller and curriculum before optimization to handle more difficult and diverse trajectories in the dataset. We ablate these strategies 
% We propose to transfer general tracking knowledge encoded in the tracking controller and the curriculum prior to the optimization process for solving difficult-to-solve problems so that we can include more difficult and diverse labeled trajectories into the dataset. We've tried to ablate such two strategies and create ``Ours (w/o data, w/o structure)'' where the final labeled dataset is created by directly optimizing each trajectory without any prior from the tracking controller or the curriculum scheduler, and ``Ours (w/o data)'' where each trajectory is optimized under the joint effort of the per-trajectory tracking optimization and the tracking prior provided by the tracking controller. Such two strategies, though using the same amount of labeled data as our full method to provide supervision, may fall short in the data quality aspect. As shown in Table~\ref{tb_exp_main}, they would lag behind our full version, illustrating the role of data quality in training the tracking controller. 
% This approach can potentially let us get better per-trajectory tracker under expansive tracking curriculum trail-and-error. However, it is extremely time-consuming and unaffordable. As presented in Table~\ref{tb_exp_main}, Ours (w/ sup.), as restricted by the quality and the diversity of the action-labeled data, typically lags behind our full method on both the GRAB dataset and the TACO dataset. It validates the importance of data quality and coverage used to train the tracking controller. Ours (w/ sup., w/ curriculum) leverages the power of curriculum learning and the benefit of per-trajectory searched accurate curriculum, and can sometimes outperform out proposed strategy, which uses the tracking controller to provide tracking priors and the curriculum scheduler to propose the tracking schedule for tracking difficult trajectories. However, leveraging this approach is highly time-consuming, and would become extremely unaffordable when the number of data increases. Our proposed strategy can not only effectively improve the data quality, but smartly reduces the time consumption. 
% using per-trajectory tracking optimization and the tracking prior from the tracking controller. 
% optimized with per-trajectory searched curriculum, other than the curriculum planned by the scheduler. 
% This demonstrate the effectiveness of the tracking curriculum and the quality of our mined curricula. 
% typically lags behind our full method,
% \todo{xxxx} 
% \todo{for the curriculum, say that the trajectories between TACO is a little bit similar so we can observe the the one with exact curriculum can achieve better performance some times}


\begin{wrapfigure}[13]{r}{0.45\textwidth} % {0pt}
\vspace{-3ex}
\includegraphics[width = 0.45\textwidth]{./figs/scaling.pdf}
\vspace{-30pt}
    \caption{\footnotesize
    Scaling the amount of demonstrations.
    }
    \label{fig:fig_scaling}
% \vspace{-30pt}
\end{wrapfigure}

\vspace{-5pt}
\noindent\textbf{Scaling the number of demonstrations.} 
To investigate the relationship between the tracking controller's performance and the number of demonstrations, we vary the size of the demonstration dataset during training and tested performance on the TACO dataset. Specifically, in the final training iteration, we down-sampled the dataset to 0.1, 0.3, 0.5, and 0.9 of its original size and re-trained the model. As shown in Figure~\ref{fig:fig_scaling}, there is a clear correlation between the amount of demonstrations and model performance. Since the curve has not plateaued, we hypothesize that increasing the amount of high-quality data could further improve performance.
% general tracking controller's performance and the amount of labeled data, 
% To explore the relation between the performance of the general tracking controller and the number of labeled data, we try to vary the number of final labeled data to train the model and test the model's performance on the TACO dataset. To be more specific, in the last training iteration, we try to down-sample the \emph{final action-labeled dataset} into $0.1, 0.3, 0.5, 0.9$ of its original size and re-train the model. As summarized in Figure~\ref{fig:fig_scaling}, there exists an obvious relation between the amount of labeled data used for training and the model's performance. Besides, the curve has not yet reached a flat raising mode in our trails. So we hypothesize that our method's performance could still be enhanced if we can manage to create more high-quality data to train the general tracking controller. 
 
% \todo{a scaling law that demonstrate the role of the data } 

% \todo{time consumption and the time efficiency}


\vspace{-10pt}
% \todo{repro statement}



==> articles_revision/intro.tex <==
\section{Introduction}
Robotic dexterous manipulation refers to the ability of a robot hand skillfully handling and manipulating objects for various target states with precision and adaptability. This capability has attracted significant attention because adept object manipulation for goals such as tool use is vital for robots to interact with the world. Many efforts have been devoted previously to push the ability of a dexterous hand toward human-level dexterity and versatility~\citep{rajeswaran2017learning,chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact,liu2024quasisim,Li2024ReinforcementLF}. This also aligns with our vision. 

Achieving human-level robotic dexterous manipulation is challenging due to two main difficulties: the intricate dynamics of contact-rich manipulation, which complicates optimization~\citep{pang2021convex,pang2023global,liu2024quasisim,Jin2024ComplementarityFreeMM}, and the need for robots to master a wide range of versatile skills beyond specific tasks. Previous approaches mainly resort to model-free reinforcement learning (RL)~\citep{chen2023visual,chen2021system,akkaya2019solving,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi} or model-based trajectory optimization (TO)~\citep{pang2021convex,pang2023global,Jin2024ComplementarityFreeMM,hwangbo2018per}. While RL requires task-specific reward designs, limiting its generalization, TO depends on accurate dynamics models with known contact states, restricting adaptability to new objects and skills. A promising alternative is to leverage human hand-object manipulation references, widely available through videos or motion synthesis, and focus on controlling a dexterous hand to track these references. This approach separates high-level task planning from low-level control, framing diverse skill acquisition as the development of a universal tracking controller.
However, challenges remain due to noisy kinematic references, differences in morphology between human and robotic hands, complex dynamics with rich contacts, and diverse object geometry and skills.
Existing methods struggle with these issues, often limiting themselves to simple tasks without in-hand manipulation~\citep{christen2022d,zhang2023artigrasp,wu2023learning,xu2023unidexgrasp,Luo2024GraspingDO,Singh2024HandObjectIP,Chen2024ViViDexLV} or certain specific skills~\citep{qin2022dexmv,liu2024quasisim,rajeswaran2017learning}.

In this work, we aim to develop a general-purpose tracking controller that can follow hand-object manipulation references across various skills and diverse objects. In particular, given a collection of kinematics-only human hand-object manipulation trajectories, the controller is optimized to drive a robotic dexterous hand to manipulate the object so that the resulting hand and object trajectories can closely mimic their corresponding kinematic sequences. 
We expect the tracking controller to exhibit strong versatility, generalize well to precisely track novel manipulations, and have strong robustness towards large kinematics noises and unexpected reference states. 


To achieve the challenging goal above, we draw three key observations: 1) learning is crucial for handling heterogeneous reference motion noises and transferring data prior to new scenarios, supporting robust and generalizable tracking control; 2) leveraging large-scale, high-quality robot tracking demonstrations that pair kinematic references with tracking action sequences can supervise and significantly empower neural controllers, as demonstrated by data-scaling laws in computer vision and NLP~\citep{Achiam2023GPT4TR,Brown2020LanguageMA}; 3) acquiring large and high-quality tracking demonstrations is challenging but we could utilize the data flywheel~\citep{Chiang2024ChatbotAA,Bai2023QwenTR} to iteratively improve the tracking controller and expand the demonstrations in a bootstrapping manner.


Based upon the previous observations, we propose \modelnamenspace, a novel neural tracking controller for dexterous manipulation, guided by human references. Specifically, given a collection of human hand-object manipulation trajectories, we first retarget the collection to kinematic robotic dexterous hand sequences to form a set of reference motions as data preparation. Our method then alternates between mining successful robot tracking demonstrations and training the controller with the mined demonstrations. To make sure the data flywheel functions effectively, we introduce two key designs. First, we carefully integrate reinforcement and imitation learning techniques to train a neural controller, ensuring its performance improves with more demonstrations while maintaining robustness against unexpected states and noise. Second, we develop a per-trajectory tracking scheme that uses the trained controller to mine diverse and high-quality tracking demonstrations through a homotopy optimization method. The scheme transfers the tracking prior from the controller to individual trajectories to ease per-trajectory tracking for better demonstration quality. Moreover, the scheme will convert a tracking reference into a series of gradually simplified reference motions so that tracking these references from simple to complex could help better track the original reference motion. This is akin to chain-of-thought and is very suitable for tracking complex reference motions to increase the demonstration diversity. The two designs above together with the iterative training enable \modelname to successfully track novel and challenging human references.


We demonstrate the superiority of our method and compare it with previous methods on challenging manipulation tracking tasks in two datasets, describing expressive hand-object interactions in daily and functional tool-using scenarios, involving complex object movements, difficult and subtle in-hand re-orientations, interactions with thin objects, and frequent hand-object rich contact variations. 
% We both conduct extensive experiments in the simulator, \emph{i.e.,} Isaac Gym~\citep{makoviychuk2021isaac}, to demonstrate the efficacy, generalization ability, and robustness of our tracker to accomplish a wide range of manipulation tracking tasks and even excellently track novel manipulation trajectories, and evaluate 
We conduct both extensive experiments in the simulator, \emph{i.e.,} Isaac Gym~\citep{makoviychuk2021isaac}, and evaluations in the real world, to demonstrate the efficacy, generalization ability, and robustness of our tracker to accomplish a wide range of manipulation tracking tasks and even excellently track novel manipulation trajectories (Figure~\ref{fig_intro_teaser}).
% both conduct 
% We conduct experiments in both the simulator, \emph{i.e.,} Isaac Gym~\citep{makoviychuk2021isaac},  and the real world to demonstrate the efficacy, generalization ability, and robustness of our tracker to accomplish a wide range of manipulation tracking tasks and even excellently track novel manipulation trajectories (Figure~\ref{fig_intro_teaser}). 
% We can track difficult manipulations involving expressive and complex object movements, detailed and subtle in-hand re-orientations, and frequent rich hand-object contact variations.
Our approach successfully surpasses the previous methods both quantitatively and qualitatively, achieving more than 10\% success rate than the previous best-performed method. Besides, we conduct further analysis and demonstrate the various recovery behaviors of our controller, demonstrating its robustness to unexpected situations. Thorough ablations are conducted to validate the efficacy of our designs.

Our contributions are threefold:
\begin{itemize} % [noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=.5cm]
    \item We present a generalizable neural tracking controller that progressively improves its performance through iterative mining and incorporating high-quality tracking demonstrations.
    \item We introduce a training method that synergistically combines reinforcement learning and imitation learning. This approach leverages abundant high-quality robot tracking demonstrations to produce a controller that is generalizable, versatile, and robust.
    \item We develop a per-trajectory optimization scheme that employs our tracking controller within a homotopy optimization framework. We propose a data-driven way to generate homotopy paths, enabling solving challenging tracking problems.
\end{itemize}





==> articles_revision/method.tex <==

% \section{Generalizable Dexterous Manipulation Tracking}
% \section{Dexterous Manipulation Tracking Control}
% \section{Generalizable Neural Tracking Control for Dexterous Manipulation}
\section{Method} \label{sec:method_sec}

\vspace{-5pt}

% \todo{add the retargeting part}
 

\begin{figure}[h]
  \centering
  \vspace{-10pt}
  \includegraphics[width=\textwidth]{figs/methdo_rb_8.pdf}
  \vspace{-20pt}
  \caption{\footnotesize
  % cks the potential for tr
  % Generalizable Dexterous Manipulation Tracking with Imitation Augmented RL and Structural Task Space Modeling. 
  % Dexterous Manipulation Tracking Control.
  % Iterative optimization to train a universal dexterous manipulation tracking controller. 
  % By augmenting RL with guidance from high-quality action-labeled data, \modelname unleashes the possibility of training a universal manipulation controller from human references. With the curriculum proposed by a curriculum scheduler that models the tracking curricula and the tracking prior provided by the tracking controller, we can in turn improve the quality of action-labeled trajectories. We adopt an interactive approach which finally offers us a universal tracking controller. 
  % \modelname unleashes the possibility of training a universal manipulation controller from human references by iteratively optimizing high-quality action-labeled trajectories and training the tracking controller via imitation-augmented RL with supervision from the labeled trajectories. Guiding RL with additional supervision from high-quality action-labeled data, \modelname effectively eases the difficulty in learning a universal tracking controller. Leveraging the tracking prior from the controller as well as the tracking curriculum proposed by a learned curriculum scheduler, we can effectively improve the quality and diversity of the action-labeled trajectories. 
  % \eric{The figure is not quite intuitive so far at the tracking prior part and the homotopy optimization part. I would suggest using a flow chart instead. I do not like the way how we visualize learning a neural network with PPO since it is not common and can not be understood immediately. We should consider checking other papers and borrowing their ways of illustration.}
  \textcolor{myblue}{\href{https://projectwebsite7.github.io/gene-dex-manip/}{\modelname} }
  % \href{https://projectwebsite7.github.io/gene-dex-manip/}{\modelname}
  learns a generalizable neural tracking controller for dexterous manipulation from human references. It alternates between training the tracking controller using abundant and high-quality robot tracking demonstrations and improving the data
  % the data
  % the data diversity and quality
  via the tracking controller through a homotopy optimization scheme.
  % By gradually optimizing the tracking controller and curating high-quality demonstration data in a bootstrapping manner, we can get a versatile, generalizable, and robust tracking controller finally. 
  % imitation-ready data 
  % unlocks the potential for training a universal manipulation controller from human references by iteratively curating high-quality, action-labeled trajectories and training the tracking controller through imitation-augmented reinforcement learning (RL) with supervision from these labeled trajectories. By guiding RL with supervision from the action-labeled data, we significantly reduce the challenges associated with learning a universal tracking controller. Utilizing the tracking prior from the controller and a tracking curriculum designed by a learned curriculum scheduler, we effectively enhance the quality and diversity of the action-labeled trajectories, driving improved performance.
  % The \textbf{parameterized quasi-physical simulator} relaxes the articulated multi rigid body dynamics as the \textit{parameterized point set dynamics}, 
  % controls the contact behavior via an unconstrained \textit{parameterized spring-damper contact model},
  % and compensates for unmodeled effects via \textit{parameterized residual physics networks}. 
  % We tackle the difficult dexterous manipulation transfer problem via \textbf{a physics curriculum}. 
  }
  \vspace{-15pt}
  \label{fig_method_pipeline}
\end{figure}

% \todo{change t to n}

% \todo{robot hand-obj kinematics dataset}

% (\emph{e.g.,} Allegro, LEAP, Shadow hand, etc.)

% The dexterous manipulation tracking control problem wishes to learn a tracking controller for a dexterous robot hand from human hand-object manipulation references. Given a manipulation sequence $(\mathbf{H}, \mathbf{O})$ describing the dexterous robot hand interacting with an object, \emph{e.g.,} obtained by kinematic retargeting from a human-object manipulation sequence, we expect the controller to robustly control the robot hand to manipulate the object so that both the resulting hand poses $\hat{\mathbf{H}}$ and the object poses $\hat{\mathbf{O}}$ can properly mimic their corresponding reference motions. We expect the controller to be able to track novel reference motions with unseen yet still challenging manipulation sequences and new objects. Such an ambitious vision is challenged by 1) the inherent difficulty underlying the tracking control problem resulting from intricate dynamics coming from frequently varying rich hand-object contacts and the complicated object movements, 2) the challenges in controlling a high-DoF dexterous robot hand to densely follow references, 3) the wish for a general tracking controller that can universally track every reference manipulations covering extremely challenging cases, and 4) the wish in high robustness and generalization ability side so that the controller can adapted to mimic unobserved references. 
% 

% The generalizable neural tracking control for dexterous manipulations from human references aims to leverage abundant and high-quality human-object interaction data to learn a generalizable manipulation tracking controller to equip a dexterous robot hand with versatile dexterous manipulation ability. Given a human-object interaction dataset containing, the tracking controller learns to track every manipulation sequence. At the test time, the tracking controller ought to generalize well to track novel, challenging human manipulation sequences with new objects, unseen hand, and object reference trajectories. Both advanced model-free RL based techniques and the model-based trajectory optimization would usually face significant challenges from the wish in the versatility and the generalization ability, the complex system, and the intricate dynamics from dynamic, rich contacts. 


% The problem is inherently difficult due to 1) the intricate dynamics involved in the dexterous manipulation that frequently challenges the optimization, 2) the high expectation in the versatility, high generalization ability, and the robustness of the controller. 

\textcolor{myblue}{\noindent\textbf{Terminologies and notations.} 
% Assuming a kinematic-only hand object state sequence, dexterous manipulation ``tracking'' means physically controlling a dexterous hand to interact with an object where the resulting state trajectory should be similar to the given goal trajectory. We use ``kinematic reference(s) (trajectories/sequences)'' to denote the kinematic-only robot hand-object state sequences retargeted from human hand-object manipulation trajectories. Each kinematic reference trajectory, denoted as  $\{ \hat{\mathbf{s}}_n \}_{n=0}^{N}$, is composed of the robot hand joint state and the object pose at each timestep $n$, \emph{i.e.,} $\hat{\mathbf{s}}_n$. A robot ``tracking demonstration'' is composed of a kinematic reference trajectory $\{ \hat{\mathbf{s}}_n \}$ and an expert action sequence for the robot hand $\{ \mathbf{a}_n^L \}$. By starting from the first frame $\mathbf{s}_0=\hat{\mathbf{s}}_0$ and controlling the robot hand using the corresponding action at each frame $\mathbf{a}_n^L$, the robot hand and object transit to the next state $\mathbf{s}_{n+1}$ according to the environment dynamics. An expert action trajectory should make sure the resulting transited state sequence $\{ \mathbf{s}_n \}_{n=0}^N$ close to the kinematic reference $\{\hat{\mathbf{s}}_n\}_{n=0}^N$. We use ``single trajectory tracking policy'' and ``trajectory-specific tracking policy'' to represent the policy that is only responsible for tracking one single trajectory. While ``neural tracking controller'' means a general tracking policy that is expected to track a diverse set of trajectories and can generalize to track new ones. 
% We say a neural controller is ``robust'' if it is resilliance towards distrubances such as large noises in the kinematic references like penetrations and unreachiable states~\citep{Li2024ReinforcementLF,Serifi2024VMPVM}. The neural tracking controller can ``generalize'' if it remains effective on unseen test scenarios involving new objects as well as unseen hand and object motions~\citep{Luo2024GraspingDO,xu2023unidexgrasp,wan2023unidexgrasp2}. The controller is with high ``adaptivity'' if it can still perform well as time-varying or time-invariant context has shifted, such as the changing contact events and varied dynamics parameters~\citep{Li2024ReinforcementLF,Qi2022InHandOR}.
% Assuming a kinematic-only hand-object state sequence, dexterous manipulation ``tracking'' involves controlling a dexterous hand to interact with an object such that the resulting state trajectory matches the goal trajectory. ``Kinematic references'' refer to robot hand-object state sequences retargeted from human manipulation trajectories, denoted as $\{\hat{\mathbf{s}}_n\}_{n=0}^N$, where $\hat{\mathbf{s}}_n$ includes the robot hand joint state and object pose at each timestep $n$. 
% A ``tracking demonstration'' consists of a kinematic reference $\{\hat{\mathbf{s}}_n\}$ and an expert action sequence $\{\mathbf{a}_n^L\}$. Starting from $\mathbf{s}_0=\hat{\mathbf{s}}_0$, the robot uses $\mathbf{a}_n^L$ at each step to transition states $\mathbf{s}_{n+1}$. 
% An ``expert action sequence'' should ensure the resulting state sequence $\{\mathbf{s}_n\}_{n=0}^N$ aligns with $\{\hat{\mathbf{s}}_n\}_{n=0}^N$. 
% A robust controller tolerates disturbances like kinematics noise and unreachable states~\citep{Li2024ReinforcementLF,Serifi2024VMPVM}. It demonstrates generalization if it performs well on unseen objects, motions, and scenes~\citep{Luo2024GraspingDO,xu2023unidexgrasp,wan2023unidexgrasp2}, and high adaptivity if it maintains performance despite shifting contexts, such as changing contact events or dynamics parameters~\citep{Li2024ReinforcementLF,Qi2022InHandOR}.
% A ``single trajectory tracking policy'' tracks one specific trajectory, while a ``neural tracking controller'' is a general policy capable of handling diverse trajectories and generalizing to new ones. 
Dexterous manipulation ``tracking'' involves controlling a robotic hand to mimic a kinematic hand-object state sequence, the goal trajectory, denoted as $\{\hat{\mathbf{s}}_n\}_{n=0}^N$. These ``kinematic references''  are retargeted from human manipulation trajectories, with $\hat{\mathbf{s}}_n$ representing the robot hand state and object pose at timestep $n$. A ``tracking demonstration'' pairs a kinematic reference $\{\hat{\mathbf{s}}_n\}$ with an expert action sequence $\{\mathbf{a}_n^L\}$, guiding the robot from $\mathbf{s}_0=\hat{\mathbf{s}}_0$ to achieve a state sequence $\{\mathbf{s}_n\}_{n=0}^N$ aligned with $\{\hat{\mathbf{s}}_n\}_{n=0}^N$. A ``robust'' controller can tolerate disturbances like kinematics noise and unreachable states. It demonstrates high ``generalization ability'' if it performs well on unseen scenarios such as new objects and novel motions, and has ``adaptivity'' if it maintains effectiveness despite shifting contexts, such as changing contacts and dynamics.
% generalize to unseen scenarios, and adapt to context shifts such as changing contact events or dynamics parameters.
}

% We use tracking prior to denote the 
% Starting from the first frame $\mathbf{s}_n$ and rollouting 
% is composed of a robot hand joint state sequence and an object pose trajectory. We use $\{ \hat{\mathbf{s}}_n \}_{n=0}^{N}$ to denote the a kinematic reference 
% a robot hand state sequence in the joint space and an object pose 
% In each tiemstep $n$, 
% we use $\mathbf{s}_n$ to denote the current state, including the robot joint states and the object pose, 
% current robot hand state (in the joint space) and the object pose 
% In each tiemstep $n$, the tracking controller/policy observes the current state $\mathbf{s}_n$, composed of the robot hand joint states and the object pose, and the goal state that we expect the hand and object to achieve in the next timestep, represented as $\hat{\mathbf{s}}_{n+1}$. It then output  
% robot hand and object state, denoted as $\mathbf{s}_n$, and the goal state that we expect the hand and object to achieve in the next timestep, represented as $\mathbf{}$ 

Given a collection of kinematic human-object manipulation trajectories, we wish to learn a generalizable neural tracking controller for a dexterous robotic hand. 
% and robust 
% versatile, 
% from these references.
% We expect the controller to equip the robot hand with a wide range of manipulation skills and also generalize well to robustly track novel and challenging manipulation tasks.
% a wide range of manipulation skills and also generalize well to robustly track novel and challenging manipulation tasks.
% tackle  novel and challenging manipulation tasks.
% track novel and challenging manipulations. 
% track 
% novel manipulation sequences with unseen object geometries and challenging, subtle in-hand manipulations. 
% to be able to 
% The problem is inherently difficult because: 1) the complex dynamics of dexterous manipulation challenge precise control, which is crucial for delicate motions; 2) there are high expectations for the controller's adaptability, generalizability, and robustness.
\textcolor{myblue}{
The problem is challenging due to the difficulty in precise dexterous manipulation, which is challenged by the underlying complex dynamics, and the high demands for the controller's generalizability and robustness.
}

% controller adaptability, generalizability, and robustness.
% diverse 

% given a collection %


% \todo{exisitng methods?}
% dyanmcis 
% The problem is challenged by the 
% Either previous model-free techniques or model-based approaches 
% various novel manipulation 
% should be able to track 
% We expect the controller can not only track every manipulation sequence in the c
% with the aim to equipping a dexterous robot hand with versatile dexterous manipulation skills. We expect the tracking controller 
% generalizable neural tracking control 
% human-object interaction dataset c


% To overcome these challenges, the key of our method lies in 
% Our method 

% We propose a method that combines reinforcement learning (RL) with imitation learning (IL) to train a generalizable tracking controller using robot tracking demonstrations. Since acquiring high-quality demonstrations with paired kinematics and action sequences is challenging, we introduce a per-trajectory tracking scheme that enhances demonstration quality and diversity via homotopy optimization. By alternating between training the controller with high-quality data and generating improved demonstrations in a bootstrapping process, we develop an effective tracking controller. Detailed explanations of these steps are provided in Sections~\ref{sec:method_il_rl},~\ref{sec:method_data}, and~\ref{sec:method_iteration}.


% To address these challenges, we propose to combine reinforcement learning (RL) and imitation learning (IL) to train a generalizable tracking controller, 
% % Since acquiring 
% % guiding the policy exploration via supervision from high-quality and 
% % empowering it with both the robustness to external disturbances benefiting from RL and
% % jointly via RL objectives and supervision from high-quality and diverse 
% % using robot tracking demonstrations. 
% \textcolor{myblue}{jointly easing the difficulty in solving the complex problem via supervision from high-quality and diverse robot tracking demonstrations and improving the policy's robustness via RL explorations. Since acquiring high-quality demonstrations with paired kinematics and action sequences is challenging, we introduce a tracking demonstration mining scheme. For each single kinematic reference trajectory, we basically leverage RL to train a trajectory-specific tracking policy, aiming to infer an action trajectory that can control the robotic hand to track the reference trajectory. Since the capability of single trajectory tracker would be limited by the RL's ability, we propose to leverage the tracking controller through a homotopy optimization scheme to enhance the demonstration quality and diversity. By iteratively mining high-quality and diverse demonstrations and training the controller with demonstrations that are gradually getting improved in a bootstrapping manner, we eventually develop an effective tracking controller. }

\textcolor{myblue}{
We address these challenges by combining reinforcement learning (RL) and imitation learning (IL) to train a generalizable tracking controller, jointly easing the difficulty in solving the complex problem via supervision from high-quality and diverse robot tracking demonstrations and improving the policy's robustness via RL explorations. We introduce a single trajectory tracking scheme to mine tracking demonstrations, composed of paired kinematic references and action sequences.
For each kinematic reference, we use RL to train a trajectory-specific policy that generates actions to track the reference. To overcome RL's limitations, we propose to leverage the tracking controller through a homotopy optimization scheme to enhance the demonstration quality and diversity. By iteratively mining better demonstrations and refining the controller in a bootstrapping manner, we develop an effective, generalizable tracking controller.
% To obtain paired kinematics and action sequences in the tracking demonstrations, we introduce a tracking demonstration mining scheme. 
}
% \textcolor{myblue}{}
% 0enhance demonstration quality and diversity via the tracking controller through a homotopy optimization scheme. 
% We basically leverage RL to train a 
% per-trajectory tracking demonstration mining sche
% introduce a per-trajectory tracking scheme that enhances demonstration quality and diversity via the tracking controller through a homotopy optimization scheme. 
% By alternating between training the controller with high-quality data and generating improved demonstrations in a bootstrapping process, we develop an effective tracking controller.
We will explain how we learn the neural tracking controller from demonstrations in Section~\ref{sec:method_il_rl}, how we mine high-quality demonstrations in Section~\ref{sec:method_data}, and how we iterate between learning controller and mining demonstrations in Section~\ref{sec:method_iteration}. 
% We will discuss how we learn the neural tracking controller from demonstrations in Section~\ref{sec:method_il_rl}, mining high-quality demonstrations in Section~\ref{sec:method_data}, and iterating between learning and mining in Section~\ref{sec:method_iteration}.
% we propose to learn from a large number of robot tracking demonstrations and combine reinforcement learning (RL) with imitation learning (IL) to effectively train the tracking controller.

% a method that combines 
% in detail 
% homotopy optimization.
% Since obtaining high-quality dexterous manipulation tracking demonstrations with paired kinematics references and action sequences is difficult, we devise a per-trajectory tracking scheme where we improve the quality and diversity of demonstration data via the tracking controller through a homotopy optimization scheme. 
% We then alternate between training the tracking controller using high-quality demonstrations and curating more diverse and higher-quality demonstrations in a bootstrapping manner, ultimately developing an effective and generalizable tracking controller. We will explain in detail how we learn the neural tracking controller from demonstrations in Section~\ref{sec:method_il_rl}, how we mine high-quality demonstrations in Section~\ref{sec:method_data}, and how we iterate between learning controller and mining demonstrations in Section~\ref{sec:method_iteration}. 
% of a generalizable, versatile, and robust neural tracking controller with a wide range of high-quality robot tracking demonstrations. 

% due to inherent challenges in dexterous manipulation tracking,

% the demonstration data
% that can benefit from a tracking controller while effectively tackling the tracking challenge via homotopy optimization.
% to ensure the data flywheel functions well.

% imitation ready data 
% high-quality imitation-ready data 
% imitation-ready data. 
% which combines the 
% Our method tackles these challenges by training a tracking controller jointly using reinforcement learning and imitation learning to empower the controller with high generalization ability and versatility by learning abundant and high-quality imitation-ready data and also maintaining robustness towards unexpected situations taking advantage of interactions with the environment via trial-and-errors. However, acquiring a large number of imitation-ready data itself is costly and difficult due to challenges in the optimization side for single trajectory tracking. Therefore, to make sure the data flywheel functions properly, we alternate between training the tracking controller and mining more diverse and higher-quality imitation-ready data leveraging the tracking controller. 
% , using the tracking controller. 
% we wish to leverage high-quality and abundant imitation-ready data to train a tracking controller jointly with RL to let the tracking controller benefit from these successful to improve the versatility and the generalization ability. Due to the inherent difficulty in dexterous manipulation, we propose an iterative optimization approach where we alternately train the tracking controller and improve the quality and diversity of the imitation-ready data so that the data flywheel can function properly. 
% Our method wishes to 

% Our method consists of two key designs to realize this vision: 1) A learning-from-demonstration strategy that trains the tracking controller jointly via imitation learning and reinforcement learning, leveraging a large number of high-quality robot tracking demonstrations; 2) A per-trajectory tracking scheme that can effectively solve difficult single trajectory tracking tasks using a tracking controller through a homotopy optimization scheme, continuously providing tracking demonstrations.
% and a homotopy path generator, by transferring tracking prior in a homotopy manner. 
% imitation-ready data; 
% 
% which gradually mines 
% imitation-augmented reinforcement learning scheme to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance; 2) a per-trajectory tracking scheme that can leverage the general tracking controller to produce better imitation-ready data; and 3) a homotopy method and a homotopy generator that can better leverage the tracking controller to solve difficult per-trajectory tracking problem for mining imitation-ready data from challenging manipulation skills. 
% to overcome these challenges: 
% that can better leverage the general tracking controller to solve 
% effective for solving difficult per-trajectory tracking problem 
% mimicking the chain of thought, to better leverage the general tracking controller for mining imitation-ready data from challenging manipulation skills. 


% We devise a basic RL-based method to train the tracking controller with delicately design action space, observations, and rewards for the general manipulation tracking problem. To let the policy benefit from the imitation-ready data, we add an additional supervised loss which, at each time, 


% First, we leverage an imitation-augmented reinforcement learning scheme to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance. We devise a basic RL-based method to train the tracking controller with delicately design action space, observations, and rewards for the general manipulation tracking problem. To let the policy benefit from the imitation-ready data, we add an additional supervised loss which, at each time, encourages the policy to imitate the action of the corresponding timestep in the trajectory.  
% Second, we develop a per-trajectory tracking scheme which can leverage the general tracking controller to produce better imitation-ready data. To obtain high-quality imitation data with action trajectories that can successfully drive the dexterous robotic hand to track the correspondence hand and object sequence, we leverage the popular modle-free RL-based method by training a per-trjaectory tracking policy using RL and use the tracking result as the optimized imitation-ready data. Desptie no expectation in the versatility and generalization ability in the per-trajectory tracker, tracking difficult tracking problem is still very challenging. to improve the data quality and include more diverse imitation-ready data into the training of tracking controller, we propose to leverage the general tracking prior encoded in the tracking controller to improve the per-trajectory tracker optimization. Third, we design a homotopy path generator, mimicking the chain of thought, to better leverage the general tracking controller for mining imitation-ready data from challenging manipulation skills. Soley relying on tracking prior encoded in the tracking controller to improve the per-trajectory tracker is still not enough to solve very difficult per-trajecotyr tracking problem. It is because that the hard-to-track trajectories are too out-of-distribution to the data prior encoded in the tracking controller, trained with mitation-ready data that has been successfully tracked. Thus such trajectory problems can hardly benefit from the tracking prior from the current tracking controller. To resolve these challenges, we propose to solve these problems in a homotopy method. Specifically, instraed of solving the difficult per-trajectyr tracking problem directly, we start from tracking a different trajectory to obtain its tracking result. After that we design a technique which allows us to let the difficult per-trajectory tracking problem benefit from the tracking result. In this way we are able to solve the difficult tracking task by starting from an easy task and gradually solve a series of tsks with the tracking results transferred to the next one. Finding such beneficial optimization paths, however, is very time-consuming. To further improve the efficiency, we propose to learn a tracking task structure prior model, which, in the inference time, can efficiently propose beneficial optimization paths for a tough single trajectory tracking problem. With the above three designs, we alternately 1) train the tracking controller and learn the tracking task structure prior model with high-quality imitation-ready data and 2) improve the data via the tracking controller and the tracking task structure prior model. The data flywheel can then function well, making it possible for us to train a strong tracking controller finally. 




% we propose to alternately train strong tracking controller and improve the imitation ready data 
% as well as the intriacat dynamics from dynamic and rich conta

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% The key idea idea lies in leveraging high-qualtiy abutndaten imitation-ready data to train a tracking controller jointly with RL and tackling the difficulties in acquiring such data by leveraging the data flywheel to curate high-quality data and improve the tracking controller in a bootstrapping manner. At train time, given a collection of human hand object manipulation trajectories, we first retarget human hands to robotic dexterous hands in the data preparation stage, resulting in a reference manipulation  set containing retareted hand trajecotires and the original object pose sequences.  Our method then alternates between mining useful imitation-ready data from the reference motion set and training the tracking controller with the mined data. W
% e have three key designs to enable the data flywheel to function effectively. First, we leverage an imitation-augmented reinforcement learning scheme to make sure the tracking controller can benefit from imitation-ready data while still being robust to state disturbance. We devise a basic RL-based method to train the tracking controller with delicately design action space, observations, and rewards for the general manipulation tracking problem. To let the policy benefit from the imitation-ready data, we add an additional supervised loss which, at each time, 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The wish in the generalization ability and versatility a
% adn versatility usually challenge popular advanced RL approaches which often requires task-specificd reward designs
% The problem is inherently chall
% The learned neural tracking controller is expected to be able to 
% At the train time, the tracking controller is optimized to track every manipulation trajectory in the training 
% Given a datset containing 
% The neural tracking control for dexterous manipulations aims at leverage human hands manipulating objects trajectories, which have abundant data sources covering the internet videos and motion synthesis models, to learn a versatile and generalizable tracking controller. Given a dataset containing diverse human-object interaction trajecotires, the controller is optimized aiming to track every manipulation trajectory in the dataset. Specifically, with the kinematics only human object manipulation trajectory as input, the tracking controller aims at output an action trajectory that can mimic the kinematic trajectory -- when letting a dexterous robot hand execute the output action trajectory, the resulting hand states and object states should be close to their corresponding kinematic trajecotires in the input sequence. A versatile and genralizable tracking controller ought be able to generalize to novel and enve challenging interactions wit new and difficult objects. At the test time, given an manipulation sequence where both the hand motion adn the object movements and the object geometry are usnee during the training, the controller is epxcted to give proper action outputs that can drive the dexterous roobt hand to precisely control the object so that the resulting hand sequence adn the object sequences are close to the input reference. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The problem of dexterous manipulation tracking control aims to develop a tracking controller for a dexterous robot hand based on human hand-object manipulation references. Given a manipulation sequence $(\mathbf{H}, \mathbf{O})$, we expect the controller to robustly control the robot hand to manipulate the object to mimic the reference motions closely. Specifically, the resulting hand poses $\hat{\mathbf{H}}$ and the object poses $\hat{\mathbf{O}}$ should accurately follow their respective reference motions. Furthermore, the controller should be capable of tracking novel reference motions involving unseen, complex manipulation sequences and new objects. This ambitious vision is challenged by several difficulties: 1) The inherent difficulty of the tracking control problem, coming from the intricate dynamics arising from frequently changing hand-object contacts and complex object movements; 2) The challenge of controlling a high-degree-of-freedom (DoF) robot hand to accurately follow dense reference points; 3) The need for a general tracking controller that can universally track diverse and highly challenging manipulation cases; 4) The requirement for high robustness and generalization, enabling the controller to adapt and accurately mimic previously unobserved reference motions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% due to the intricate dynamics arising from 
% \(\hat{\mathbf{H}}\) and object poses \(\hat{\mathbf{O}}\) 

% so that the resulting hand and object trajectories could closely mimic the reference motions. 
% in a way that closely mimics the reference motions.
% which describes the interaction between the robot hand and an object (\textit{e.g.}, obtained via kinematic retargeting from a human-object manipulation sequence), the goal is for the controller to robustly manage the robot hand to manipulate the object in a way that closely mimics the reference motions. 

% hindered by several challenges: 
% 1. The inherent difficulty of the tracking control problem due to the intricate dynamics arising from frequently changing hand-object contacts and complex object movements.
% 2. The challenge of controlling a high-degree-of-freedom (DoF) robot hand to accurately follow dense reference points.
% 3. The need for a general tracking controller that can universally track diverse and highly challenging manipulation cases.
% 4. The requirement for high robustness and generalization, enabling the controller to adapt and accurately mimic previously unobserved reference motions.

% The manipulation sequence may contain novel manipulation sequences and new object geometries that the controller is never aware of. We still expect the controller to be able to deal with such novel tracking targets. 

% inherent difficulty of controlling a dexterous hand to densely track a manipulation trajectory with complex object motions, the intricate dynamics resulting from the rich and changing contacts between the hand and the object, the difficulty of controlling a high DoF dexterous hand, and the morphology difference, 2) the vision of learning a single policy that can universally track all trajectories, and 3) the wish of the high generalization ability to unseen and difficult manipulations for the policy. 

% Given a set of human hand-object manipulation demonstrations $\mathcal{S}=\{ ( \mathbf{H}, \mathbf{O} ) \}$, the dexterous manipulation tracking control problem aims at learning a single tracking controller that can control a dexterous robot hand to manipulate the object so that both resulting hand poses and the object poses can accurately follow their corresponding references in the kinematic demonstration. Given new manipulations involving novel interactions and unseen object geometries, we expect the controller to generalize well and robustly track those unobserved manipulations. 
% % the generalizable dexterous manipulation tracking aims at learn a single general tracking policy that 1) can successfully track each trajectory in the dataset and 2) can generalize well to novel manipulation trajectories unseen during training.
% Formally, given a multi-fingered dexterous robot hand (\emph{e.g.,} Allegro, LEAP, Shadow hand, etc.) we wish to learn a tracking controller $\mathbf{\pi}(\cdot\vert \cdot)$ from the given kinematic-only human-object interaction demonstrations $\mathcal{S}$. 
% For each manipulation trajectory $(\mathbf{H}, \mathbf{O})$, $\mathbf{\pi}(\cdot\vert \cdot)$ should be able to output a physically plausible control sequence $\mathbf{A}$ that is able to drive the dexterous robot hand to manipulate the object so that the resulting hand trajectory $\hat{\mathbf{H}}$ and the object trajectory $\hat{\mathbf{O}}$ are close to the reference motion $(\mathbf{H}, \mathbf{O})$. 
% % the object according to the kinematic demonstration $(\mathbf{H}, \mathbf{O})$, where both the resulting hand sequence and the object sequence should be close to their corresponding target trajectories. 
% Besides, given a novel manipulation trajectory unseen during the training, we wish $\mathbf{\pi}(\cdot\vert \cdot)$ can generalize well and output a reasonable manipulation trajectory that can physically track the demonstration accordingly. The vision of learning a generalizable tracker is challenged by 1) the inherent difficulty of controlling a dexterous hand to densely track a manipulation trajectory with complex object motions, the intricate dynamics resulting from the rich and changing contacts between the hand and the object, the difficulty of controlling a high DoF dexterous hand, and the morphology difference, 2) the vision of learning a single policy that can universally track all trajectories, and 3) the wish of the high generalization ability to unseen and difficult manipulations for the policy. 

% primarily in the locomotion domain, % 
% Considering the above huge challenges, directly training a policy aiming to track each manipulation trajectory would challenge both current advanced model-based and model-free techniques. Inspired by the data scaling law in other spaces, we propose to leverage a large number of imitation-ready data with both demonstrations and action sequences that can correctly drive the hand to precisely mimic the reference trajectory to train a general tracking controller. However, optimizing a large number of high-quality imitation-ready data itself is very challenging. Therefore, we propose to facilitate and enhance the per-trajectory tracking optimization via data prior from the tracking controller and the task structure. Specifically, instead of solving each tracking problem alone, we propose to solve difficult tasks via a homotopy method. It tries to solve a difficult problem by gradually solving each task in the optimization path and transferring results to the next. To efficiently find correct optimization paths, we further propose to encode such structural relations into a model, which is leveraged to propose optimization paths directly during the inference. We then present an iterative optimization strategy that gradually improves each side and finally lets us arrive at a general tracking controller. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% could let us arrive at a general tracking controller finally. 
% Letting the model propoe correct optimization paths could spare us lots of time cost in the trail and error in finding optimization paths. We then present an iterative optimization strategy that could let us arrive at a general tracking controller finally. 
% through an optimization path. This path contains a series of per-trajectory tracking problems. A good path can let us solve the final problem better by solving each problem and transferring results to the next task one-by-one. 

% interactive strategy that could let us arrive at a general 
% Consideirng the dependencies between the tracking controller, tracking task structural prior, 

% To improve the efficiency of finding correct optimization paths, we further propose to search such beneficial optimization paths 
% The task structural prior 
% The homotopy method optimizes a tracking task of interest 
% tracking task structure prior. The tracking task structure encodes cross-task relations 
% The tracking task structural prior 
% Specifically, we leverage RL to train per-trajectory tracking policies. 
% We further propose to use tracking prior from the tracking controller 
% to solve difficult pre-trajectory tracking problem and impro
% is not feasible 
% We adopt a model-free approach to solve the problem considering the recent success achieved by model-free RL in developing strong and even universal controllers~\citep{Luo2024GraspingDO,xu2023unidexgrasp,wan2023unidexgrasp2,Luo2023PerpetualHC,Luo2023UniversalHM}. However, despite the strong capability of RL demonstrated in other tasks, directly training a policy aiming to track each manipulation trajectory is not feasible due to the above huge challenges. Compared to using a universal tracking controller, single trajectory tracking is an easier problem to solve. Observing recent trials and success in combining expert demonstrations or policies with RL, \todo{add refs}, we explore the possibility of learning a tracking controller with the joint effort of RL and guidance from high-quality action-labeled data. However, despite the eased difficulty in training per-trajectory trackers, advanced solutions would still fall short in resolving very difficult tracking problems or are extremely time-consuming~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}. This makes optimizing for abundant and high-quality action-labeled trajectories itself a very difficult problem. Observing the power of the foundation model in solving downstream tasks effectively and inspired by the recent success in leveraging curriculum learning to tackle difficult tasks~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}, we propose to improve the quality and diversity of action-labeled dataset via tracking prior from the tracking controller and correct tracking curriculum. Since finding correct curricula will cost a lot of time and requires trial and error, we present an automatic tracking curricula mining strategy and propose to learn a curriculum scheduler, which can be used to propose good curricula, from the mined valid curricula. The dependencies between high-quality per-trajectory trackers and the general tracking controller as well as the curriculum scheduler pose us a ``chicken-and-egg''  puzzle. We therefore propose an iterative approach that progressively enhances each side and finally lets us arrive at a universal tracking controller. 


% We adopt a model-free approach to tackle this problem, motivated by the recent success of model-free reinforcement learning (RL) in developing robust and even universal controllers~\citep{Luo2024GraspingDO,xu2023unidexgrasp,wan2023unidexgrasp2,Luo2023PerpetualHC,Luo2023UniversalHM}. However, despite the demonstrated strength of RL in other tasks, directly training a policy to track individual manipulation trajectories is not feasible due to the significant challenges outlined earlier. While using a universal tracking controller is highly complex, tracking a single trajectory presents a more manageable problem. 
% Recent advancements combining expert demonstrations or policies with RL have shown promise in addressing these challenges \todo{add refs}. Building on this, we explore the potential of developing a tracking controller by integrating RL with high-quality, action-labeled data. Although training per-trajectory trackers is more straightforward, even advanced solutions often fall short when faced with exceptionally difficult tracking problems, or they become prohibitively time-consuming~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}. As a result, optimizing a large, high-quality action-labeled dataset remains a complex task.
% Inspired by the power of foundation models to solve downstream tasks effectively, and drawing from recent successes in curriculum learning for tackling difficult challenges~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim}, we propose enhancing the quality and diversity of the action-labeled dataset by leveraging a tracking prior from the controller and applying a refined tracking curriculum. Given the trial-and-error nature and time costs associated with identifying the correct curricula, we introduce an automatic tracking curriculum mining strategy. Additionally, we propose learning a curriculum scheduler that can suggest effective curricula based on the mined valid ones.
% The interdependencies between high-quality per-trajectory trackers, the general tracking controller, and the curriculum scheduler create a “chicken-and-egg” problem. To address this, we propose an iterative approach that progressively improves both components, ultimately leading to the development of a universal tracking controller.


% to effecitly improving the quality and diversity of action-labeld trajecotries taking advantage the joint power of per-trajectory tracking policy optimization, 
% due to the inherent difficulty in the manipulation tracking problem and the vision of tackling multiple and heterogeneous trajectory tracking problems at once.
% Considering the recent success achieved by model-free reinforcement learning in developing strong and even universal controllers~\citep{Luo2024GraspingDO,xu2023unidexgrasp,wan2023unidexgrasp2,Luo2023PerpetualHC,Luo2023UniversalHM}, and the little assumption in the known system dynamics, which may be very difficult to model to model for dexterous manipulations, we adopt a model-free approach and wish to leverage the reinforcement learning to learn a tracking policy for solving the problem. Directly training a policy aiming to track each manipulation trajectory in the dataset is not a feasible solution due to the inherent difficulty in the manipulation tracking problem and the vision of tackling multiple and heterogeneous trajectory tracking problems at once.
% where 
% \todo{some descriptions w.r.t. the distinctions and heter. within trajs?} 
% Based on the key observation in the benefit brought by the supervision provided by successful tracking trajectories\todo{rewrite this}, we pursue a strategy that can leverage the power of action-labeled manipulation trajectories to ease the difficulty in learning a universal tracking controller\todo{rewrite this -- unleash the power of data in xxx}. This further leads us to the problem of efficiently acquiring abundant high-quality action-label trajectories in an affordable time budget. Recent advances in model-free or model-based strategies to optimize an action trajectory that can successfully track a single trajectory either fall short in quality or is highly inefficient~\citep{christen2022d,zhang2023artigrasp,liu2024quasisim}. Successful trials in curriculum learning to solve difficult problems~\citep{zhang2023learning,Zhuang2023RobotPL,liu2024quasisim} let us explore what's good structural relations we can explore in this problem that is beneficial to improve single trajectory tracking. However, despite the effectiveness, curriculum learning itself is time-expensive with additional requirements in the trial-and-error to find correct curricula. With the observation of the general knowledge encoded in the foundation model to zero-shot solving specific problems, we wonder about the possibility of leveraging the tracking knowledge learned by the tracking controller to help single trajectory tracking. This further led us to wonder if can we learn a curriculum scheduler from cross-trajectory relations encoding cross-task optimization synergies so that the scheduler can efficiently plan a task curriculum for us to solve each difficult tracking problems? The dependencies between high-quality per-trajectory trackers and the general tracking controller as well as the curriculum scheduler pose us a ``chicken-and-egg''  puzzle. We therefore propose an iterative approach that progressively enhances each side and finally lets us arrive at a universal tracking controller. 

% However we face a ``chicken-and-egg'' puzzle since acquiring  high-quality abundant action-labeled data efficiently is itself not feasible due to restrictions of current techniques.  Therefore, 
% However, despite the recent achievements, 
% Optimizing for an effective policy that can track a single manipulation trajectory is already extremely challenging considering the difficulties of the non-smooth dynamics and frequent rich contact variations. Training a generalist policy that can solve such a tough manipulation tracking problem is even more difficult. Training a single controller capable of tracking diverse motions often challenges advanced RL techniques. However, optimizing out a reasonable control trajectory for each not-too-difficult single manipulation sequence is feasible under the support of current techniques. Therefore, a natural question is can we design a strategy that can resolve difficulties in single trajectory tracking and manage to get a specialist policy and then leverage such optimized specialist policies to train the generalist policy? However, acquiring such as generalist for each single trajectory is too expensive and almost unaffordable due to the heavy time cost. Moreover, optimizing each trajectory independently may still struggle with solving extremely challenging problems. This naturally leads us to find cross-tracking task synergies to enhance each single task's performance. With the above considerations, we propose a specialist-generalist-specialist training scheme and a task curriculum, powered by a heuristic-guided task relational space exploration and modeling, for iteratively improving the capability of the generalist policy and enhancing the single manipulation trajectory tracking performance. 
% \todo{rewrite this paragraph.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Our method comprises three key designs: 1) an imitation augmented RL algorithm that can effectively optimize a tracking controller taking the joint effort from RL and guidance from action-labeled trajectories (Sec.~\ref{sec:method_il_rl}), 2) a homotopy optimization scheme for solving difficult per-trajectory tracking problem, an optimization path searching strategy, and a tracking task structure prior model that encode optimization paths (Sec.~\ref{sec:method_task_space_modeling}), and 3) an iterative optimization scheme which alternately improve the imitation-ready data and train the tracking controller for optimizing a powerful tracking controller finally (Sec.~\ref{sec:method_sgs}).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% a tracking task structure modeling strategy, and tracking task structure prior model that can efficiently propose correct optimization paths in the inference time to solve difficult problems via a homotopy method (Sec.~\ref{sec:method_task_space_modeling}), and 3) an iterative optimization scheme which alternately improve the imitation-ready data and train the tracking controller for optimizing a powerful tracking controller finally (Sec.~\ref{sec:method_sgs}).
% n automatic tracking curriculum searching strategy and a curriculum scheduler that models valid tracking curricula, which can be used to propose correct curricula for tracking very difficult trajectories  (Sec.~\ref{sec:method_task_space_modeling}), 3) an interactive optimization approach that progressive 1) improve the universal tracking controller, and 2) enalarge and improve the action-labeled dataset via tracking prior from the tracking controller as well as the curriculum scheduling (Sec.~\ref{sec:method_sgs}).
% such relations via a conditional diffusion model
% could benef
% general tracking controller's training from abundant high-quality action-labeled data 

% ``specialist-generalist-specialist'' training strategy which iteratively optimizing out better specialists, leveraging the cross-task synergies from the task relational model and the generalist policy, and improving the generalist performance by training with more and better specialists 
% task relational space modeling scheme with a heuristic-guided searching algorithm for constructing the task relational space and a conditional diffusion model for describing such relations 
% that could leverage action-labeled data to 
% enhance the performance of the generalist policy 
% % cross-task synergy modeling scheme 

% effectively let the generalist policy benefit from more and better action-labeled single trajectory manipulation's optimization result and 
% a heuristic-guided searching method for building the structural task relational space, which summarizes the cross-task optimization synergies in the manipulation tracking problem, 
% 2) an effective optimization scheme that 

% as well as an offline action trajectory and then leveraging such 
% that can manage to optimize for a reasonable control sequence for each manipulation trajectory 
% Directly leveraging davnaced RL techniques to train a single tracker capable of tracking diverse motions 

% \textcolor{red}{(TODO: explain why we employ a generalist-specialist-generalist approach, why we start from the specialist training; Explain the overall high level motivations at first and then continue with the key designs)}
% Our method comprises two key designs to tackle these challenges: 1) an imitation augmented RL algorithm that could leverage action-labeled data to learn a general tracking policy, 2) an effective optimization scheme for solving difficult tracking problems with an automatically explored hierarchical trajectory space, a distilled task translation model, and a task curriculum, and 3) an interactive model training and action-labeled data acquisition and improvement scheme leveraging the universal policy and the distilled task translation model. 
% \textcolor{red}{(TODO: Add section labels)}
% \textcolor{red}{(TODO: may be swap 1 and 2)}

% \todo{action labeled dataset for training the tracking controller}

% \todo{curriculum scheduler}

% \todo{using the above two tools to improve per-trajectory trackers}


% Consider %

% specialist formulation
% specialist formulation --- 
% d

% \todo{add some explanations on the kinematic retargeting}

% \todo{though the retargeted trajectories have noise, actually we would not be restricted by such noise}

% \todo{add the residual policy --- actually it is somewhat interesting and would not restrict us into adjacent part of the original kinematic trajectory}



% \subsection{Generalist Training via Imitation Augmented RL} \label{sec:method_il_rl}
% \subsection{Tracking Controller Training via Imitation Augmented RL} \label{sec:method_il_rl} 
% \subsection{Tracking Controller Training via Imitation Augmented RL} \label{sec:method_il_rl} 

\vspace{-5pt}
\subsection{Learning a Neural Tracking Controller from Demonstrations} \label{sec:method_il_rl} 
\vspace{-5pt}
% \eric{Imitation-augmented RL refers to a pretty broad range of methods and there are already a lot of similar algorithms in the literature. We don't necessarily need to come up with a name for this algorithm since it is probably not a very big deal. We could simply use ``learning a neural tracking controller from demonstrations'' as the subsection title. We could first motivate the usage of RL and IL together since RL is better at coping with dynamic state disturbance while IL can benefit from a large number of demonstrations. Then describe the RL part. Later, incorporate the IL part. Finally, conceptually analyze the framework a bit. see below.}

% \eric{We should conceptually compare with the old DAPG paper (Learning Complex Dexterous Manipulation with
% Deep Reinforcement Learning and Demonstrations) and also add ablations in the experiment section to motivate the necessity of coming up with the current approach. 
% For me, the difference sounds to be that we are doing tracking so even using RL the explored states will not deviate from the given trajectory too much, making the current design possible. In the current design, from RL's perspective, the imitation loss biases RL policy's action toward the imitation source to improve sampling efficiency. From IL's perspective, RL is injecting noises into the states to make learning more robust similar to DART.}

% We could first motivate the usage of RL and IL together since RL is better at coping with dynamic state disturbance while IL can benefit from a large number of demonstrations. Then describe the RL part. Later, incorporate the IL part. Finally, conceptually analyze the framework a bit. see below.

% \eric{Imitation-augmented RL refers to a pretty broad range of methods and there are already a lot of similar algorithms in the literature. We don't necessarily need to come up with a name for this algorithm since it is probably not a very big deal. We could simply use ``learning a neural tracking controller from demonstrations'' as the subsection title. We could first motivate the usage of RL and IL together since RL is better at coping with dynamic state disturbance while IL can benefit from a large number of demonstrations. Then describe the RL part. Later, incorporate the IL part. Finally, conceptually analyze the framework a bit. see below.}

% To train a tracking controller that can benefit from a large number of imitation-ready data and also be robust to dynamic state disturbances, we leverage reinforcement learning and imitation learning to train a tracking controller. Specifically, we propose an RL-based training strategy with carefully designed action apace, observations and rewards for the manipulation tracking problem. We further present an additional imitation loss so that we can train the tracking controller with additional supervision from the imitation-ready data with high-quality action sequences. 

% Given a collection of human-object manipulation trajectories and a set of high-quality robot tracking demonstrations, we wish to learn an effective and generalizable neural tracking controller. 
% In the beginning, we retarget human hand-object manipulation to a robotic hand as a data pre-processing step. 
% We combine RL and IL to develop a generalizable and robust neural tracking controller. 
% Taking advantage of imitating diverse and high-quality robot tracking demonstrations, we can effectively let the tracking controller master diverse manipulation skills and also equip it with high generalization ability. Jointly leveraging the power of RL, the controller would not get overfit to imitating successful tracking results covering a narrow distribution, maintaining strong robustness to dynamic state disturbances. Specifically, we design an RL-based learning scheme for training the tracking controller, including the carefully-designed action space, observations, and the reward tailored for the manipulation tracking task. We also introduce an IL-based strategy that lets the tracking controller benefit from imitating high-quality demonstration data. 
% By integrating these two approaches, we effectively address the complex problem of generalizable tracking control.


Given a collection of human-object manipulation trajectories and a set of high-quality robot tracking demonstrations, our goal is to learn an effective and generalizable neural tracking controller. 
In the beginning, we retarget human hand-object manipulation to a robotic hand as a data preprocessing step. We combine RL and IL to develop a generalizable and robust neural tracking controller. 
Taking advantage of imitating diverse and high-quality robot tracking demonstrations, we can effectively let the tracking controller master diverse manipulation skills and also equip it with high generalization ability. 
% Jointly leveraging the power of RL, the controller would not get overfit to imitating successful tracking results covering a narrow distribution, therefore maintaining strong robustness to dynamic state disturbances. 
Jointly leveraging the power of RL, the controller avoids overfitting to successful tracking results limited to a narrow distribution, thereby maintaining robust performance in the face of dynamic state disturbances.
Specifically, we design an RL-based learning scheme for training the tracking controller, including the carefully-designed action space, observations, and the reward tailored for the manipulation tracking task. We also introduce an IL-based strategy that lets the tracking controller benefit from imitating high-quality demonstration data. 
By integrating these two approaches, we effectively address the complex problem of generalizable tracking control.


% Combining the best of the two worlds, we finally succeed in the complex generalizable tracking control problem. 
% from the trajectories. 

% Then, in our formulation, the neural tracking controller is an agent that interacts with the environment according to a tracking policy $\pi$. At each timestep $n$, the policy observes the state $\hat{\mathbf{s}}_n$, consisting of the current state of the robotic dexterous hand and the object state, and the next goal $\mathbf{s}_{n+1}$, commanded as the next state of the robotic hand in the retargeted sequence and the next goal object state. Then the agent then samples an action $\mathbf{a}_n$ from the policy $\mathbf{a}_n\sim \pi(\cdot \vert \mathbf{s}_n, \mathbf{s}_{n+1})$. After applying action to the robotic dexterous hand, the hand transits and physically interacts with the object. The resulting hand state and the object state should be close to their corresponding nextstep state in the reference trajectory. 
% tracking policy $\pi_{\theta}$. At 
% We then combine reinforcement learning (RL) and imitation learning (IL) to develop a generalizable, versatile~\eric{we are using versatile a lot from the very beginning but it is not quite clear what it indeed refers to.}, and robust neural tracking controller. 

% reinforcement learning (RL) and imitation learning (IL) 
% leveraging knowledge learned 
% from the abundant data. 
% imitation-ready data, 
% Jointly leveraging the power of the reinforcement learning, we 
% equip the tracking controller with 
% we let the tracking controller 
% so that it can benefit from abundant imitation-ready data while maintaining robustness to dynamic state disturbances. 

% a well-defined action space, observations, and the reward 
% We design an RL-based strategy for solving the tracking controller problem, including a well-defined action space, observation framework, and reward structure tailored for the manipulation tracking task. 
% We begin by motivating the integration of RL, which excels in handling dynamic challenges, with IL, which benefits from extensive demonstration data. 
% Our RL-based strategy includes a well-defined action space, observation framework, and reward structure tailored for the manipulation tracking task. 

% let the 
% To guide the learning of the tracking controller, we introduce an imitation learning scheme to jointly train the controller with RL. 

% imitation loss 
% exploration of the RL's agent, we introduce an
% and to let us succeed in the generalizable tracking control problem, we 

% We will illustrate details as follows. 
% benefit the tracking controller 
% to enhance training by adding additional supervision from high-quality demonstration data. 
% with high-quality action sequences from the demonstration data, allowing for additional supervision. Finally, we will conceptually analyze this framework to highlight its effectiveness in training a neural tracking controller from demonstrations.
% which adds additional supervision 
% as an additional super


% To develop a generalizable and versatile neural tracking controller that can benefit from abundant imitation-ready data while maintaining robustness to dynamic state disturbances, we combine reinforcement learning (RL) and imitation learning (IL). 
% benefiting from abundant imitation-ready data while 
% that is versatile 
% utilizes abundant imitation-ready data 

% consider an approach where

% We design an imitation augmented RL algorithm to train the tracking controller. It is composed of a basic tracking policy and an action supervised loss. Given an action-labeled dataset composed of trajectories with high-quality action sequences, we can overcome the difficulty of training the general controller solely via RL leveraging the additional supervision provided by the action-labeled trajectories. 
% can benefit the tracking controller's learning via this strategy. 
% Optimizing the tracking controller aiming to solve multiple tracking problems is difficult considering the inherent poor multi-task ability of RL. \todo{add refs}
% Directly using advanced RL to train a tracking controller is an extremely challenging problem considering the inherent difficulty of dexterous manipulations and the high demand for generalization ability, versatility, and robustness. In comparison, single trajectory tracking, expecting no generalization ability or versatility, is an easier problem. Inspired by recent exploration and achievements on introducing supervision, either from the offline dataset, online trajectory optimization, or experts, into RL~\citep{rajeswaran2017learning,Liu2023BlendingIA}, we design an imitation augmented RL algorithm, composed of a basic tracking policy and an action supervised loss. Given an action-labeled dataset composed of trajectories with  high-quality action sequences, we can benefit the tracking controller's learning via this strategy. 
% with dedicated   to train the tacking controller, composed of a basic tracking 
% Single trajectory tracking is an 
% Inspired by 
% % Training a general tracking controller with the expectation of tracking all trajectories directly always turns out to be a problem that is too difficult to solve by current reinforcement learning techniques. 
% Therefore, instead of optimizing the general tracker directly,  we propose to augment the training with supervision from the action-labeled dataset to ease the training~\citep{Jenelten2023DTCDT,rajeswaran2017learning,Liu2023BlendingIA}. We delicately design the observations and rewards so that by leveraging advanced RL as the base approach we can solve many single trajectory tracking problems. With high-quality action-labeled trajectories rollout by their optimized per-trajectory trackers, we then propose an imitation augmented RL training scheme to ease the training and improve the general tracking controller. 
% How to leverage experts or offline datasets to improve RL training is still an active research topic currently. 
% Despite previous successful trials in other scenarios~\citep{Jenelten2023DTCDT,rajeswaran2017learning,Liu2023BlendingIA}, how to unleash the power of this trend of methods for dexterous manipulation tracking generalist poses many unique challenges. 
% Instead of directly training a generalist policy aiming to track all trajectories directly, which always turns out to be a problem that is too difficult to solve by current RL techniques, we propose to augment the training with the supervision from action labeled dataset for ease and speed up the policy learning. \todo{some references w.r.t. this approach} 
% \todo{rewrite the next sentence}
% To fulfill this vision, we need to curate action-labeled trajectories. Therefore, we again propose to leverage RL to train a trajectory-specific tracking policy to infer actions for the trajectory. 

\noindent\textbf{Neural tracking controller.} 
% In our formulation, the neural tracking controller is an agent that interacts with the environment according to a tracking policy $\pi$. At each timestep $n$, the policy observes the observation $\mathbf{o}_n$. $\mathbf{o}_n$ is computed based upon the current state $\mathbf{s}_n$, the next goal $\hat{\mathbf{s}}_{n+1}$ which is commanded as the next goal state of the robotic hand and the next goal object state, and the object geometry.
% Then, the agent samples an action $\mathbf{a}_n$ from the policy $\mathbf{a}_n\sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})$. After applying action to the robotic dexterous hand, the hand moves and physically interacts with the object. After that, both the hand and the object transit into the next state according to the environment dynamics, \emph{i.e.,} ${\mathbf{s}}_{n+1} \sim p(\cdot \vert {\mathbf{s}}_n, \mathbf{a}_n)$. 
% The resulting hand state and object state should closely match their respective next goal states.
In our formulation, the neural tracking controller acts as an agent that interacts with the environment according to a tracking policy \(\pi\). At each timestep \(n\), the policy observes the observation \(\mathbf{o}_n\) and the next goal \(\hat{\mathbf{s}}_{n+1}\) (designated as the target state for the robotic hand and the object). The policy then computes the distribution of the action. Then the agent sample an action $\mathbf{a}_n$ from the policy, \emph{i.e.,} \(\mathbf{a}_n \sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})\). The observation $\mathbf{o}_n$ primarily contains the current state $\mathbf{s}_n$ and the object geometry. 
% which is primarily computed based on the current state \(\mathbf{s}_n\) and the next goal \(\hat{\mathbf{s}}_{n+1}\) (designated as the target state for the robotic hand and the object). The policy then computes the distribution of the action. Then the agent sample an action $\mathbf{a}_n$ from the policy, \emph{i.e.,} \(\mathbf{a}_n \sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})\). The observation $\mathbf{o}_n$ primarily contains the current state $\mathbf{s}_n$ and the object geometry. 
% Then the agent 
% and the object geometry. 
% computed based on the current state \(\mathbf{s}_n\), the next goal \(\hat{\mathbf{s}}_{n+1}\) (designated as the target state for the robotic hand and the object), and the object geometry.
% The agent then samples an action \(\mathbf{a}_n\) from the policy, \emph{i.e.,} \(\mathbf{a}_n \sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})\). 
Upon executing the action with the robotic dexterous hand, the hand physically interacts with the object, leading both the hand and the object to transition into the next state according to the environment dynamics, represented as \(\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)\). 
% An effective tracking controller should let the resulting hand and object states should closely align with their respective next goal states.
An effective tracking controller should ensure that the resulting hand and object states closely align with their respective next goal states.
% The resulting hand and object states should closely align with their respective next goal states.

% which is computed based upon the current state $\mathbf{s}_n$, the next goal $\hat{\mathbf{s}}_{n+1}$, commanded as the next state of the robotic hand in the retargeted sequence and the next goal object state, and the object geometry.
% ~\eric{the writing is a bit confusing here. Does $\mathbf{o}_n$ include $\hat{\mathbf{s}}_{n+1}$ and the object geometry or it only includes $\mathbf{s}_n$? Why the object geometry is not a part of the policy input in the next formula?} % state-goal pair $(\mathbf{s}_n, \hat{\mathbf{s}}_{n+1})$ 
% primarily encodes the current hand and object state, object geometry, 
% the policy observes the state ${\mathbf{s}}_n$, consisting of the current state of the robotic dexterous hand and the object state, 
% and the next goal $\hat{\mathbf{s}}_{n+1}$, 
% commanded as the next state of the robotic hand in the retargeted sequence and the next goal object state. 

% The resulting hand state and the object state should be close to their corresponding next goal state. 
% nextstep state in the reference trajectory. 




% \todo{adapt to the tracking controller}
% \noindent\textbf{Per-trajectory tracker training.} 
% \noindent\textbf{Tracking controller optimization via RL.} 
% \noindent\textbf{Basic RL for training the tracking controller.} 
% \noindent\textbf{Training the tracking controller via RL.} 
\noindent\textbf{Reinforcement learning.}  
% Our single trajectory specialist training scheme leverages PPO to optimize for a tracking policy $\mathbf{\pi}(\cdot\vert \cdot)$. 
% Given a kinematic manipulation trajectory $(\mathbf{H}, \mathbf{O})$, we aim at optimizing a tracking policy $\mathbf{\pi}(\cdot\vert\cdot )$ that can control a dexterous robot hand to track the reference kinematic trajectory. 
% We use PD control to drive the hand. % links and joints %
% We carefully design the action space, and observation space as well as the reward and develop an RL-based optimization scheme for learning a tracking policy. Considering the poor sample efficiency of RL, instead of letting the tracking policy learn absolute positional target $\mathbf{a}_n$ at each timestep $n$, we assume there exists a basic trajectory, which is usually set to the kinematic reference trajectory, and let RL learn residual relative target $\Delta \mathbf{a}_n$ at each timestep $n$. For each timestep $n$, denote the hand state in the basic trajectory as $\mathbf{h}_n^b$, we calculate the final positional target as follows: 
% \begin{align}
%     \mathbf{a}_n = \mathbf{h}_n^b + \sum_{k=1}^n \Delta \mathbf{a}_k. 
% \end{align}
% In addition to the possibility in speeding up the training, the basic trajectory $\mathbf{H}^b=\{ \mathbf{h}_n^b \}$ gives us an additional dimension for optimizing the single trajectory tracking policy. For instance, we can initialize the basic trajectory as the tracking result of a different tracking task and re-optimize the residual policy to try to improve the single trajectory tracking. 
% \eric{The explanation should be more logical. We should start from introducing the state space, and then explain the common action space, e.g., joint positional targets, followed by mentioning our residual design. Finally rewards. I like how the \href{https://research.nvidia.com/labs/par/maskedmimic/assets/SIGGRAPHAsia2024_MaskedMimic.pdf}{MaskedMimic} paper introduces these.}
% We design 
% leverage 
% reinforcement learning scheme to 
% In the RL-based training scheme, the agent receives a reward $r_{n} = r({\mathbf{s}}_n, \mathbf{a}_n, \hat{\mathbf{s}}_{n+1}, \mathbf{s}_{n+1})$ after each transition. The training objective is maximizing the discounted cumulative reward: 
% \begin{align}
%     J = \mathbb{E}_{p(\tau\vert \pi)} \left[  \sum_{n=0}^{N} \gamma^{n}r_n  \right],
% \end{align}
% where $p(\tau\vert \pi) = p({\mathbf{s}}_0) \Pi_{n=0}^{N-1}p(\mathbf{s}_{n+1}\vert \mathbf{o}_n, \mathbf{a}_n)\pi(\mathbf{a}_n\vert \mathbf{s}_n,\hat{\mathbf{s}}_{n+1})$ is the likelihood of a transition trajectory of the agent $\tau = (\mathbf{s}_0,\mathbf{a}_0,r_0,...,\mathbf{s}_{N-1},\mathbf{a}_{N-1},r_{N-1}, \mathbf{s}_N)$. The discount factor $\gamma \in [0,1)$ determines the effective horizon length of the policy. 
% In the tracking control problem, the next goal state $\hat{\mathbf{s}}_{n+1}$ usually consists of the next step hand state and the object state in the kinematic reference sequence. 
% We control the robotic hand via a proportional derivative (PD) controller, following previous literature~\citep{Luo2024GraspingDO,Luo2023PerpetualHC,christen2022d,zhang2023artigrasp}. The action $\mathbf{a}_n$ then contains the target position commands of all hand joints. To improve the sample efficiency of RL, instead of letting the tracking policy learn the absolute positional target, we introduce a residual action space. Specifically, we introduce a baseline hand trajectory and train the policy to learn the residual relative target  $\Delta\mathbf{a}_n$ in each timestep. 
% The baseline trajectory is always available for the tracking problem -- one can trivially set it to the kinematic reference trajectory. 
% In each timestep $n$, we compute the position target via $\mathbf{a}_n = \mathbf{s}_n^{b} + \sum_{k=0}^{n}\Delta \mathbf{a}_k$, where $\mathbf{s}_n^{b}$ is the $n$-th step hand state in the baseline trajectory. 
% The observation at each timestep $n$ encodes the current hand and object state, the next goal state, baseline trajectory, actions, velocities, and the object geometry: 
% \begin{align}
%     \mathbf{o}_n = \{ \mathbf{s}_n, \dot{\mathbf{s}}_n, \hat{\mathbf{s}}_{n+1}, \mathbf{s}^b_n, \mathbf{a}_n, \text{feat}_{\text{obj}}, \text{aux}_n \}, \label{eq_obs}
% \end{align}
% where $\text{feat}_{\text{obj}}$ is the object feature produced by a pre-trained object point cloud encoder. We additionally introduce an auxiliary feature $\text{aux}_n$, computed based upon available states, to expose the agent with more informative information. We will explain in detail in Appendix~\ref{sec:supp_method}. 
% Our reward for manipulation tracking encourages the transited hand state and the object state to be close to their corresponding reference states and the hand-object affinity: 
% \begin{align}
%     r = w_{o, p} r_{o, p} + w_{o, q} r_{o, q} + w_{\text{wrist}} r_{\text{wrist}} + w_{\text{finger}} r_{\text{finger}} + w_{\text{affinity}} r_{\text{affinity}}, \label{eq_rew}
% \end{align}
% where $r_{o,p},r_{o, q},r_{\text{wrist}},r_{\text{finger}},r_{\text{affinity}}$ are rewards for object position, object orientation, hand wrist, hand fingers, and hand-object affinity, $w_{o, p},  w_{o, q}, w_{\text{wrist}}, w_{\text{finger}},  w_{\text{affinity}}$ are their weights. Details of the reward computation are deferred to the Appendix~\ref{sec:supp_method}. 
In the RL-based training scheme, the agent receives a reward \(r_{n} = r({\mathbf{s}}_n, \mathbf{a}_n, \hat{\mathbf{s}}_{n+1}, \mathbf{s}_{n+1})\) after each transition. The training objective is to maximize the discounted cumulative reward:
\begin{align}
    J = \mathbb{E}_{p(\tau\vert \pi)} \left[  \sum_{n=0}^{N-1} \gamma^{n}r_n  \right],
\end{align}
where \(p(\tau\vert \pi) = p({\mathbf{s}}_0) \prod_{n=0}^{N-1} p(\mathbf{s}_{n+1}\vert \mathbf{o}_n, \mathbf{a}_n)\pi(\mathbf{a}_n\vert \mathbf{s}_n,\hat{\mathbf{s}}_{n+1})\) is the likelihood of a transition trajectory of the agent \(\tau = (\mathbf{s}_0,\mathbf{a}_0,r_0,...,\mathbf{s}_{N-1},\mathbf{a}_{N-1},r_{N-1}, \mathbf{s}_N)\). The discount factor \(\gamma \in [0,1)\) determines the effective horizon length of the policy.
In the tracking control problem, the next goal state \(\hat{\mathbf{s}}_{n+1}\) typically comprises the subsequent hand state and the object state from the kinematic reference sequence. We control the robotic hand using a proportional derivative (PD) controller, following previous literature~\citep{Luo2024GraspingDO,Luo2023PerpetualHC,christen2022d,zhang2023artigrasp}. The action \(\mathbf{a}_n\) contains the target position commands for all hand joints. 
To enhance the sample efficiency of RL, rather than allowing the tracking policy to learn the absolute positional targets, we introduce a residual action space. Specifically, we introduce a baseline hand trajectory and train the policy to learn the residual relative target \(\Delta\mathbf{a}_n\) at each timestep. The baseline trajectory is consistently available for the tracking problem and can be trivially set to the kinematic reference trajectory. 
In each timestep $n$, we compute the position target via $\mathbf{a}_n = \mathbf{s}_n^{b} + \sum_{k=0}^{n}\Delta \mathbf{a}_k$, where $\mathbf{s}_n^{b}$ is the $n$-th step hand state in the baseline trajectory. 
% The observation at each timestep \(n\) encodes the current hand and object states, the next goal state, the baseline trajectory, actions, velocities, and the object geometry:
The observation at each timestep $n$ encodes the current hand and object state, the baseline trajectory, actions, velocities, and the object geometry:
% the next goal state, 
% baseline trajectory, actions, velocities, and the object geometry: 
\begin{align}
    % \mathbf{o}_n = \{ \mathbf{s}_n, \dot{\mathbf{s}}_n, \hat{\mathbf{s}}_{n+1}, \mathbf{s}^b_n, \mathbf{a}_n, \text{feat}_{\text{obj}}, \text{aux}_n \}, \label{eq_obs}
    \mathbf{o}_n = \{ \mathbf{s}_n, \dot{\mathbf{s}}_n, \mathbf{s}^b_n, \mathbf{a}_n, \text{feat}_{\text{obj}}, \text{aux}_n \}, \label{eq_obs}
\end{align}
where \(\text{feat}_{\text{obj}}\) is the object feature generated by a pre-trained object point cloud encoder. We also introduce an auxiliary feature \(\text{aux}_n\), computed based on available states, to provide the agent with more informative context. Further details will be explained in Appendix~\ref{sec:supp_method}.
Our reward for manipulation tracking encourages the transited hand state and the object state to closely match their respective reference states, as well as promoting hand-object affinity:
\begin{align}
    r = w_{o, p} r_{o, p} + w_{o, q} r_{o, q} + w_{\text{wrist}} r_{\text{wrist}} + w_{\text{finger}} r_{\text{finger}} + w_{\text{affinity}} r_{\text{affinity}}, \label{eq_rew}
\end{align}
where \(r_{o,p}, r_{o, q}, r_{\text{wrist}}, r_{\text{finger}}, r_{\text{affinity}}\) represent rewards for object position, object orientation, hand wrist, hand fingers, and hand-object affinity, respectively, while \(w_{o, p}, w_{o, q}, w_{\text{wrist}}, w_{\text{finger}}, w_{\text{affinity}}\) are their corresponding weights. Details regarding the reward computation are deferred to Appendix~\ref{sec:supp_method}.



% ~\eric{should be ``trivially''. Please use Grammarly to carefully check the whole paper to avoid grammar errors.} 
% $\mathbf{b}_n$ 

% , $\text{aux}_n$ is the auxiliary features, computed based upon available states~\eric{at least we should explain the purpose of including some auxiliary features?}, which we will explain in detail in Appendix~\ref{sec:supp_method}. 

% Our reward for manipulating tracking comprises three components: the hand reward $r_{h}$, the object reward $r_o$, and the hand-object affinity reward $r_d$. The object reward encourage the transited object position and the orientation close to their kinematic references: $r_o = w_p r_{o,p} + w_q r_{o,q}$. 
% The object reward includes both position and orientation rewards, defined as: 
% \begin{align}
%     r_o = w_p(0.9 - \Vert \mathbf{s}_n^p - \hat{\mathbf{o}}_n^p \Vert_2 ) + w_q(\text{np.pi} - \text{Diff\_Angle}(\mathbf{o}_n^q - \hat{\mathbf{o}}_n^q )), \label{eq:rew_obj}
% \end{align}
% where $w_p$ and $w_q$ are the weights for position and orientation rewards, respectively, and $\text{Diff\_Angle}(\cdot, \cdot)$  computes the rotation angle difference between two quaternions. The hand reward is calculated as the negative weighted sum of the current hand joint positions and the reference positions:
% \begin{align}
%     r_h = -(w_{\text{trans}} \Vert \mathbf{h}_n[:3] - \hat{\mathbf{h}}_n[:3] \Vert_1 + w_{\text{ornt}} \Vert \mathbf{h}_n[3:6] - \hat{\mathbf{h}}_n[3:6] \Vert_1 + w_{\text{finger}} \Vert \mathbf{h}_n[6:] - \hat{\mathbf{h}}_n[6:] \Vert_1  ), \label{eq:rew_hand}
% \end{align}
% % we include in the observation, 
% % The tracking controller for manipulation should be aware of the geometry of the object. So we include the object feature, produced by a pre-trainedd object point cloud encoder, into the state. The final state contains 

%%%%%%%%%%%%%%%%%%%%%% baseline trajs %%%%%%%%%%%%%%%%%%%%%%
% This approach benefits us from two ways. First, the RL exploration needs to explore around the baseline trajectory only, thereby accelerating the convergence. Second, it offers us an additional dimension for optimizing the tracking policy -- 
% needs to explore around a baseline hand trajectory. 
% it can accelerate the training 
% we introduce a baseline hand trajectory
% The action $\mathbf{a}_n$ contains the joint torque commands applied to all hand joints. We follow the literature and adopt 
% contains the positional target of each hand joint. 
% is the positional target of each hand joint
% in the kinematic reference sequence
% aims at optimizing $\pi$ 
% Our RL-based scheme for training the tracking controller aims at optimizing the tracking policy $\pi$ with the objective to maximize the discounted cumulative reward: 
% \begin{align}
%     J = \mathbb{E}_{p(\tau\vert )}
% \end{align}
% We carefully design the action space, observation space, and reward to develop an RL-based optimization scheme for learning a tracking controller. To address the poor sample efficiency of RL, instead of letting the tracking policy learn the absolute positional target $\mathbf{a}_n$ at each timestep $n$, we introduce a basic trajectory~\eric{base trajectory or basic trajectory? I would suggest the former. Please make sure we modify all terms together.}, commonly the kinematic reference trajectory, and allow RL to learn the residual relative target $\Delta \mathbf{a}_n$ at each timestep. For each timestep $n$, denote the hand state in the basic trajectory as $\mathbf{h}_n^b$, we compute the final positional target as follows: 
% % we denote the hand state in the basic trajectory as $\mathbf{h}_n^b$ and compute the final positional target as follows:
% \begin{align}
%     \mathbf{a}_n = \mathbf{h}_n^b + \sum_{k=1}^n \Delta \mathbf{a}_k. 
% \end{align}
% This approach not only accelerates training but also provides an additional dimension for optimizing the single trajectory tracking policy. For instance, we can initialize the basic trajectory using the tracking results from a different task and then re-optimize the residual policy to enhance the single trajectory tracking performance.
%%%%%%%%%%%%%%%%%%%%%% baseline trajs %%%%%%%%%%%%%%%%%%%%%%


% using the action trajectory sampled 
% In our method, we try to improve the single trajectory tracking by varying the basic trajectory from its own kinematic reference motion to the rollout action trajectory produced by a well-trained expert for a different task or from the general tracking policy, followed by re-optimizing the residual policy. 

%%%%%%%%%%%%%%%%%%%%%% observation space %%%%%%%%%%%%%%%%%%%%%%
% At each timestep $n$, the observation includes information about the current hand and object states, the next frame tracking target, the current cumulated residual targets, the next step hand state in the basic trajectory, and the pre-processed object feature $\text{feat}_{\text{obj}}$. The $n$-th step observation, denoted as $\mathbf{o}\mathbf{b}\mathbf{s}_n$, is calculated as follows:
% \begin{align}
%     \mathbf{o}\mathbf{b}\mathbf{s}_n = \{ \hat{\mathbf{h}}_n, \hat{\mathbf{o}}_n,  \hat{\dot{\mathbf{h}}}_n, \hat{\dot{\mathbf{o}}}_n, \mathbf{f}_n,  \mathbf{h}_{n+1}, \mathbf{o}_{n+1}, \mathbf{h}_{n+1} - \hat{\mathbf{h}}_n, \mathbf{o}_{n+1} \ominus \hat{\mathbf{o}}_n, \sum_{k=1}^n\Delta\mathbf{a}_k, \mathbf{h}_{n+1}^b, \text{feat}_{\text{obj}}   \}, \label{eq:observations}
% \end{align}
% where $\hat{\mathbf{h}}_n$ and $\hat{\mathbf{o}}_n$ represent the observed positions of hand joints and object orientation at timestep $n$, $\hat{\dot{\mathbf{h}}}_n$ and $\hat{\dot{\mathbf{o}}}_n$ denote the velocities of hand joints and object linear and angular velocities, respectively, $\mathbf{f}_n$ indicates the hand finger positions in the world space.
%%%%%%%%%%%%%%%%%%%%%% observation space %%%%%%%%%%%%%%%%%%%%%%






% At each timestep $n$, the observation comprises the current hand and object state information, the next frame tracking target, the current cumulated residual targets, the next step basic hand state, and the pre-processed object feature $\text{feat}_{\text{obj}}$ as input and output the hand action for the hand to achieve the next state. Specifically, at each timestep $n$, we calculate the observation $\mathbf{o}\mathbf{b}\mathbf{s}_n$ as follows: 
% \begin{align}
%     \mathbf{o}\mathbf{b}\mathbf{s}_n = \{ \hat{\mathbf{h}}_n, \hat{\mathbf{o}}_n,  \hat{\dot{\mathbf{h}}}_n, \hat{\dot{\mathbf{o}}}_n, \mathbf{f}_n,  \mathbf{h}_{n+1}, \mathbf{o}_{n+1}, \mathbf{h}_{n+1} - \hat{\mathbf{h}}_n, \mathbf{o}_{n+!} \ominus \hat{\mathbf{o}}_n, \sum_{k=1}^n\Delta\mathbf{a}_k, \mathbf{h}_{n+1}^b, \text{feat}_{\text{obj}}   \}, \label{eq:observations}
% \end{align}
% where $\hat{\mathbf{h}}_n$ and $\hat{\mathbf{o}}_n$ are observed hand joint DoF positions and the object orientation as well as positions at the timestep $t$, $\hat{\dot{\mathbf{h}}}_n$ and $\hat{\dot{\mathbf{o}}}_n$ are hand DoF velocities and object linear as well as angular velocities respectively, $\mathbf{f}_n$ denotes the hand finger positions in the world space. 

% $\mathbf{h}_{n+1}$ and $\mathbf{o}_{n+1}$ are the kinematic targets of the hand DoF positions and the object state in the next timestep. 

% The reward consists a hand tracking reward $r_{h}$, object tracking reward $r_o$, and the hand-object affinity reward $r_d$. Specifically, the object reward contains the object position reward and the orientation reward: 
% \begin{align}
%     r_o = w_p(0.9 - \Vert \mathbf{o}_n^p - \hat{\mathbf{o}}_n^p \Vert_2 ) + w_q(\text{np.pi} - \text{Diff\_Angle}(\mathbf{o}_n^q - \hat{\mathbf{o}}_n^q )), \label{eq:rew_obj}
% \end{align}
% where $w_p$ and $w_q$ are weights of the position reward and the orientation reward respectively, $\text{Diff\_Angle}(\cdot, \cdot)$ calculates the rotation angle difference of two rotations represented as quaternions. The hand reward is the negative of the weighted sum of the current hand DoF positions and the reference positions: 
% \begin{align}
%     r_h = -(w_{\text{trans}} \Vert \mathbf{h}_n[:3] - \hat{\mathbf{h}}_n[:3] \Vert_1 + w_{\text{ornt}} \Vert \mathbf{h}_n[3:6] - \hat{\mathbf{h}}_n[3:6] \Vert_1 + w_{\text{finger}} \Vert \mathbf{h}_n[6:] - \hat{\mathbf{h}}_n[6:] \Vert_1  ), \label{eq:rew_hand}
% \end{align}
% where $w_{\text{trans}}, w_{\text{ornt}}$, and $w_{\text{finger}}$ are weights. The hand-object affinity reward encourages the hand palm and fingers to get close to the object: 
% \begin{align}
%     r_d = -(w_{\text{palm}} \Vert \mathbf{p}_n^{\text{palm}} - \hat{\mathbf{o}}_n^p \Vert + w_{\text{finger}} \sum_{i=1}^{n_f} \Vert \mathbf{f}_{n,i} - \hat{\mathbf{o}}_n^p \Vert),  \label{eq:rew_affinity}
% \end{align}
% where $w_{\text{palm}}$ and $w_{\text{finger}}$ are weights of the palm-object and finger-object affinities respectively, $n_f$ denotes the number of fingers, $\mathbf{f}_{n,i}$ represents the position of the $i$-th finger in the current frame $n$. 
% Finally, the overall reward is composed as the sum of these three components: $r = r_h + r_o + r_d$. 
% We leverage PPO~\citep{Schulman2017ProximalPO} implemented in rl\_games~\citep{rlgames2021} to train our policy. 


%%%%%%%%%%%%%%%%%%%%%% reward function %%%%%%%%%%%%%%%%%%%%%%
% The reward function comprises three components: the hand-tracking reward $r_{h}$, the object-tracking reward $r_o$, and the hand-object affinity reward $r_d$. The object reward includes both position and orientation rewards, defined as:
% \begin{align}
%     r_o = w_p(0.9 - \Vert \mathbf{o}_n^p - \hat{\mathbf{o}}_n^p \Vert_2 ) + w_q(\text{np.pi} - \text{Diff\_Angle}(\mathbf{o}_n^q - \hat{\mathbf{o}}_n^q )), \label{eq:rew_obj}
% \end{align}
% where $w_p$ and $w_q$ are the weights for position and orientation rewards, respectively, and $\text{Diff\_Angle}(\cdot, \cdot)$  computes the rotation angle difference between two quaternions. The hand reward is calculated as the negative weighted sum of the current hand joint positions and the reference positions:
% \begin{align}
%     r_h = -(w_{\text{trans}} \Vert \mathbf{h}_n[:3] - \hat{\mathbf{h}}_n[:3] \Vert_1 + w_{\text{ornt}} \Vert \mathbf{h}_n[3:6] - \hat{\mathbf{h}}_n[3:6] \Vert_1 + w_{\text{finger}} \Vert \mathbf{h}_n[6:] - \hat{\mathbf{h}}_n[6:] \Vert_1  ), \label{eq:rew_hand}
% \end{align}
% % degrees of freedom (DoF) 
% % \[
% % r_h = -\left(w_{\text{trans}} \|\mathbf{h}_n[:3] - \hat{\mathbf{h}}_n[:3]\|_1 + w_{\text{ornt}} \|\mathbf{h}_n[3:6] - \hat{\mathbf{h}}_n[3:6]\|_1 + w_{\text{finger}} \|\mathbf{h}_n[6:] - \hat{\mathbf{h}}_n[6:]\|_1\right), \label{eq:rew_hand}
% % \]
% with weights $w_{\text{trans}}, w_{\text{ornt}}$, and $w_{\text{finger}}$. The hand-object affinity reward encourages proximity between the hand palm and fingers and the object:
% \begin{align}
%     r_d = -(w_{\text{palm}} \Vert \mathbf{p}_n^{\text{palm}} - \hat{\mathbf{o}}_n^p \Vert + w_{\text{finger}} \sum_{i=1}^{n_f} \Vert \mathbf{f}_{n,i} - \hat{\mathbf{o}}_n^p \Vert),  \label{eq:rew_affinity}
% \end{align}
% % \[
% % r_d = -\left(w_{\text{palm}} \|\mathbf{p}_n^{\text{palm}} - \hat{\mathbf{o}}_n^p\| + w_{\text{finger}} \sum_{i=1}^{n_f} \|\mathbf{f}_{n,i} - \hat{\mathbf{o}}_n^p\|\right), \label{eq:rew_affinity}
% % \]
% where $w_{\text{palm}}$ and $w_{\text{finger}}$ are the weights for the palm-object and finger-object affinities, respectively, $n_f$ is the number of fingers, and $\mathbf{f}_{n,i}$ denotes the position of the $i$-th finger at timestep $n$. The overall reward is then computed as the sum of these three components: $r = r_h + r_o + r_d$.  
% % We utilize PPO~\citep{Schulman2017ProximalPO} as implemented in rl\_games~\citep{rlgames2021} to train our policy.
%%%%%%%%%%%%%%%%%%%%%% reward function %%%%%%%%%%%%%%%%%%%%%%


% \todo{bonus reward? }

% \textcolor{red}{(TODO: add the reward design here)}
% \textcolor{red}{(TODO: add the residual policy here --- it is important since we need to justify the task curriculum here)}

% By re-optimizng the residual policy, we can possibly arrive at a better 
% For instance, by setting the base trajectory to an action trajectory produced by an expert trained for a different trajectory, 
% It opens the opportunity to transfer 
% This strategy natrualy afford us an additional dimension in optimizing the single trajectory tracking policy. 
% we train the tracker to output a residual relative target $\Delta \mathbf{a}_n$. 
% letting the policy learn absolute positional targets $\mathbf{a}_n$, we 
% residual policies whose outputs are treated as residual positional targets added to a base trajectory. Formally, 
% given a base trajectory containing the hand DoF positos at each  timestep, \emph{i.e.,} $\mathbf{H}^b = \{ \mathbf{h}_n^b \}_{n=1}^N$, we let the policy to learn a residual positional 
% To further improve the RL's sample efficiency, instead of letting the policy to output abs

% \todo{residual policy here!!!}

% \noindent\textbf{Single manipulation trajectory specialist tracking policy.}  Given a kinematic manipulation trajectory $(\mathbf{H}, \mathbf{O})$, training a specialist policy aims at optimizing a tracking policy $\mathbf{\pi}(\cdot\vert\cdot )$ that can control a dexterous robot hand to track the reference kinematic trajectory. 
% We train a specialist policy leveraging RL to solve the problem. 
% Considering the intricate dynamics involved in the dexterous manipulation resulting from the high DoF of a dexterous hand and the rich and changing hand-object contacts, we resort to model free approaches and leverage RL to optimize the manipulation tracking policy. 
% \noindent\textbf{Trajectory specific specialist policy.} Given a kinematic manipulation trajectory $(\mathbf{H}, \mathbf{O})$, training a specialist policy aims at optimizing a tracking policy $\mathbf{\pi}(\cdot\vert\cdot )$ that can control a dexterous robot hand to track the reference kinematic trajectory. 
% Assuming the physical model is unknown and non-differentiable, we leverage reinforcement learning to optimize the policy. 

% \noindent\textbf{Imitation augmented RL for learning a general tracking controller.} 
% \noindent\textbf{Imitation augmented RL.} 

% \noindent\textbf{Additional Imitation Loss.}  

% \noindent\textbf{Imitation loss.}
% \noindent\textbf{Learning from tracking demonstration.} 
\noindent\textbf{Imitation learning.} 
% To let the tracking controller benefit from a large number of robot tracking demonstration data, we train 
% of imitation-ready data, we train the actor to imitate successful tracking results, aiming at distill ``tracking knowledge'' from these trajectories into the tracking controller. 
% Leveraging the powe
% Relying on RL solely can hardly let us train a strong tracking controller due to its restriction 
% The RL-based learning scheme, restricted by sample inefficiency and the incapability to master multiple tracking problems, can hardly solve the generalizable tracking control problem, as evidenced by our early experiments. Therefore, we propose an IL-based strategy and try to distill successful, abundant, and diverse ``tracking knowledge'' to the tracking controller. Specifically, we train the tracking agent to imitate a large number of high-quality robot tracking demonstrations. 
% In this way, we can effectively guide the agent to produce ``expert actions'' that can successfully track the reference state. Besides, by imitating diverse tracking demonstrations, the agent can avoid repeatedly experiencing low rewards in difficult tracking scenarios, while also preventing over-exploitation of easier tracking tasks. 
% Formally, a robot tracking demonstration of length $N$ contains a kinematic reference sequence $(\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_{N})$, and an expert's state-action trajectory $(\mathbf{s}_0^L, \mathbf{a}_0^L, ..., \mathbf{s}_{N-1}^L, \mathbf{a}_{N-1}^L, \mathbf{s}_N^L)$.
% In addition to the actor loss, we add an action supervision loss to bias the policy's prediction at each timestep towards its corresponding expert action in the demonstration: 
% \begin{align}
%     \mathcal{L}_a = \mathbb{E}_{\mathbf{a}_n\sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})} \Vert \mathbf{a_n} - \mathbf{a}^L_{n}  \Vert. 
% \end{align}
% In this way, we can guide the policy’s exploration via these demonstrations, ultimately speeding up convergence and improving the performance in the complex problem.  From the IL's perspective, the RL exploration adds noise to the states to make the imitation more robust to noise in a similar flavor to DART~\citep{laskey2017dart}. 
% Since the agent should not and will not explore states too far from the reference states in the tracking control task, it is possible to optimize the policy via both the imitation loss and RL reward simultaneously.
The RL-based learning scheme, hindered by sample inefficiency and its inability to handle multiple tracking problems, struggles to solve the generalizable tracking control problem, as demonstrated by our early experiments. Therefore, we propose an IL-based strategy to distill successful, abundant, and diverse ``tracking knowledge'' into the tracking controller. Specifically, we train the tracking agent to imitate a large number of high-quality robot tracking demonstrations. 
This approach effectively guides the agent to produce ``expert actions'' that can successfully track the reference state. Additionally, by imitating diverse tracking demonstrations, the agent can avoid repeatedly encountering low rewards in challenging tracking scenarios, while also preventing over-exploitation of easier tasks.
Formally, a robot tracking demonstration of length \(N\) consists of a kinematic reference sequence \((\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_{N})\) and an expert's state-action trajectory \((\mathbf{s}_0^L, \mathbf{a}_0^L, ..., \mathbf{s}_{N-1}^L, \mathbf{a}_{N-1}^L, \mathbf{s}_N^L)\). 
In addition to the actor loss, we incorporate an action supervision loss to bias the policy's predictions at each timestep towards the corresponding expert action in the demonstration:
\begin{align}
    \mathcal{L}_a = \mathbb{E}_{\mathbf{a}_n\sim \pi(\cdot \vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})} \Vert \mathbf{a_n} - \mathbf{a}^L_{n}  \Vert. 
\end{align}
This guidance allows the policy’s exploration to be informed by these demonstrations, ultimately speeding up convergence and enhancing performance in complex problems. From the perspective of IL, the RL exploration introduces noise into the states, making the imitation more robust, in a similar flavor to DART~\citep{laskey2017dart}. 
Since the agent should not and will not explore states too far from the reference states in the tracking control task, it is feasible to optimize the policy using both the imitation loss and RL reward simultaneously.


% the agent can avoid continuously experiencing low rewards in hard tracking cases, thereby free of exploiting easy tracking problems. 
% getting stuck in exploiting easy tracking problems due to low positive reward from hard tracking cases.
% ~\eric{due to low positive reward from hard tracking cases?}. 

% ~\eric{In addition to the actor loss,} 

% action prediction for the state-goal pair $(\mathbf{s}_n, \hat{\mathbf{s}}_{n+1})$ towards its corresponding expert action in the demonstration: 

% encourage the policy predict 
% when training the agent to solve the tracking problem with a kinematic sequence $(\hat{\mathbf{s}}_0, .., \hat{\mathbf{s}}_N)$ and the expert action trajectory $(\mathbf{a}^L_0, ..., \mathbf{a}^L_{N-1})$ from the demonstration, we add an action supervision loss to the policy's predicted action $\mathbf{a}_n$ at each timestep: 
% \begin{align}
%     \mathcal{L}_a = \sum_{n=0}^{N-1} \mathbb{E}_{\mathbf{a}_n\sim \pi(\cdot\vert \mathbf{o}_n, \hat{\mathbf{s}}_{n+1})} \Vert \mathbf{a_n} - \mathbf{a}^L_{n}  \Vert.  
% \end{align}

% making it possible to optimize with both the imitation loss and RL reward simultaneously.
% In the tracking control task, where the RL should not and will not explore states too far from the reference states, making it possible to optimize with both the imitation loss and RL reward simultaneously.
% the demonstrations can guide 
% The demonstrations bias the policy toward the supervision data. It can thereby 

% for each tracking demonstration containing the expert action sequence $(\mathbf{a}^L_0, ..., \mathbf{a}^L_{N-1})$ for tracking the kinematic sequence $(\hat{\mathbf{s}}_0, .., \hat{\mathbf{s}}_N)$, we add an action supervision loss to the policy's predicted action $\mathbf{a}_n$ at each timestep
% hardly offer us a strong tracking controller. 
% can hardly let us get a strong tracking controller. 
% To facilitate the learning of the tracking controller, we propose to distill successful ``tracking knowledge'' from high-quality robot tracking demonstrations. 
% % Specifically, we propose to train the  tracking controller to imitate high-quality robot tracking demonstrations. 
% % propose to leverage the joint power of RL and IL and train the tracking 
% Specifically, instead of relying on the RL-based training scheme solely, we additionally train the tracking controller to imitate high-quality robot tracking demonstrations. 
% % in addition to the RL-based training scheme, 
% Formally, for each trajectory with the action sequence $(\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L)$, we incorporate the following action supervision loss into the policy's prediction at each timestep \((\mathbf{\mu}_n, \mathbf{\sigma}_n)\) to  encourage the actor to mimic this trajectory: 
% % encourage the actor to mimic this trajectory at each timestep by incorporating the following action supervision loss into the policy's prediction at each timestep \((\mathbf{\mu}_n, \mathbf{\sigma}_n)\):
% \begin{align}
%     \mathcal{L}_a = \Vert \mathbf{\mu}_n -  \mathbf{a}_n \Vert, 
% \end{align} 
% where \(\mathbf{a}_n\) denotes the action taken at the \(n\)-th timestep from the action trajectory $\mathbf{A}_L$.


% This strategy aims to align the action trajectory produced by the current policy with the optimized successful action sequence from the dataset, resembling the approach used in DART~\citep{laskey2017dart}~\eric{from RL's perspective, the demonstrations bias the policy toward the supervision data. from IL's perspective, the RL exploration adds noise to the states to make the imitation more robust to noise in a similar flavor to DART}.~\eric{Also mention that since this is the tracking task, the RL policy should not and will not explore states too far from the reference states, making it possible to optimize with both the imitation loss and RL reward simultaneously.}


% s at each timestep \((\mathbf{\mu}_n, \mathbf{\sigma}_n)\):
% an imitation loss to the 
% Given a dataset containing paired kinematic trajectories and action sequences $\mathcal{S}_L=\{ (\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L) \}$, we introduce an additional action supervision loss to the actor loss, aimed at distilling successful ``tracking knowledge'' from these trajectories into the tracking controller. 

% Formally, for each labeled trajectory \((\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L)\), we incorporate the following action supervision loss into the policy's predictions at each timestep \((\mathbf{\mu}_n, \mathbf{\sigma}_n)\):
% \begin{align}
%     \mathcal{L}_a = \Vert \mathbf{\mu}_n -  \mathbf{a}_n \Vert, 
% \end{align}
% where \(\mathbf{a}_n\) denotes the action taken at the \(n\)-th timestep from the optimized action trajectory. This strategy aims to align the current trajectory with the optimized successful trajectory from the dataset, resembling the approach used in DART~\citep{laskey2017dart}.

% \noindent\textbf{Additional imitation loss.} 
% Given a dataset containing paired kinematic trajectories and action sequences $\mathcal{S}_L=\{ (\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L) \}$, we add an additional action supervision loss to the actor loss to distill successful ``tracking knowledge'' from these trajectories to the tracking controller. 
% Formally, for each labeled trajectory $(\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L)$, the following action supervised loss is additionally added on the policy's prediction in each timestep $(\mathbf{\mu}_n, \mathbf{\sigma}_n))$ to train the policy:
% \begin{align}
%     \mathcal{L}_a = \Vert \mathbf{\mu}_n -  \mathbf{a}_n \Vert, 
% \end{align}
% where $\mathbf{a}_n$ denotes $n$-th step action taken from the optimized action trajectory. This strategy tries to bias the current trajectory towards the optimized successful trajectory in the dataset, in a similar flavor to DART~\citep{laskey2017dart}. 


% With the carefully designed specialist policy training strategy and the task relational space exploration and modeling scheme, it is possible for us to optimize for a satisfactory result for each single manipulation trajectory tracking task. However, it is still not enough to acquire a generalist that can not only achieve good performance in each sequence but even generalize to unseen trajectories. Simply following the above RL scheme and training a single policy on multiple tasks is not feasible as demonstrated in our early experiments. As the number of training tasks increases, the RL would even struggle with effectively optimizing a strong policy that can solve every training task, letting alone generalize to unseen trajectories and resolve the novel manipulation sequence tracking challenge. We suppose such pool fitting phenomenon comes from the inherent deficiency of RL in solving multiple tasks. We therefore propose to introduce labeled single trajectory optimization results into the training process of RL, \textit{i.e.,} providing additional action labels as the supervision signals to train the policy together with RL. Specifically, 
% n action-labeled dataset 

% wthe imitation augmented RL involves adding an additional action supervision loss to the actor loss to distill successful ``tracking knowledge'' from these trajectories to the tracking controller. 
% where each trajectory $(\mathbf{H}_L, \mathbf{O}_L)$ is augmented with an additional action sequence $\mathbf{A}_L$, 
% we add an action supervision loss to the actor loss. 
% produced by well-trained per-trajectory trackers,
% Intuitively, this strategy tries to distill knowledge form the action-labeled trajectories to the tracking controller. 
% optimized knowledge in per-trajectory trackers to the general tracking controller. 

% $(\mathbf{\mu}_n, \mathbf{\sigma}_n) = \mathbf{\pi}(\cdot \vert \hat{\mathbf{s}}_n)$ to train the policy:

% to train the policy $\mathbf{\pi}(\cdot\vert \cdot)$  


% \todo{need to say we usthe same model-free tacking algo as that for the tracking controller}
\vspace{-5pt}
\subsection{Mining High-Quality Robot Tracking Demonstrations Using Neural Controller through a Homotopy Optimization Scheme} 
\label{sec:method_data}
\vspace{-5pt}
% To prepare demonstrations to train the tracking controller, we need to infer action sequences from kinematic-only trajectories to create paired data with kinematic references and the action sequence. We primarily leverage model-free reinforcement learning techniques to train the tracking policy for each single trajectory to acquire its corresponding action sequence.~\eric{we should briefly explain the naive way of doing per-trajectory tracking. No one knows its relation with the controller at this moment and we should not assume that is straightforward to understand.} Though this straightforward solution can successfully track lots of trajectories~\eric{I think we should mention that a lot of trajectories can not be tracked by this naive method instead of emphasizing that it is already quite successful?}, relying solely on optimizing per-trajectory tracking policy independently presents challenges for complex tracking scenarios. To resolve difficulties in tracking challenging trajectories to improve the diversity and the quality of tracking demonstrations, we then explore the possibility of~\eric{this expression sounds weak} using the tracking controller through a homotopy optimization scheme to improve per-trajectory tracking by 1) transferring tracking prior from the tracking controller and 2) learning a homotopy path generator which can propose useful homotopy paths that we can leverage to track previously difficult-to-track trajectories through a homotopy optimization method. 
% % directly training a policy leveraging RL with the above designs 

% Preparing demonstrations to train the training controller

% Preparing demonstrations to train the tracking controller requires us to infer the action 
% To prepare a demonstration to train the tracking controller, we need to infer the action sequence $(\mathbf{a}^L_0,...,\mathbf{a}^L_{N-1})$ that can successfully track the kinematic reference trajectory $(\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)$. A naive way is leveraging RL to train a single trajectory tracking policy $\pi$ and take its resulting action sequence as the demonstration. However, leveraging this strategy alone can hardly provide us with a diverse and high-quality tracking demonstration dataset because RL would be challenged by the inherent difficulties in dexterous manipulation. To improve the diversity and the quality of robot tracking demonstrations, we propose to leverage the tracking controller and a homotopy optimization scheme to improve the per-trajectory tracking results. 

To prepare a demonstration from a kinematic reference trajectory \((\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)\) for training the tracking controller, we need to infer the action sequence \((\mathbf{a}^L_0, ..., \mathbf{a}^L_{N-1})\) that successfully tracks the reference sequence.  
% trajectory \((\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)\). 
A straightforward approach is to leverage RL to train a single-trajectory tracking policy \(\pi\) and use its resulting action sequence directly. 
% as the demonstration. 
However, relying solely on this strategy often fails to provide a diverse and high-quality dataset of tracking demonstrations, as RL struggles with the inherent challenges of dexterous manipulation.
To enhance both the diversity and quality of robot tracking demonstrations, we propose utilizing the tracking controller in conjunction with a homotopy optimization scheme to improve the per-trajectory tracking results.

% We first think present a naive solution 

% ~\eric{train a single policy or train a per-trajectory tracking policy?
% }

% of the inherent difficulty of dexterous manipulation tracking that would 
% which will challenge the optimization of RL, especially in difficult manipulation tracking problems.

% this strategy can hardly provide 
% Specifically, we can formulate is as a single trajectory tracking problem. Given the kinematic references, we aim at optimizing a tracking policy $\pi$ that can track the reference trajectory. In each tiemstep, $\pi$ observes the current state $\mathbf{s}_n$ and the next goal state $\hat{\mathbf{s}}_{n+1}$; and predict the distribution of the current action $\mathbf{a}_n$. $\pi$ is optimized to minimize the difference between the transited state $\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)$ in each timestep $n$ is close to the goal state $\hat{\mathbf{s}}_{n+1}$. 
% By sampling from the $\pi$ in each step and transiting to the next state, we can  
% However, this way of doing per-trajectory tracking cannot provide us with 

\noindent\textbf{RL-based single trajectory tracking.} 
% A basic solution to acquire the demonstration is leveraging RL to solve the per-trajectory tracking problem and taking the resulting action sequence as the demonstration. Given a kinematic reference trajectory, we aim at optimizing a tracking policy $\pi$ that can track the reference trajectory. In each timestep, $\pi$ observes the current state $\mathbf{s}_n$ and the next goal state $\hat{\mathbf{s}}_{n+1}$. It then predicts the distribution of the current action $\mathbf{a}_n$. 
% The policy $\pi$ is optimized to minimize the difference between the transited state $\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)$ at each timestep $n$ and the goal state $\hat{\mathbf{s}}_{n+1}$. Similar to our design for the RL-based learning scheme for the tracking controller, we adopt a residual action space. We introduce a baseline trajectory $(\mathbf{s}^b_0,...,\mathbf{s}^b_N)$ for each tracking task, while only leveraging RL to learn a residual policy. Observations and reward are the same to our design for tracking controller (see Eq.~\ref{eq_obs}~\ref{eq_rew}). Once $\pi$ has been optimized, we can sample the action $\mathbf{a}_n$ from $\pi$ in each timestep. By iteratively transferring to the next state using the predicted action and querying the policy $\pi$ to generate a new action, we can get the expert action sequence $(\mathbf{a}_0^L, ..., \mathbf{a}_{N-1}^L)$ for the input kinematic reference trajectory. 
A basic approach to acquiring demonstrations is to leverage RL to address the per-trajectory tracking problem, using the resulting action sequence as the demonstration. Given a kinematic reference trajectory, our goal is to optimize a tracking policy \(\pi\) that can accurately track this reference trajectory. At each timestep, \(\pi\) observes the current state \(\mathbf{s}_n\) and the next goal state \(\hat{\mathbf{s}}_{n+1}\), and it predicts the distribution of the current action \(\mathbf{a}_n\).
The policy \(\pi\) is optimized to minimize the difference between the transited state \(\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)\) at each timestep \(n\) and the goal state \(\hat{\mathbf{s}}_{n+1}\). Similar to our design for the RL-based learning scheme for the tracking controller, we adopt a residual action space. For each tracking task, we introduce a baseline trajectory \((\mathbf{s}^b_0, ..., \mathbf{s}^b_N)\) and only learn a residual policy using RL. The observations and rewards follow the same design as for the tracking controller (see Eq.~\ref{eq_obs} and Eq.~\ref{eq_rew}).
Once \(\pi\) has been optimized, we can sample the action \(\mathbf{a}_n\) from \(\pi\) at each timestep. By iteratively transitioning to the next state using the predicted action and querying the policy \(\pi\) to generate a new action, we can obtain the expert action sequence \((\mathbf{a}_0^L, ..., \mathbf{a}_{N-1}^L)\) for the input kinematic reference trajectory.


% $\pi$ is optimized to minimize the difference between the transited state $\mathbf{s}_{n+1} \sim p(\cdot \vert \mathbf{s}_n, \mathbf{a}_n)$ in each timestep $n$ is close to the goal state $\hat{\mathbf{s}}_{n+1}$.~\eric{this sentence is grammarly incorrect.}

% with those designed for the tracking controller (see Eq.~\ref{eq_obs}~\ref{eq_rew}). 
% each kinematic trajectory, while 



% naive per-trajectory tracking 

% \noindent\textbf{Transferring tracking prior.} 
\noindent\textbf{Transferring \textcolor{myblue}{``tracking prior''}.} 
% To improve the quality and diversity of the demonstrations, we devise a strategy that utilizes the general ``tracking knowledge'' encoded in the universal tracking controller to improve trajectory-specific tracking policies. Specifically, to track a kinematic reference trajectory $(\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)$, we first track it via the tracking controller with the baseline trajectory set to the kinematic reference. We then set the baseline trajectory to the resulting action sequence and re-optimize the residual policy leveraging the RL-based single trajectory tracking method. The tracking controller can help us find a better baseline trajectory, which eases policy learning and improves the single trajectory tracking result. 
To \textcolor{myblue}{improve the demonstrations, we devise a strategy that takes advantage of the tracking controller, which has already encoded ``knowledge'' that can track lots of trajectories (named as ``tracking prior''), to improve trajectory-specific tracking policies}.
% improve the quality and diversity of demonstrations, we devise a strategy that takes advantage of the general ``tracking knowledge'' encoded in the universal tracking controller to improve trajectory-specific tracking policies. 
Specifically, to track a reference trajectory \((\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)\), we first utilize the tracking controller to track it, with the baseline trajectory set to thew reference sequence. We then adjust the baseline trajectory to the resulting action sequence and re-optimize the residual policy using the RL-based single trajectory tracking method. This approach can help us find a better baseline trajectory, facilitating single-trajectory tracking policy learning and improving the per-trajectory tracking results. 
% the result. 
% the single trajectory tracking result. 
% allows the tracking controller to find a better baseline trajectory, facilitating policy learning and improving the single trajectory tracking result. 

% ~\eric{it might confuse the reader here since the tracking policy refers to a per-trajectory tracker while the tracking controller refers to the general tracker. I think it would be better if we could use a more distinctive term to differentiate in this whole section. Maybe trajectory-specific tracking policy v.s. universal tracking controller?} 

% per-trajectory tracking. 

% The tracking controller can help us find a better baseline trajectory that would ease the policy learning, thereby facilitating the per-trajectory tracking. 

% per-trajectory tracking.
% Then we set the baseline trajectory as the
% use the tracking controller to track 
% to track a 
% % for a 
% kinematic reference trajectory $(\hat{\mathbf{s}}_0, ..., \hat{\mathbf{s}}_N)$, we first query the tracking controller to generate an action sequence $(\mathbf{a}^{\text{prior}}_0, ..., \mathbf{a}^{\text{prior}}_{N-1})$. After that, we set the baseline trajectory as the sampled actions and optimize the residual policy leveraging the RL-based per-trajectory tracking scheme. The tracking controller can help us find a better baseline trajectory that would ease the policy learning, thereby facilitating the per-trajectory tracking. 
% If the action sequence we've sampled from the tracking controller proved to serve as a better baseline trajectory for the single trajectory tracking policy, we then take the new tracking result as its action sequence and improve the demonstration. 
% Since the tracking controller 
% Once the residual policy have been optimized, we can get its tracking results. If we can better track the kinematic references in this way than adopting the original approach, 
% without transferring the tracking prior, 
% the resulting action 
% If the action sequence 

% can get a better tracking result. 
% baseline trajectory that we've sampled from the tracking controller proves to serve asa 
% transfer the general knowledge encoded in the tracking controller to improve the per
% Considering the 
% the limitations of leveraging RL to solve the per-trajectory tracking 
% With the tracking controller, which has already been optimized to be able to track lots of manipulation trajectories, we devise a method that can let the single trajectory tracking benefit from the tracking controller. Specifically, for a tracking task $T$ that is difficult to solve, we first query the tracking controller for an action sequence $\mathbf{A}$. After that, we initialize $\mathbf{A}$ as the basic trajectory in the single trajectory tracking policy~\eric{since we did not explain how to do the per-trajectory tracking above, it is weird here to talk about the base trajectory.}. We then optimize the residual policy aiming to track the trajectory $T$.  Taking advantage of the general tracking prior encoded in the tracking controller, we can potentially~\eric{do not use these very vague term} get better tracking results than directly tracking $T$ with the kinematic sequence as the basic trajectory. 
% After that, we optimize the residual policy aiming to track the trajectory $T$.



% \noindent\textbf{Learning a homotopy path generator and tracking via a homotopy method.} 

% \noindent\textbf{Solving difficult tracking problem via a homotopy optimization scheme.} 
\noindent\textbf{A homotopy optimization scheme.}
% The tracking controller's training relies on the results from previously successfully tracked trajectories, which would limit its ability.~\eric{this sentence seems redundant. maybe remove it and just keep the next sentence.} 
Training the controller with data mined from itself can introduce biases and reduce diversity, hindering its generalization capabilities. To address this issue, we propose a homotopy optimization scheme to improve the per-trajectory tracking performance and to tackle previously unsolvable single-trajectory tracking problems. For the tracking problem $T_0$, instead of solving it directly, the homotopy optimization iteratively solves each tracking task in an optimization path, \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$, and finally solves $T_0$, in a similar flavor to ``chain-of-thought''~\citep{Wei2022ChainOT}. In the beginning, we leverage the RL-based tracking method to solve $T_K$. After that, we solve each task $T_m$ via the RL-based tracking method with the baseline trajectory set to the tracking result of $T_{m+1}$. This transfer of tracking results from other tasks helps us establish better baseline trajectories, ultimately yielding higher-quality tracking outcomes.
% solves it via iteratively solving each tracking task in an optimization path, \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$, 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Transferring the tracking results of other tasks can help us find better baseline trajectories, thereby offering us better tracking results with improved quality. 
% an optimization path,  \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$. 
% Instead of tracking a trajectory directly, the homotopy optimization 
% solving each single-trajectory tracking problem directly, 
% % a strategy that utilizes RL and transfers tracking knowledge to tackle previously unsolvable single-trajectory tracking problems. 
% Instead of addressing each single-trajectory problem directly, we employ a homotopy optimization method, inspired by the "chain-of-thought" approach~\citep{Wei2022ChainOT}, to enhance tracking results. Specifically, the homotopy optimization addresses the tracking problem for task \(T_0\) through an optimization path, \((T_K, T_{K-1}, ..., T_0)\). Initially, we use RL to solve for \(T_K\). Subsequently, we address each task \(T_m\) by applying the RL-based tracking method, using the tracking result of \(T_{m+1}\) as the baseline trajectory. This transfer of tracking results from other tasks enables us to establish better baseline trajectories, ultimately yielding higher-quality tracking outcomes.

% Considering the fact that the tracking controller is trained with the supervision from the tracking results of the already successfully tracked trajectories, its ability would be restricted.  Using data mined by the controller to train the controller could suffer from data biases and diversity issues, which may hinder the generalization ability of the tracking controller. To mitigate this issue, we need a strategy that can solve previously unsolvable single trajectory tracking problems by leveraging RL and even transferring the tracking prior. Therefore, instead of solving each single-trajectory tracking problem directly, we propose to leverage a homotopy optimization method, mimicking ``chain-of-thought''~\citep{Wei2022ChainOT}, to improve the tracking results. Specifically, the homotopy optimization solves the racking problem of task $T_0$ via an optimization path,  \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$. At the beginning, we leverage the RL to solve $T_K$. After that, we solve each task $T_m$ via the RL-based tracking method with the baseline trajectory set to the tracking result of $T_{m+1}$. Transferring the tracking results of other tasks can help us find better baseline trajectories, thereby offering us better tracking results with improved quality. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% may be restricted in the ability to solve 
% relatively simple tracking problems.
% Therefore, using the data mined 
% that can effectively improve the diversity and quality 
% ~\eric{Need to mention that the using the data mined by the controller to train the controller could suffer from data biases and diversity issues, which could hinder the generalizability of the controller to novel and challenging cases. Therefore we need bias mitigation techniques.} Solving very difficult single trajectory tracking problems would still pose lots of challenges. 

% optimizing the per-trajectory tracker alone, we propose to leverage a 

% to improve the tracking results of very difficult trajectories~\eric{very difficult trajectories sound like just a very small portion of the data? it is better to give the feeling that the method is generally helpful}.

% higher-quality
% by the controller to train the controller could suffer from data biases and diversity issues, which may hinder the generalization ability of the tracking controller. To mitigate this issue, we need a strategy that can solve previously unsolvable single trajectory tracking problems by leveraging RL and even transferring the tracking prior. 
% by transferring the tracking result of $T_{m+1}$ as the baseline trajectory. x

% In this way, we leverage the tracking knowled
% If the tracking result of $T_0$ can achieve can achieve better tracking performance
% Iteratively solving each problem 
% transfer the tracking results of $T_{m+1}$ as the baseline trajectory of the tracking task $T_m$  
% solve the per-
% for a tracking task $T_0$, 
% $T_0$ that is hard to solve, we propose to solve $T_0$ via a homotopy path, \emph{e.g.,} $(T_K, T_{K-1}, ..., T_0)$. Starting from solving the first task $T_K$, we transfer the tracking result obtained in the current task to initialize the basic trajectory of the next tracking task. By gradually transferring tracking results from the previous task and solving each problem gradually in this manner, we could potentially~\eric{again, this is a very weak term and should be avoided} get better tracking results of task $T_0$. 

\noindent\textbf{Finding effective homotopy optimization paths.}
% Although leveraging the homotopy optimization scheme to solve previously unsolvable tracking problems proves to be an effective strategy for many tracking tasks, it relies on effective optimization paths. A naive way to find an effective homotopy path is brute-force searching. Specifically, given a collection of kinematic references, we optimize their per-trajectory tracking results at first. We also identify neighbors for each tracking task, \emph{e.g.,} based upon the similarity between every two kinematic reference trajectories. After that, we iteratively transfer the optimization results from neighbors and re-optimize the residual policy for each tracking task. We record the neighbor that can give the current tracking task a better baseline trajectory than its kinematic reference sequence as an effective ``parent task''. After we've reached the maximum number of iterations, \emph{i.e.,} $K$, to find effective homotopy paths for the tracking task $T_0$, we can start from $T_0$ and backtrace effective ``parent tasks''. We regard $(T_{K}, ..., T_0)$ as an effective homotopy path of $T_0$ if for each $0\le m \le K$, $T_{m+1}$ is an effective parent task of $T_m$. 
While leveraging the homotopy optimization scheme to solve previously unsolvable problems has proven effective for many tasks, it depends on identifying effective optimization paths. A straightforward approach is brute-force searching. Specifically, given a set of kinematic references, we first optimize their per-trajectory tracking outcomes. We then identify neighbors for each task based on the similarity between pairs of kinematic reference trajectories. Next, we iteratively transfer optimization results from neighboring tasks and re-optimize the residual policy for each tracking task. For a specific task, we consider a neighbor that provides a better baseline trajectory than its kinematic trajectory as an effective ``parent task''.
% We consider a neighbor that provides a better baseline trajectory than the original kinematic reference as an effective ``parent task''. 
After reaching the maximum number of iterations, $K$, we can find effective homotopy paths for a task, \emph{i.e.,} $T_0$, by starting from $T_0$ and backtracing
% begin from the target task to optimize $T_0$ and backtrace 
% the
effective ``parent tasks''. We define $(T_{K}, ..., T_0)$ as an effective homotopy path for $T_0$ if, for each $0 \leq m \leq K$, $T_{m+1}$ is 
% serves as 
an effective parent task for $T_m$.


% In each iteration, for each tracking task, we try to transfer the tracking result of each of its neighbors as its baseline trajectory and re-optimize the residual tracking policy. 

% suppose we wish to 
% several iterations, 

% the best initialization as the best ``parent task''. After several iterations, \emph{i.e.,} $K$, if we can solve the current target tracking task successfully (\emph{i.e.,} achieving the tracking error smaller than a success threshold), we then start from the current tracking task and backtrace to find an effective homotopy optimization path. In more detail, starting from the task $T_0$, we can find its best ``parent task'' $T_1$. Then for each $1\le m\le K-1$, we find its best ``parent task'' $T_{m+1}$. Finally, we get an effective optimization path $(T_{K}, ..., T_0)$ for the task $T_0$. 

% If we can get better tracking result, we record the 
% every tracking task, we try to transfer th 


% \noindent\textbf{Learning a homotopy generator by encoding effective optimization paths.} 
\noindent\textbf{Learning a homotopy generator for efficient homotopy path planning.} 
% Leveraging the homotopy optimization scheme to 
% Since finding effective homotopy optimization paths is costly, which is unaffordable during the inference time 
% Finding effective homotopy optimization paths for tracking each trajectory is extremely costly and unaffordable during inference time. Therefore, we propose to learn a homotopy path generator $\mathcal{M}$ from a small set. Then, we can use the homotopy generator to propose effective homotopy paths for a tracking task efficiently. The most critical part of finding a homotopy path is finding effective ``parent tasks''. We re-formulate the homotopy path generator learning problem as a tracking task transformation problem. For each tracking task $T_0$, we wish the generator $\mathcal{M}$ to give us a distribution of its effective ``parent tasks'': $\mathcal{M}(\cdot\vert T_0)$, considering the fact that a single tracking task may have multiple effective ``parent tasks''. Once $\mathcal{M}$ has been trained, for $T_0$, we can iteratively query $\mathcal{M}$ to generate a homotopy path: $(T_K, ..., T_0)$, where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m), \forall 0\le m\le K-1$. 
% We propose to learn a conditional diffusion model as the tracking task transformer, taking advantage of its strong distribution modeling ability. Given a collection of tracking tasks, described using the kinematic reference trajectories of the hand and the object, and the object geometry, we first train a diffusion model to describe the distribution of tracking tasks. 
% To prepare data to fine-tune the diffusion model into a conditional diffusion model, we first search effective homotopy paths from the tracking task collection. 
% Having completed the search, we can obtain a set of paired data of (tracking task $T_c$, effective ``parent task'' $T_p$). 
% We then use these data to tune the diffusion model into a conditional diffusion model, \emph{i.e.,} $T_p \sim \mathcal{M}(\cdot\vert T_c)$. A well-trained $\mathcal{M}$ can propose an effective ``homotopy path'' by recursively finding the parent: $(T_K,...,T_0)$, where $T_{m+1}\sim \mathcal{M}(\cdot \vert \mathcal{T}_m),\forall 0\le m\le K-1$.
Finding effective homotopy optimization paths for tracking each trajectory is computationally expensive and impractical during inference. To address this, we propose learning a homotopy path generator $\mathcal{M}$ from a small dataset, enabling efficient generation of effective homotopy paths for other tracking tasks. The key problem in identifying homotopy paths lies in finding  effective ``parent tasks''. We reformulate this problem as a tracking task transformation problem,
% , 
aiming for a generator $\mathcal{M}$ that provides a distribution of effective ``parent tasks'' for each tracking task $T_0$: $\mathcal{M}(\cdot \vert T_0)$, considering the fact that a single tracking task may have multiple effective ``parent tasks''.
Once $\mathcal{M}$ is trained, we can find a homotopy path by iteratively finding parent tasks.
% iteratively query it to generate a homotopy path for a tracking task. 
% for $T_0$: $(T_K, ..., T_0)$, where $T_{m+1} \sim \mathcal{M}(\cdot \vert T_m)$ for all $0 \le m \le K-1$.
We propose training a conditional diffusion model as the tracking task transformer, leveraging its strong distribution modeling capability. Given a set of tracking tasks, characterized by the kinematic reference trajectories of the hand and object, as well as object geometry, we first train a diffusion model to capture the distribution of tracking tasks.
To fine-tune this diffusion model into a conditional model, we first search for effective homotopy paths within the tracking task dataset. This yields a set of paired data of the tracking task $T_c$ and their corresponding effective ``parent task'' $T_p$. We then use this data to tune the diffusion model into a conditional diffusion model, such that $T_p \sim \mathcal{M}(\cdot \vert T_c)$. A well-trained $\mathcal{M}$ can efficiently propose an effective homotopy path for a tracking task, \emph{i.e.,} $T_0$, by starting from $T_0$ and recursively finding the parent task, resulting in  $(T_K, ..., T_0)$, where $T_{m+1} \sim \mathcal{M}(\cdot \vert T_m)$ for all $0 \le m \le K-1$.
% propose an effective homotopy path by recursively finding parent tasks: $(T_K, ..., T_0)$, where $T_{m+1} \sim \mathcal{M}(\cdot \vert T_m)$ for all $0 \le m \le K-1$.


% that can efficiently generate an effective homotopy path $(T_K, ...., T_0)$ for a tracking task $T_0$. 
% With the learned generator $\mathcal{M}$, we can leverage it to efficiently
% With the learned generator $\mathcal{M}$, 
% Then we can transfer the knowledge of ``homotopy paths'' encoded in $\mathcal{M}$ to more diverse trajectories and plan effective homotopy paths for them using $\mathcal{M}$ in an efficient manner. 

% apply the homotopy generator 
% effectively transfer the 
% Since t


% With a well-trained $\mathcal{M}$, we can recursively find 
% ~\eric{Need a summary sentence describing the inference time behavior?} 

% the collection of tracking tasks. 
% a collection of 
% We first train a diffusion model to describe the distribution of 
% To prepare data, we first search effective homotopy paths from a collection of tracking tasks. Having completed the search, we can obtain a set of paired data of (tracking task, effective ``parent task''). 
% After the search 
% Each searched path can give us a collection of paried tracking 

% can be leveraged to propose effective homotopy optimization paths efficiently during the inference. 



% Taking the tracking task $T_0$ as the example, in each iteration, we try to transfer the optimization result of each  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \noindent\textbf{Learning a homotopy generator by encoding beneficial optimization paths.} 
% \noindent\textbf{Learning a homotopy generator by encoding beneficial optimization paths.} 
% Solving each difficult tracking task in this fashion~\eric{what fashion? make sure every time when you use pronoun, it is clear}, though proved to enough effective, relies on correct~\eric{effective or correct? there does not seem to be a only correct answer for homotopy path} homotopy paths.~\eric{need to explain the naive way to build these paths first (the basic trial and error stuff) before you comment on the cost below.} Searching for correct paths for each difficult-to-track trajectory from scratch, however, is very costly. Therefore, we propose to learn a homotopy generator that can directly propose beneficial homotopy paths at the inference time.~\eric{comment on its connection of chain of though}
% Learning a homotopy generator requires valid optimization paths.~\eric{it is not clear since people dont know you are learning in a supervised manner. You assume too much context here.} Thus we first design an automatic tracking task structure exploration strategy for finding beneficial homotopy paths. We then train a homotopy generator to encode the mined paths~\eric{for efficient inference}.

% Specifically, we try to explore beneficial homotopy optimization paths from the trajectories in the training dataset via a breadth-first-searching strategy. 
% % Specifically, we iteratively explore beneficial cross-tracking task relations from a set of kinematic trajectories
% % We iteratively explore  beneficial cross-.
% % We explore beneficial homotopy paths from the trajectories in the training dataset via a 
% In each searching iteration, we iteratively explore beneficial cross-tracking task relations~\eric{this term is weird and not intuitive. An easier way to introduce what you what to do is to define the term first and then use it. It seems we are using terms first and deine later...Here for every two trajectories, we can evaluate whether their tracking results can benefit the tracking process of each other and we use directional edges to encode such relations.} from a set of kinematic trajectories. For each trajectory, we first identify its neighborhood from other kinematic trajectories via the similarity between two kinematic sequences. After that, we first run the per-trajectory tracking optimization to get their tracking results. Then we try to construct cross-tracking task relations via an iterative BFS approach. 
% In each iteration, for each tracking task $T$, we try to transfer the tracking result of its neighbour $T_p$ to initialize its basic trajectory and re-train the residual policy. If we can get better tracking results using the initialization from $T_p$, we say $T_p\rightarrow T$ a beneficial cross-task relation. We regard $T_p$ as the ``parent trajectory'' of $T$. We record the best tracking result for each trajectory obtained at this iteration.
% After severe iterations, we have obtained a beneficial cross-task relation set $\mathcal{C} = \{ (T_p\rightarrow T) \}$ which contains each beneficial cross-task relation. With $\mathcal{C}$, we regard $(T_{K}, T_{K-1}, ..., T_0)$ is a valid homotopy path if $T_{m+!}$ is the parent task of $T_m$ for each $0\le m \le K - 1$. 



% We propose to train a model that transforms each trajectory $T_c$ to the parent trajectory $T_p$ to model the tracking task structure.~\eric{need to talk about the motivation. the previous mined relationship is only a small set due to the heavy computation cost and we need to use the model to cover more diverse trajectories} 
% Considering the fact that a single child trajectory $T_c$ may have multiple different parent trajectories $T_p$, we formulate it as a conditional trajectory generation problem where the goal is to generate the parent trajectories conditioned on the child $T_c$. Therefore, we train a conditional diffusion model to accomplish this vision. Specifically, we first train a trajectory diffusion model $\mathcal{M}$ which models the distribution of all kinematic trajectories. After that, we fine-tune it to a conditional generative model that describes the distribution of the parent trajectory of each child trajectory. By sampling from the conditional generative model, we transform each tracking task to its parent tracking task, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. We can construct a homotopy path by iteratively querying the conditional generative model to sample the parent tasks, \emph{i.e.,} $(T_K, T_{K-1}, ..., T_0)$ where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m)$, $0\le m \le  K - 1$. 

% At the inference time, we let the homotopy generator propose a homotopy path for a hard-to-solve task $T$.~\eric{when to stop?} We gradually solve each tracking task in the path and transfer tracking results to the next task to solve the problem finally. 


% These tracking results are regarded as 
% For each trajectory, we first identify a neighborhood for it from other kinematic trajectories via the similarity between two kinematic trajectories. We first run the per-trajectory tracking optimization to get their individual tracking results. Then we try to construct cross-task relations using an iterative BFS approach. 
% % \todo{all trajs with the initially optimized results} \todo{at first jwe identify ja neighborhood set } 
% In each iteration, for each 





% homotopy path exploration strategy for 
% automatic tracking task structure exploration strategy for finding beneficial homotopy paths. Then we train a homotopy generator to encode the mined paths.


% previous tracking task to initialize the basic trajectory of the next tracking task. By gradually solving each problem in this manner in the series, we could potentially get better results in the task $T$, taking advantage of the basic trajectory initialized from other tracking tasks. 

% % to explore the tracking task
% % explore the tracking task structure and leverage a homotopy method to resolve these challenges by borrowing knowledge from other problems. 
% % Specifically, for a tracking task 
% % to explore


% The homotopy method, though proved to enough effective in resolving challenges in very difficult tracking tasks, relies on correct homotopy paths. 




\vspace{-5pt}
\subsection{Improving the Tracking Controller via Iterative Optimization}
\label{sec:method_iteration}
\vspace{-5pt}

% We employ an iterative approach that alternates between training the tracking controller using abundant robot tracking demonstrations and curating more diverse and higher-quality tracking demonstrations using the controller. Our method consists of three stages. 
% In the first stage, we sample a small set of tracking tasks and generate a demonstration set by applying reinforcement learning (RL) to obtain single trajectory tracking results for each task.  With these demonstrations, we train a tracking controller using RL and IL. We do not learn the homotopy path generator at this stage because the generalization ability of the learned model will be restricted by the number of effective homotopy paths used for training. 
% In the second stage, we sample a trajectory dataset from the remaining tasks, weighted by the tracking error of the controller. We use RL, with attempts to transfer tracking prior, to obtain per-trajectory tracking results, search for homotopy paths, and learn a homotopy generator based on these results. The best tracking results of all successfully tracked trajectories are then curated into a new demonstration set, which we use to re-train the tracking controller.

We adopt an iterative approach that alternates between training the tracking controller with abundant robot tracking demonstrations and curating more diverse, higher-quality demonstrations using the controller. Our method is divided into three stages.
In the first stage, we sample a small set of tracking tasks and generate an initial demonstration set by applying RL to obtain single-trajectory tracking results for each task. Using these demonstrations, we train the tracking controller with both RL and IL. At this stage, we do not train the homotopy path generator, as the model's generalization ability would be limited by the small number of effective homotopy paths available for training.
In the second stage, we sample a dataset of trajectories from the remaining tasks, weighted according to the controller's tracking error. We then use RL, incorporating tracking priors, to optimize per-trajectory tracking, search for homotopy paths, and train a homotopy path generator based on the resulting data. The best tracking results from all successfully tracked trajectories are curated into a new demonstration set, which is used to re-train the tracking controller.
In the third stage, we resample tracking tasks from the remaining set and leverage RL, the tracking controller, and the homotopy generator to curate another set of tracking demonstrations. This final set is used to optimize the tracking controller, resulting in our final model.

% With the above designs, we then adopt an iterative approach where we alternate between 1) training the tracking controller using abundant robot tracking demonstrations and 2) curating a large number of tracking demonstrations using the tracking controller. 
% To balance between the effectiveness of the tracking controller and the time cost in its training, our method consists of three stages as detailed as follows. In the first stage, we sample a small amount of tracking tasks $\mathcal{S}_1$ from all training tasks. 
% Since we do not have the tracking controller or the homotopy generator at the beginning, we create a robot tracking demonstration set by directly leveraging RL to obtain the single trajectory tracking result for each tracking task in $\mathcal{S}_1$. With these demonstrations, we train a tracking controller using RL and IL. The homotopy path generator is not learned at this stage because the generalizaton ability of the learned model will berestricted by the number of effective homotopy paths used for training. 
% In the second stage, we additionally sample a trajectory dataset from the remaining training tracking tasks, with weight positively proportional to the tracking error of the tracking controller. We then jointly leverage RL and the tracking controller to obtain per-trajectory tracking results. We also search the homotopy paths and learn a homotopy generator using searched results. We then curate a demonstration set from the best per-trajectory tracking results we've obtained. 
% With these demonstrations, we re-train a tracking controller.  
% In the third stage, we re-sample tracking tasks from the remaining set. Jointly leveraging RL, the tracking controller, and the homotopy generator, we curate a new robot tracking demonstration set. We then re-train the tracking controller with the supervision provided by these demonstrations. We take it as the final optimized tracking controller. 
% Specifically, 

% data from the whole training dataset. 


% Denote the total tracking task set sampled till now as $\mathcal{S}_2$, 




% We then try to get the per-trajectory tracking results taking the joint effort of per-trajectory tracking optimization, tracking data prior from the tracking controller and the homotopy generator. Having obtained current action-labeled trajectories, we re-train the tracking controller with the supervision provided by those trajectories. We then take it as the final optimized tracking controller.~\eric{Here we only introduce what we do but do not explain the rationality. Why only homotopy in the third stage but not the second stage? Why only three stages in total but not more? At least we should comment a bit on this since with high chance reviewers will ask about it as well. It is better to say something before the others ask.}

% To learn a homotopy generator, we search effective homotopy optimization paths and j
% to get single trajectory tracking result for each 
% We then try~\eric{avoid using these weak terms} to get the per-trajectory tracking result for each trajectory in both the re-sampled dataset and the original dataset taking the joint effort of both the per-trajectory tracking optimization and the tracking data prior provided by the tracking controller. After that, we obtained the second version of the demonstration data. We then re-train the trajectory controller with the supervision from action sequences in the dataset. In this stage, we construct the tracking task structure by searching homotopy optimization paths from trajectories in the dataset. We train a homotopy generator that encodes the searched optimization paths. In the third stage, we re-train the tracking controller via labeled trajectories obtained till now. In the third stage, 
% By optimizing the per-trajectory tracker for each trajectory in the dataset, we get the first version of demonstration data containing trajectories with high-quality action sequences. After that, the labeled dataset is leveraged to train the tracking controller. Then in the second stage, 

% and the tracking task structure prior provided by the tracking task structure prior model. 
% a tracking task structure prior model which encodes the optimization paths. 
% via the imitation-augmented RL. 
% is composed of three stages. 
% e then adopt an interactive approach to gradually get a strong tracking controller. 











% Considering the fact that the tracking controller is trained with the supervision from the tracking results of the already successfully tracked trajectories, it may be restricted in the ability to solve relatively simple tracking problems. Solving very difficult single trajectory tracking problems would still pose lots of challenges. Therefore, instead of optimizing the per-trajectory tracker alone, we propose to explore the tracking task structure and leverage a homotopy method to resolve these challenges by borrowing knowledge from other problems. 
% Specifically, for a tracking task $T$ that is hard to solve, we propose to solve $T$ via a homotopy path, \emph{e.g.,} $(T_A, T_B, ..., T)$. Starting from solving the first task $T_A$, we transfer the tracking result obtained in the previous tracking task to initialize the basic trajectory of the next tracking task. By gradually solving each problem in this manner in the series, we could potentially get better results in the task $T$, taking advantage of the basic trajectory initialized from other tracking tasks. 


% for difficult-to-solve problems 
% to facilitate the per-trajectory tracking problem solving, and 2) 
% introduce two techniques to improve the per-trajectory tracking policy
% with the  tracking controller, we try to 
% With the tracking controller, we try

% th successful action sequences, we need to infer action 
% we need to infer action sequences for kinematics
% We devise a per-trajectory tracking scheme to extract a large volume of high-quality imitation-ready data from kinematic-only trajectories. Initially, single trajectory tracking simplifies the problem by not requiring versatility or generalization, making it more manageable than training a general tracking controller. For various straightforward manipulation trajectories, per-trajectory tracking can effectively leverage the basic RL-based training scheme outlined earlier. However, relying solely on RL to track each trajectory independently presents challenges for more complex tracking scenarios. To address this, we introduce two techniques that enable single trajectory tracking to benefit from the neural controller and the structure of the tracking tasks. The first technique involves transferring tracking data to the controller to enhance single trajectory performance. The second explores the tracking task structure, employing a homotopy method to mitigate the difficulties associated with challenging single trajectory tracking problems.
% % We devise a per-trajectory tracking scheme to mine a large number of high-quality imitation-ready data from kinematic-only trajectories. First, single trajectory tracking, without the demand on versatility or the generalization ability, reduced to a simpler problem than training a general tracking controller. For various manipulation trajectories that are not very difficult, per-trajectory tracking is a solvable problem leveraging the basic RL-based training scheme detailed above. However, solely relying on tracking every single trajectory independently via RL would still face challenges in resolving very difficult tracking problems. Therefore, we propose two techniques to let the single trajectory tracking benefit from the neural controller and the tracking task structure. The first one involves transferring the tracking data prior to the tracking controller to facilitate the single trajectory tracking. The second one tries to explore the tracking task structure and leverage a homotopy method to ease the difficulty in challenging single trajectory tracking problems. 
% % if leveraging advanced model-free RL techniques. 
% % By leveraging the RL to train a single trajectory tracking policy, leveraging the above designed action space, observations, and the reward, we can already get high-quality tracking results for lots of manipulation trajectoreis. 


% \noindent\textbf{Improving per-trajectory tracking via tracking data prior.} With the tracking controller, which has already been optimized to be able to track lots of manipulation trajectories, we devise a method that can let the single trajectory tracking benefit from the tracking controller's tracking capability. Specifically, for a tracking task $T$ that is difficult to solve, we first query the tracking controller for a reasonable action sequence $\mathbf{A}$. After that, we initialize $\mathbf{A}$ as the basic trajectory in the single trajectory tracking policy. After that, we optimize the residual policy aiming to track the trajectory $T$. Taking advantage of the general tracking prior encoded in the tracking controller, we can potentially get better tracking results than directly tracking $T$ with the kinematic sequence as the basic trajectory. 

% \noindent\textbf{A homotopy method for solving difficult per-trajectory tracking.} Considering the fact that the tracking controller is trained with the supervision from the tracking results of the already successfully tracked trajectories, it may be restricted in the ability to solve relatively simple tracking problems. Solving very difficult single trajectory tracking problems would still pose lots of challenges. Therefore, instead of optimizing the per-trajectory tracker alone, we propose to explore the tracking task structure and leverage a homotopy method to resolve these challenges by borrowing knowledge from other problems. 
% Specifically, for a tracking task $T$ that is hard to solve, we propose to solve $T$ via a homotopy path, \emph{e.g.,} $(T_A, T_B, ..., T)$. Starting from solving the first task $T_A$, we transfer the tracking result obtained in the previous tracking task to initialize the basic trajectory of the next tracking task. By gradually solving each problem in this manner in the series, we could potentially get better results in the task $T$, taking advantage of the basic trajectory initialized from other tracking tasks. 

% \noindent\textbf{Learning a homotopy generator by mining beneficial optimization paths.} The homotopy method, though proved to enough effective in resolving challenges in very difficult tracking tasks, relies on correct homotopy paths. Searching for correct paths for each difficult-to-track trajectory from scratch, however, is very costly. Therefore, we propose to learn a homotopy generator that can directly propose beneficial homotopy paths at the inference time. 
% Learning a homotopy generator requires valid homotopy paths. Thus we first design an automatic tracking task structure exploration strategy for finding beneficial homotopy paths. Then we train a homotopy generator to encode the mined paths.

% We explore beneficial homotopy paths from the trajectories in the training dataset via a breadth-first-searching strategy. Specifically, we iteratively explore beneficial cross-tracking task relations from a set of kinematic trajectories.
% For each trajectory, we first identify a neighborhood for it from other kinematic trajectories via the similarity between two kinematic trajectories. We first run the per-trajectory tracking optimization to get their individual tracking results. Then we try to construct cross-task relations using an iterative BFS approach. 
% % \todo{all trajs with the initially optimized results} \todo{at first jwe identify ja neighborhood set } 
% In each iteration, for each tracking task $T$, we try to transfer the tracking result of its neighboring tracking task $T_p$ to initialize its basic trajectory and re-train the residual policy. If we can get better tracking results in this manner, we say $T_p\rightarrow T$ a beneficial cross-task relation. We regard $T_p$ as the ``parent trajectory'' of $T$. We record the best tracking result for each trajectory obtained at this iteration After severe iterations, we have obtained a beneficial cross-task relation set $\mathcal{C} = \{ (T_p\rightarrow T) \}$ which contains each beneficial cross-task relation. With $\mathcal{C}$, we regard $(T_{K}, T_{K-1}, ..., T_0)$ is a valid homotopy path if $T_{m+!}$ is the parent task of $T_m$ for each $0\le m \le K - 1$. 

% We propose to train a model that transforms each trajectory $T_c$ to the parent trajectory $T_p$ to model the tracking task structure. 
% Considering the fact that a single child trajectory $T_c$ may have multiple different parent trajectories $T_p$, we formulate it as a conditional trajectory generation problem where the goal is to generate the parent trajectories conditioned on the child $T_c$. Therefore, we train a conditional diffusion model to accomplish this vision. Specifically, we first train a trajectory diffusion model $\mathcal{M}$ which models the distribution of all kinematic trajectories. After that, we fine-tune it to a conditional generative model that describes the distribution of the parent trajectory of each child trajectory. By sampling from the conditional generative model, we transform each tracking task to its parent tracking task, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. We can construct a homotopy path by iteratively querying the conditional generative model to sample the parent tasks, \emph{i.e.,} $(T_1, T_2, ..., T_k)$ where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m)$, $1\le m \le k-1$. 

% At the inference time, we let the homotopy generator propose a homotopy path for a hard-to-solve task $T$. We gradually solve each tracking task in the path and transfer tracking results to the next task to solve the problem finally. 



% \noindent\textbf{Iterative optimization for progressively improving the tracking controller. } We then adopt an interactive approach to gradually get a strong tracking controller. Specifically, our method is composed of three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing the per-trajectory tracker for each trajectory in the dataset, we get the first version of imitation-ready data containing trajectories with high-quality action sequences. After that, the labeled dataset is leveraged to train the tracking controller via the imitation-augmented RL. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories with weight positively proportional to the tracking error of the first version controller. We then try to get the per-trajectory tracking result for each trajectory in both the re-sampled dataset and the original dataset taking the joint effort of both the per-trajectory tracking optimization and the tracking data prior provided by the tracking controller. After that, we obtained the second version of the imitation-ready data. We then re-train the trajectory controller with the supervision from action sequences in the dataset. In this stage, we construct the tracking task structure by searching homotopy optimization paths from trajectories in the dataset. We train a tracking task structure prior model which encodes the optimization paths. In the thrid stage, we re-train the tracking controller via labeled trajectories obtained till now. In the third stage, we re-sample a subste from the remaining trajectories. We then try to get the per-trajectory tracking results taking the joint effort of per-trajectory tracking optimization, tracking data prior from the tracking controller, and the tracking task structure prior provided by the tracking task structure prior model. Having obtained current action-labeled trajectories, we re-train the tracking controller with the supervision provided by those trajectories. We then take it as the final optimized tracking controller. 


% e further propose a homotopy method to resolve challenges in those problems. 
% propose to tackle difficult
% tackle difficult per-trajectory trac
% it may still be very hard for us to get good results in
% % Leveraging advanced RL with our dedicated designs for tracking, we can solve lots of per-trajectory tracking problems to a satisfactory extent. However, this strategy still struggles to solve very difficult tracking problems considering the inherent challenges of manipulation tracking. 
% % restrictions of RL. 
% Therefore, we propose to tackle difficult per-trajectory tracking problems via a homotopy method. 
% % a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% % Therefore, we propose a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% Specifically, for the trajectory $A=(\mathbf{H}_A, \mathbf{O}_A)$ that is difficult to track directly, instead of directly tracking the trajectory $A$, we propose to find an optimization path consisting of a series of tracking tasks that can help us solve the tracking problem of $A$. We then try to track $A$ by tracking each trajectory in the path and transfer results to the next in a one-by-one manner. If in this way we can get better tracking results for $A$ than directly solving $A$, we regard it as a good optimization path for $A$. We then further propose to encode such tracking task structure into a model so that it can propose useful optimization paths during the inference time efficiently. To fulfill this vision, we propose to first mine useful optimization paths from trajectories in the training dataset. We then encode the searched optimization paths into a model so that it can provide us with good optimization paths during the inference period efficiently. 



% to benefit single trajectory tracking from 
% the demand on the tracking
% resuded as a simpler problem than training a general racking controller, 
% To acquire a large number of high-quality tracking results, we devise a per-trajectory tracking scheme
% acquire high-quality per-trajectory tracking results 
% Training a high quality tracking controller requires 
% Training the tracking controller requires a large j
% Single tracjectoyr tracking control, tho
% Solving the per-trajectory tracking problem directly would still make it hard to address the challenge in tracking very difficult trajectories. To improve tracking results in these so that we can get more diverse imitation ready data with high quality action sequences in more tracking cases, we design a strategy where we can leverage the general tracking controller and the tracking task structure prior to better solve per-trajectory tracking problem. With the tracking controller, we devise two strategies to improve per-trajectory tracking performance. First, we try to leverage the general tracking prior encoded in the tracking controller to facilitate difficult per-trajectory tracking problem solving. The tracking controller trained to track lots of manipulation trajectories, with the supervision from high-quality imitation-ready data, already has the capability to give reasonable tracking results for various manipulation trajectories. So we design a strategy where we can let difficult per-trajectory tracking benefit from such tracking prior from the tracking controller. Second, instead of solving the per-trajectory tracking problem alone, we propose a homotopy method whih can effectively solve a difficult tracking problem by solving the task via an optimization path, and a homotopy generator which can propose beneficial homotopy optimization paths efficiently for a problem that is difficult to solve. We will detail them as follows. 


% \noindent\textbf{}



% % \noindent\textbf{Improving per-trajectory trackers via tracking prior and curriculum scheduling.} 
% \noindent\textbf{Improving per-trajectory trackers via tracking data prior and task structure prior.} The general tracking controller and the tracking task structure prior offer us two ways to improve the per-trajectory tracking result of a specific trajectory that is difficult to track, denoted as $A$. Firstly, we sample the action sequence from the general tracking controller for the current tracking task. We then initialize the basic trajectory as the sampled action sequence and re-train the residual policy to try to get better tracking results. Secondly, we let the tracking task structure prior model propose an optimization path consisting of a series of tracking tasks. After that, we solve the tracking problem of $A$ by gradually solving each task in the optimization path and transferring the results to the next one. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \noindent\textbf{A homotopy method for solving difficult per-trajectory tracking problem.} 
% % We propose 
% Leveraging advanced RL with our dedicated designs for tracking, we can solve lots of per-trajectory tracking problems to a satisfactory extent. However, this strategy still struggles to solve very difficult tracking problems considering the inherent challenges of manipulation tracking. 
% % restrictions of RL. 
% Therefore, we propose to tackle difficult per-trajectory tracking problems via a homotopy method. 
% % a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% % Therefore, we propose a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% Specifically, for the trajectory $A=(\mathbf{H}_A, \mathbf{O}_A)$ that is difficult to track directly, instead of directly tracking the trajectory $A$, we propose to find an optimization path consisting of a series of tracking tasks that can help us solve the tracking problem of $A$. We then try to track $A$ by tracking each trajectory in the path and transfer results to the next in a one-by-one manner. If in this way we can get better tracking results for $A$ than directly solving $A$, we regard it as a good optimization path for $A$. We then further propose to encode such tracking task structure into a model so that it can propose useful optimization paths during the inference time efficiently. To fulfill this vision, we propose to first mine useful optimization paths from trajectories in the training dataset. We then encode the searched optimization paths into a model so that it can provide us with good optimization paths during the inference period efficiently. 


% \noindent\textbf{Learning a homotopy generator by mining beneficial optimization paths. } 
% Given a trajectory set containing $K$ trajectories, we find useful tracking task optimization paths via breadth-first search. For each trajectory, we first identify its potential parent set via cross-trajectory similarity. Then in each searching iteration, for each task $A$, we try to use the best-tracked action trajectory of each of its parent task $B$ to initialize its tracking policy and see whether the policy optimization could benefit from the initialization. If the tracking result of trajectory $B$ can help us track the trajectory $A$, we regard $B$ as a beneficial parent tracking task of $A$. After several iterations, we identify a set of optimization paths $\mathcal{C} = \{ (T_n, ..., T_1) \} $, where for each  $1\le k \le n-1$, $T_{k+1}$ is the parent task of $T_k$.  

% Having obtained the optimization path set $\mathcal{C}$, we propose to train a model that transform each trajectory $T_c$ to the parent trajectory $T_p$ to model the tracking task structure. 
% % to model the tracking task structure. 
% Considering the fact that a single child trajectory $T_c$ may have multiple different parent trajectories $T_p$, we formulate it as a conditional trajectory generation problem where the goal is to generate the parent trajectories conditioned on the child $T_c$. Therefore, we train a conditional diffusion model to accomplish this vision. Specifically, we first train a trajectory diffusion model $\mathcal{M}$ which models the distribution of all kinematic trajectories. After that, we fine-tune it to a conditional generative model that describes the distribution of the parent trajectory of each child trajectory. By sampling from the conditional generative model, we transform each tracking task to its parent tracking task, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. We can construct an optimization path by iteratively querying the conditional generative model to sample the parent tasks, \emph{i.e.,} $(T_1, T_2, ..., T_k)$ where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m)$, $1\le m \le k-1$. 


% % \noindent\textbf{Planning the homotopy paths for solving difficult problems. } 


% \noindent\textbf{Iterative optimization for progressively improving the tracking controller. } We then adopt an interactive approach to gradually get a strong tracking controller. Specifically, our method is composed of three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing the per-trajectory tracker for each trajectory in the dataset, we get the first version of imitation-ready data containing trajectories with high-quality action sequences. After that, the labeled dataset is leveraged to train the tracking controller via the imitation-augmented RL. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories with weight positively proportional to the tracking error of the first version controller. We then try to get the per-trajectory tracking result for each trajectory in both the re-sampled dataset and the original dataset taking the joint effort of both the per-trajectory tracking optimization and the tracking data prior provided by the tracking controller. After that, we obtained the second version of the imitation-ready data. We then re-train the trajectory controller with the supervision from action sequences in the dataset. In this stage, we construct the tracking task structure by searching homotopy optimization paths from trajectories in the dataset. We train a tracking task structure prior model which encodes the optimization paths. In the thrid stage, we re-train the tracking controller via labeled trajectories obtained till now. In the third stage, we re-sample a subste from the remaining trajectories. We then try to get per-trajectory tracking result taking the joint effort of per-trajectory tracking optimization, tracking data prior from the tracking controller, and the tracking task structure prior provided by the tracking task structure prior model. Having obtained current action-labeled trajectories, we re-train the tracking controller with the supervision provided by those trajectories. We then take it as the final optimized tracking controller. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% propose to build the tracking task structure
% lots of imitation-ready data 
% the tracking controller is trained to mimic 
% with the tracking controller which already has the ability to track various manipulation 
% transfer tracking data prior encoded in the tracking controller to better solve per-trajectory tracking problem. Specifically, to solve the problem of tracking the trajectory $A$, we first try to query the trajectory controller to obtain the tracking result, an action sequence, of $A$. After that, we try to use the sampled action sequence to initialize the per-trajectory tracking 
% can leverage the tracking prior encoded in the tracking 


% \subsection{Per-Trajectory Tracking via Tracking Data Prior}
% \todo{todo} % 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Solving per-trajectory tracking directly would still make it hard to address the challenge in tracking very difficult trajectories. To improve tracking results in these difficult cases so that we can get more diverse imitation ready data with high quality action sequences in more tracking cases, we design a strategy where we can transfer tracking data prior encoded in the tracking controller to better solve per-trajectory tracking problem. Specifically, to solve the problem of tracking the trajectory $A$, we first try to query the trajectory controller to obtain the tracking result, an action sequence, of $A$. After that, we try to use the sampled action sequence to initialize the per-trajectory tracking 
% can leverage the tracking prior encoded in the tracking 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% % \subsection{Homotopy Path Generator Learning} 

% % tracking task structural modeling 

% % % \subsection{Structural Cross-Task Synergy Modeling}
% % \subsection{Structural Task Relational Space Modeling} \label{sec:method_task_space_modeling}
% % \subsection{Curriculum Scheduler Modeling via Mining and Modeling Cross-Trajectory Relations} \label{sec:method_task_space_modeling}
% % \subsection{Curriculum Scheduler Modeling} \label{sec:method_task_space_modeling}
% % \subsection{Learning Curriculum Scheduler via Modeling Tracking Curricula} \label{sec:method_task_space_modeling}
% % \subsection{Modeling Tracking Task Structure via Encoding Beneficial Optimization Paths} \label{sec:method_task_space_modeling}
% \subsection{Tracking Task Structure Modeling via Encoding Homotopy Optimization Paths} \label{sec:method_task_space_modeling}
% Leveraging advanced RL with our dedicated designs for tracking, we can solve lots of per-trajectory tracking problems to a satisfactory extent. However, this strategy still struggles to solve very difficult tracking problems considering the inherent challenges of manipulation tracking. 
% % restrictions of RL. 
% Therefore, we propose to tackle difficult per-trajectory tracking problems via a homotopy method. 
% % a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% % Therefore, we propose a tracking curriculum to tackle difficult per-trajectory tracking problems. 
% Specifically, for the trajectory $A=(\mathbf{H}_A, \mathbf{O}_A)$ that is difficult to track directly, instead of directly tracking the trajectory $A$, we propose to find an optimization path consisting of a series of tracking tasks that can help us solve the tracking problem of $A$. We then try to track $A$ by tracking each trajectory in the path and transfer results to the next in a one-by-one manner. If in this way we can get better tracking results for $A$ than directly solving $A$, we regard it as a good optimization path for $A$. We then further propose to encode such tracking task structure into a model so that it can propose useful optimization paths during the inference time efficiently. To fulfill this vision, we propose to first mine useful optimization paths from trajectories in the training dataset. We then encode the searched optimization paths into a model so that it can provide us with good optimization paths during the inference period efficiently. 
% % inference-time tracking task prior 
% % tracking task structure into a model so that it can provide us with inference-time tracking task structure prior efficiently. 
% % useful optimization paths into a model so that it 

% % and  and track $A$ by 
% % propose to track $A$ 
% % to solve the problem by solving each tracking 
% % the tracking curriculum tries to transfer the optimized action trajectory of a different tracking task, \emph{e.g.,} $B=(\mathbf{H}_B, \mathbf{O}_B)$ to initialize the tracking policy of $A$. If the re-optimized tracker can achieve better results than the original one, such a trail ($B\rightarrow A$) is regarded as a good curriculum. We say trajectory $B$ is the ``parent'' trajectory of $A$. Although the tracking curriculum is provided highly effective in our experiments, finding a good curriculum for solving each hard-to-track problem requires lots of trial and error and is thus very time-inefficient. Therefore, we propose to use a curriculum scheduler to expressively model tracking curricula so that that scheduler can be leveraged to propose tracking curricula efficiently. To fulfill this vision, we propose to first mine such tracking curricula from a batch of data, followed by learning a curriculum scheduler to model such tested effective curricula. 
% % rollout by a successful tracker 
% % We propose a tracking curriculum to tackle difficult per-trajectory tracking problems that continuously challenge RL when being optimized alone. 

% % \noindent\textbf{Constructing the tracking task structure.} 
% \noindent\textbf{Searching optimization paths.}
% Given a trajectory set containing $K$ trajectories, we find useful tracking task optimization paths via breadth-first search. For each trajectory, we first identify its potential parent set via cross-trajectory similarity. Then in each searching iteration, for each task $A$, we try to use the best-tracked action trajectory of each of its parent task $B$ to initialize its tracking policy and see whether the policy optimization could benefit from the initialization. If the tracking result of trajectory $B$ can help us track the trajectory $A$, we regard $B$ as a beneficial parent tracking task of $A$. After several iterations, we identify a set of optimization paths $\mathcal{C} = \{ (T_n, ..., T_1) \} $, where for each  $1\le k \le n-1$, $T_{k+1}$ is the parent task of $T_k$.  
% % we identify a set of parent tasks for each task, which further construct our tracking task structure. 
% % Such relations then form our tracking task structure. 
% % we regard $B\rightarrow A$ 
% % as a valid curriculum. After several iterations, two times in our experiments, we can identify a set of valid tracking curricula $\mathcal{C} = \{ T_p \rightarrow T_c \}$, where $T_p$ denotes the parent trajectory and $T_c$ represents the child trajectory. 
% % we find tracking curricula via breadth-first search. For each trajectory, we first identify its potential parent set via 

% % \noindent\textbf{Searching tracking curricula.} 

% \noindent\textbf{Modeling tracking task structure.}  Having obtained the optimization path set $\mathcal{C}$, we propose to train a model that transform each trajectory $T_c$ to the parent trajectory $T_p$ to model the tracking task structure. 
% % to model the tracking task structure. 
% Considering the fact that a single child trajectory $T_c$ may have multiple different parent trajectories $T_p$, we formulate it as a conditional trajectory generation problem where the goal is to generate the parent trajectories conditioned on the child $T_c$. Therefore, we train a conditional diffusion model to accomplish this vision. Specifically, we first train a trajectory diffusion model $\mathcal{M}$ which models the distribution of all kinematic trajectories. After that, we fine-tune it to a conditional generative model that describes the distribution of the parent trajectory of each child trajectory. By sampling from the conditional generative model, we transform each tracking task to its parent tracking task, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. We can construct an optimization path by iteratively querying the conditional generative model to sample the parent tasks, \emph{i.e.,} $(T_1, T_2, ..., T_k)$ where $T_{m+1}\sim \mathcal{M}(\cdot \vert T_m)$, $1\le m \le k-1$. 
% % we then complete the trajectory transformation 
% % complete the trajectory transformation problem, \emph{i.e.,} $T_p\sim \mathcal{M}(\cdot \vert T_c)$. 
% % % \noindent\textbf{Learning curriculum scheduler via modeling tracking curricula.}
% % $\mathcal{M}_{\mathcal{C}}: T_c $


% % With our carefully designed reward and observation space, the PPO can effectively optimize a specialist policy that achieves satisfactory performance on easy or medium manipulation tracking tasks. However, it would still struggle with achieving a reasonable solution for very difficult tasks involving intricate hand-object interactions such as subtle in-hand re-orientations and frequent contact shifting. Therefore, to further enhance the single trajectory tracking performance for providing better supervision for the tracking controller's training, we propose to explore trajectory curricula to better solve difficult tracking problems. Specifically, if we can transfer the optimized action sequence from tracking problem $A=(\mathbf{H}_A, \mathbf{O}_A)$ to $B=(\mathbf{H}_B, \mathbf{O}_B)$ as the start point of the task $B$'s optimization (\emph{i.e.,} setting the action sequence $\mathbf{A}_B$ that can successfully solve $B$ as the basic trajectory of $A$ and re-optimize the residual policy), which we also observe can achieve better performance than directly tracking $B$, we regard the problem of tracking $B$ can be benefit from tracking $A$, \emph{i.e.,} saying task $A$ is the ``parent'' trajectory of $B$. We then aim to leverage such cross-trajectory relations to construct a curriculum for each trajectory that is hard to optimize. To efficiently and effectively find such relations, we wish to learn a model that can tell us what's the most suitable ``parents'' for the current trajectory. It is hard to heuristically define a rule-based criterion such as based on the kinematic similarities or object geometry affinities, that exactly refect such relations. Therefore, we formulate this problem as a trajectory transformation and aim at learning  model $\mathcal{M}_{\mathcal{S}}$ from the trajectory dataset $\mathcal{S}$ to solve it. In detail, given a difficult-to-track trajectory $(\mathbf{H}, \mathbf{O})$, we want the model $\mathcal{M}_{\mathcal{S}}$ to transform it to its ``parent'' $(\mathbf{H}^p, \mathbf{O}^p)$. Considering the fact that there may be multiple instances that can serve as the ``parent'' for a single trajectory, the trajectory transformation ought to be a stochastic process where $\mathcal{M}_{\mathcal{S}}$ models the distribution of the parent, \textit{i.e.,} $(\mathbf{H}^p, \mathbf{O}^p) \sim \mathcal{M}_{\mathcal{S}}(\cdot\vert (\mathbf{H}, \mathbf{O}))$.

% % cross-task synergies to improve the training of a difficult task. 

% % To fulfill this vision, we further formulate the learning problem of the model $\mathcal{M}_{\mathcal{S}}$ as a conditional generative model training problem. Specifically, $\mathcal{M}_{\mathcal{S}}$ takes a trajectory $(\mathbf{H}, \mathbf{O})$ as the input and generates its parent trajectory. Therefore, we first train a diffusion model to describe the distribution of all kinematic trajectories contained in the dataset $\mathcal{S}$. After that, to acquire data for tuning it to a conditional generative model for the task transformation purpose, we propose a BFS approach to mine such ``parent-child'' paired data from the dataset. Detailed steps regarding the curriculum searching and the curriculum scheduler's training are deferred to Appendix~\ref{}. 


% %%%%%%%%%%%%%%%% move to appendix %%%%%%%%%%%%%%%
% % The BFS-based approach for constructing the task relational space and the conditional diffusion model training are detailed as follows. 

% % \todo{ add a picture for this structural space construction}

% % \todo{add the retargeted motions such as same trajectory different objects}

% % \todo{details w.r.t. how we identify the cross task affinities? }

% % \todo{extended task set?}

% % \noindent\textbf{Heuristic guided BFS for structural task relational space construction.} Given all manipulation trajectories from the training dataset $\mathcal{S}$, we first construct an expanded task set by augmenting each single task $(\mathbf{H}_A, \mathbf{O}_A, m_A)$ into $(\mathbf{H}_C, \mathbf{O}_A, m_A)$ and $(\mathbf{H}_A, \mathbf{O}_A, m_C)$. The structural task relational space wants to quantify the cross-task relations for each two different tasks in the expanded task set. One can imagine a most ideal way that is trying to test each pair of two manipulation trajectories $(A, B)$ to test whether one task, for instance task $B$ can benefit from task $A$. However, such a strategy is too expensive with the time complexity $\vert \mathcal{S}\vert^2$. If we wish not to be restricted to the first order cross-task relations only and also want to explore the high-order relations, for instance, the current task $C$ can benefit from the optimization result of task $B$ with the initialization of task $A$, the brute-force searching would cost $K\vert \mathcal{S}\vert^2$. Therefore, we adopt a heuristic guided searching strategy to reduce the time consumption to an affordable amount. 

% % Specifically, we first identify potential neighbours for each task via trajectory similarities and object geometry similarities. Having restricted the number of potential neighbours to a reasonable value, \emph{i.e.,} $K_{\text{nei}}$, we only conduct the affinity test between each potential neighbours. With this strategy, we can reduce the timeconsumption to $K K_{\text{nei}} \vert \mathcal{S}\vert$. By tuning $K$ and $K_{\text{nei}}$, we can balance the accuracy and the efficiency of the task relation space construction process. Please refer to the Supp. for more details. 
% % % Besides, it may overlook the high-order task relations, where the current task $C$ can benefit from the optimization result of task $B$ with the initialization of task $A$.  

% % % Specifically, \textcolor{red}{(TODO: add the description for the BFS part)}

% % \noindent\textbf{Conditional diffusion model for task relation modeling.} 
% % \todo{how we obtain the pairs to train the diffusion model -- both the high order and the first order} 
% % \todo{how to train the model}

% % \todo{re-check this part}
% %%%%%%%%%%%%%%%% move to appendix %%%%%%%%%%%%%%%

% % \todo{details w.r.t. how to improve per-trajectory tracker via tracking prior and the curriculum scheduler}


% % \textcolor{red}{(TODO: pharse it into a specialist-generalist-specialist iteration? )}
% % \noindent\textbf{Progressive generalist model training and labeled dataset improvement.}
% % \subsection{Progressive Generalist Model Training via ``Specialist-Generalist-Specialist'' Iterations} \label{sec:method_sgs}

% % \subsection{Progressively Improving the Tracking Controller via Iterative Optimization} \label{sec:method_sgs}

% \subsection{Iterative Optimization for Progressively Improving Tracking Controller} \label{sec:method_sgs}
% Based on the above designs, we then propose an iterative approach where the tracking controller is progressively improved by alternately executing the following two steps: 1) improving per-trajectory trackers with the joint effort of per-trajectory tracking optimization, data prior from the tracking controller, and the homotopy optimization path from the tracking task structure prior model; 2) training better tracking controller with the supervision from the improved imitation-ready data with action sequences. 
% % improving the action-labeled dataset by training better per-trajectory trackers on more trajectories leveraging the power of tracking prior provided by the general tracking controller and the optimization path from the tracking task structure prior; 2) training better tracking controller via supervision from the improved action-labeled dataset. 
% % the trajectory curriculum proposed by the curriculum scheduler; 

% % \noindent\textbf{Improving per-trajectory trackers via tracking prior and curriculum scheduling.} 
% \noindent\textbf{Improving per-trajectory trackers via tracking data prior and task structure prior.} The general tracking controller and the tracking task structure prior offer us two ways to improve the per-trajectory tracking result of a specific trajectory that is difficult to track, denoted as $A$. Firstly, we sample the action sequence from the general tracking controller for the current tracking task. We then initialize the basic trajectory as the sampled action sequence and re-train the residual policy to try to get better tracking results. Secondly, we let the tracking task structure prior model propose an optimization path consisting of a series of tracking tasks. After that, we solve the tracking problem of $A$ by gradually solving each task in the optimization path and transferring the results to the next one. 
% % tracker of a specific trajectory. Firstly, we can sample 
% % The sampled action sequence is init %
% % % , \emph{e.g.,} $A$. 
% % Firstly, we can use the action trajectory sampled from the general tracking controller on the current trajectory as the basic trajectory in its policy. By re-optimizing the residual policy, we may get better results than the original optimization. Secondly, by transforming trajectory $A$ into its parent trajectory $B$ via the curriculum scheduler and using the successful rollout action trajectory on the trajectory $B$ as the basic trajectory of $A$'s tracking policy, we re-optimize the residual policy for $A$ to try to get a better tracker for $A$. 
% % the curriculum scheduler
% % curriculum scheduler %

% \noindent\textbf{Iteratively improving tracking controller and the action-labeled dataset.} We then adopt an interactive approach to gradually get a strong tracking controller. Specifically, our method is composed of three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing the per-trajectory tracker for each trajectory in the dataset, we get the first version of imitation-ready data containing trajectories with high-quality action sequences. After that, the labeled dataset is leveraged to train the tracking controller via the imitation-augmented RL. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories with weight positively proportional to the tracking error of the first version controller. We then try to get the per-trajectory tracking result for each trajectory in both the re-sampled dataset and the original dataset taking the joint effort of both the per-trajectory tracking optimization and the tracking data prior provided by the tracking controller. After that, we have obtained the second version of the imitation ready data. We then re-train the trajectory controller with the supervision from action sequences in the dataset. In this stage, we construct the tracking task structure by searching homotopy optimization paths from trajectories in the dataset. We train a tracking task structure prior model which encodes the optimization paths. In the thrid stage, we re-train the tracking controller via labeled trajectories obtained till now. In the third stage, we re-sample a subste from the remaining trajectories. We then try to get per-trajectory tracking result taking the joint effort of per-trajectory tracking optimization, tracking data prior from the tracking controller, and the tracking task structure prior provided by the tracking task structure prior model. Having obtained current action-labeled trajectories, we re-train the tracking controller with the supervision provided by those trajectories. We then take it as the final optimized tracking controller. 
% % The tracking controller 
% % by encoding such optimization paths. 
% % The resampled dataset is leveraged the action-labeled dataset, \emph{i.e.,} $\mathcal{A}_1$. After that, the labeled dataset is leveraged to train the tracking controller. With the trained general controller, we evaluate it on all training tasks. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories where the weight is positively proportional to the tracking error of the first version controller. The resampled dataset is then labeled by optimizing their per-trajectory trackers. 
% % Combining these optimized trajectories and labeled trajectories in the first stage, we obtain the second version of the labeled dataset $\mathcal{A}_2$. The tracking controller is then trained via the supervision provided by $\mathcal{A}_2$. We mine trajectory curricula to improve tracking results of the currently selected trajectory. With the resulting tracking curricula, we then train a curriculum scheduler. In the third stage, we re-sample a subset from the remaining trajectories and use the tracking controller as well as the curriculum scheduler to label them, resulting in the third version of labeled dataset $\mathcal{A}_3$. After that, we re-train the tracking controller with supervision provided by $\mathcal{A}_3$. 
% % In the third stage, 
% % with the re-trained controller, we then construct the 
% % task relations space and try to improve the single trajectory optimization results leveraging the task relations space and the knowledge encoded in the generlaist model. Denote the improved labeled dataset as $\mathcal{A}_3$, the final controller is then trained with the supervision guidance from $\mathcal{A}_3$. 
% % % a specialist policy for each single trajectory in the initially sampled small dataset, we obtain the first version of the labeled dataset $\mathcal{A}_1$. 


% % \begin{itemize}
% %     \item 
% % \end{itemize}

% % Despite the effectiveness of the above single trajectory specialist policy optimization strategy leveraging RL and the task curriculum, it is infeasible for us to optimizing out a tracking policy for each individual trajectory in the training dataset considering the unaffordable computation and time consumption. Moreover, the task relation modeling may fail to explore valuable cross-trajectory relations when we only have a limited number of labeled data. Therefore the single trajectory optimization may still not that perfect due to the under-explored task relations. To leverage high-quality labeled data for training the tracking controller and to balance the amount of the labeled data with the time consumption, we propose a progressive policy training and labeled data improvement strategy. Specifically, the model is gradually trained via three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing a specialist policy for each single trajectory in the initially sampled small dataset, we obtain the first version of the labeled dataset $\mathcal{A}_1$. After that, the labeled dataset is leveraged to train the tracking controller via the above imitation augmented RL training strategy. With the trained tracking controller, we evaluate it on all training tasks. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories where the weight is positively proportional to the tracking error of the first version policy. The resampled dataset is then labeled via the specialist training. Combining theses optimized trajectories and labeled trajectories in the first stage, we obtain the second version of the labeled dataset $\mathcal{A}_2$. The tracking controller is then trained via the additional supervision provided by $\mathcal{A}_2$. In the third stage, with the re-trained controller, we then construct the task relations space and try to improve the single trajectory optimization results leveraging the task relations space and the knowledge encoded in the generlaist model. Denote the improved labeled dataset as $\mathcal{A}_3$, the final controller is then trained with the supervision guidance from $\mathcal{A}_3$. 




% % \subsection{Structural Cross-Task Synergy Modeling}







% % Following the above specialist policy training strategy, we can optimize a trajectory specific policy the inferred action sequence for each single manipulation trajectory. With such action-labeled trajectories $\mathcal{A}$, we train the generalist policy together with the imitation supervision provided by the action labeled trajectories and the RL. 

% % for each single manipulation trajectory


% % To efficiently optimizing single action-labeled trajectory with minimal hand tuning effort, we wish for a single suit of reward and observation design with which we can effectively optimize for a specialist policy for each single single trajectory. 
% % However, considering the inherent difficulties underlying the dexterous manipulation tracking, the RL algorithm may struggle with tracking some very difficult manipulation trajectories, \textit{e.g.,} with difficult object movements such as subtle re-orientations or involving grasping extremely thin objects. Therefore, we propose to ease the difficult single trajectory optimization problem by transferring knowledge from other trajectories. Specifically, we propose to explore cross-trajectory relations. That is, for each single trajectory that is hard to track, we aim to find its ``parent tasks'' whose optimization results can benefit its optimization. 
% % % employ model-free approach 


% % \textcolor{red}{(TODO: in this paragraph, the focus is how to train the specialist policy -- we can directly use the specialist policy (exactly the term) here )}

% % \subsection{Dexterous Manipulation Tracking via RL and Automatic Task Curriculum}

% % \textcolor{red}{(TODO: move the MDP and the model-free approach training and learning --- the model-free approach, the model unknown assumption, the MDP formulation to the beginning of the paragraph)}
% % % Automatic task
% % Considering the intricate dynamics involved in the dexterous manipulation resulting from the high DoF of a dexterous hand and the rich and changing hand-object contacts, we employ a model-free approach for tackle the problem. 
% % \textcolor{red}{(TODO: add the MDP formulation that frequently appear in other papers)}
% % Given a single kinematic manipulation trajectory $(\mathbf{H}, \mathbf{O})$, the trajectory specific specialist training aims at optimizing a tracking policy $\mathbf{\pi}(\cdot\vert\cdot )$ that can control a dexterous robot hand to track the reference kinematic trajectory. Assuming the physical model is unknown and non-differentiable, we leverage reinforcement learning to optimize the policy. To efficiently optimizing single action-labeled trajectory with minimal hand tuning effort, we wish for a single suit of reward and observation design with which we can effectively optimize for a specialist policy for each single single trajectory. However, considering the inherent difficulties underlying the dexterous manipulation tracking, the RL algorithm may struggle with tracking some very difficult manipulation trajectories, \textit{e.g.,} with difficult object movements such as subtle re-orientations or involving grasping extremely thin objects. Therefore, we propose to ease the difficult single trajectory optimization problem by transferring knowledge from other trajectories. Specifically, we propose to explore cross-trajectory relations. That is, for each single trajectory that is hard to track, we aim to find its ``parent tasks'' whose optimization results can benefit its optimization. \textcolor{red}{(TODO: rephrase this sentence, given xxx , we aim at xxx )}
% % Specifically, we propose a BFS based searching strategy that can automatically explore the trajectory relational space, quantifying relations between each trajectory pair from the datasets. After acquiring cross-trajectory relations, we propose to distill the explored trajectory relational space into a trajectory relational model. The trajectory relational model can then serve as a task relational prior model for providing knowledge w.r.t. cross-trajectory affinities. Then for each hard to track trajectory, we can leverage this model to transform it into a different trajectory, saying  the ``parent trajectory''. By first tracking the ``parent trajectory'' and then optimizing based on the tracked sequence of the parent trajectory, we can better track the original difficult trajectory finally. 



% % \noindent\textbf{Specialist policy training.} Our single trajectory specialist training scheme leverages PPO to optimize for a tracking policy $\mathbf{\pi}(\cdot\vert \cdot)$. The policy takes the current observation, comprising the current hand and object state information and the next frame tracking target as input and output the hand action for the hand to achieve the next state. Specifically, at each timestep $t$, we calculate the observation $\mathbf{o}\mathbf{b}\mathbf{s}_t$ as follows: 
% % \begin{align}
% %     \mathbf{o}\mathbf{b}\mathbf{s}_t = \{ \hat{\mathbf{h}}_t, \hat{\mathbf{o}}_t, \hat{\dot{\mathbf{h}}}_t, \hat{\dot{\mathbf{o}}}_t, \mathbf{f}_t,  \mathbf{h}_{t+1}, \mathbf{o}_{t+1}, \mathbf{h}_{t+1} - \hat{\mathbf{h}}_t, \mathbf{o}_{t+!} \ominus \hat{\mathbf{o}}_t   \}, 
% % \end{align}
% % where $\hat{\mathbf{h}}_t$ and $\hat{\mathbf{o}}_t$ are observed hand joint DoF positions and the object orientation as well as positions at the timestep $t$, $\hat{\dot{\mathbf{h}}}_t$ and $\hat{\dot{\mathbf{o}}}_t$ are hand DoF velocities and object linear as well as angular velocities respectively, $\mathbf{f}_t$ denotes the hand finger positions in the world space, $\mathbf{h}_{t+1}$ and $\mathbf{o}_{t+1}$ are the kinematic targets of the hand DoF positions and the object state in the next timestep. 

% % The reward consists a hand tracking reward $r_{h}$, object tracking reward $r_o$, and the hand-object affinity reward $r_d$. Specifically, xxx 
% % \textcolor{red}{(TODO: add the reward design here)}
% % \textcolor{red}{(TODO: add the residual policy here --- it is important since we need to justify the task curriculum here)}
    
% % % the observation $\mathbf{o}_t$ 


% % % \noindent\textbf{Trajectory relational space exploration via BFS.} 
% % \noindent\textbf{Trajectory relational space exploration and modeling.} 
% % We propose an automatic task curriculum to tackle difficult manipulation trajectories that are hard to track directly. Treating each single trajectory tracking problem as a task, for a tough task, the task curriculum tries to find its affinity tasks and transferring the optimized control trajectories for these tasks as the initialization for the current task to improve the tracking performance. \textcolor{red}{(TODO: add details here)} Such an approach requires us to find affinity tasks, which act as ``parent tasks'' for the current hard to solve problem. The current difficult task should be able to benefit from the optimization results of the ``parent tasks''. It is hard to heuristically define a rule-based criterion such as based on the kinematic similarities or object geometry affinities, that exactly refect such relations. Therefore, we formulate this problem as a trajectory transformation and aim at learning  model $\mathcal{M}_{\mathcal{S}}$ from the trajectory dataset $\mathcal{S}$ to solve it. In detail, given a difficult task, described as a kinematic trajectory $(\mathbf{H}, \mathbf{O})$, we want the model $\mathcal{M}_{\mathcal{S}}$ to transform it to its ``parent task'', described via a kinematic trajectory $(\mathbf{H}^p, \mathbf{O}^p)$ as well. Considering the fact that there may be multiple tasks that can serve as the ``parent task'' for a single difficult task, the trajectory transformation ought to be a stochastic process where $\mathcal{M}_{\mathcal{S}}$ models the distribution of the parent, \textit{i.e.,} $(\mathbf{H}^p, \mathbf{O}^p) \sim \mathcal{M}_{\mathcal{S}}(\cdot\vert (\mathbf{H}, \mathbf{O}))$.

% % To fulfill this vision, we further formulate the learning problem of the model $\mathcal{M}_{\mathcal{S}}$ as a conditional generative model training problem. Specifically, $\mathcal{M}_{\mathcal{S}}$ takes a trajectory $(\mathbf{H}, \mathbf{O})$ as the input and generates its parent tasks. Therefore, we first train a diffusion model to describe the distribution of all kinematic trajectories contained in the dataset $\mathcal{S}$. After that, to acquire data for tuning it to a conditional generative model for the task transformation purpose, we propose a BFS approach to mine such ``parent-child'' paired data from the dataset. Specifically, \textcolor{red}{(TODO: add the description for the BFS part)}




% % % Given a tracking task $(\mathbf{H}, \mathbf{O})$, 
% % % model outhgt to model a distribution of the parent.
% % % we aim at learning a model $\mathcal{M}_{\mathcal{S}}$ from the trajectory dataset $\mathcal{S}$ 
% % % We therefore propose a BFS based approach for mining cross-task relations for constructing the task relational space from the given trajectory dataset $\mathcal{S}$. 
% % % BFS based approach for mining cross-task relations 

% % % the task curriculum tries to fi


% % % \noindent\textbf{Trajectory relation modeling via conditional diffusion.}  

% % % aiming to find ``parent tasks'' 
% % % with difficult object movements such as subtle re-orientations or involving grasping thin objects, 
% % % Considering the vision to efficiently optimizing single action-labeled trajectory with minimal hand tuning effort, we wish for a single suit of reward and observation design for each trajectory. 

% % % For each manipulation reference trajectory, we wish to d


% % % Given the unknown model assumption, we leverage reinforcement learning to optimize the policy. 


% % % For single trajectory specific specialist policy training, 


% % \subsection{General Tracking Policy via Imitation Augmented RL}
% % With the carefully designed specialist policy training strategy and the task relational space exploration and modeling scheme, it is possible for us to optimize for a satisfactory result for each single manipulation trajectory tracking task. However, it is still not enough to acquire a generalist that can not only achieve good performance in each sequence but even generalize to unseen trajectories. Simply following the above RL scheme and training a single policy on multiple tasks is not feasible as demonstrated in our early experiments. As the number of training tasks increases, the RL would even struggle with effectively optimizing a strong policy that can solve every training task, letting alone generalize to unseen trajectories and resolve the novel manipulation sequence tracking challenge. We suppose such pool fitting phenomenon comes from the inherent deficiency of RL in solving multiple tasks. We therefore propose to introduce labeled single trajectory optimization results into the training process of RL, \textit{i.e.,} providing additional action labels as the supervision signals to train the policy together with RL. Specifically, given an action-labeled  dataset $\mathcal{S}_L=\{ (\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L) \}$, where each trajectory is augmented with an additional action sequence $\mathbf{A}$, we add an additional action supervision loss to train the policy together with RL, trying to distill optimized knowledge to the policy. Formally, for each labeled trajectory $(\mathbf{H}_L, \mathbf{O}_L, \mathbf{A}_L)$, the following action supervised loss is additionally added on the policy's prediction in each timestep $(\mathbf{\mu}_t, \mathbf{\sigma}_t) = \mathbf{\pi}(\cdot \vert \hat{\mathbf{s}}_t)$ to train the policy:
% % % to train the policy $\mathbf{\pi}(\cdot\vert \cdot)$  
% % \begin{align}
% %     \mathcal{L}_a = \Vert \mathbf{\mu}_t -  \mathbf{a}_t \Vert, 
% % \end{align}
% % where $\mathbf{a}_t$ denotes $t-$th step action taken from the optimized action trajectory. This strategy tries to bias the current trajectory towards the optimized successful trajectory in the dataset, in a similar flavor to DART~\citep{laskey2017dart}. 
% % % the action superv ised loss -- 



% % \textcolor{red}{(TODO: pharse it into a specialist-generalist-specialist iteration? )}
% % \noindent\textbf{Progressive generalist model training and labeled dataset improvement.}
% % Despite the effectiveness of the above single trajectory specialist policy optimization strategy leveraging RL and the task curriculum, it is infeasible for us to optimizing out a tracking policy for each individual trajectory in the training dataset considering the unaffordable computation and time consumption. Moreover, the task relation modeling may fail to explore valuable cross trajectory relations when we only have a limited number of labeled data. Therefore the single trajectory optimization may still not that perfect due to the under-explored task relations. To leverage high-quality labeled data for training the generalist policy and to balance the amount of the labeled data with the time consumption, we propose a progressive policy training and labeled data improvement strategy. Specifically, the model is gradually trained via three stages. In the first stage, we sample a small amount of data from the whole training dataset. By optimizing a specialist policy for each single trajectory in the initially sampled small dataset, we obtain the first version of the labeled dataset $\mathcal{A}_1$. After that, the labeled dataset is leveraged to train the generalist policy via the above imitation augmented RL training strategy. With the trained generalist, we evaluate it on all training tasks. Then in the second stage, we additionally resample a trajectory dataset from the remaining training trajectories where the weight is positively proportional to the tracking error of the first version policy. The resampled dataset is then labeled via the specialist training. Combining theses optimized trajectories and labeled trajectories in the first stage, we obtain the second version of the labeled dataset $\mathcal{A}_2$. The generalist is then trained via the additional supervision provided by $\mathcal{A}_2$. In the third stage, with the re-trained generalist, we then construct the task relations space and try to improve the single trajectory optimization results leveraging the task relations space and the knowledge encoded in the generlaist model. Denote the improved labeled dataset as $\mathcal{A}_3$, the final generalist model is then trained with the supervision guidance from $\mathcal{A}_3$. 




% % % maximize the potential benefit of the labeled data for training the generalist tracking policy and to 
% % % To tackle theses issues and 
% % % o fully exploit the potential of leveraging labeled 
% % % have a limited number of labeled dataset
% % % task relation modeling may fail to explore valuable trajectory 




% % % The RL would even struggle to optimize an effective policy that can solve every task when the size of the training task set
% % % us to obtain good result in each single trajectory tracking 


% % % for enhancing the multi-task performance of RL to learn a universal 

% % % each manipulation trajectory 
% % % that can output a physically plausible control sequence $\mathbf{A}$ for each manipulation trajectory $(\mathbf{H}, \mathbf{O})$ which is able to drive a dexterous robot 



==> articles_revision/related.tex <==

% \usepa

\vspace{-10pt}

\section{Related Work}

\vspace{-5pt}

% \noindent\textbf{Dexterous manipulation skill acquisition.} 

Equipping robots with human-level dexterous manipulation skills is crucial for future advancements. Previous approaches either rely on model-based trajectory optimization or model-free reinforcement learning (RL). Model-based methods face challenges due to the complexity of dynamics, often requiring approximations~\citep{pang2023global,Jin2024ComplementarityFreeMM,pang2021convex}. Model-free approaches, using RL~\citep{rajeswaran2017learning,chen2023visual,chen2021system,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact}, focus on goal-driven tasks with task-specific rewards, limiting their generalization across diverse tasks.
% limiting generalization to diverse tasks.
Our work explores a general controller for dexterous manipulations. Besides, learning via mimicking kinematic trajectories has recently become a popular train to equip the agent with various expressive skills~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC,Luo2023UniversalHM}. DTC~\citep{Jenelten2023DTCDT} proposes a strategy that can combine the power of model-based motion planning and RL to overcome the sample inefficiency of RL. 
% overcome the deficiency of the sample inefficiency of RL. 
In the humanoid motion tracking space, PHC~\citep{Luo2023PerpetualHC} proposes an effective RL-based training strategy to develop a general humanoid motion tracker. Recently, OmniGrasp~\citep{Luo2024GraspingDO} proposes to train a universal grasping and trajectory following policy. The policy can generalize to unseen objects as well as track novel motions. However, their considered motions are still restricted in grasping and trajectory following, leaving the problem of tracking more interesting and difficult trajectories such as those with subtle in-hand manipulations largely not explored. In this paper, we focus on these difficult and challenging manipulations. Moreover, we are also related to recent trials on combining RL with imitation learning. To overcome the sample inefficiency problem of RL and to facilitate the convergence, various approaches have been developed aiming to augment RL training with demonstrations~\citep{Sun2018TruncatedHP,Hester2017DeepQF,Booher2024CIMRLCI,Liu2023BlendingIA}. In our work, we wish to leverage high-quality demonstrations to guide the agent's explorations. Unlike previous work where demonstrations are readily available, acquiring a sufficient amount of high-quality robot tracking demonstrations remains a significant challenge in our task.
% Different from previous literature where demonstrations are assumed available, how to acquire abundant high-quality robot tracking demonstrations is a challenging problem in our task. 





% , however, struggle with the complexity of dynamics and often require approximations
% Equipping robots with human-level dexterous manipulation skills is critical for advancing robotics. Previous approaches largely rely on either model-based trajectory optimization or model-free reinforcement learning (RL). Model-based methods face challenges due to the complexity of dynamics, often requiring approximations~\citep{pang2023global,Jin2024ComplementarityFreeMM,pang2021convex}. On the other hand, model-free methods, using RL~\citep{rajeswaran2017learning,chen2023visual,chen2021system,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact}, focus on task-specific rewards, limiting their generalization across diverse tasks. In our work, we aim to develop an agent with versatile manipulation skills. Recently, learning by mimicking kinematic trajectories has gained popularity as a way to equip robots with a wider range of expressive skills~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC,Luo2023UniversalHM}. For instance, DTC~\citep{Jenelten2023DTCDT} presents a hybrid strategy that combines model-based motion planning with RL, addressing RL's sample inefficiency. In humanoid motion tracking, PHC~\citep{Luo2023PerpetualHC} introduces an effective RL-based training approach to develop a generalized humanoid motion tracker. Recently, OmniGrasp~\citep{Luo2024GraspingDO} has trained a universal policy for grasping and trajectory tracking that generalizes to unseen objects and novel motions. However, the motions considered are limited to grasping and trajectory following, with more complex tasks remaining largely unexplored. Our paper focuses on these challenging manipulation tasks. Additionally, we explore the integration of RL with IL to overcome the sample inefficiency problem and enhance convergence. Several methods have been developed to augment RL with demonstrations~\citep{Sun2018TruncatedHP,Hester2017DeepQF,Booher2024CIMRLCI,Liu2023BlendingIA}. Unlike previous work where demonstrations are readily available, acquiring a sufficient amount of high-quality robot tracking demonstrations remains a significant challenge in our task.
% remains a significant challenge


% Recent methods combining RL with motion imitation~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC} enhance expressiveness, yet they focus on simpler motions like grasping. In contrast, we target complex manipulations involving subtle in-hand re-orientations. To improve RL efficiency, imitation learning with demonstrations~\citep{Sun2018TruncatedHP,Liu2023BlendingIA} has been explored, but obtaining high-quality robot tracking demonstrations remains a challenge in our task.

% Equipping an embodied agent with dexterous manipulation skills is a vital step towards a future robot. Previous methods either adopt a model-based trajectory optimization approach or resort to a model-free method aiming to train a policy without assumptions on prior knowledge about the system. Developing a model-based method to solve dexterous manipulation is extremely challenging due to the complexity of the underlying dynamics. Therefore, previous methods would typically develop an approximated model~\citep{pang2023global,Jin2024ComplementarityFreeMM,pang2021convex}. A more popular approach is assuming the system dynamics is unknown and training a policy using advanced reinforcement learning~\citep{rajeswaran2017learning,chen2023visual,chen2021system,christen2022d,zhang2023artigrasp,qin2022dexmv,liu2022herd,wu2023learning,gupta2016learning,wang2023physhoi,mordatch2012contact}. Despite recent promising advances that have been demonstrated in the literature, they typically focus on learning goal-driven skills and require task-specific reward designs~\citep{chen2023visual,chen2021system,rajeswaran2017learning,christen2022d,zhang2023artigrasp,qin2022dexmv}, preventing them from generalizing to a wide range of diverse and novel tasks. In this work, we take a step further and explore the problem of learning a general controller for dexterous manipulations. Besides, learning a controller via mimicking kinematic trajectories has recently become a popular train to equip the controller with various expressive skills~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC,Luo2023UniversalHM}. DTC~\citep{Jenelten2023DTCDT} proposes a strategy that can combine the power of model-based motion planning and RL to overcome the deficiency of the sample inefficiency of RL. In the humanoid motion tracking space, PHC~\citep{Luo2023PerpetualHC} proposes an effective RL-based training strategy to develop a general humanoid motion tracker. Recently, OmniGrasp~\citep{Luo2024GraspingDO} proposes to train a universal grasping and trajectory following policy. The policy can generalize to unseen objects as well as track novel motions. However, their considered motions are still restricted in grasping and trajectory following, leaving the problem of tracking more interesting and difficult trajectories such as those with subtle in-hand re-orientations largely not explored. In this paper, we focus on these difficult and challenging manipulations. Moreover, we are also related to recent trials on combining RL with imitation learning. To overcome the sample inefficiency problem of RL and to facilitate the convergence, various approaches have been developed aiming to augment RL training with demonstrations~\citep{Sun2018TruncatedHP,Hester2017DeepQF,Booher2024CIMRLCI,Liu2023BlendingIA}. In our work, we wish to leverage high-quality demonstrations to guide the agent's explorations. Different from previous literature where demonstrations are assumed available, how to acquire abundant high-quality robot tracking demonstrations is a challenging problem in our task. 
% such as in-hand re-orientation using the hand with a fixed base~\citep{chen2023visual,chen2021system}~\citep{chen2023visual,chen2021system}, grasping, re-locating, relatively simple tool-using~\citep{rajeswaran2017learning,christen2022d,zhang2023artigrasp,qin2022dexmv}, or single manipulation trajectory mimicking~\citep{liu2024quasisim}. 
% Recent trials only learning general skills are still restricted to relatively simple tasks such as grasping~\citep{xu2023unidexgrasp,wan2023unidexgrasp2}. 

% want to take a step further and explore the possibility of learning a general tracking controller that can accomplish a wide range of challenging manipulation tasks. 

% via using planned motions to give dense rewards, and also at the same time keep the robustness of RL in the final controller.

% where RL is leveraged to train a tracking policy with hard mining strategies. 

% action-labeled data is itself a difficult question in our problem. 
% in training a general tracking controller using RL. 
% such as complex tool-using with non-trivial object motions and subtle manipulations using fingers. 
% even the MoCap trajectories that are never seen during the training. 
% Leveraing 
% Training a general tracking 
% Our method is also related 
% \todo{learning from humans? }
% mimicking a diverse range of challenging 
% Although there are recent trails that try to learn general controller, they are still restricted to 
% Althrough there are recent trails on learning general controllers 
% is leveraging a model-free 
% Despite impressive achievements they have demonstrated, 
% a simplified model such as using a relaxed soft contact model~\citep{pang2023global,drake,Jin2024ComplementarityFreeMM}.

% \noindent\textbf{Tracking control.} Learning a controller via mimicking kinematic trajectories has recently become a popular train to equipe the controller with various expressive skills~\citep{Jenelten2023DTCDT,Luo2023PerpetualHC,Luo2023UniversalHM}. DTC~\citep{Jenelten2023DTCDT} proposes a strategy that can combine the power of model-based motion planning and RL to overcome the deficiency of the sample inefficiency of RL via using planned motions to give dense rewards, and also at the same time keep the robustness of RL in the final controller. In the humanoid motion tracking space, PHC~\cite{Luo2023PerpetualHC} proposes an effective training strategy where RL is leveraged to train a tracking policy with hard mining strategies. Recently, OmniGrasp~\citep{Luo2024GraspingDO} proposes to train a universal grasping and trajectory following policy. The policy can generalize to unseen objects as well as track novel motions, even the MoCap trajectories that are never seen during the training. However, the difficulty of their considered motion is still restricted in grasping and trajectory following, leaving the problem of tracking more interesting and difficult trajectories such as those with complex object movements with subtle in-hand re-orientations largely not explored. In this paper, we focus on difficult and challenging manipulations such as complex tool-using with non-trivial object motions and subtle manipulations using fingers. 

% \noindent\textbf{Reinforcement learning with imitation learning.} 
% How to combine RL with imitation learning has attracted lots of attention. To overcome the sample inefficiency problem of RL and to facilitate the convergence, various approaches are developed aiming to augment RL training with demonstrations~\citep{Sun2018TruncatedHP,Hester2017DeepQF,Booher2024CIMRLCI,Liu2023BlendingIA}. In our work, we wish to leverage high-quality offline data to ease the difficulty in training a general tracking controller using RL. Different from previous literature where the labeled dataset is assumed available, how to acquire enough and high-quality action-labeled data is itself a difficult question in our problem. \todo{reifne this para.}
% the training difficulty of RL in solving the 
% the difficulty of training a general tracking controller 
% Despite their achievements, what's a proper way to combine the power of both sides in the dexterous manipulation space remains largely unexplored. Moreover, 

\vspace{-5pt}

==> articles_revision/repro_state.tex <==
\section{Reproducibility Statement}

\noindent \textbf{Novel Models and Algorithms.}
Our method is composed of two novel designs: 
1) The tracking controller training strategy which combines RL and IL. We have provided detailed explanations of the algorithm in Section~\ref{sec:method_il_rl} and Appendix~\ref{sec:supp_method}. Besides, we have included the source code in the Supplementary Materials, where the implementations of the algorithm are contained. Please refer to \emph{Key Implementations} section in the file \emph{DexTrack-Code/README.md} in our Supplementary Materials. 
% The \rep representation. We have provided detailed explanations of the representation in Section~\ref{sec:geneoh} and Appendix~\ref{sec_appen_rep_design}. Besides, we have included the source code in the Supplementary Materials, where the implementations of \rep are contained. Please refer to \emph{Key Implementations} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 
2) The homotopy optimization scheme, the homotopy path searching strategy as well as the homotopy path generator. 
% tracking curriculum and the tracking curricula mining strategy as well as the curriculum scheduler. 
We have provided detailed explanations in Section~\ref{sec:method_data} and Appendix~\ref{sec:supp_method}. Besides, we have included the source code in the Supplementary Materials. Please refer to the \emph{Key Implementations} section in the file \emph{DexTrack-Code/README.md} in our Supplementary Materials. 
3) The iterative optimization approach. We have provided detailed explanations in Section~\ref{sec:method_iteration} and Appendix~\ref{sec:supp_method}.  Besides, we have included the source code in the Supplementary Materials. Please refer to the \emph{Key Implementations} section and \emph{Usage} section in the file \emph{DexTrack-Code/README.md} in our Supplementary Materials. 
% The progressive HOI denoising method. We have provided detailed explanations of the denoising method in Section~\ref{sec:diffusion} and Appendix~\ref{sec_genenoh_diffusion_details}. Model, training, and evaluation details are included in Appendix~\ref{sec_appen_model_details} and~\ref{sec_appen_training_details}. Besides, we have included the source code in the Supplementary Materials. Please refer to the \emph{Key Implementations} section and \emph{Usage} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 

% \noindent \textbf{Theoretical Results.}
% Please refer to section~\ref{sec_appen_rep_design} in the Appendix for the proof of the property of leveraging the stage-wise denoising can clean the noisy input where each stage would not comprise the naturalness achieved after previous denoising stages. 

% \noindent \textbf{Datasets.}
% Please refer to Section~\ref{sec_exp_settings} and Appendix~\ref{sec_appen_datasets} for a detailed explanation of the datasets used. The data preprocessing part can be found in the \emph{Data Preprocessing} section in the file \emph{Geneoh-Diffusion-Code/README.md} in our Supplementary Materials. 

\noindent \textbf{Experiments.} 
For experiments, we provide 1) Source code.
Please refer to the folder \emph{DexTrack-Code} in our Supplementary Materials for details. 
2) Experimental details of our method and compared baselines. Please refer to the Section~\ref{sec:exp_setting} and in the Appendix~\ref{sec:supp_exp_details} for details. 
We also provide related information and instructions in the \emph{DexTrack-Code/README.md} file. 


==> articles_revision/teaser_figure.tex <==
\begin{figure}[htbp]
  % \includegraphics[width=\textwidth]{figs/teaser_8.pdf}
  % \includegraphics[width=\textwidth]{figs/teaser_15.pdf}
  \includegraphics[width=\textwidth]{figs/teaser_rb_6.pdf}
  \vspace{-23pt}
  \caption{ \footnotesize
  % By only Training on limited data, 
 %  \href{https://projectwebsite7.github.io/gene-dex-manip/}{
 % \eric{It is very hard to see the teaser figure even after zooming in. The text in the figure should be at least as large as the caption text size. The images are so small and the highlight can hardly be seen even after zooming in by 200\%. The captions should also highlight the key: our neural tracking controller can track diverse and novel human hand object manipulation references once trained.} \modelname}
 % \eric{The figure font size is still much smaller than t  he caption font size. Please adjust and increase the font size. Also, I think for kinematic references, maybe it is better to show the original human motion. The red circles are highlighting something invisible... We should reduce the number of figures to increase the size of each figure. Please make sure the figure is still visible when printed out using A4 paper.}
 \href{https://projectwebsite7.github.io/gene-dex-manip/}{\modelname} learns a generalizable neural tracking controller for dexterous manipulation from human references. 
 % \textcolor{myblue}{Our neural tracking controller (\emph{Fig. (a)}) can generalize to track novel and difficult manipulation trajectories with thin objects as well as intricate interactions with complex object movements and intriguing in-hand manipulations (\emph{Fig. (b)}), exhibits resilience to large kinematics noise, and is valuable in real-world applications (\emph{Fig. (c)}). }
 % \textcolor{myblue}{Our neural tracking controller takes kinematic references as input, and outputs hand action commands, aiming to make the tracking results close to input references (\emph{Fig. (a)}). It can generalize to track novel and difficult manipulation trajectories with thin objects as well as intricate interactions with complex object movements and intriguing in-hand manipulations (\emph{Fig. (b)}), exhibits resilience to large kinematics noise, and is valuable in real-world applications (\emph{Fig. (c)}). }
  % \textcolor{myblue}{Our neural tracking controller processes kinematic references to generate hand action commands, ensuring close tracking of input trajectories (\emph{Fig. (a)}). It generalizes to challenging tasks, such as thin-object manipulation and intricate in-hand interactions with complex movements (\emph{Fig. (b)}), demonstrating robustness to significant kinematics noise and practical utility in real-world scenarios (\emph{Fig. (c)}). }
    \textcolor{myblue}{
    % \href{https://projectwebsite7.github.io/gene-dex-manip/}{\modelname} learns a generalizable neural tracking controller for dexterous manipulation from human references. 
    It generates hand action commands from kinematic references, ensuring 
    % processes kinematic references to generate hand action commands, ensuring
    close tracking of input trajectories (\emph{Fig. (a)}), generalizes to novel and challenging tasks involving thin objects, complex movements and intricate in-hand manipulations (\emph{Fig. (b)}), 
    % , such as thin-object manipulation and intricate in-hand interactions with complex movements (\emph{Fig. (b)}), 
    and demonstrates robustness to large kinematics noise and utility in real-world scenarios (\emph{Fig. (c)}).
    Kinematic references are illustrated in \textcolor{orange}{orange rectangles} and \textcolor{orange}{background}. 
    % Our neural tracking controller processes kinematic references to generate hand action commands, ensuring close tracking of input trajectories (\emph{Fig. (a)}). It generalizes to challenging tasks, such as thin-object manipulation and intricate in-hand interactions with complex movements (\emph{Fig. (b)}), demonstrating robustness to significant kinematics noise and practical utility in real-world scenarios (\emph{Fig. (c)}). 
    }
 % Our neural controller can adeptly generalize to track novel manipulation trajectories with unseen objects, involving difficult interactions with thin objects (\emph{Fig. (a)}), intricate tool-using with intriguing re-orientations (\emph{Fig. (b)}),  exhibits high robustness towards large kinematics noise, and is valuable in real-world applications (\emph{Fig. (c)}). 
 % Figures in \textcolor{orange}{orange rectangles} with \textcolor{orange}{orange background} illustrate kinematic references.
 % ~\eric{should use more bold color instead of gray. it is very hard to see the gray rectangles or background.} 
 % with complex movements and 
 % The controller can 
 % various and novel manipulation trajectories involving difficult manipulations with thin objects (\emph{Fig. (a)}), intricate tool-using with complex movements and subtle in-hand re-orientations (\emph{Fig. (b)}),  exhibits high robustness towards large kinematics noise, and is valuable in real-world applications (\emph{Fig. (c)}). Figures in \textcolor{gray}{gray rectangles} with \textcolor{gray}{gray background} illustrate kinematic references. 
 % and out-of-domain (OOD) interactions involving objects from a brand new category (\emph{Fig. (c)}) 
 % The controller can adeptly control a dexterous robot hand to accomplish various challenging manipulations involving novel and difficult manipulations with complex object movements and intricate in-hand re-orientations (\emph{Fig. (a)}), new and challenging object geometries (\emph{Fig. (b)}),  and is robust to large kinematics noise and out-of-domain (OOD) interactions involving objects from a brand new category (\emph{Fig. (c)}). 
 % dexterous manipulation tracking controller from human manipulation references. 
  }
  \vspace{-1pt}
  \label{fig_intro_teaser}
\end{figure}
